Data Flow Refinement Type Inference

Refinement types enable lightweight verification of functional programs. Algorithms for statically inferring refinement types typically work by reduction to solving systems of constrained Horn clauses extracted from typing derivations. An example is Liquid type inference, which solves the extracted constraints using predicate abstraction. However, the reduction to constraint solving in itself already signifies an abstraction of the program semantics that affects the precision of the overall static analysis. To better understand this issue, we study the type inference problem in its entirety through the lens of abstract interpretation. We propose a new refinement type system that is parametric with the choice of the abstract domain of type refinements as well as the degree to which it tracks context-sensitive control flow information. We then derive an accompanying parametric inference algorithm as an abstract interpretation of a novel data flow semantics of functional programs. We further show that the type system is sound and complete with respect to the constructed abstract semantics. Our theoretical development reveals the key abstraction steps inherent in refinement type inference algorithms. The trade-off between precision and efficiency of these abstraction steps is controlled by the parameters of the type system. Existing refinement type systems and their respective inference algorithms, such as Liquid types, are captured by concrete parameter instantiations. We have implemented our framework in a prototype tool and evaluated it for a range of new parameter instantiations (e.g., using octagons and polyhedra for expressing type refinements). The tool compares favorably against other existing tools. Our evaluation indicates that our approach can be used to systematically construct new refinement type inference algorithms that are both robust and precise.

==> dataflow_informal.tex <==
% !TEX root = ../thesis.tex
\section{Data Flow Semantics}
\label{sec:df-dataflow}

To help us introduce the generalization of Liquid types, we first present several data flow semantics
of which Liquid types are an abstraction in the style of abstract interpretation. We start by informally
introducing a concrete \textit{data flow} semantics of untyped functional programs that explicitly models
how data flows in higher order programs. We then show two abstractions of the concrete semantics, 
\textit{relational} and \textit{collapsed} data flow semantics, that represent intermediate steps in 
designing Liquid types, thus formally modeling the points where Liquid type inference loses precision.


\subsection{Concrete Data Flow Semantics}

The main idea behind the concrete data flow semantics is to mimic the data flow propagation
of Liquid types but on the concrete level. While Liquid type inference propagates relations
represented by Liquid types, the concrete semantics propagates concrete values. Whereas
Liquid type inference assings types to (program expressions identified with) program locations
in a context-insensitive fashion, the concrete semantics assigns meaning to each location
subject to the context at hand. There is also a difference in which we present the concrete
semantics compared to original formulation of Liquid type inference. The latter encodes
the higher-order data flow using the subtyping constraints. Our concrete semantics on the 
other hand explicitly models how data is propagated, e.g., how inputs flow from call sites
to function definitions and how outputs propagate back in the other direction. One thing
the original Liquid types and the concrete semantics have in common is that they both
compositionally perform their respective inference purely on the structure of program expressions.


%We now proceed to the formal presentation of our data flow semantics for untyped higher-order programs.

\smartparagraph{Semantic Domains}
\label{sec:dfs-sdomains}
%
The concrete semantics assigns the meaning to every unique execution point called
an \textit{execution node} (or simply node) $\cnode \in \cnodes$. We distinguish
\emph{expression nodes} $\cenodes$ and \emph{variable nodes} $\cvnodes$. An expression
node $\pair{\cenv}{\elabel}$, denoted $\cn{\cenv}{\elabel}$, captures the execution
point where a subexpression $e^\elabel$ is evaluated in the environment $\cenv$.
As we shall see later, one of the abstraction steps performed by Liquid types is to
completely drop the environment when assigning types to program expressions.
\begin{align*}
\cnode \in \cnodes \; \Def= {}  \; \cenodes \cup \cvnodes \ind 
\cenodes \; \Def= {}  \; \cenvironments \times \elabels  \ind 
\cvnodes \; \Def= {}  \; \cenvironments \times \cenodes \times \vars \\
%
\cenv \in \cenvironments \; \Def= {}  \; \vars \pto_{\mi{fin}} \cvnodes \ind
\cmap \in \cmaps \; \Def= {}  \; \cnodes \to \cvalues \ind[2]\\
%
\cval \in \cvalues \; ::= {} \; \bot \mid \cerr \mid \const \mid \ctable \ind
\ctable \in \ctables \; \Def= {}  \; \ccallsites \to \cvalues \times \cvalues \ind[2]
\end{align*}


An environment $\cenv$ is a (finite) partial map binding variables to
variable nodes. A variable node $\pair{\cenv}{\ccsite, x}$, denoted 
$\cvn{\cenv}{\ccsite}{x}$, models the execution point where an argument value
is bound to a formal parameter of a function. Here, $\cenv$ is the environment
of the expression node where the function was defined. The expression node
$\ccsite$ is referred to as the \emph{call site} of the variable node. Intuitively,
this is the node of the subexpression that emits the function value being applied.
That is, if the call came from the expression
$(e_1^{\elabel_1} \, e_2^{\elabel_2})$, then the location of $\ccsite$ is
$\elabel_1$ and the environment of $\ccsite$ is the environment
used when evaluating the function application. The call site
is included in the variable node to uniquely identify the
binding. This way, we implicitly model the call stack of a program. 
Finally, $x$ is the formal parameter that is being bound to the variable node. 

%We explain the role of expression and variable nodes in
%more detail later. For any node $\cnode$, we
%denote by $\nenv(\cnode)$ the environment component of $\cnode$ and by
%$\cnode$ is an expression node $n=(\cenv, \elabel)$, then we write
%$\nloc(\cnode)$ the location component.
%
% We denote an extension of an environment $\cenv$ with a new binding of
% a variable $x$ to a variable node $\cvnode$ with
% $\cenv.(x\!:\cvnode)$. We further write $\cenv(x)$ for the variable
% node in the most recent (i.e. right-most) binding of $x$ in $\cenv$ if
% such a binding exists.
%A pair $\pair{e}{\cenv}$ is called well-formed if $\cenv(x)$ is defined for
%every variable $x$ that occurs free in $e$.  

\smartparagraphnb{Values and execution maps}
%
There are four kinds of (data flow) values $\cval \in \cvalues$. First, every constant
$\const$ is also a value. The value $\bot$ stands for nontermination or
unreachability of a node, and the value $\cerr$ models execution
errors. Functions are represented by \emph{tables} $\ctable$. A table
maintains an input/output value pair for each call site. We use square bracket notation
for tables and write $\tentry{a}{\cval_1}{\cval_2}$ for a table
entry that maps call site $a$ to the value pair $\pair{\cval_1}{\cval_2}$.
We denote by $\ctable_{\bot}$ 
%and $\ctable_{\cerr}$ the tables that map every call 
%site to the pairs $\pair{\bot}{\bot}$ and $\pair{\cerr}{\cerr}$, respectively.
the empty table that maps every call site to the pair $\pair{\bot}{\bot}$.
Hence, we use $[\tentry{\ccsite}{\cval_1}{\cval_2}]$
as shorthand for the table $\ctable_{\bot}[\ccsite \mapsto \pair{\cval_1}{\cval_2}]$.
We say that a table $\ctable$ has been called
at a call site $\ccsite$, denoted $\ccsite \in \ctable$, if the associated input value is not $\bot$:
$\pi_1(\ctable(\ccsite)) \not = \bot$. 
%The set $\csseen(\ctable)$ consists of all call sites for which $\ctable$ is called.

The data flow semantics computes \emph{execution maps}
$\cmap \in \cmaps$, which map nodes to values.
We write $\cmap_{\bot}$ ($\cmap_{\cerr}$) for
the execution map that assigns $\bot$ ($\cerr$) to every node.

Let us provide intuition on the execution maps through an
example. Consider the program and an excerpt of its execution map
shown in Fig.~\ref{ex:concrete-semantics-example}. Each expression
in the program is annotated with its unique location. E.g., the
using occurrence of \lstinline+x+ on line 1 is annotated with location
$g$. We use a simplified notation for nodes based on the following simple
observation. Only the expression with the location $g$ is visited more
than once, when analyzing the two calls to \lstinline+id+, so all other
reachable nodes in the map can be identified with their location only
for the presentation purposes. We will go into more details
on the nodes $g^a$ and $g^d$ shortly.
%
\begin{figure}[h!]
\begin{minipage}[t]{.38\textwidth}
\begin{flushleft}
{\begin{lstlisting}[language=Caml,mathescape=true,
  columns=fullflexible]
let id x = x${}^{g}$ in
let u = (id${}^{a}$ 1${}^{b}$)${}^{c}$ in
(id${}^{d}$ 2${}^{e}$)${}^{f}$
\end{lstlisting}}
\end{flushleft}
\end{minipage}%
\begin{minipage}[t]{.62\textwidth}
  \begin{flushright}
    %\vspace{-0.5em}
    \[%\left \{
        \begin{array}{@{}l@{}}
          \texttt{id} \mapsto [ \tentry{a}{1}{1},\; \tentry{d}{2}{2}] \;\quad\; \texttt{u},b,c,g^a \mapsto 1\\[1ex]
          a \mapsto [ \tentry{a}{1}{1} ] \;\quad\; d \mapsto [ \tentry{d}{2}{2}] \;\quad\; e,f,g^d \mapsto 2
        \end{array}
      %\right \}
    \]
  \end{flushright}
\end{minipage}
\caption{Program 1 and excerpt of its execution map~\label{ex:concrete-semantics-example}}
\end{figure} 

The mapping $e, f, g^a \mapsto 2$ indicates that the result computed
at nodes $e$, $f$, and $g^a$ is $2$. The nodes $g^a$ and $g^d$
correspond to the evaluations of the expression at location $g$
for each of the two calls to \lstinline+id+ at call sites
$a$ and $d$, respectively. We use the superscript notation informally
in our examples to indicate the environment associated with the
node for each of the two calls. For instance, consider the node
$g^d$. The actual definition of this node is $g^d \triangleq \cn{\cenv_1}{g}$
where $\cenv_1$ maps $x$ to the variable node $\cvn{\epsilon}{d}{x}$
and $\epsilon$ is an empty environment. The basic intuition is that
we are visiting the location $g$ in the context $\cenv_1$ where we
reached the enclosing function in the empty environment $\epsilon$
and we are analyzing the function body for the input argument $x$ emmited at 
the call site expression node $d$. The definition of $d$ can be given
similarly. By nesting the call site nodes in the environments we
implicitly model the program call stack.

Some of the nodes are mapped to function values. The function
\lstinline+id+ is represented by the table
$[ \tentry{a}{1}{1},\; \tentry{d}{2}{2} ]$ that stores input-output
values for the two calls to \lstinline+id+ at $a$ and $d$.
The nodes corresponding to the two usages of
\lstinline+id+ are also mapped to tables. However, these tables only
have a single entry each. Intuitively, \lstinline+id+ takes two
separate data flow paths in the program starting from its definition
(which we associate with \lstinline+id+ itself). For each node on
these two paths, the associated table captures how \lstinline+id+ will
be used at the nodes on any data flow path that continues from that point onward. The
tables stored at nodes $a$ and $d$ thus only contain information
about the input and output for the respective call site whereas the
table stored at \lstinline+id+ captures both call sites because the
node for the definition of \lstinline+id+ occurs on both paths.

\smartparagraph{Concrete transformer and semantics}
As a precursor to defining the data flow semantics, we define a
\emph{computational ordering} $\cvord$ on values. In this ordering,
$\bot$ is the smallest element, $\cerr$ is the largest element, and
tables are ordered recursively on the pairs of values for each call
site:
\begin{align*}
  \cval_1 \cvord \cval_2 {\Def\iff} &  \cval_1 = \bot \vee \cval_2 = \cerr
                                       \vee (\cval_1, \cval_2 \in \consts
                                       \wedge \cval_1 = \cval_2)  \;\vee \\
  & (\cval_1,\cval_2 \in \ctables
                                   \wedge \forall \ccsite.\,
                                   \cval_1(\ccsite) \mathrel{\vecop{\cvord}}
                                   \cval_2(\ccsite))
\end{align*}
Defining the error value as the largest element of the ordering is
nonessential but simplifies the presentation~\cite{PavlinovicThesis}.
The data flow semantics of an expression $e$ is defined as the least
fixpoint of a concrete transformer, $\ctransname$, on execution
maps. The idea is that we start with the map $\cmap_\bot$ and then
use $\ctransname$ to consecutively update the map with new values as more
and more nodes are reached. The signature of this transformer is as follows:
\[
  \ctransname: \Exp \to \cenvironments \to \cmaps \to \cmaps
\]
Essentially, $\ctransname$ takes an expression $e$ and an environment
$\cenv$ and returns a transformer
$\ctrans[k]{e}(\cenv): \cmaps \to \cmaps$ on execution maps. The
definition of $\ctrans[k]{e}(\cenv)$ is studied in~\cite{PavlinovicThesis}
and defined using induction over the structure of $e$, enabling
an easier formal connection to Liquid typing rules. The concrete
semantics $\csem \llbracket e \rrbracket$ of a program $e$ is defined
as the least fixpoint of $\ctransname$ over the complete lattice of
execution maps. We use the example from
Fig.~\ref{ex:concrete-semantics-example} to describe how the data flow
computation works on a high level. In Fig.~\ref{fig:running-example-maps},
we show the intermediate data flow maps for Program 1 obtained in each
step of the fixpoint computation. For simplicity, we only show the entries
for nodes storing tables.
%
\begin{figure}[t]
\small
\[\arraycolsep=10pt
\begin{array}{cccc}
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(1)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto &\;\; \bot\\
          a \mapsto&\;\; \bot\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
&
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(2)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; []\\
          a \mapsto&\;\; \bot\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
&
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(3)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; []\\
          a \mapsto&\;\; []\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
&
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(4)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; []\\
          a \mapsto&\;\; [\tentry{a}{1}{\bot}]\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
\end{array}\]
\noindent\makebox[\linewidth]{\rule{.99\textwidth}{0.2pt}}
\[\arraycolsep=11pt
\begin{array}{ccc}
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(5)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{\bot}]\\
          a \mapsto&\;\; [\tentry{a}{1}{\bot}]\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
&        
	\begin{array}{@{}l@{}l@{}}
	\mathbf{(6)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}]\\
          a \mapsto&\;\; [\tentry{a}{1}{\bot}]\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
&
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(7)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}]\\
          a \mapsto&\;\; [\tentry{a}{1}{1}]\\
          d \mapsto&\;\; \bot\\
        \end{array}
	\end{array}
\end{array}\]
\noindent\makebox[\linewidth]{\rule{.99\textwidth}{0.2pt}}
\[\arraycolsep=8pt
\begin{array}{ccc}
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(8)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}]\\
          a \mapsto&\;\; [\tentry{a}{1}{1}]\\
          d \mapsto&\;\; []\\
        \end{array}
	\end{array}
&
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(9)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}]\\
          a \mapsto&\;\; [\tentry{a}{1}{1}]\\
          d \mapsto&\;\; [\tentry{d}{2}{\bot}]\\
        \end{array}
	\end{array}
&	
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(10)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}, \tentry{d}{2}{\bot}]\\
          a \mapsto&\;\; [\tentry{a}{1}{1}]\\
          d \mapsto&\;\; [\tentry{d}{2}{\bot}]\\
        \end{array}
	\end{array}
\end{array}\]
\noindent\makebox[\linewidth]{\rule{.99\textwidth}{0.2pt}}
\[\arraycolsep=8pt
\begin{array}{cc}
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(11)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}, \tentry{d}{2}{2}]\\
          a \mapsto&\;\; [\tentry{a}{1}{1}]\\
          d \mapsto&\;\; [\tentry{d}{2}{\bot}]\\
        \end{array}
	\end{array}
&
        \begin{array}{@{}l@{}l@{}}
	\mathbf{(12)}  & {}\; 
        \begin{array}{@{}r@{}l@{}}
          \texttt{id} \mapsto&\;\; [\tentry{a}{1}{1}, \tentry{d}{2}{2}]\\
          a \mapsto&\;\; [\tentry{a}{1}{1}]\\
          d \mapsto&\;\; [\tentry{d}{2}{2}]\\
        \end{array}
	\end{array}
\end{array}\]
\caption{Fixpoint iterates of the data flow semantics for Program 1 in Fig.~\ref{ex:concrete-semantics-example}}
\label{fig:running-example-maps}
\vspace{-1em}
\end{figure}
%
Initially, no useful information for nodes \lstinline+id+, $a$, and $d$ is known,
denoted with $\bot$ in the map (\textbf{1}). After evaluating the \lstinline+id+ 
function definition expression, the node \lstinline+id+ is
assigned the empty table $[\,]$ (\textbf{2}). This table indicates that the meaning of \lstinline+id+ is a function
with currently no information on how this function is used in the program. 
In the next step (\textbf{3}), the node $a$ is reached and is also assigned $[\,]$ 
based on the value of \lstinline+id+. However, in the next step (\textbf{4}) our semantics
observes that \lstinline+id+ is called with 1 at node $a$; the table associated 
with $a$ hence contains this information.
This information is then propagated back to the
table associated with \lstinline+id+ in the next step (\textbf{5}). 

The propagation of information is formally defined as an exchange of
data between the table at \lstinline+id+ and $a$. Formally, the transformer
uses the data propagation function $\cprop$ defined in 
Fig.~\ref{fig:concrete-prop}.
%
\begin{figure}[t]
\begin{minipage}[t]{0.65\textwidth}
\[\begin{array}{r l}
%\cprop(\const, \bot) \Def=& \pair{\const}{\const} \ind[4] \cprop(\ctable, \bot) \Def= \;\pair{\ctable}{\ctable_{\bot}} \ind[4] \cprop(\cerr, \bot) \Def= \;\pair{\cerr}{\cerr}  \\[1.25ex]
\cprop(\ctable_1, \ctable_2) \Def=& \\ 
\multicolumn{2}{l}{\sind \Mlet \ctable' = \Lambda \ccsite. } \\[0.5ex]
\multicolumn{2}{l}{\sind[2]\Mif \ccsite \not\in \ctable_2 \;\Mthen \pair{\ctable_1(\ccsite)}{\ctable_2(\ccsite)} \;\Melse} \\[0.5ex]
\multicolumn{2}{l}{\sind[2]\Mlet \pair{\cval_{1i}}{\cval_{1o}} = \ctable_1(\ccsite) \Mend \pair{\cval_{2i}}{\cval_{2o}} = \ctable_2(\ccsite)} \\ [0.5ex]
\multicolumn{2}{l}{\sind[3]\;\;\pair{\cval'_{2i}}{\cval'_{1i}} = \cprop(\cval_{2i}, \cval_{1i}) \Mend \pair{\cval'_{1o}}{\cval'_{2o}} = \cprop(\cval_{1o}, \cval_{2o})} \\[0.5ex]
%&\ind[2] \;\; \pair{\cval'_{1o}}{\cval'_{2o}} = \Mif \cval'_{1i} = \cval'_{2i} \;\Mthen \cprop(\cval_{1o}, \cval_{2o}) \;\Melse \pair{\cval_{1o}}{\cval_{2o}} \\[0.5ex]
\multicolumn{2}{l}{\sind[2] \Min (\pair{\cval'_{1i}}{\cval'_{1o}}, \pair{\cval'_{2i}}{\cval'_{2o}}) \quad\quad\quad \ind[4]} \\[0.5ex]
\multicolumn{2}{l}{\sind \Min \pair{\Lambda \ccsite.\; \pi_1(\ctable'(\ccsite))}{\Lambda \ccsite.\; \pi_2(\ctable'(\ccsite))}} 
\end{array}\]
\end{minipage}%
\begin{minipage}[t]{0.34\textwidth}
\[\begin{array}{r l}
\cprop(\ctable, \bot) \Def= &  \pair{\ctable}{\ctable_{\bot}}\\[5.5ex]
\cprop(\ctable, \cerr) \Def=&  \pair{\cerr}{\cerr} \\[5.5ex]
%\cprop(\cval_1, \cval_2) \Def= &  \pair{\cval_1}{\cval_2} \ind[3] \textbf{(otherwise)}
\cprop(\cval_1, \cval_2) \Def= &  \pair{\cval_1}{\cval_1 \cvjoin \cval_2}\\
\multicolumn{2}{c}{\textbf{(otherwise)}}
\end{array}\]
\end{minipage}
\caption{Value propagation in the concrete data flow semantics\label{fig:concrete-prop}}
\end{figure}
%
The value propagation works as follows. First, it simply pushes constant
values forward. The interesting cases are when we propagate information between tables. 
The idea is that seen inputs are propagated backwards whereas outputs
for these inputs flow forward. For our current example of propagation between
tables at \lstinline+id+ and $a$, the input seen at the call site $a$ is propagated
to \lstinline+id+. As we shall see next, the output computed by \lstinline+id+ for
this input will be propagated back to the table at $a$. In general, inputs flow from
call sites to function definitions whereas outputs flow back to the call sites. 
This change of direction in propagation between tables corresponds to the change
of direction in subtyping for functions input and output types.


Now that \lstinline+id+ has seen input 1, our semantics evaluates the body of \lstinline+id+ with 1, 
producing 1 as the result (\textbf{6}). In the next step (\textbf{7}), this output is propagated
back in the other direction to the table stored at $a$~\cite{pierce}. After this step, the node $d$
becomes reachable and is assigned the empty table $[\,]$ (\textbf{8}). The data flow computation
then continues in the similar fashion as described earlier. 
%Note how a data flow value stored at some execution point, such as \

\input{intermediate}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> defs.tex <==
% !TEX root = paper.tex

%Zvonimir: rotate bigsqcup to get bigsqcap


%technical report
\newif\iftr
\trtrue
\newcommand{\less}[1]{\iftr \else #1 \fi}
\newcommand{\more}[1]{\iftr #1 \else \fi}
\newcommand{\lessmore}[2]{\iftr #2 \else #1 \fi}


\newcommand{\mn}[1]{\operatorname{#1}}

\newcommand{\m}[1]{\mathsf{#1}}
\newcommand{\mi}[1]{\mathit{#1}}

\newcommand{\kw}[1]{\bm{\mathsf{#1}}} % keyword in pseudo code

%meta-language
\newcommand{\Mlet}{\kw{let}\;}
\newcommand{\Min}{\kw{in}\;}
\newcommand{\Mif}{\kw{if}\;}
\newcommand{\Melse}{\kw{else}\;}
\newcommand{\Melif}{\kw{else\;if}\;}
\newcommand{\Mthen}{\kw{then}\;}
\newcommand{\Mand}{\;\kw{and}\;}
\newcommand{\Mend}{\kw{;}\;}
%\newcommand{\Mend}{\Mand}

\newcommand{\bdiamond}{\mathbin{\diamond}}

\newcommand{\stacklabel}[1]{\stackrel{\smash{\scriptscriptstyle \mathrm{#1}}}}
\newcommand{\Def}{\stacklabel{\mathrm{def}}}


% misc

\newcommand{\tool}[1]{\textsf{#1}\xspace}
\newcommand{\ourtool}{\tool{DART\_IT}}

\newcommand{\NN}{\mathbb{N}}

\newcommand{\lfp}{\m{lfp}}

\newcommand{\dom}{\operatorname{\mathsf{dom}}}
\newcommand{\rng}{\operatorname{\mathsf{rng}}}

\newcommand{\qd}{\;\;}
\newcommand{\pto}{\rightharpoonup}
\newcommand{\tto}{\mathbf{\to}}

\newcommand{\set}[1]{\{#1\}}
\newcommand{\pset}[2]{\set{\,#1\mid#2\,}}

\newcommand{\sqleq}{\sqsubseteq}

\newcommand{\Repeat}[2]{\foreach \n in {1, ..., #1}{#2}}
\newcommand{\setc}[2]{\{#1 \mid #2\}}
\newcommand{\pwset}[1]{\mathcal{}}
\newcommand{\powerset}{\mathcal{\wp}}
\newcommand{\ite}[3]{#1 \,\mathbf{?}\; #2 \;\mathbf{:}\; #3}

\newcommand{\pair}[2]{\langle #1, #2 \rangle}
\newcommand{\vecop}[1]{{\dot #1}}
\newcommand{\dvecop}[1]{{\ddot #1}}

\newcommand{\ind}[1][1]{\quad\Repeat{#1}{\quad}}
\newcommand{\sind}[1][1]{\;\Repeat{#1}{\;}}
\newcommand{\ssind}[1][1]{\,\Repeat{#1}{\,}}
%language
\newcommand{\elabels}{Loc}
\newcommand{\elabel}{\ell}
\newcommand{\vlabels}{Loc}
\newcommand{\vlabel}[1][x]{\elabel_{#1}}

\newcommand{\vars}{\mi{Var}}
\newcommand{\Exp}{\mi{Exp}}
\newcommand{\const}{c}
\newcommand{\consts}{\mi{Cons}}
\newcommand{\bools}{\mi{Bool}}
\newcommand{\btrue}{\mi{true}}
\newcommand{\bfalse}{\mi{false}}
\newcommand{\ifte}[3]{#1\,?\,#2:#3}



%(concrete) dataflow semantics
\newcommand{\cdesignation}{c}
\newcommand{\cn}[2]{#1{\bdiamond}#2}
\newcommand{\cns}[3]{#1{\bdiamond}#2{\bdiamond}#3}
\newcommand{\cvn}[3]{#1{\bdiamond}#2{\bdiamond}#3}
\newcommand{\csseen}{\mi{cld}}



\newcommand{\nenv}{env}
\newcommand{\nloc}{loc}

\newcommand{\cerr}{\omega}
\newcommand{\cval}{v}
\newcommand{\cvalues}{\mathcal{V}}
\newcommand{\ctable}{T}
\newcommand{\ctables}{\mathcal{T}}

\newcommand{\cmap}{M}
\newcommand{\cmaps}{\mathcal{M}}

\newcommand{\cenvironments}{\mathcal{E}}
\newcommand{\cenv}{\Gamma}
\newcommand{\cnodes}{\mathcal{N}}
\newcommand{\cnode}{n}
\newcommand{\cenodes}{\mathcal{N}_e}
\newcommand{\cenode}{n}
\newcommand{\cvnodes}{\mathcal{N}_{x}}
\newcommand{\cvnode}{n}
\newcommand{\ccallsites}{\cenodes}
\newcommand{\ccsite}{\cvnode_{\m{cs}}}
%\newcommand{\csinp}{\mathit{in}}
%\newcommand{\csout}{\mathit{out}}
\newcommand{\cstack}{s}
\newcommand{\cstacks}{\mathcal{S}}

\newcommand{\cvord}{\sqsubseteq}
\newcommand{\cvmeet}{\sqcap}
\newcommand{\cvjoin}{\sqcup}

\newcommand{\cmord}{\vecop{\cvord}}
\newcommand{\cmmeet}{\vecop{\cvmeet}}
\newcommand{\cmjoin}{\vecop{\cvjoin}}
\newcommand{\cmjoinb}{\vecop{\bigsqcup}}

\newcommand{\complete}{comp}
\newcommand{\cprop}{\mathsf{prop}}
\newcommand{\fuel}{k}
\newcommand{\fuels}{\mathbb{N}}

\newcommand{\ctransname}{\m{step}}
%\newcommand{\ctrans}[2][k+1]{\ctransname_{#1}\llbracket#2\rrbracket}
\newcommand{\ctrans}[2][k+1]{\ctransname_{\more{#1}}\llbracket#2\rrbracket}
\newcommand{\ccoll}{\mathbf{C}}
\newcommand{\csem}{\mathbf{S}}
\newcommand{\cdomain}{\mathcal{P}}
\newcommand{\cdomelem}{K}
\newcommand{\csafe}{\cmaps_{\m{safe}}}
\newcommand{\psafe}{P_{\m{safe}}}

%relational semantics
\newcommand{\rdesignation}{\mathsf{r}}

\newcommand{\rscope}{N}

\newcommand{\rbot}{\bot^{\rdesignation}}
\newcommand{\rerr}{\top^{\rdesignation}}
\newcommand{\rval}{r}
\newcommand{\rvalues}[1][\rscope]{\cvalues^{\rdesignation}_{#1}}
\newcommand{\rtable}{T^{\rdesignation}}
\newcommand{\rtables}[1][\rscope]{\ctables^{\rdesignation}_{#1}}

\newcommand{\rbools}{\bools^{\rdesignation}}
\newcommand{\rtrue}{\btrue^{\rdesignation}}
\newcommand{\rfalse}{\bfalse^{\rdesignation}}

\newcommand{\relname}{R}
\newcommand{\relsname}[1][\rscope]{\mathcal{R}_{#1}}
\newcommand{\rel}{\relname^{\rdesignation}}
\newcommand{\rels}[1][\rscope]{\relsname^{\rdesignation}}

\newcommand{\row}[2]{\pair{#1}{#2}}

\newcommand{\dmapname}{D}
\newcommand{\dmapsname}{\mathcal{\dmapname}}
\newcommand{\dmap}{\dmapname^{\rdesignation}}
\newcommand{\dmaps}{\dmapsname^{\rdesignation}}
\newcommand{\rdf}{\mathsf{F}}

\newcommand{\rmap}{\cmap^{\rdesignation}}
\newcommand{\rmaps}{\cmaps^{\rdesignation}}

\newcommand{\rvord}{\sqleq^{\rdesignation}}
\newcommand{\rvmeet}{\sqcap^{\rdesignation}}
\newcommand{\rvjoin}{\sqcup^{\rdesignation}}
\newcommand{\rvmeetb}{\mathsf{\bigsqcap}^{\rdesignation}}
\newcommand{\rvjoinb}{\bigsqcup^{\rdesignation}}

\newcommand{\rvecord}{\vecop{\sqleq}^{\rdesignation}}

\newcommand{\rmord}{\mathrel{\vecop{\sqleq^{\rdesignation}}}}
\newcommand{\rmmeet}{\mathop{\vecop{\sqcap^{\rdesignation}}}}
\newcommand{\rmjoin}{\mathop{\vecop{\sqcup^{\rdesignation}}}}
\newcommand{\rmjoinb}{\vecop{\bigsqcup^{\rdesignation}}}
\newcommand{\rmmeetb}{\vecop{\bigsqcap^{\rdesignation}}}

\newcommand{\dgamma}{\gamma^{\m{d}}}
\newcommand{\rgamma}[1][\rscope]{\gamma^{\rdesignation}_{#1}}
\newcommand{\ralpha}[1][\rscope]{\alpha^{\rdesignation}_{#1}}
\newcommand{\rmgamma}{\vecop{\gamma^{\rdesignation}}}
\newcommand{\rmalpha}{\vecop{\alpha^{\rdesignation}}}

\newcommand{\rprop}{\cprop^{\rdesignation}}
\newcommand{\rupdate}[3]{#1\rupd{#2}{#3}}
\newcommand{\rupd}[2]{[#1 \leftarrow #2]}
\newcommand{\rrescope}[2]{\rstrengthen{#1}{#2}}
\newcommand{\rstrengthen}[2]{#1[#2]}
\newcommand{\requality}[3]{\rstrengthen{#1}{#2 {=} #3}}
\newcommand{\rsubst}[3]{#1|[#2/#3 |]}
\newcommand{\rstrength}{\mathsf{strength^{\rdesignation}}}
\newcommand{\rconst}{c^{\rdesignation}}

\newcommand{\rtransname}{\ctransname^{\rdesignation}}
%\newcommand{\rtrans}[2][k+1]{\rtransname_{#1}\llbracket #2 \rrbracket}
\newcommand{\rtrans}[2][k+1]{\rtransname_{\more{#1}}\llbracket #2 \rrbracket}
\newcommand{\rcoll}{\mathbf{C}^{\rdesignation}}
\newcommand{\rmean}{\mathbf{U}^{\rdesignation}}
\newcommand{\rdomain}{\cdomain^{\rdesignation}}
\newcommand{\rdomelem}{P^{\rdesignation}}
\newcommand{\rdgamma}{{\dvecop{\gamma}}^{\rdesignation}}
\newcommand{\rdalpha}{{\dvecop{\alpha}}^{\rdesignation}}
\newcommand{\rdord}{\mathrel{\dvecop{\sqleq^{\rdesignation}}}}





%collapsed semantics
\newcommand{\penvironments}{\hat{\cenvironments}}
\newcommand{\penv}{\hat{\cenv}}
\newcommand{\pnodes}{\hat{\cnodes}}
\newcommand{\pnode}{\hat{\cnode}}
\newcommand{\penodes}{\hat{\cenodes}}
\newcommand{\penode}{\hat{\cenode}}
\newcommand{\pvnodes}{\hat{\cvnodes}}
\newcommand{\pvnode}{\hat{\cvnode}}

\newcommand{\absn}{z}
\newcommand{\absns}{\mathit{DVar}}
\newcommand{\ptvar}{\mi{dx}}
\newcommand{\ptio}{{io}}

\newcommand{\pdesignation}{\mathsf{cr}}

\newcommand{\pscope}{{\hat{\rscope}}}

\newcommand{\perr}{\top^{\pdesignation}}
\newcommand{\pbot}{\bot^{\pdesignation}}
\newcommand{\pval}{u}
\newcommand{\pvalues}[1][\pscope]{\cvalues^{\pdesignation}_{#1}}
\newcommand{\ptable}{T^{\pdesignation}}
\newcommand{\ptables}[1][\pscope]{\ctables^{\pdesignation}_{#1}}
\newcommand{\ptab}[3][\absn]{\langle #1, #2, #3 \rangle}

\newcommand{\pbools}{\bools^{\pdesignation}}
\newcommand{\ptrue}{\btrue^{\pdesignation}}
\newcommand{\pfalse}{\bfalse^{\pdesignation}}

\newcommand{\prel}{\relname^{\pdesignation}}
\newcommand{\prels}[1][\pscope]{\relsname[#1]^{\pdesignation}}

\newcommand{\pdmap}{\dmapname^{\pdesignation}}
\newcommand{\pdmaps}{\dmapsname^{\pdesignation}}

\newcommand{\pmap}{\cmap^{\pdesignation}}
\newcommand{\pmaps}{\cmaps^{\pdesignation}}

\newcommand{\pvord}[1][\pscope]{\sqleq^{\pdesignation}_{#1}}
\newcommand{\pvecord}{\mathrel{\vecop{\sqleq}^{\pdesignation}}}
\newcommand{\pvmeet}[1][\pscope]{\sqcap^{\pdesignation}_{#1}}
\newcommand{\pvjoin}[1][\pscope]{\sqcup^{\pdesignation}_{#1}}
\newcommand{\pvmeetb}[1][\pscope]{\mathsf{\bigsqcap}^{\pdesignation}_{#1}}
\newcommand{\pvjoinb}[1][\pscope]{\mathsf{\bigsqcup}^{\pdesignation}_{#1}}

\newcommand{\pmord}{\vecop{\sqleq^{\pdesignation}}}
\newcommand{\pmmeet}{\vecop{\sqcap^{\pdesignation}}}
\newcommand{\pmjoin}{\vecop{\sqcup^{\pdesignation}}}
\newcommand{\pmjoinb}{\vecop{\bigsqcup^{\pdesignation}}}
\newcommand{\pmmeetb}{\vecop{\bigsqcap^{\pdesignation}}}

\newcommand{\pgammac}{\gamma^{\pdesignation}}
\newcommand{\palphac}{\alpha^{\pdesignation}}
\newcommand{\pgamma}[1][\pscope]{\gamma^{\pdesignation}_{#1}}
\newcommand{\palpha}[1][\pscope]{\alpha^{\pdesignation}_{#1}}
\newcommand{\pmgamma}{\vecop{\gamma^{\pdesignation}}}
\newcommand{\pmalpha}{\vecop{\alpha^{\pdesignation}}}

\newcommand{\pprop}{\cprop^{\pdesignation}}
\newcommand{\pupdate}[3]{#1\rupd{#2}{#3}}
\newcommand{\pupd}[2]{|[#1 := #2|]}
\newcommand{\prescope}[2]{\mathsf{rescope}^{\pdesignation}(#1, #2)}
\newcommand{\pequality}[3]{#1|[#2 = #3|]}
\newcommand{\psubst}[3]{#1|[#2/#3 |]}
\newcommand{\pstrengthen}[2]{#1[#2]}
\newcommand{\pstrength}{\mathsf{strength^{\pdesignation}}}
\newcommand{\pconst}{c^{\pdesignation}}

\newcommand{\ptransname}{\ctransname^{\pdesignation}}
%\newcommand{\ptrans}[2][k+1]{\ctransname^{\pdesignation}_{#1}\llbracket#2\rrbracket}
\newcommand{\ptrans}[2][k+1]{\ctransname^{\pdesignation}_{\more{#1}}\llbracket#2\rrbracket}
\newcommand{\pcoll}[1][\cdot]{\mathbf{C}^{\pdesignation}\llbracket#1\rrbracket}
\newcommand{\pmean}{\mathbf{U}^{\designation}}
\newcommand{\pdomain}{\mathcal{P}^{\pdesignation}}
\newcommand{\pdomelem}{P^{\pdesignation}}
\newcommand{\pdgamma}{{\dvecop{\gamma}}^{\pdesignation}}
\newcommand{\pdalpha}{{\dvecop{\alpha}}^{\pdesignation}}


%general refinement type semantics
\newcommand{\tdesignation}{\mathsf{t}}

\newcommand{\tbot}{\bot^{\tdesignation}}
\newcommand{\terr}{\top^{\tdesignation}}
\newcommand{\tval}{t}
\newcommand{\tvalues}[1][\pscope]{\cvalues^{\tdesignation}_{#1}}
\newcommand{\ttable}{T^{\tdesignation}}
\newcommand{\ttables}[1][\pscope]{\ctables^{\tdesignation}_{#1}}
\newcommand{\ttab}[3][\absn]{#1\!:#2 \to #3}

\newcommand{\tbools}{\bools^{\tdesignation}}
\newcommand{\ttrue}{\btrue^{\tdesignation}}
\newcommand{\tfalse}{\bfalse^{\tdesignation}}

\newcommand{\basetypes}{\mathsf{B}}
\newcommand{\basetype}{\mathsf{b}}

\newcommand{\paramdomain}[1][\pscope]{\mathcal{A}_{#1}}
\newcommand{\paramelem}{\mi{a}}
\newcommand{\parambot}{\bot^{\paramdesignation}}
\newcommand{\paramtop}{\top^{\paramdesignation}}
\newcommand{\paramtrue}{\paramelem_{\mi{t}}}
\newcommand{\paramfalse}{\paramelem_{\mi{f}}}
\newcommand{\paramdesignation}{\mathsf{a}}
\newcommand{\paramord}[1][\pscope]{\sqleq^{\paramdesignation}_{#1}}
\newcommand{\parammeet}[1][\pscope]{\mathsf{\sqcap}^{\paramdesignation}_{#1}}
\newcommand{\paramjoinb}[1][\pscope]{\mathsf{\bigsqcup}^{\paramdesignation}_{#1}}
\newcommand{\parammeetb}[1][\pscope]{\mathsf{\bigsqcap}^{\paramdesignation}_{#1}}
\newcommand{\paramjoin}[1][\pscope]{\mathsf{\sqcup}^{\paramdesignation}_{#1}}
\newcommand{\paramalpha}[1][\pscope]{\alpha^{\paramdesignation}}
\newcommand{\paramgamma}[1][\pscope]{\gamma^{\paramdesignation}}
\newcommand{\paramwid}[1][\pscope]{\mathop{\triangledown^{\paramdesignation}_{#1}}}

\newcommand{\trel}[2][\basetype]{\{\nu\!:#1\;|\;#2\}}
\newcommand{\trelv}[1][\pscope]{\relname^{\tdesignation}}
\newcommand{\trels}[1][\pscope]{\relsname[#1]^{\tdesignation}}

\newcommand{\tmap}{\cmap^{\tdesignation}}
\newcommand{\tmaps}{\cmaps^{\tdesignation}}

\newcommand{\tvord}[1][\pscope]{\sqleq^{\tdesignation}_{#1}}
\newcommand{\tvecord}{\vecop{\sqleq}^{\tdesignation}}
\newcommand{\tvmeet}[1][\pscope]{\sqcap^{\tdesignation}_{#1}}
\newcommand{\tvjoin}[1][\pscope]{\sqcup^{\tdesignation}_{#1}}
\newcommand{\tvmeetb}[1][\pscope]{\bigsqcap^{\tdesignation}_{#1}}
\newcommand{\tvjoinb}[1][\pscope]{\bigsqcup^{\tdesignation}_{#1}}

\newcommand{\tmord}{\dot{\sqleq}^{\tdesignation}}
\newcommand{\tmmeet}{\dot{\sqcap}^{\tdesignation}}
\newcommand{\tmjoin}{\dot{\sqcup}^{\tdesignation}}
\newcommand{\tmjoinb}{\dot{\bigsqcup}^{\tdesignation}}
\newcommand{\tmmeetb}{\dot{\bigsqcap}^{\tdesignation}}

\newcommand{\tvgamma}[1][\pscope]{\gamma^{\tdesignation}_{#1}}
\newcommand{\tvalpha}[1][\pscope]{\alpha^{\tdesignation}_{#1}}
\newcommand{\tmgamma}{\vecop{\gamma^{\tdesignation}}}
\newcommand{\tmalpha}{\vecop{\alpha^{\tdesignation}}}

\newcommand{\tprop}{\cprop^{\tdesignation}}
\newcommand{\tupdate}[3]{#1\tupd{#2}{#3}}
\newcommand{\tupd}[2]{|[#1 := #2|]}
\newcommand{\trescope}[2]{\mathsf{rescope}^{\tdesignation}(#1, #2)}
\newcommand{\tequality}[3]{#1|[#2 = #3|]}
\newcommand{\tsubst}[3]{#1|[#2/#3 |]}
\newcommand{\tstrength}{\mathsf{strength^{\tdesignation}}}
\newcommand{\tconst}{c^{\tdesignation}}

\newcommand{\ttransname}{\ctransname^{\tdesignation}}
\newcommand{\ttrans}[2][k+1]{\mathsf{step}^{\tdesignation}\llbracket#2\rrbracket}
\newcommand{\tcoll}[1][\cdot]{\mathbf{C}^{\tdesignation}\llbracket#1\rrbracket}
\newcommand{\tmean}{\mathbf{U}^{\tdesignation}}
\newcommand{\tdomain}{\mathcal{P}^{\tdesignation}}
\newcommand{\tdomelem}{P^{\tdesignation}}
\newcommand{\tdgamma}{{\dvecop{\gamma}}^{\tdesignation}}
\newcommand{\tdalpha}{{\dvecop{\alpha}}^{\tdesignation}}

\newcommand{\wid}{\mathop{\triangledown}}
\newcommand{\shapewid}[1][\pscope]{\mathop{\triangledown^{\m{sh}}_{#1}}}
\newcommand{\shape}{\m{sh}}
\newcommand{\twid}[1][\pscope]{\mathop{\triangledown^{\tdesignation}_{#1}}}
\newcommand{\tmwid}{\dot{\wid}^{\tdesignation}}
\newcommand{\trelwid}[1][\pscope]{\mathop{\triangledown^{\m{ra}}_{#1}}}

\newcommand{\btype}[1]{\mathsf{#1}}
\newcommand{\tint}{\btype{int}}
\newcommand{\tbool}{\btype{bool}}
\newcommand{\rtype}[2]{\{\nu\!: #1 \mid #2\}}

\newcommand{\Qualifiers}{\mathcal{Q}}
\newcommand{\qualifiers}{Q}
\newcommand{\qualifier}{q}

\newcommand{\veufa}{\mathtt{ValidEUFA}}
\newcommand{\subtype}{<:}
\newcommand{\liqenv}{\xi}
\newcommand{\liqenvs}{\Xi}

%comments

\newcommand{\zp}[1]{{\color{blue} zvonimir: #1}}


\newcommand{\qtransname}{\ctransname^{q}}
\newcommand{\qcoll}[1][\cdot]{\mathbf{C}^{q}\llbracket#1\rrbracket}
\newcommand{\liqsub}{{<:}^{q}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> design.tex <==
\section{Design Space of Data Flow Refinement Type Inference}
\label{sec:design-space}

We next describe the design space of type inference algorithms built
using our abstract interpretation framework. We think of this design
space as the points where the inference loses precision relative to
the concrete semantics. These points are
made explicit in the choice of the domains and Galois connections as
well as the widening operators used to guarantee the soundness and
termination of the analysis. We discuss these points in more detail by
working with Program~2 of Fig.~\ref{ex:running-example}.


\subsubsection*{Concrete Semantics} Enriching our concrete data flow
semantics can yield more powerful type analyses. For instance, by
augmenting concrete tables with the node at which they were created
allows one to define refinement types that additionally capture how
the control flows in higher-order programs.  For instance, the entry
for node $b$ in the concrete map of Program 2 could be
$[\tentry{b}{[\tentry{a^b}{1}{0}]^{g1}}{0}]^h$. Compared to the
corresponding table of the original map, the augmented table
additionally remembers the node $h$ where the corresponding function
was defined. The same applies for the contents of the augmented
table. E.g. the observed input at call site $b$ originates from node
$g1$. Such augmented tables are naturally abstracted by relational,
collapsed, and refinement type tables that keep track of a
finite set of possible program locations at which functions are
defined.
% The size of such location sets is bounded by the program size.
The corresponding analysis would infer the following function
type for \lstinline+g+
\[g::\langle {g1}, {g2}\rangle\; x:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu \leq 1 \wedge \nu \geq 0}.\]
Here, the designation $\langle g1, g2 \rangle$ indicates that the
functions flowing to \lstinline+g+ are possibly $g1$ and $g2$. 
We note that the results presented in this paper already allow 
data flow refinement type inference algorithms to be used in 
combination with existing control flow 
analyses~\cite{DBLP:journals/csur/Midtgaard12,DBLP:conf/iccl/CousotC94}
via reduced products~\cite{cousot1979systematic}.

\subsubsection*{Relational Semantics} Our relational semantics does not 
maintain precise dependencies between functional values in the current scope.
We made this design choice to faithful model Liquid types. However, a
more precise analysis could discover useful dependencies on functional 
values. For instance, the following refinement type \'a la Liquid types 
can be assigned to the function \lstinline+h+ 
\[h:: g:\!(x:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu \leq 1 \wedge \nu \geq 0}) \to \rtype{\tint}{\nu = g\;1}. \]
Note here that the output type of \lstinline+h+ denotes the integer results 
of calling \lstinline+g+ with 1, which in turn always has to be in the interval [0, 1].
%Another direction of improving the Liquid type inference is to discover 
%relations over richer notions of scope. 
%Developing analyses that infer
%such powerful relations we leave as future work.

\subsubsection*{Collapsed Semantics} One way to improve the precision
of the collapsed semantics is to let tables maintain an input-output
relation for every location in the program (or some other partition of
the set of concrete nodes).  In such a semantics, a variable node is
defined as a pair of an abstract environment and a location. The
abstract transformer for the recursive function definition evaluates
in parallel the function body for every location from which inputs to
the function have been observed.
%Other transformer rules, as well as
%the abstract propagation, are defined in the expected way.
Similarly, the general refinement type analysis obtained from this
semantics is defined as the one presented in this paper, except that a
single function type is now replaced by a function type for every
program location. This corresponds to an intersection type indexed by program
locations as in~\cite{DBLP:conf/pldi/FreemanP91,DBLP:conf/vmcai/ZhuJ13}.
For example, the intersection refinement type inferred for the function
\lstinline+h+ would be:
\begin{align*}
h::\;\; & b:(x\!:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu = 0}) \to \rtype{\tint}{\nu = 0}   \;\;\;\wedge\\
    & d:(x\!:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu = x}) \to \rtype{\tint}{\nu = 1}.
\end{align*}
Observe how \lstinline+h+ is typed for each of its call site locations separately.
Consequently, the refinement type for the divisor expression in Program~2 is $\rtype{\tint}{\nu=1}$,
since it is typed based on the type of \lstinline+h+ for call site location $d$.
Hence, this semantics is able to show that Program~2 is safe, recovering from the loss of precision
introduced by our collapsed semantics. This new type inference 
is still guaranteed to terminate since there is only a finite number of locations in the program.

Our abstract interpretation framework provides the operating levers
that allow one to systematically explore these alternative inference
algorithms while easily retaining soundness.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> intermediate.tex <==
\section{Intermediate Abstract Semantics}

We next present two abstract semantics that represent crucial
abstraction steps in calculationally obtaining Liquid Type
inference from our concrete data flow semantics. Our formal exposition
focuses mostly on the aspects of these semantics that are instrumental
in understanding the loss of precision introduced by the two semantics.
Other technical details can be found in designated appendices.


\subsection{Relational Semantics}
\label{sec:arelational}
%
%We next show the first abstraction of the concrete data flow
%semantics in the sequence of abstract semantics leading up to the
%generalized Liquid type inference.
%
As we shall see later, a critical abstraction step performed by Liquid
types is to conflate the information in tables that are propagated
back from different call sites of that function. That is, a pair of
input/output values that has been collected from one call site will
also be considered as a possible input/output pair at other call sites
to which that function flows. However, in order for Liquid type inference
not to lose too much precision, output values observed for a particular 
call site explicitly remember the corresponding input value.
We refer to this semantics as the \textit{relational data flow semantics}.


\smartparagraph{Abstract domains}
%
The definitions of nodes, stacks, and environments in the relational semantics
are the same as in the concrete semantics. The relational abstractions of values,
constants, and tables are defined with respect to \emph{scopes}, which
are finite sets $\rscope \subseteq \cnodes \cup \absns$ of nodes and 
\textit{dependency variables} $\absn \in \absns$. Dependency variables
are intuitively used to describe how function output values depend on
the input values, similar to the way input-output relations are captured in
dependent types. The scope of a node $\cnode$, denoted $\rscope_{\cnode}$,
is the range of $\cnode$'s environment: $\rscope_{\cnode} \Def= \rng(\nenv(\cnode))$.
The new domains are defined as follows:
%
\begin{align*}
\rval_{\rscope} \in \rvalues & ::= {} \; \rbot \mid \rerr \mid \rel_{\rscope} \mid \rtable_{\rscope} &
\dmap_{\rscope} \in \dmaps_N & \Def= {} \; \rscope \cup \set{\nu} \to \consts \cup \{\rdf\} \\
%
\rel_{\rscope} \in \rels & \Def= {}\; \powerset(\dmaps_{\rscope}) &
\rtable_{\rscope} \in \rtables & \Def= {} \; \Sigma \absn \in \absns,
\Pi{\ccsite \in \ccallsites}.\; 
	\rvalues[\rscope \setminus \{\absn\}] \times \rvalues[\rscope \cup \{\absn\}]\\
%
&&\rmap \in \rmaps & \Def= \; \Pi{\cnode \in \cnodes}.\;\rvalues[\rscope_{\cnode}]
\end{align*}
%
Relational values $\rval_\rscope$ model how concrete values, stored at
some node, depend on the concrete values of nodes in the current scope
$\rscope$. The relational value $\rbot$ again models nontermination or
unreachability and imposes no constraints on the values in its
scope. The relational value $\rerr$ models every possible concrete
value, including $\cerr$. Concrete constant values are abstracted by
relations $\rel_\rscope$, which are sets of \emph{dependency vectors}
$\dmap_\rscope$. A dependency vector tracks the dependency between a
constant value stored at the current node, represented by the special
symbol $\nu$, and the values stored at the other nodes in the current
scope $\rscope$. Here, we assume that $\nu$ is not contained in $\rscope$.

We only track dependencies between constant values precisely: if a
node in the scope stores a table, we abstract it by the symbol $\rdf$
which stands for an arbitrary concrete table. We assume $\rdf$ to be
different from all other constants. We also require that for all
$\dmap_\rscope \in \rel_\rscope$, $\dmap(\nu) \in \consts$.
%
Relational tables $\rtable$ are defined analogously to concrete tables
except that they now map call site stacks $\ccsite$ to
pairs of relational values $\pair{\rval_i}{\rval_o}$ rather than
concrete values. We also associate a symbolic dependency variable 
$\absn$ with a call site stacks to express input-output dependencies; $\absn$
is not allowed to be in the scope of the input relational $\rval_i$ 
but is explicitly added to the scope of $\rval_o$. The idea is that
$\rval_o$ tracks the dependency between the output value and
the input values described by $\rval_i$ via $\absn$.
%We denote by $\rtable_{\bot}$ 
%the empty relational table that maps every call site to the pair $\pair{\rbot}{\rbot}$.
%We denote the fact that a relational table $\rtable$ has been invoked at a
%call site $\ccsite$ by $\ccsite \in \rtable$.
%
Relational execution maps $\rmap$ assign each node $\cnode$ a relational
value with scope $\rscope_\cnode$. 
%We denote by $\rmap_{\bot}$ ($\rmap_{\cerr}$)  
%the relational execution maps that assign $\rbot$ ($\rerr$) to every node.
%The definitions for bottom/top 
%relational maps and pointwise comparison of maps are as expected.

%We denote by $\rvalues[]$ the union of all $\rvalues$ and use similar
%notation for the sets of all dependency relations and relational
%tables. For the members of these sets we sometimes omit the subscript
%indicating the scope when it is irrelevant or clear from the context.

We provide the intuition behind the relational semantics through an 
example revisiting program 1 from Fig.~\ref{ex:concrete-semantics-example}.
%revisiting Program 2 from Fig.~\ref{ex:running-example}. 
We only show the entries for the nodes that store tables.
%
\begin{small}
\begin{align*}
\texttt{id} \mapsto {} & \absn:[ \tentry{a}{\{(\nu\!:1)\}}{\{(\absn\!:1, \nu\!:1)\}},\;
			 \tentry{d}{\{(\nu\!:2)\}}{\{(\absn\!:2, \nu\!:2)\}} ] \\
\texttt{a} \mapsto {} & \absn:[ \tentry{a}{\{(\texttt{id}\!:\rdf, \nu\!:1)\}}{\{(\texttt{id}\!:\rdf, \absn\!:1, \nu\!:1)\}}] \\
\texttt{d} \mapsto {} & \absn:[\tentry{d}{\{(\texttt{id}\!:\rdf, u\!:1, \nu\!:2)\}}{\{(\texttt{id}\!:\rdf, u\!:1, \absn\!:2, \nu\!:2)\}} ]
\end{align*}
\end{small}%
%
The relational semantics abstracts a concrete value $\cval$ by a
relational value that relates $\cval$ with the values observed at the
nodes that are in the scope of the node where $\cval$ was observed. 
Consider the entry for node \lstinline+id+. As expected, this entry 
is a table that has seen inputs at call site stacks identified with
$a$ and $d$, i.e, the table
has entries indexed by $a$ and $d$.
The actual input stored for call site $a$  
is now a relation consisting of the single row $(\nu:1)$, and
similarly for call site $d$. As the node \lstinline+id+ 
has no other nodes in its scope, these input relations are
essentially just representing the original input values $1$ and $2$. 
We associate these original values with the symbolic node $\nu$. The
output relation for $a$ consists of the single row $(\absn:1, \nu:1)$, 
stating that for the input value $1$ (associated with $\absn$), the
output value is also $1$ (associated with $\nu$). Observe how we use the dependency variable $\absn$
to explicitly capture the dependencies between the input and output values. 
%In general, we use the notation $\ccsite \bowtie \absn$ to
%denote that a table has seen an input from call site stack $\ccsite$ and we use
%the symbolic variable $\absn$ to bind the input value in the output relations of $\ccsite$.

The entry for \lstinline+a+ is similar to the one for \lstinline+id+, 
except that the relation also has an additional entry $\texttt{id}:\rdf$. 
This is because \lstinline+id+ is in the scope of the definition of
\lstinline+a+. The value of $\texttt{id}$ in the execution map is a table,
which we capture in the relations using the symbolical value
$\rdf$. That is, the relational semantics only tracks relational
dependencies between primitive values precisely whereas function
values are abstracted by $\rdf$. A similar description can be given for
the table stored at node $d$. Here, we also have the variable node $u$
in the scope whose value is $1$. As expected, the relational tables for
\lstinline+a+ and \lstinline+d+ contain a subset of entries of the table
stored at \lstinline+id+.

\smartparagraph{Abstraction}
%
We define the meaning of relational execution maps in terms of a
Galois connection between $\rmaps$ and the complete lattice of sets of
concrete execution maps $\powerset(\cmaps)$\lessmore{.}{, which we can
  then lift to properties $\cdomain = \NN \to \powerset(\cmaps)$.}
The details of this construction and the resulting abstract
transformer of the relational semantics can be found in \S~\ref{appendix:relational-semantics}.
%
We here focus on the key idea of the abstraction by formalizing the
intuitive meaning of relational values given above. Our formalization
assumes a function $\iota\!:(\cnodes \cup \absns) \mapsto \cnodes$
whose main purpose is to map dependency variables used in tables to 
their corresponding (non-empty) call stacks. We then define a family
of concretization functions 
$\rgamma[\iota]: \rvalues[] \to \powerset(\cmaps \times \cvalues)$, 
parameterized by scopes $\rscope$, between relational values and
sets of pairs of execution maps and values.
%
\begin{align*}
\rgamma[\iota](\rbot) \Def=\; & \cmaps \times \set{\bot} \ind[7] \quad \rgamma[\iota](\rerr) \Def=\; \cmaps \times \cvalues \\
%
\rgamma[\iota](\rel_{\rscope}) \Def=\; & \setc{\pair{\cmap}{c}}{\dmap {\in} \rel_\rscope \wedge \dmap(\nu) = c \land  
 \forall \cnode {\in} \rscope.\; \cmap(\cnode) \in \dgamma(\dmap(\iota(\cnode)))} \cup \rgamma[\iota](\rbot)\\
%
\rgamma[\iota](\absn: \rtable_{\rscope}) \Def=\; & \{ \pair{\cmap}{\ctable}\;|\; \forall \ccsite.\;
  \ctable(\ccsite) = \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) = \pair{\rval_i}{\rval_o} 
  \wedge \pair{\cmap_i}{\cval_i} \in \rgamma[\iota](\rval_i) \;\wedge\\ 
  &\ind[2] \pair{\cmap_o}{\cval_o} \in \rgamma[{\iota[\absn \mapsto \ccsite]}](\rval_o) \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap \wedge \cmap_o = \cmap_i[\ccsite \mapsto \cval_i]\} \cup \rgamma[\iota](\rbot)
\end{align*}
%
Here, the function $\dgamma$, which is used to give meaning to dependency
relations, is defined by $\dgamma(c) = \set{c}$ and $\dgamma(\rdf)=\ctables$.
Observe how we extend $\iota$ with a mapping from a dependency variable
$\absn$ to the corresponding call site stack $\ccsite$ when concretizing
output relations in tables. In effect, we simply use $\iota$ to keep track
of how dependency variables have been chosen for each call site stack.

%\smartparagraph{Design space} As pointed out, our relational data flow
%semantics does not maintain precise dependencies between functional
%values in the current scope. We made this design choice to
%faithfully model Liquid types, which do not
%precisly track functional dependencies. This choice of modeling
%relations represents another point in the design space of Liquid
%types. That is, a more precise analysis could discover useful
%dependencies on functional values. For instance, the following
%refinement type \'a la Liquid types
%%
%\[h:: g:\!(x:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu \leq 1 \wedge \nu \geq 0}) \to \rtype{\tint}{\nu = g\;1}. \]
%%
%can be assigned to the function \lstinline+h+ indicating that the output of
%\lstinline+h+ is the result of applying the input function \lstinline+g+ to $1$.
%Note here that the output type of \lstinline+h+ denotes the integer results 
%of calling \lstinline+g+ with 1, which in turn always has to be in the interval [0, 1].


\subsection{Collapsed Semantics}

We now describe a key abstraction step in the construction of our data
flow refinement type semantics. We formalize this step in terms of a
\textit{collapsed (relational data flow) semantics}. The main goal of
this semantics is to collapse the entries in function tables into
boundedly many while controlling how much stack information is being
abstracted, thereby allowing for different notions of call-site
context sensitivity.

\smartparagraph{Abstract domains}
%
The collapsed semantics is parameterized by a \textit{finite} set ofabstract stacks $\pstack \in \pstacks$ and an abstract concatenation operator
$\pconcat\!:\pstacks \times \pnodes \to \pstacks$. Here, $\pnodes$ is a set
of abstract nodes induced by abstract stacks, as defined below.
%
%
\[\begin{array}{c}
\pnode \in \pnodes \Def=  \penvironments \times \locs \times \pstacks \;\;\;\;
\pvnode \in \pvnodes \Def=  \penvironments \times \vars \times \pstacks \;\;\;\;
\penv \in \penvironments \Def= \vars \pto_{\mi{fin}} \pnodes \;\;\;\;
\prel_{\pscope} \in \prels \Def= {} \powerset(\pdmaps_{\pscope})\\[1.2ex]
%
%
\pval \in \pvalues ::=  \pbot \mid \perr \mid \prel_{\pscope} \mid \ptable_{\pscope} \ind 
\ptable_{\pscope} \in \ptables \Def= \Sigma \absn \in \absns, \, \Pi \pcsite \in \pstacks .\;\pvalues[\pscope \setminus \{\absn\}] \times \pvalues[\pscope \cup \{\absn\}] \\[1.2ex]
\pdmap_{\pscope} \in \pdmaps_{\pscope} \Def= (\pscope \cup\{\nu\}) \to (\consts \cup \{\rdf\})
%%
 \ind
\pmap \in \pmaps \Def= \Pi{\pnode \in \pnodes}.\;\pvalues[\pscope_{\pnode}]
\end{array}\]
%
Effectively, abstract nodes and environments have the same structure as
the concrete nodes except that concrete stacks are replaced with abstract
stacks. As expected, \emph{abstract scope} $\pscope$ is defined as a finite
set of abstract nodes and dependency variables
$\pscope \subseteq_{\mathit{fin}} (\pnodes \cup \absns)$. Analogous to
concrete scopes, we define the abstract scope
of an abstract node $\pnode$ as
$\pscope_{\pnode} \Def= \mathsf{rng}(\nenv(\pnode))$.
%For simplicity, we will often use $\pnode$ to
%range over both kinds of elements of abstract scopes.  The set of

Collapsed values $\pval_{\pscope} \in \pvalues$ are implicitly indexed
by an abstract scope $\pscope$ and closely resemble relational
values. The only major difference is in
the definition of tables. A \emph{collapsed table} $\ptable_{\rscope} \in \ptables$
now track an input-output relation for every abstract call stack 
via dependency variables $\absn$, where $\absn$ cannot appear in the scope of
the input relational value $\pval_1$ but is included in the scope of
output relational value $\pval_2$.

\smartparagraph{Example}
%
Let us provide the intuition behind the collapsed semantics through the example in Fig.~\ref{ex:concrete-semantics-example}
We assume the set of abstract stacks has a single element $\hat{o}$. In other
words, we with to perform a context-insensitive relational analysis on our
running example. For simplicity, we omit writing the abstract stack $\hat{o}$
in tables and only use dependency variables instead.

The collapsed semantics yields the following \emph{collapsed execution map} for
our running program, which abstracts the relational execution map for this program
shown earlier.
%
\[\begin{array}{@{}c@{}}
\small
%\textbf{a)}\\
%g1, c \to [ a^c \mapsto \pair{1}{0}] \quad g2, e \to [ a^e \mapsto \pair{1}{1}] \\[1ex]
%b  \to  [ c \mapsto \pair{[ a^c \mapsto \pair{1}{0}]}{0}] \quad d  \to  [ e \mapsto \pair{[ a^e \mapsto \pair{1}{1}]}{1}]\\[1ex]
%h  \to  [ c \mapsto \pair{[ a^c \mapsto \pair{1}{0}]}{0},  e \mapsto \pair{[ a^e \mapsto \pair{1}{1}]}{1}] \\[1ex] \hline \\
%
%\textbf{b)}\\
%g1, c \to [ a^c \mapsto \pair{\{(\nu\!:1)\}}{\{(a^c\!:1, \nu\!:0)\}}] \quad g2, e \to [ a^e \mapsto \pair{\{(\nu\!:1)\}}{\{(a^e\!:1, \nu\!:1)\}}] \\[1ex]
%b  \to  [ c \mapsto \pair{[ a^c \mapsto \pair{\{(\nu\!:1)\}}{\{(a^c\!:1, \nu\!:0)\}}]}{\{(c\!:\rdf, \nu\!:0)\}}]\\
%d  \to  [ e \mapsto \pair{[ a^e \mapsto \pair{\{(\nu\!:1)\}}{\{(a^e\!:1, \nu\!:1)\}}]}{\{(e\!:\rdf, \nu\!:1)\}}]\\[1ex]
%h  \to  [ c \mapsto\pair{[ a^c \mapsto \pair{\{(\nu\!:1)\}}{\{(a^c\!:1, \nu\!:0)\}}]}{\{(c\!:\rdf, \nu\!:0)\}},  \\
%\quad\quad\;\; e \mapsto \pair{[ a^e \mapsto \pair{\{(\nu\!:1)\}}{\{(a^e\!:1, \nu\!:1)\}}]}{\{(e\!:\rdf, \nu\!:1)\}}] \\[1ex] \hline \\
%
%\textbf{c)}\\
\texttt{id} \mapsto\; \ptab[\absn]{\{(\nu\!:1), (\nu\!:2)\}}{\{(\absn\!:1, \nu\!:1), (\absn\!:2, \nu\!:2)\}} \\[1ex]
a \mapsto\; \ptab[\absn]{\{(\nu\!:1)\}}{\{(\absn\!:1, \nu\!:1)\}} \quad
d \mapsto\; \ptab[\absn]{\{(\nu\!:2)\}}{\{(\absn\!:2, \nu\!:2)\}}
\end{array}\]
%
Again, we only show the entries for functions. Since the semantics does
not maintain any stack information, the relational tables do not track
where tunctions are being called in the program. 

Consider first the entry in the above map that assigns
\lstinline+id+.  This \textit{collapsed} table
indicates that \lstinline+id+ is a function called at some concrete
call site nodes, symbolically represented as $\absn$, with inputs 1 and
output 2. Note that while the precise call site stack information
of \lstinline+id+ is no longer maintained, the symbolic variable
$\absn$ still captures the relational dependency between the input and
output values for all the calls to \lstinline+id+.

Different kinds of call site context sensitivity can be obtained
by different notions of abstract stacks. For instance, classical
$k$-length callstring context-sensitive analyses can be obtained
by defining abstract stacks as lists of locations of length up to $k$.
The abstract concatenation operation $\pconcat$ then puts the location
of the input abstract node to the top of the stack and ensures the
stack length is less or equal to $k$.

%The ramifications of abstracting from the precise call site information
%in tables is best understood by considering a slightly more involved example.
%Consider a function \lstinline{let f g x = g x} and suppose \lstinline+f+
%is called with \lstinline+id+ and 1 at node $a$, and with increment function
%\lstinline+inc+ and 1 at node $b$. The collapsed semantics assigns to $f$ table
%$\ptab[\absn_1]{(\ptab[x]{\cdots}{\cdots})}{\ptab[\absn_2]{\{(\absn_1:\rdf, \nu\!:1)\}}
%{\{(\absn_1:\rdf, \absn_2\!:1, \nu\!:1), (\absn_1:\rdf, \absn_2\!:1,\nu\!:2)\}}}$.
%Essentially, the collapsed meaning of \lstinline+f+ is a function that
%takes another function (whose table we omit for simplicity) and integer
%1 as inputs, and returns integers 1 and 2.
%Since the table for \lstinline+f+ does not keep precise dependencies on
%functions and does not distinguish inputs based on their call sites $a$ and $b$,
%the collapsed semantics returns a relation consisting of values 1 and 2
%as the return values for both nodes $a$ and $b$. Concrete and relational
%semantics, on the other hand, precisely return values 1 and 2 for nodes
%$a$ and $b$, respectively.

 
\smartparagraph{Abstraction}
%
In order to provide the meaning of collapsed execution maps and
values, we also assume that the analysis is parameterized with
\textit{stack abstraction} function $\rho: \cstacks \to \pstacks$
that captures how the abstract stacks lose the precision compared
to concrete stacks. Such function are immediate for context
insensitive and $k$-length callstring context-sensitive analyses
described earlier.

We then use the stack abstraction function formally relate concrete
and abstract nodes, environments, and scopes. To this end, we raise
the stack abstraction function to define
the \textit{node abstraction} function $\rho:\cnodes \to \pnodes$ as
$\rho(\cnode) \Def= \cns{(\rho \circ \nenv(\cnode))}{\nloc(\cnode)}{\rho(\nstack(\cnode))}$.
%
%\begin{align*}
%\rho \Def= &\; \Lambda \cnode.\;\Mlet \cenv = \nenv(\cnode) \\
%&\ind[2]\;\; \penv = \Lambda x \in dom(\cenv).\; \rho(\cenv(x))\\
%&\ind\; \Min \cn{\penv}{\nloc(\cnode)}
%\end{align*}
%
In essence, $\rho$ recursively replaces concrete stacks with the concrete
ones in variable nodes. 
%For instance, if suppose $\rho$ maps two concrete
%variable nodes $\cvn{\cenv}{\ccsite}{x}$ and
%$\cvn{\cenv}{\ccsite'}{x}$ for distinct call sites $\ccsite$ and
%$\ccsite'$ to the same abstract node $\cn{(\rho \circ
%  \cenv)}{x}$. 
Next, we want to abstract relations over concrete nodes in $\rscope$ by
relations over abstract nodes in $\pscope$ which may contain
dependency variables standing for arbitrary expression nodes at call
sites. The corresponding concretization function therefore needs to be
defined with respect to a specific matching
$\delta:\pscope \to \rscope$ of abstract to concrete nodes. These
matching functions need to be consistent with node abstraction. We
formalize this consistency property by defining the set of all
\emph{scope consistent matchings} $\Delta(\pscope,\rscope)$ as
%
{\small
\begin{align*}
 \Delta(\pscope,\rscope) \Def= \pset{\delta: \pscope {\to} \rscope}{
 \forall \pvnode \in \pscope. (\pvnode \in \pnodes \Rightarrow \rho(\delta(\pvnode)){=}\pnode) 
  \wedge (\pvnode \in \absns \Rightarrow \delta(\pvnode) = \pvnode)}
\end{align*}
}%
%
We require that the matching of abstract nodes with concrete nodes is
consistent with $\rho$ and that dependency variables are equal.
%
The meaning of collapsed values $\pvalues$ with respect to relational
values $\rvalues$ is then given subject to a scope consistent matching
$\delta \in \Delta(\pscope, \rscope)$ by the concretization function
$\pgammac_{\delta} : \pvalues \to \rvalues$, defined as
follows:
% 
\begin{gather*}
\pgammac_{\delta}(\pbot) \Def= \rbot \ind \pgammac_{\delta}(\perr) \Def= \rerr \\
\pgammac_{\delta}(\absn:\ptable) \Def=\; \absn:\Lambda \ccsite\;
	\pair{\pgammac_{\delta}(\ptable_i(\rho(\ccsite)))}{\pgammac_{\delta}(\ptable_o(\rho(\ccsite), \absn))} \\
%
\pgammac_{\delta}(\prel_{\pscope}) \Def=\;
\setc{\dmap}{ \pdmap \in \prel \wedge \pdmap(\nu) = \dmap(\nu) \;\wedge \forall \pnode \in \pscope.\; \dmap(\delta(\pnode)) = \pdmap(\pnode)}
%
\end{gather*}
%
In the above, we use $\ptable_i(\pcsite, \absn)$ to denote the input
of $\ptable$ for call site stack $\pcsite$ with dependency variable $\absn$.
We use a similar notation $\ptable_o$ for outputs of collapsed tables.
The concretization function simply renames the abstract variable nodes used in
dependency vectors to dependency vectors using concrete variable nodes using $\delta$.
For tables, it assigns the same pair of relational values to every
possible concrete call site stack using $\rho$.
%(modulo renaming of $\ccsite$ in the output
%relation). 
%Note that the extended matching function
%$\delta[\absn \mapsto \ccsite]$ 
%is scope consistent for $\pscope \cup \set{\absn}$ and
%$\rscope \cup \set{\ccsite}$.


Details on the abstract transformer and other aspects of the collapsed
semantics are in \S~\ref{appendix:collapsed-semantics}.
%Appendix~\ref{appendix:collapsed-semantics}.

%\smartparagraph{Design space} One way to improve the precision
%of the collapsed semantics is to let tables maintain an input-output
%relation for every location in the program (or some other partition of
%the set of concrete nodes).  In such a semantics, a variable node is
%%defined as a pair of an abstract environment, the program variable being
%bound, and a location. Such a collapsed
%semantics leads to Liquid type inference where 
%each function is typed separately for the (over-approximation of) inputs
%coming from each individual call site location in the program. This corresponds to an 
%intersection type indexed by program locations as in~\cite{DBLP:conf/pldi/FreemanP91,DBLP:conf/vmcai/ZhuJ13}.
%For example, the intersection refinement type inferred for the function
%\lstinline+h+ would be:
%\begin{align*}
%h::\;\; & b:(x\!:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu = 0}) \to \rtype{\tint}{\nu = 0}   \;\;\;\wedge\\
%    & d:(x\!:\rtype{\tint}{\nu=1} \to \rtype{\tint}{\nu = x}) \to \rtype{\tint}{\nu = 1}.
%\end{align*}
%Here, \lstinline+h+ is typed for each of its call site locations separately.
%Hence, the refinement type for the divisor expression in Program~2 is $\rtype{\tint}{\nu=1}$,
%since it is typed based on the type of \lstinline+h+ for call site location $d$.
%Hence, this semantics is able to show that Program~2 is safe, recovering from 
%the loss of precision introduced by our collapsed semantics. %This new type inference 
%%is still guaranteed to terminate since there is only a finite number of locations in the program.

%Our abstract interpretation framework provides the operating levers
%that allow one to systematically explore these alternative inference
%algorithms while easily retaining soundness.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> language.tex <==
% !TEX root = main.tex
\section{Language}
\label{sec:language}

We work with a simple call-by-value higher-order language where all of the function
definitions appear at the top level. This choice simplifies our exposition,
but does not lose on generality as nested function definitions can be moved
to the top level using the techniques of lambda lifting~\cite{DBLP:conf/fpca/Johnsson85}.


\paragraph{\textbf{Syntax}.} 
Programs in our work are essentially recursion equation systems. 
That is, a program $p \in \Progs$ consists of $n$ functions each of 
which accepts exactly $k$ arguments.
\[\begin{array}{l}
f_1\; x_1 \cdots x_k\; =\; e_1 \\[0.25ex]
.\Repeat{5}{\quad}. \\[0.25ex]
.\Repeat{5}{\quad}. \\[0.25ex]
.\Repeat{5}{\quad}. \\[0.25ex]
f_n\; x_1 \cdots x_k\; =\; e_n
\end{array}\]
\noindent Bodies of program functions are expressions $e$ whose grammar is
shown in Figure~\ref{fig:language}. The expression language is standard, 
supporting branching statements and higher-order computation by treating
functions as first-class citizens.

\begin{figure}[h!]
\centering
\begin{tabular}{l l r}
$e \in \Exp$ & $::=$ & expressions \\[1ex]

$\quad|\;$ & $x_i$ & function parameter \\[1ex]

$\quad|\;$ & $f_i$ & function name \\[1ex]

$\quad|\;$ & $\const$ & constant \\[1ex]

$\quad|\;$ & $e_1 (e_2)$ & function application \\[1ex]

$\quad|\;$ & $\ifte{e}{e_1}{e_2}$ & if-then-else conditional
\end{tabular}
\caption{Expression syntax}
\label{fig:language}
\end{figure}

\noindent We denote the set of function indices with $I = \{1, \dots, n\}$.
Also, we assume the existence of constants $true$ and $false$ which we use to 
assign meaning to conditional statements.


\subsection{Semantic Domains}

The semantics of our language, that we shortly introduce, rely on several
semantic domains. 

\paragraph{Values.} In order to faithfully model Liquid type systems, we 
distinguish several kinds of values. \textit{Simple values} are either base 
$\base \in \Bases$ values or closures.   

\[\begin{array}{r l r}
\wz, \vz ::= & \base \quad|\quad c & \Repeat{4}{\quad} \text{simple values } \Valsz \\[1ex]
c ::= & [i\; \env] & \text{closures } \Closures \\[1ex]
\env ::= & \multicolumn{2}{l}
{\underbrace{\langle\his{}{C_0}, \vh_1, \dots, \vh_l, \unr, \dots,\unr\rangle}_{k+1}}\\[1ex]
\multicolumn{3}{r}{\text{environments } \envs\; (i \in I, 0 \leq l \leq k, C_0 \subseteq \Closures)} \\[1ex]
\wh, \vh ::= & \his{\vz}{C} & \text{history values } \Valsh \\[2ex]

w, v \in \Vals \triangleq & \Valsz \cup \{\omega, \bot\} & \text{values}
\end{array}\]

\noindent Closures model function calls. A closure hence consists
of an index of a function that is being called and an \textit{environment}
that captures the information about arguments currently passed to the function. 
Simple values paired with a finite set of closures are called \textit{history values}.
Actual values returned by programs are simple values together with non-termination
$\bot$ and error $\omega$ values. We will use symbols $C, D$ to range over 
(finite) sets of closures. The intuition behind history values 
is best understood in the context of environments.


\paragraph{Environments.} An environment $\env$ is a vector of history values, 
representing current argument values equipped with a set of closures $C$ called 
a \textit{history}. Histories capture information on how the encompassing closure 
was passed around to other closures. The argument vectors are padded 
to the right with $\unr$, intuitively capturing the fact that there are several
other arguments yet to be passed before the corresponding function can be 
evaluated. An environment that has not seen all $k$ arguments is considered partial, 
denoted with $par(\env)$.

To get a better understanding of closures and environments,
consider the closure $c = [i \;\langle \his{}{\{c_1\}}\; \his{1}{\{c_2\}, \unr, \dots, \unr} \rangle]$.  
Intuitively, this value tells us that the initial closure 
$c' = [i \;\langle \his{}{\emptyset}\; \unr, \dots, \unr \rangle]$ 
of the function $f_i$ was first passed as an argument to another closure $c_1$,
resulting in the closure $c'' = [i \;\langle \his{}{\{c_1\}}\; \unr, \dots, \unr \rangle]$ .
Later on during the computation, $c''$ was itself passed an argument value $1$,
yielding the closure $c''' = [i \;\langle \his{}{\{c_1\}}\; \his{1}{\emptyset}, \unr, \dots, \unr \rangle]$.
This closure, in turn, was later passed to $c_2$, resulting in $c$. As it can 
be seen, closures keep track of how they were passed along in the program. 
Closure values of this form are required for precise modeling of higher-order 
contracts. 

In the rest of this paper, we will use $E \in \powerset{\Envs}$ to range
over sets of environments and $\vec{E} \in \powerset{\Envs}^n$ for vectors
of sets of environments. We will also make use of functions $lai(\env)$
that returns the index of the last argument in the environment vector, 
$arg(\env, i)$ that returns argument value at position $i$ in the environment, 
and $his(\env)$ that returns the set of histories attached to argument values.
%\noindent On a high-level, this predicates holds when the first environment is a predecessor
%of the second one, i.e., the second environment belongs to a closure that earlier in
%the computation held the first environment.


\paragraph{Relations.}
We model program functions as relations $R \in \Rels \triangleq \Envs \times \Vals$.
To lookup values that program functions produce, we use 
\[\lookup{R}{\env} \triangleq \setc{v}{\langle \env, v \rangle \in R 
				\vee (\env \not \in dom(R) \Rightarrow v = \bot)}.\]
 
\noindent In the rest of the paper, we will use $\vec{R} \in \Rels^n$ to range over 
vectors of relations. Relation vectors form a \textit{concrete domain} in the sense 
they form a complete lattice subject to the pointwise subset ordering.

\begin{lemma}[Concrete domain]
$(\Rels^n, \vec{\subseteq}, \vec{R}_{\bot}, \vec{R}^{\top}, \vec{\cap}, \vec{\cup}).$
\end{lemma}

\noindent In the above, $\vec{R}^{\bot}$ is the vector of empty relations and
$\vec{R}^{\top}$ is the vector of relations $\Envs\times\Vals$.

\subsection{Semantics}

We now introduce the semantics of our language. The basic idea is as follows.
For a given program, we assume we are also given an initial set of inputs/environments
for each function. These inputs are tantamount to initial states in the context of 
semantics of imperative programs. Each function is assigned meaning in an iterative
fashion using a \textit{concrete transformer} that (1) computes outputs the functions 
only for the inputs seen so far, (2) collects new inputs for the functions, and (3) updates
appropriatelly closure values so they maintain the correct history information.

\paragraph{Concrete transformer.} 
The concrete transformer is modeled as a relation
$\ctrans{\cdot}:\Exp \to \Rels^n \to (\Envs \times \Vals \times \powerset{\Envs}^n)$
akin to a transition system. It relates an expression, the approximation of program functions given
in terms of relation vector $\vec{R}$, current input environment $\env$, with a value the expression 
evalutes to and calls observed for each function during the evaluation.


\begin{figure}[h!]
\centering
\[\begin{array}{l l l}
% \multicolumn{3}{l}{\forall e, \vec{R}, \env, v, \vec{E}.\; \ctransr{e}{\vec{R}}{\env}{v}{\vec{E}} \implies \neg par(\env)}\\[1.5ex]

%---variable---
\langle \env, v, \emptyset^n \rangle \in \ctrans{x_i}(\vec{R}) &\iff&  arg(\env, i) = v \\[1.5ex]

%---constant---
\langle \env, \base, \emptyset^n \rangle \in \ctrans{\const}(\vec{R}) &\iff& \base \in \Bases \\[1.5ex]

%---function names---
\langle \env, [i\; \env_1], \vec{E} \rangle \in \ctrans{f_i}(\vec{R}) &\iff& 
	\vec{E} = \vecupd{\emptyset^n}{i}{\{\env_1\}} \;\wedge \\[1ex]
\multicolumn{3}{r}{\;\env_1 = \langle \his{}{\emptyset}, \unr, \dots, \unr\rangle} \\[1.5ex]

%---if-then-else---
\langle\env, v, \vec{E}\rangle \in \ctrans{\ifte{e}{e_1}{e_2}}(\vec{R})&\iff& \\[0.5ex]
\multicolumn{3}{l}{\qd\exists v_0, v_1, v_2, \vec{E}_0, \vec{E}_1, \vec{E}_2.\;
			\langle\env, v_0, \vec{E}_0\rangle \in \ctrans{e}(\vec{R}) \;\wedge}\\[0.5ex]	
\multicolumn{3}{l}{\quad\quad\quad \langle\env, v_1, \vec{E}_1\rangle \in \ctrans{e_1}(\vec{R}) 
				\wedge \langle \env, v_2, \vec{E}_2\rangle \in \ctrans{e_2}(\vec{R}) \;\wedge}\\[0.5ex]	

\multicolumn{3}{l}{\qd \Mif v_0  = \bot\;\Mthen v = \bot \wedge \vec{E} = \vec{E}_0 }\\[0.5ex]
\multicolumn{3}{l}{\qd \Melse \Mif v_0 \not \in \{\true, \false\}\;\Mthen v = \omega \wedge \vec{E} = \vec{E}_0}\\[0.5ex]
\multicolumn{3}{l}{\qd \Melse\Mif v_0 = \true \;\Mthen  v = v_1 \wedge \vec{E} = \vec{E}_0 \;\vec{\cup}\; \vec{E}_1} \\[0.5ex]
\multicolumn{3}{l}{\qd \Melse v = v_2 \wedge \vec{E} = \vec{E}_0 \;\vec{\cup}\; \vec{E}_2}\\[2ex]

%---function application---
\langle \env, v, \vec{E}\rangle \in \ctrans{e_1(e_2)}(\vec{R}) &\iff& \exists v_1, v_2, \vec{E}_1, \vec{E}_2.\;\\[0.5ex]	
\multicolumn{3}{c}{\langle \env, v_1, \vec{E}_1\rangle \in \ctrans{e_1}(\vec{R}) \wedge 
				\langle \env, v_2, \vec{E}_2\rangle \in \ctrans{e_2}(\vec{R})  \;\wedge}\\[0.5ex]	


\multicolumn{3}{l}{\qd \Mif v_1  = \bot \vee v_1 = \omega \;\Mthen v = v_1 \wedge \vec{E} = \vec{E}_1}\\[0.5ex]
\multicolumn{3}{l}{\qd \Melse \Mif v_1  \in Base \;\Mthen v = \omega \wedge \vec{E} = \vec{E}_1}\\[0.5ex]
\multicolumn{3}{l}{\qd \Melse \Mif v_2 = \bot \vee v_2 = \omega \;\Mthen v = v_2 \wedge \vec{E} = \vec{E}_1 \;\vec{\cup}\; \vec{E}_2}\\[0.5ex]
\multicolumn{3}{l}{\qd \Melse}\\[0.5ex]

\multicolumn{3}{l}{\qd\qd \Mlet [i\; \langle\his{}{C_0}, \vh_1, \dots, \vh_l, \unr, \dots,\unr\rangle] =v_1 \Min}\\[0.5ex]
\multicolumn{3}{l}{\qd\qd \Mlet \langle v'_2, \vec{E}_3\rangle = }\\[0.5ex]
\multicolumn{3}{l}{\Repeat{3}{\qd} \Mif v_2 \in Base \;\Mthen \langle v_2, \emptyset^n\rangle}\\[0.5ex]
\multicolumn{3}{l}{\Repeat{3}{\qd} \Melse}\\[0.5ex]
\multicolumn{3}{l}{\Repeat{4}{\qd} \Mlet [j\; \langle\his{}{C_0}, \dots, \his{\wz_m}{C_m}, \unr, \dots,\unr\rangle] = v_2 \Min}\\[0.5ex]
\multicolumn{3}{l}{\Repeat{4}{\qd} \Mlet \env_2 = \langle\his{}{C_0}, \dots, \his{\wz_m}{(C_m \cup \{v_1\})}, \unr, \dots,\unr\rangle \Min}\\[0.5ex]
\multicolumn{3}{l}{\Repeat{5}{\qd} \langle  [j\; \env_2], \vecupd{\emptyset^{n}}{j}{\{\env_2\}} \rangle}\\[0.5ex]

\multicolumn{3}{l}{\qd\qd \Min}\\[0.5ex]

\multicolumn{3}{l}{\qd\qd \Mlet \env_1 = \langle\his{}{C_0}, \vh_1, \dots, \vh_l,  \his{v'_2}{\emptyset}, \unr, \dots,\unr\rangle \Min }\\[0.5ex]
\multicolumn{3}{l}{\qd\qd \Mlet \vec{E}_0 = \vec{E}_1 \;\vec{\cup}\; \vec{E}_2 \;\vec{\cup}\; \vec{E}_3 \;\vec{\cup}\; \vecupd{\emptyset^n}{i}{\{\env_1\}} } \\[1ex]
\multicolumn{3}{l}{\Repeat{3}{\qd} \Mif l = k -1 \;\Mthen v \in \lookup{\vecat{\vec{R}}{i}}{\env_1} \wedge \vec{E} = \vec{E}_0}\\[0.5ex]
\multicolumn{3}{l}{\Repeat{3}{\qd} \Melse v = [i\; \env_1] \wedge \vec{E} = \vec{E}_0}
\end{array}\]
\caption{Concrete transformer for the language}
\label{fig:concrete-transformer}
\end{figure}

Before going into the details of the transformer shown in Figure~\ref{fig:concrete-transformer}, 
we first highlight some of its main features. First, program expressions are not evaluated with 
partial inputs/environments.This fact is assumed in the above definition,
but it can be made explicit by adding the $\neg par(\env)$ condition for environments.
This restriction is a simple consequence of the fact that our language
employs call-by-value evaluation strategy. Second, although environments contain history information
for each argument, such histories do not affect the evaluation. Their only purpose is to remember
the information required to model higher-order contracts. Lastly, the definition of the transformer
is compositional and abstracts away from how programs execute step-by-step. 

The function application construct has arguably the most interesting definition. If either
$e_1$ of $e_2$ diverge or return an error, that value is simply propagated as the result. Also, $e_1$ is required
to evaluate to a closure; otherwise error is returned. Next, the environment of the closure of $e_1$ is 
extended with the value $v_2$ of $e_2$. If the extended environment is full, i.e., with no placeholders, 
the result of the whole function application is the value that $\vec{R}$ holds for the underlying function 
on the full environment. If the environment is not full, the result is a new extended closure of $v_1$. 
Additional care needs to be taken if $v_2$ is a closure itself. In that case, the transformer first 
extends $v_2$ with the information that it is being passed to $v_1$, resulting in a new closure $v'_2$. 
Only then is $v_1$ extended with $v'_2$. Also, the transformer saves environments of $v'_2$ and 
extended $v_1$ as observed inputs of their respective functions, although these inputs might be partial. 
We remember partial inputs because Liquid types infer relations between arguments of partial inputs
provided to functions as well. 


\paragraph{Collecting semantics.} 
The collecting semantics $\coll{\cdot}:\Progs \to \Cenvs \to \Crels$ uses the concrete transformer 
to compute the meaning of a program as relation vector $\vec{R}$ that abstracts every function
with a relation.

\[\begin{array}{@{}l}
\coll{f_1\; x_1\cdots x_k =e_1\dots f_n\;x_1\cdots x_k = e_n}(\vec{E_0}) \triangleq \\[1ex]
\mathbf{lfp}^{\vec{\subseteq}}_{\vec{er}(\vec{E_0})}\; \lambda \vec{R}.\; \vec{R} \quad\vec{\cup}\\[1ex]
\multicolumn{1}{r}{\langle rel(e_1, \vec{R}, re(\vecat{\vec{R}}{1})), \dots, rel(e_n, \vec{R}, re(\vecat{\vec{R}}{n}))\rangle \quad\vec{\cup}}\\[1ex]
\multicolumn{1}{r}{er(envs(e_1, \vec{R}, re(\vecat{\vec{R}}{1}))) \;\vec{\cup} \cdots \vec{\cup}\; er(envs(e_n, \vec{R}, re(\vecat{\vec{R}}{n})))}\\[3ex]

er(E) \triangleq \setc{\langle \env, \bot\rangle}{\env \in E}\\[1ex]
re(R) \triangleq \setc{\env}{\langle\env, v\rangle \in R} \\[1ex]
rel(e, \vec{R}, E) \triangleq \setc{\langle \env, v \rangle}{\env \in E \wedge \exists \vec{E}.\;\langle\env, v, \vec{E}\rangle \in \ctrans{e}(\vec{R})} \\[1ex]
envs(e, \vec{R}, E) \triangleq \vec{\bigcup}\; \setc{\vec{E}}{\env \in E \wedge \exists v.\;\langle\env, v, \vec{E}\rangle \in \ctrans{e}(\vec{R})}
\end{array}\]

\noindent Starting with an initial set of inputs $\vec{E}$ for every function, the fixpoint of the 
collecting semantics in each iteration assigns value to every observed function input and adds new 
unseen inputs to the relation. When new inputs are added to a relation, we make they are assigned 
$\bot$. For each function, 
an input environment can hence be assigned non-termination value $\bot$ and potentially the result of 
evaluating the function on the input if the evaluation terminates. This explains the need for 
abstracting functions
by relations, which additionally permits modeling non-deterministic languages. We note that this
semantics would not be suitable for type systems where one is interested in differentiating between
non-terminating and terminating computations. However, conventional type systems including Liquid
types do not make such distinctions.


\paragraph{Environment-set collecting semantics.} Our ultimate goal is to create a refinement type system
that is at the core of mainstream refinement type systems found in practice. As we show formally in
Section~\ref{sec:general-ref}, the meaning of a type environment is a certain set of concrete environments.
To facilitate easier correspondence between abstract (type) and concrete semantics, we modify the 
concrete transformer so it provides meaning to expressions subject to a set of environments instead
of a single environment. A nice feature of this modification is that the new transformer 
$\strans{\cdot}: \Exp \to \Rels^n \to \powerset{\Envs} \to \powerset{\Envs \times Vals \times \powerset{\Envs}^n}$
is now a functional.
%\[\strans{e}(\vec{R})(E) \triangleq \setc{a}{a = \langle\env, v, \vec{E} \rangle \wedge \env \in E \wedge a \in \ctrans{e}(\vec{R})(\env)} \]
The new \textit{environment-set} collecting semantics $\scoll{\cdot}:\Progs \to \Cenvs \to \Crels$,
however, retains the same signature. In the rest of this paper, the term collecting semantics will
exclusively stand for this \textit{environment-set} semantics. The actual definitions of the new transformer
and the collecting semantics are straigftforward extensions of the original versions, so we omit them
in the interest of saving space.









==> liquid.tex <==
% !TEX root = ../thesis.tex
\subsection{Liquid Type Semantics}
\label{sec:liquid-types-ai}

To obtain an instance of our data flow refinement type analysis, one
has to choose a stack abstraction, basic types, the abstract domain of
type refinements and a shape widening operator. We now show how to
obtain Liquid type inference in this manner.

\smartparagraph{Stack abstraction} As liquid type inference is a
context-insensitive analysis, we choose the trivial stack abstraction
$\pstacks=\{\epsilon\}$ introduced in
Example~\ref{ex:collapsed-semantics}. We hence omit abstract stacks in
the notation for refinement tables and just use the usual notation for
dependent function types.

\smartparagraph{Basic types and abstract refinement domains}
The set of basic types consists of types such as $\tint$ and $\tbool$
where the base typing function $\mi{ty}: \consts \to \basetypes$
is implemented by, say, the Hindley-Milner algorithm.
The abstract domain of type refinements $\paramdomain$ is
$\powerset(Q_{\pscope})$ where $Q_{\pscope}$ is a finite set of
logical formulas whose free variables range over $\pscope \cup \{\nu\}$ and that
includes all equality constraints between these variables. The
elements of $\paramdomain$ are interpreted conjunctively and
quotiented by the pre-order induced by entailment modulo some
appropriate decidable first-order theory (e.g., linear arithmetic with
uninterpreted functions as in~\cite{DBLP:conf/pldi/RondonKJ08}). This
quotient forms a complete lattice.
%The domain operations are simply implemented using
%appropriate logical operations. For example,
%$\requality{a}{\nu}{\pnode}$ is $a \land \nu = \pnode$ and
%$\rupdate{a}{\pnode}{a'}$ is $a \land a'[\pnode/\nu]$. 
%Note that
%Liquid Types assume the set of qualifiers $Q$ to include equality
%atoms $\nu = x$ and $x = y$ where $x,y$ can then be instantiated for the
%abstract nodes in each scope. 

\smartparagraph{Domain operations}
The strengthening operations on our Liquid types are defined structurally on types
by relying on the strengthening operations provided by $\paramdomain$. 
These operations correspond to the logical operations used in the original Liquid types work. For
instance, for a refinement domain element $\paramelem$, the operation $\requality{a}{\nu}{x}$ 
yields $a \land \nu = x$ and $\rupdate{a}{x}{a'}$ 
is $a \land a'[x/\nu]$ where $a'[x/\nu]$ is the formula obtained by
syntactically substituting $x$ for $\nu$ in $a'$. 
%Also, Liquid types avoid using the
%rescoping operation in the strengthening operations by renaming dependency
%variables, thus making sure that variables in types are always unique.


\smartparagraph{Widening} First note that the refinement domains
$\paramdomain$ have finite height. The type refinement widening
operator $\paramwid$ is therefore simply the join operator on
$\paramdomain$. Liquid type inference solves the issue of shape
widening by first inferring basic types using standard Hindley-Milner
type inference, which effectively rejects any program where the
nesting depth of tables is unbounded. We could have similarly considered only
programs that are well-typed according to Hindley-Milner in our
general refinement type semantics, thus avoiding the need for shape
widening. However, we designed the data flow refinement semantics so
that it performs the two inference phases simultaneously, thereby not
forcing the analysis to make an a priori decision about how the shapes
of the types of recursive functions should be approximated.  To obtain
Liquid types in our framework, we thus need a shape widening operator
that mimics the approximation of recursive functions performed by the
Hindley-Milner type system on which Liquid type inference is
based. The connection between this approximation and widening is
already known~\cite{cousot1997types} and explored
elsewhere~\cite{monsuez1993polymorphic,gori2003properties,gori2002experiment}.

\smartparagraph{Connection to Liquid typing rules}
The original Liquid type inference is formalized with respect to
typing rules. In the following, we formally relate the fixpoints of our
analysis to the typing derivations obtained by these rules.
%\lessmore{First, we can identify program variables in
%Liquid Types with abstract nodes in the data flow refinement type
%semantics.}{
%First, A-normalization ensures that we can identify program variables in
%Liquid Types with abstract nodes in the data flow refinement type
%semantics.}Thus, a \emph{Liquid scope} $\vec{x}$ corresponds to an
%abstract scope $\pscope$ in our setting. 
The subtyping relation on our Liquid types is defined as 
%
\[\begin{array}{@{}c}
%\tbot \;\liqsub\; \tval \ind[2] \terr \;\liqsub\; \terr \\
\rtype{\basetype}{\paramelem_1} \;\liqsub\; \rtype{\basetype}{\paramelem_2} {\Def\iff} \paramelem_1 \paramord[] \paramelem_2 \\
z{:} \tval_1 {\to} \tval_2 \;\liqsub\; z{:} \tval_3 {\to} \tval_4 {\Def\iff} \tval_3 \,\liqsub\, \tval_1 \wedge \rupdate{\tval_2}{z}{\tval_3} \,\liqsub\, \rupdate{\tval_4}{z}{\tval_3} 
%\tval_1 {<:} \tval_2 \Def\iff {} \tval_1, \tval_2 {\in} \trels \land \basetype(\tval_1) = \basetype(\tval_2) \wedge \paramelem(\tval_1) \paramord[] \paramelem(\tval_2) \;\vee\\ 
%\ind[2]  \tval_1, \tval_2 \in \ttables \wedge \mi{inp}(\tval_2) \,{<:}\, \mi{inp}(\tval_1) \wedge 
%                                        \mi{out}(\tval_1) \,{<:}\, \mi{out}(\tval_2) 
\end{array}\]
%Again, we implicitly assume that dependency variables match when comparing function
%types. Also, we use $\mi{inp}$ and $\mi{out}$ to extract function input and output
%types, respectively. 
%Our subtyping relation coincides with the original one~\cite[p. 6]{DBLP:conf/pldi/RondonKJ08}.
The only difference to the original subtyping relation defined
in~\cite[p. 6]{DBLP:conf/pldi/RondonKJ08} is that we do not need a
typing environment here because we push the constraints imposed on
variables in the environment directly into the type refinements.
%except for the $\tbot$ and $\terr$ types that are not considered by the original Liquid 
%type system. Also, 
The following lemma relates subtyping and propagation between the involved types.
%
%\begin{lemma}~\label{thm:liq-subtyping}
%If $\pair{\tval_1}{\tval_2} = \tprop(\tval_1, \tval_2)$, then $\tval_1 \,{\liqsub}\, \tval_2$.
%\end{lemma}
%
\begin{lemma}~\label{thm:liq-subtyping-prop-fixpoint}
If $\tval_1 \,{\liqsub}\, \tval_2$, then $\pair{\tval_1}{\tval_2} =
\tval_1 \tiprop \tval_2$.
\end{lemma}
%
\noindent We use this fact to show that any valid derivation of a
Liquid typing judgment represents a fixpoint of $\ttransname$, which means
that it the typing rules are sound with respect to our concrete
dataflow semantics. To this end, we first
define Liquid typing judgments $\liqenv \liqtyp e : \tval$ adapted
from~\cite[p. 6]{DBLP:conf/pldi/RondonKJ08}. Here, $\liqenv \in \liqenvs \Def = \vars \rightharpoonup
\tvalues[]$ is a standard typing environment, mapping variables to
Liquid types. The rules defining the judgment relation are given in Fig.~\ref{fig:adapted-lq-rules}.

% We define the typing rules with respect to standard
% typing environments $\liqenv \in \liqenvs \Def = \vars \rightharpoonup
% \tvalues[]$ that map program variables to types. 
% %Given a type map $\tmap$ and an (injective)
% %abstract environment $\penv$, we define an induced type environment 
% %$\liqenv_{\tmap, \penv} \Def= \tmap \circ \penv$ that simply returns a 
% %type in $\tmap$ for every variable in $\penv$. Just as Liquid types, our data 
% %flow refinement type semantics visits every program expression only once. That is, 
% %the body of each lambda expression is always analyzed with the same abstract 
% %environment in each iteration. Due to the uniqueness
% %of program variables in programs of $\Exp$, the (potentially) reachable environment 
% %nodes can thus be precomputed statically and represented using the binding variables 
% %of the lambda expressions, just as in the original Liquid types work. That is, 
% %for every program variable $x$ bound by some lambda abstraction in $p$, we 
% %can compute, based on the syntax tree of $p$, the variable node created for $x$ 
% %by the refinement type semantics, assuming $p$ is analyzed with the initial
% %empty abstract environment $\emptyset$. Let $\kappa_p \in \vars(p) \to \pnodes$ 
% %be such an (injective) mapping from variables of $p$ to their corresponding environment
% %nodes. We use this map to perform type strengthening in typing rules.
% In order to connect the typing rules with the results produced by our abstract
% interpretation, we define the rules subject to an injective mapping 
% $\kappa:\vars \to \pnodes$ from variables to abstract nodes. Let $\liqenvs^{\kappa}$ 
% be the set of liquid typing environments whose domain is $\m{dom}(\kappa)$.
% The abstract scope induced by $\kappa$ is then simply $\pscope_{\kappa} \Def= \m{rng}(\kappa)$.
% Also, the induced abstract environment is
% $\kappa(\liqenv) \Def= \Lambda x \in \m{dom}(\liqenv).\kappa(x)$.
% %We also define the abstract scope induced by $\kappa$ as $\pscope_{\kappa} \Def= \m{rng}(\kappa)$.
% Given an encoding of abstract environment nodes $\kappa$, our Liquid typing relation 
% %$\liqtyp:\Sigma \liqenv \in \liqenvs^{\kappa}.\, \Exp \times \tvalues[\pscope_{\kappa}]$
% $\liqtyp:\Sigma \liqenv \in \liqenvs^{\kappa}.\, \Exp \times \tvalues[\pscope_{\kappa}]$
% is given by the typing rules shown in Figure~\ref{fig:adapted-lq-rules}.
%
\begin{figure}[t]
%\[\begin{array}{c}
%\infer{\liqenv \liqtyp x : \tval}{x \in \m{dom}(\liqenv) & \liqenv(x)\;\liqsub\;\tval} \ind[3]
%
%\infer{\liqenv \liqtyp \const : \tconst[\liqenv]^{\kappa}}{} \\[2ex]
%
%\infer{\liqenv \liqtyp e_1 e_2: \tval}
%{\begin{array}{c c}\liqenv \liqtyp e_1: \tval_1 & \liqenv \liqtyp e_2: \tval_2 \\[0.5ex] \tval_2 \not= \terr & \tval_1 \;\liqsub\; \ptvar(\tval_1)\!:\tval_2 \to \tval\end{array}} \\[2ex]
%
%\infer{\liqenv \liqtyp \mu f \lambda x.\,e : \tval}
%{\begin{array}{c c}\pi_1(\ptio(\tval)) \not\in \{\tbot, \terr\} & \ptvar(\tval)\!:\tval_x \to \tval_1 \;\liqsub\; \tval \\[0.5ex] \tval \;\liqsub\; \tval_f & \liqenv.x:\tval_x.f:\tval_f \liqtyp e:\tval_1\end{array}}
%
%\more{\\[2ex]
%\infer{\liqenv \liqtyp (\ite{x}{e_1}{e_2}): \tval}
%{\begin{array}{c c}
%\liqenv \liqtyp x: \tval_0 \quad \tval_0 \tvord[] \tbools & \tval_1 \,\liqsub\, \tval \quad \tval_2 \,\liqsub\, \tval\\[0.5ex]
%\liqenv_1 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \ttrue}
%&  
%\liqenv_1 \liqtyp e_1: \tval_1 \\[0.5ex] 
%\liqenv_2 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \tfalse}
%& \liqenv_2 \liqtyp e_2: \tval_2
%\end{array}}
%}
%\end{array}\]
\[\begin{array}{c}
% \infer{\liqenv \liqtyp x : \tval}{x \in \m{dom}(\liqenv) & \liqenv(x)\;\liqsub\;\tval & \tval = \rstrengthen{\requality{\liqenv(x)}{\nu}{\kappa(x)}}{\liqenv}^\kappa } \ind[3]
% %
% \infer{\liqenv \liqtyp \const : \tconst[\liqenv]^{\kappa}}{} \\[1.5ex]
\infer{\liqenv \liqtyp x : \tval}{x \in \m{dom}(\liqenv) &
\rstrengthen{\requality{\liqenv(x)}{\nu}{x}}{\liqenv} \liqsub \tval } \ind[3]
%
\infer{\liqenv \liqtyp \const : \tval}{\tconst[\liqenv] \liqsub \tval} \\[1.5ex]
%
\infer{\liqenv \liqtyp e_1 \, e_2 : \exists \absn.\, \tval}
{  \liqenv \liqtyp e_1 : \tval_1 & \liqenv \liqtyp e_2 :
\tval_2 &
   \tval_1 \liqsub \absn\!:\tval_2 \to \tval
}\ind[2]
%
\infer{\liqenv \liqtyp \lambda x.\,e_1 : \tval}
{
\liqenv_1 = \liqenv.x\!:\tval_x & \liqenv_1 \liqtyp e_1 : \tval_1 & x\!:\tval_x \to \tval_1 \liqsub \tval
}

\more{\\[2ex]
\infer{\liqenv \liqtyp (\ite{x}{e_1}{e_2}) : \tval}
{\begin{array}{c c}
\liqenv \liqtyp x: \tval_0 \quad \tval_0 \,\liqsub\, \tbools & \tval_1 \,\liqsub\, \tval \quad \tval_2 \,\liqsub\, \tval\\[0.4ex]
\liqenv_1 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \ttrue}
&  
\liqenv_1 \liqtyp e_1 : \tval_1 \\[0.4ex] 
\liqenv_2 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \tfalse}
& \liqenv_2 \liqtyp e_2 : \tval_2
\end{array}}
}
\end{array}\]
\caption{Adapted Liquid typing rules}
\label{fig:adapted-lq-rules}
\vspace{-1em}
\end{figure}
%
\noindent 
%Here, constant abstractions are defined as 
%$\tconst \Def= \tvalpha(\pconst)$ (or, alternatively,
%as $\tconst \Def= \rtype{\mi{ty}(c)}{\paramtop[\nu=c]}$ where
%We assume we are given an existing base typing function $\mi{ty}: \consts \to \basetypes$
%(e.g., Hindley-Milner) for constants and an existing strengthening operation 
%$\paramelem[\nu=c]$ on type refinements that sets $\nu$ to $\const$ in the concrete
%(implemented as adding a logical conjunct $\nu = c$ to $\paramelem$). 
%We use these operations and $\kappa$ to properly strengthen constants with the
%environment assumptions. That is, 
%We use $\tconst[\liqenv]^{\kappa}$ as a shorthand 
%for $\tconst[\tmap]$ where 
%$\tmap = \Lambda \pnode.\,\ite{\pnode \in \m{rng}(\kappa)}{\liqenv(\kappa^{-1}(\pnode%))}{\tbot}$.

\more{
Apart from the use of $\kappa$, the first obvious difference between our typing rules 
and the original Liquid typing rules is that the rules in the original
paper are nondeterministic: the subtyping rule can be applied at any 
point in the typing derivation. Our rules, on the other hand, are 
deterministic as we directly push subtyping constraints at any point 
where there is a potential flow of data. Second, we assume for simplicity 
that conditionals are A-normalized, as is the case with the original Liquid type inference 
algorithm implementation~\cite[sec. 4.4]{DBLP:conf/pldi/RondonKJ08}.}{
The only notable difference between our typing rules 
and the original Liquid typing rules is that our rules are
deterministic: instead of allowing subtyping to be applied at any
point in a typing derivation, our rules apply subtyping only at those
points where there is an application of $\tprop$ in the data flow semantics.
}

To state the soundness theorem we need one more definition: we say that a typing
environment is \textit{valid} if it does not map any variable to $\tbot$ or $\terr$. 
%\begin{theorem}~\label{thm:liquid-types}
%Let $e^{\ell}$ be a program and $\tmap = \tcoll[e^{\ell}]$.
%If $\tmap$ is safe, then $\epsilon \vdash_{\mi{q}}^{\kappa_p} e : \tmap(\cn{\epsilon}{\ell})$.
%\end{theorem}
\begin{theorem}[Soundness]~\label{thm:liquid-types}
Let $e^{\ell}$ be an expression, $\liqenv$ a valid typing environment, and
$\tval \in \tvalues[]$. If $\liqenv \liqtyp e^{\ell}: \tval$, 
then there exists an environment $\penv$ and a safe type map $\tmap$
such that $\liqenv = \tmap \circ \penv$, $\tval =
\tmap(\cn{\penv}{\ell})$, and $\tmap = \ttrans{e^\ell}(\penv,\epsilon,\tmap)$.
\end{theorem}
%
%
%Here, dependency variables correspond to program variables since the original Liquid Type 
%inference encodes abstract nodes using program variables. 
%The typing relation $\vdash_{\mi{q}}$, discussed in more depth in \S~\ref{sec:lq-typing-rules},
%coincides with the original Liquid typing relation~\cite[p. 6]{DBLP:conf/pldi/RondonKJ08}.
%\noindent The proof goes by showing that one can construct a safe type map from the typing derivation
%corresponding to $\liqenv \liqtyp e^{\ell}: \tval$. This map is then shown to be a fixpoint
%of the abstract transformer.
Theorem~\ref{thm:liquid-types} and
Lemma~\ref{thm:liq-subtyping-prop-fixpoint} can be generalized to
arbitrary domains of type refinements under certain mild assumptions,
such as idempotency of the domain operations.


%\smartparagraph*{Design space}
%We note that our Liquid type inference is sound by construction and
%the points where the analysis loses precision are made explicit in our
%choice of widening operators and Galois connections used in the
%relational, collapsed, and refinement type semantics. This is in
%contrast to the original Liquid types work where the soundness of the
%inference is argued as follows.  Given an expression $e$, a Liquid
%type environment $\Gamma$, and a qualifier set $Q$, it is first shown
%that for a Liquid type $\tau$ inferred by the algorithm
%$\m{Solve}(\Gamma, e, Q)$, the original Liquid typing relation holds
%$\Gamma \vdash_{Q} e : \tau$~\cite[Theorem
%2]{DBLP:conf/pldi/RondonKJ08}.  Then, this relation is shown to be
%conservative subject to an ``exact" typing relation
%$\Gamma \vdash e : \tau$~\cite[Theorem 1]{DBLP:conf/pldi/RondonKJ08},
%which is in turn proven to be sound subject to a standard operational
%semantics elsewhere~\cite{DBLP:conf/esop/KnowlesF07}.  This indirect soundness
%argument obscures where the analysis loses precision. In particular,
%it does not make formally explicit how $\vdash_{Q}$ abstracts $\vdash$ and
%how $\vdash$ abstracts the concrete semantics.



% We next establish the connection between the refinement type abstract transformer $\ttrans[]{\cdot}$ and
% the Liquid Typing relation $\vdash_{Q}$ given by the typing rules found in~\cite{DBLP:conf/pldi/RondonKJ08}.
% Since Liquid Type refinements are predicates in the EUFA logic, we will informally interpret types $\tval$ 
% as logical formulas. Similarly, the interpretation of a Liquid Type $\tval$ in the environment $\liqenv$ is an 
% implication $\bigwedge_{x \in \mathsf{dom}(\liqenv)}[x/\nu]\liqenv(x) \implies \tval$.


% We now apply a sequence of safe transformations to the above rule in order to get the rule Liquid
% Types actually use. First, we A-normalize the expression $e_1 e_2$ to \lstinline+let x1 = e1 in let x2 = e2 in x1 x2+.
% Also, we replace $T$ with $T_o$ in the subtyping requirement in the rule antecedent. This replacement 
% serves as a safe optimization: (1) setting $T$ to $T_o$ clearly satisfies the subtyping requirement 
% as the strongest solution and (2) by the syntax of the language $T$ can only be 
% propagated to other types, i.e., appear on the left hand side of the subtyping checks. Note that we do not implement 
% this optimization in our transformer as it is non-essential. As subtyping corresponds to propagation 
% between types, the actual output type for the whole expression is $\rupdate{\tval_o}{x}{\tval_2}$ by the definition
% of $\tprop$. The new rule is now
% %
% \begin{align*}
% \infer{\liqenv_0 \vdash_{Q} x_1 x_2\!:\exists x.\rupdate{T_o}{x}{T_2}}{\liqenv_0 \vdash_{Q} x_1\!:(x:\tval_x \to \tval_o) & \liqenv_0 \vdash_{Q} x_2\!:\tval_2  & \liqenv_0 \vdash_Q \tval_2 \subtype \tval_x }
% \end{align*}
% %
% where $\liqenv_0 = \liqenv.(x_1\!:(x:\tval_x \to \tval_o)).(x_2\!:\tval_2)$. Since $x$ is not in the current scope of $\liqenv$,
% the type of the whole expression removes $x$ from its implicit
% scope. This is denoted using the existential quantification over
% $x$.
% By the logical view of domain operations mentioned in Section~\ref{sec:arelational},
% $\tval' \Def= \exists x.\rupdate{\tval_o}{x}{\tval_2}$ can be viewed as $\exists x.\tval_o \wedge \tval_2[x/\nu]$.
% By the definition of abstract transformer/typing rule for the case of program variables, we have $\tval_2 \implies x_2 = \nu$.
% This in turn implies that $\tval' \equiv \exists x.\tval_o \wedge \tval_2[x/\nu] \wedge x_2 = x$.
% The last equality makes the existential quantification redundant so $\tval'$ can be simplified to $\tval_o[x_2/x] \wedge \tval_2[x_2/\nu]$.
% Finally, since $x_2:\tval_2 \in \liqenv$ then $\tval_2[x_2/\nu]$ is contained in the environment assumptions so 
% $\tval'$ can be further simplified to $\tval' \equiv [x_2/x]\tval_o$, which is the resulting type used in the rules 
% of the original Liquid Types work.

% We note that the original Liquid typing rule for function application does not rely on A-normalization and it assigns
% the $[e_2/x]\tval_o$ type to the whole function application expression. However, replacing $x$ with an arbitrary expression $e_2$ 
% in the type refinement of $\tval_o$ might not yield a predicate that is an instantiation of the given qualifier set $Q$ 
% or a predicate admissible by SMT solvers. As pointed out in the original work on Liquid Types~\cite{DBLP:conf/pldi/RondonKJ08},
% the actual Liquid Type inference algorithm performs A-normalization so the refinement type of the subexpression 
% $e_2$ is stored in the environment and its information is then used for computing the type of the whole expression, in the
% same style as presented above.
%\begin{comment}
%\smartparagraph*{Shape widening}
%\lessmore{
%We note that the Liquid Type inference first infer basic types
%and only then it infers type refinements. Our data flow refinement semantics
%performs the two inference phases simultaneously, thus not forcing the
%analysis to make an a priori decision about how the shapes of the
%types of recursive functions should be approximated. To obtain Liquid
%Types in our framework, we need a shape widening operator that mimics
%the approximation of recursive functions performed by the
%Hindley-Milner type system on which Liquid Types are based. The
%connection between this approximation and widening is already well
%understood~\cite{cousot1997types}.
%}{
%We note that Liquid Types split the analysis into two phases: (1)
%inferring the shape of types and the constraints on the refinement
%predicates, and (2) solving the constraints to synthesize the
%refinement predicates. For this reason, Liquid Types do not need an
%explicit shape widening operator. Our data flow refinement semantics
%performs the two inference phases simultaneously, thus not forcing the
%analysis to make an a priori decision about how the shapes of the
%types of recursive functions should be approximated. To obtain Liquid
%Types in our framework, we need a shape widening operator that mimics
%the approximation of recursive functions performed by the
%Hindley-Milner type system on which Liquid Types are based. The
%connection between this approximation and widening is already well
%understood~\cite{cousot1997types}. Alternatively, we can mirror the
%two-phase approach of Liquid Types and start the analysis with a type
%map that is already initialized with the shapes inferred by
%Hindley-Milner but where the base type refinements are all set to the
%least element $\parambot$ of the type refinement domain. In this case,
%the shape widening operator simply reduces to join.
%}
%\end{comment}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> monadic.tex <==
\section{Monadic Transformers}

\begin{figure}[t]
\[\begin{array}{@{}l|l}
\begin{array}{@{}l}
%constant
\ttrans{c_\elabel}(\penv, \pstack) \Def= \\
\sind \Mdo \pnode = \cn{\elabel}{\penv} \,\Mend \tenv \mto
\menv(\penv) \,\Mend
\tval' \mto \mupd{\pnode}{\rstrengthen{\tconst}{\tenv}} \\[0.4ex]
\sind \Mreturn \tval'\\[2ex]
%var
\ttrans{x_\elabel}(\penv, \pstack) \Def= \\
\sind \Mdo  \pnode = \cn{\elabel}{\penv} \, \Mend \pnode_x = \penv(x)
\, \Mend \tval \mto \mread{\pnode} \Mend \, \tenv \mto \menv(\penv) \, \\[0.4ex]
\sind[6] \tval' \mto \mupd{\pnode_x,\,
\pnode}{\rstrengthen{\tenv(x)\tvareq{x}}{\tenv} \tiprop \rstrengthen{\tval\tvareq{x}}{\tenv}}\\
\sind \Mreturn \tval'\\[2ex]
%
%function application
\ttrans{(e_\elabela \, e_\elabelb)_\elabel}(\penv, \pstack) \Def=  \\
\sind 	\Mdo  \pnode = \cn{\elabel}{\penv} \,\Mend \pnode_\elabela =
\cn{\elabela}{\penv}
		\,\Mend \pnode_\elabelb = \cn{\elabelb}{\penv} \,
\Mend \tval \mto \mread{\pnode}\\[0.4ex]
\sind[6] \tval_\elabela \mto \ttrans[k]{e_\elabela}(\penv, \pstack) \,\Mend
\massert{\tval_\elabela \in \ttables[]}\\[0.4ex]
\sind[6] \tval_\elabelb \mto \ttrans[k]{e_\elabelb}(\penv, \pstack)\\[0.4ex]
%\ind[2]	\Mif \tval_2 = \tbot \;\Mthen \tmap_2 \;\Melif \tval_2 = \terr \;\Mthen \tmap_{\terr} \;\Melse\\[0.75ex]
\sind[6] \tval'_\elabela,\, \absn:[\tentry{\elabela \pconcat \pstack}{\tval_\elabelb'}{\tval'}] = \tval_\elabela \tiprop
\absn:[\tentry{\elabela \pconcat \pstack}{\tval_\elabelb}{\tval}]\\[0.4ex]
\sind[6] \tval''	\mto \mupd{\pnode_\elabela,\, \pnode_\elabelb,\,
\pnode}{\tval'_\elabela,\, \tval'_\elabelb,\, \tval'}\\[0.4ex]
\sind \Mreturn \tval''
\end{array}
&
%lambda abstraction
\begin{array}{@{}l}
\ttrans{(\lambda x.e_\elabela)_\elabel}(\penv, \pstack) \Def= \\ 
\sind	\Mdo \pnode = \cn{\elabel}{\penv} \,\Mend \tval \mto
\mupd{\pnode}{x:\ttable_{\bot}} \\[0.5ex]
\sind[6] \tval' \mto \Mfor \pstack' \in \tval \;\Mdo \tstepbody(x,
e_\elabela, \pnode, \penv, \tval)\\[0.5ex]
\sind[6] \tval'' \mto \mupd{\pnode}{\tval'}\\[0.5ex] 
\sind[2] \Mreturn \tval'' \\[2ex]
%
%
\tstepbody(x, e_\elabela, \pnode, \penv, \tval)(\pstack') \Def= \\
\sind  \Mdo  \pnode_x = \cns{x}{\penv}{\pstack'} \,\Mend
                  \penv_\elabela = \penv.x\!:\!\pnode_x \,\Mend
\pnode_\elabela = \cn{\elabela}{\penv_\elabela}\\[0.5ex]
%\sind[6] \massert{\tval(\pstack') \neq \terr}\\[0.5ex]
\sind[6] \tval_x \mto \mread{\pnode_x} \,\Mend \tval_\elabela \mto \ttrans[k+1]{e_\elabela}(\penv_\elabela,
\pstack') \\[0.5ex]
\sind[6]  x:[\ttab[\pstack']{\tval_x'}{\tval_\elabela'}], \tval' = x:[\ttab[\pstack']{\tval_x}{\tval_\elabela}] \tiprop \tval(\pstack') \\[0.5ex]
\sind[6]  \_ \mto \mupd{\pnode_x,\, \pnode_\elabela}{\tval'_x,\, \tval'_\elabela} \\[0.5ex]
\sind  \Mreturn \tval'
\end{array}
\end{array}\]
\caption{Abstract transformer for data flow refinement semantics\label{fig:refinement-transformer}}
\vspace{-1em}
\end{figure}

% \begin{figure}[t]
%   \[\ttransname: \Exp \to \pstacks \to \penvironments \to \tmaps \to
%     \tmaps \times \tvalues[]\]
% \[\begin{array}{@{}l|l}
% \begin{array}{@{}l}
% %constant
% \ttrans{c^\elabel}(\pstack) \Def=
% \Mdo \tval \mto \mupd{\elabel}{\tconst} \, \Min \tval \\[2ex]
% %var
% \ttrans{x^\elabel}(\pstack) \Def= \\
% \sind \Mdo \tval_x \mto \mread{x} \Mend \tval \mto \mread{\ell} \\[0.4ex]
% \sind[5]\;  \pair{\tval_x'}{\tval'} =
% \tprop(\requality{\tval_x}{\nu}{x}, \tval) \\[0.4ex] 
% \sind[5]\; \_ \mto \mupd{x}{\tval_x'} \Mend \tval'' \mto
% \mupd{\elabel}{\tval'}\\[.4ex]
% \sind \Min \tval''\\[2ex]
% %
% %function application
% \ttrans{(e_1^{\elabel_1} e_2^{\elabel_2})^\elabel}(\pstack) \Def=  \\
% \sind 	\Mdo \tval_1 \mto \ttrans[k]{e_1}(\pstack) \Mend \massert{\tval_1 \in \ttables[]}\\[0.4ex]
% \sind[5] \tval_2 \mto \ttrans[k]{e_2}(\pstack) \Mend \tval \mto
% \mread{\elabel} \Mend \pstack_1 = \elabel_1 \pconcat \pstack\\[0.4ex]
% %\ind[2]	\Mif \tval_2 = \tbot \;\Mthen \tmap_2 \;\Melif \tval_2 = \terr \;\Mthen \tmap_{\terr} \;\Melse\\[0.75ex]
% \sind[5]	\pair{\tval'_1}{\absn:[\tentry{\pstack_1}{\tval_2'}{\tval'}]} = \tprop(\tval_1,
% \absn:[\tentry{\pstack_1}{\tval_2}{\tval}])\\[0.4ex]
% \sind[5] \_ \mto \mupd{\elabel_1}{\tval_1'} \Mend \_ \mto
% \mupd{\elabel_2}{\tval_2'} \Mend \tval'' \mto \mupd{\elabel}{\tval'}\\[0.4ex]
% \sind \Min \tval''
% \end{array}
% &
% %lambda abstraction
% \begin{array}{@{}l}
% \ttrans{(\lambda x.e_1^{\elabel_1})^{\elabel}}(\pstack) \Def= \\ 
% \sind	\Mdo \absn:\ttable \mto \mupd{\elabel}{\absn:\ttable_{\bot}} \\[0.5ex]
% \sind[5]  \absn:{\ttable}' \mto \Mfor \pcsite \in \ttable \, \Mdo\\[0.5ex] 
% \sind[7]  \massert{\ttable(\ccsite) \neq \terr} \Mend \mbind{x}{\pcsite} \\[0.5ex]
% \sind[7]  \tval_x \mto \mread{x} \Mend \tval_1 \mto \ttrans[k+1]{e_1}(\pcsite)\\[.5ex]
% \sind[7]  \pair{\absn:\ttable_x}{\absn:{\ttable}''} = \tprop\\[0.5ex]
% \sind[9]     (\absn:[\ttab[\pcsite]{\tval_x}{\requality{\tval_1}{\absn}{x}}], \absn:\ttable) \\[0.5ex]
% \sind[7]   \pair{\tval'_x}{\tval'_1} = \ttable_x(\pcsite) \\[0.5ex]
% \sind[7]   \_ \mto \mupd{x}{\tval_x'} \Mend \_ \mto \mupd{\elabel_1}{\tval'_1} \\[0.5ex]
% \sind[5] \Min \absn:{\ttable}''\\[0.5ex]
% \sind[5] \absn:{\ttable}''' \mto \mupd{\elabel}{\absn:{\ttable}'}\\[0.5ex]
% \sind \Min \absn:{\ttable}'''
% %\sind \Min \tmap[\pnode \mapsto \ttable] \tmjoin \tmjoinb_{\pcsite} \;\overline{\tmap}(\pcsite)
% \end{array}
% \end{array}\]
% \caption{Abstract transformer for data flow refinement semantics\label{fig:refinement-transformer}}
% \vspace{-1em}
% \end{figure}

\begin{figure}
  \begin{align*}
    \mread{\pnode} \Def= {} & \Lambda \tmap.\, \pair{\tmap}{\tmap(\pnode)}\\
    \mupd{\pnode}{\tval} \Def= {} & \Lambda \tmap.\, \Mlet \tval'
= \tmap(\pnode) \tvjoin[] \tval \,\Min \pair{\tmap[\pnode \mapsto \tval']}{\tval'}\\
    \menv(\penv) \Def= {} & \Lambda \tmap.\, \pair{\tmap}{\tmap \circ \penv}\\
    \Mfor \pstack \in \ttable \, \Mdo F \Def= {} & \Lambda 
\tmap.\, \tmjoinb_{\pstack \in \ttable} F(\pstack)(\tmap)\\
   \den{\Mdo [] \Mreturn t} \, \Def= {} & \Lambda \tmap.\, \pair{\tmap}{t}\\
   \den{\Mdo v \mto F \Mend \mathit{bs} \, \Min t} \Def= {} & \Lambda \tmap.\, \Mlet
\pair{{\tmap}'}{u} = F(\tmap) \Min\\
& \sind[10] \Mif {\tmap}' = \tmap_\top \, \Mthen
\pair{\tmap_\top}{\terr} \, \Melse \den{\Mdo \mathit{bs} \, \Mreturn t[u/v]}({\tmap}')\\
   \den{\Mdo v = u \Mend \mathit{bs} \, \Mreturn t} \Def= {} & \Lambda \tmap.\,\den{\Mdo \mathit{bs} \, \Mreturn t[u/v]}(\tmap)\\
    \den{\Mdo \massert{P} \Mend \mathit{bs} \, \Min t} \Def= {} & \Lambda \tmap.\, \Mif P
\,\Mthen  \den{\Mdo \mathit{bs} \, \Mreturn t}(\tmap) \, \Melse \pair{\tmap_\top}{\terr}
  \end{align*}
  \caption{Monad transformers for abstract state machine}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> old-defs.tex <==
% !TEX root = main.tex

%language
\newcommand{\labels}[0]{\mathit{Label}}
\newcommand{\expressions}[0]{\mathit{Expr}}
\newcommand{\integers}[0]{\mathit{Int}}
\newcommand{\vars}[0]{\mathit{Var}}
\newcommand{\ifte}[3]{\mathbf{if}\;#1\;\mathbf{then}\;#2\;\mathbf{else}\;#3}
\newcommand{\llabs}[0]{\lambda^l x. e}
\newcommand{\constants}{\mathit{Const}}




%semantics
\newcommand{\dordering}{\sqsubseteq}

\newcommand{\values}[0]{\mathit{Val}}

\newcommand{\dconsts}[0]{\mathit{C}}
\newcommand{\dconst}[0]{\mathit{c}}

\newcommand{\envs}[0]{\mathit{Env}}

\newcommand{\sdomain}[0]{\mathbb{S}}
\newcommand{\properties}[0]{\mathbb{P}}

\newcommand{\semantics}[2]{\mathbf{S}_{#1}|[#2|]}
\newcommand{\ctsemantics}[3]{\mathbf{S}_{#1}^{#2}|[#3|]}

\newcommand{\msemantics}[1]{\mathbf{M}|[#1|]}

\newcommand{\collecting}[1]{\mathbf{C_s}|[#1|]}
\newcommand{\mcollecting}[1]{\mathbf{C_m}|[#1|]}



% concrete refinement type system
\newcommand{\bbool}{\mathbf{bool}}
\newcommand{\bases}{\mathbb{B}}

\newcommand{\reftype}[2]{\langle \nu:#1\;|\;#2\rangle}
\newcommand{\deptype}[2]{x:#1 \to #2}
\newcommand{\crefinement}{\Theta}
\newcommand{\ctop}{\top^c}
\newcommand{\cbot}{\bot^c}

\newcommand{\expsat}[3]{|[#2|]_{#3}^{#1}}

\newcommand{\ctypes}{\mathbb{T}}
\newcommand{\ctype}{t}
\newcommand{\ctord}{\preceq}
\newcommand{\ctords}{<:}
\newcommand{\ctg}{\gamma}
\newcommand{\cta}{\alpha}


\newcommand{\ctenvs}{\mathbb{H}}
\newcommand{\ctenv}{H}
\newcommand{\ctenvord}{\overset{\cdot}{\ctord}}
\newcommand{\ctenvg}{\overset{\cdot}{\ctg}}
\newcommand{\ctenva}{\overset{\cdot}{\cta}}
\newcommand{\ctenvstren}[4]{{#1}^{{#2},{#3}, #4}}

\newcommand{\ctypings}{\mathbb{I}}
\newcommand{\ctyp}{I}
\newcommand{\ctypord}{\overset{\cdot\cdot}{\ctord}}
\newcommand{\ctypg}{\overset{\cdot\cdot}{\ctg}}
\newcommand{\ctypa}{\overset{\cdot\cdot}{\alpha}}


\newcommand{\ctyping}[2]{\mathtt{T}_{#1}|[{#2}|]}
\newcommand{\ctransformer}[2]{\vdash_{#1}^{#2}}





% abstract refinement type system
\newcommand{\prefdomain}{D}
\newcommand{\prefinement}{d}
\newcommand{\ptop}{\top_d}
\newcommand{\pbot}{\bot_d}

\newcommand{\pexpsat}[3]{|#2|_{#3}^{#1}}
%\newcommand{\pexpsat}[2]{|[#1|]^{\prefinement}_{#2}}

\newcommand{\ptypes}{\mathbb{P}}
\newcommand{\ptype}{p}
\newcommand{\ptord}{\leq_p}
\newcommand{\ptg}{\gamma_p}
\newcommand{\pta}{\alpha_p}

\newcommand{\ptenvs}{\mathbb{U}}
\newcommand{\ptenv}{U}
\newcommand{\ptenvord}{\overset{\cdot}{\ptord}}
\newcommand{\ptenvg}{\overset{\cdot}{\ptg}}
\newcommand{\ptenva}{\overset{\cdot}{\pta}}
\newcommand{\ptenvstren}[4]{{#1}^{#2, #3, #4}}

\newcommand{\ptypings}{\mathbb{V}}
\newcommand{\ptyp}{V}
\newcommand{\ptypord}{\overset{\cdot\cdot}{\ptord}}
\newcommand{\ptypg}{\overset{\cdot\cdot}{\ptg}}
\newcommand{\ptypa}{\overset{\cdot\cdot}{\alpha}}







\newcommand{\abstrans}{\mathcal{T}}

\newcommand{\Qualifiers}{\mathcal{Q}}
\newcommand{\qualifiers}{Q}
\newcommand{\qualifier}{q}

\newcommand{\veufa}{\mathtt{ValidEUFA}}


%comments

\newcommand{\zp}[1]{{\color{blue} zvonimir: #1}}
\newcommand{\tw}[1]{{\color{red} thomas: #1}}



%repeat command
\newcommand{\Repeat}[2]{\foreach \n in {1, ..., #1}{#2}}




\newcommand{\anyenv}[0]{\bullet}

%helper functions
\newcommand{\tv}[1]{tv(#1)}
\newcommand{\fpv}[1]{fpv(#1)}
\newcommand{\setc}[2]{\{#1 \mid #2\}}
\newcommand{\pwset}[1]{\mathcal{}}
\newcommand{\powerset}[1]{\mathcal{P}{(#1)}}
\newcommand{\diverge}[2]{divg_{#1}(#2)}
\newcommand{\ite}[3]{(#1 \mathbf{?}\; #2 \;\mathbf{|}\; #3)}
\newcommand{\arrfun}[2]{(#1 \hookrightarrow #2)}
\newcommand{\varen}[2]{[#1/#2]}



==> proofs/c-semantics-inductive-properties.tex <==
\subsubsection{Inductive Properties}

We define inductive properties $P$ of a program $m$ as a set of triples consisting of locations in the program, 
concrete maps, and environments that is closed subject to the concrete transformer $\ctransname$. 
More precisely, given a program $m$, we say that $P  \in \powerset(\locs \times \cmaps \times \cenvironments)$ 
is an \textit{inductive invariant} (of $\ctransname$) if
%
\[(\ell, \cmap, \cenv) \in P \implies (\ell, \ctrans[\fuel]{e^\ell}(\cenv)(\cmap), \cenv) \in P\]
%
where $e^\ell \in m$ and $(e, \cenv)$ is well-formed. We additionally require that
all potential recursive calls of $\ctransname$ for the subexpressions of $e$
are closed subject to $P$, as follows:
%
\begin{itemize}
\item $e^\ell = e_1^{\ell_1} e_2^{\ell_2}$.
\begin{gather*}
\infer
%{(\ell_1, \ctrans[\fuel]{e_1^{\ell_1}}(\cenv)(\cmap), \cenv) \in P_\fuel}
{(\ell_1, \cmap, \cenv) \in P}
{(\ell, \cmap, \cenv) \in P}\\
%
\infer
{(\ell_2, \cmap_1, \cenv) \in P}
{
\begin{array}{c c}
(\ell, \cmap, \cenv) \in P & (\ell_1, \cmap_1, \cenv) \in P \\
\cmap_1 = \ctrans[\fuel]{e_1^{\ell_1}}(\cenv)(\cmap) & \cmap_1(\cn{\cenv}{\ell_1}) \not\in \{\bot, \cerr\}
\end{array}
}
\end{gather*}

%\item $e^\ell = (\ifte{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}})^\ell$.
%\begin{gather*}
%\infer
%{(\ell_0, \cmap, \cenv) \in P}
%{(\ell, \cmap, \cenv) \in P}\\
%
%\infer
%{(\ell_1, \cmap, \cenv) \in P}
%{
%\begin{array}{c c}
% (\ell, \cmap, \cenv) \in P & (\ell_0, \cmap_0, \cenv) \in P \\
%\cmap_0 = \ctrans[\fuel]{e_0^{\ell_0}}(\cenv)(\cmap) & \cmap_0(\cn{\cenv}{\ell_0}) = \btrue
%\end{array}
%}\\
%
%\infer
%{(\ell_2, \cmap, \cenv) \in P}
%{
%\begin{array}{c c}
% (\ell, \cmap, \cenv) \in P & (\ell_0, \cmap_0, \cenv) \in P \\ 
%\cmap_0 = \ctrans[\fuel]{e_0^{\ell_0}}(\cenv)(\cmap) & \cmap_0(\cn{\cenv}{\ell_0}) = \bfalse
%\end{array}
%}
%\end{gather*}

\item $e^\ell = (\mu f.\lambda x. e_1^{\ell_1})^\ell$.
\begin{gather*}
\infer
{(\ell_1, \cmap_1, \cenv_1) \in P}
{
\begin{array}{c}
\begin{array}{c c c}
\cmap(\cn{\ell}{\cenv}) = \ctable & \ccsite \in \ctable & \pi_1(\ctable(\ccsite)) \not\in \{\bot, \cerr\} \\
\cnode_x = \cvn{\cenv}{\ccsite}{x} & \cnode_f = \cvn{\cenv}{\ccsite}{f} & \cenv_1 = \cenv.x\!:\cnode_x.f\!:\cnode_f \\
\end{array}\\
\begin{array}{c}
\pair{\ctable'_x}{\ctable'} = \cprop([\ccsite \mapsto \pair{\cmap(\cnode_x)}{\cmap(\cn{\cenv_1}{\ell_1})}], \ctable)\\
\pair{\ctable''}{\ctable'_f} = \cprop(\ctable, \cmap(\cnode_f)) \ind[2] \pair{\cval'_x}{\cval'_1} = \ctable'x(\ccsite) \\
\cmap_1 = \cmap[\cn{\cenv}{\ell} \mapsto \ctable' \cvjoin \ctable'', \cnode_x \mapsto \cval'_x, \cnode_f \mapsto \ctable'_f, \cn{\cenv_1}{\ell_1} \mapsto \cval'_1]\\
(\ell, \cmap, \cenv) \in P
\end{array}
\end{array}
}
%\\
%
%\infer
%{(\ell_1, \ctrans[\fuel]{e_1^{\ell_1}}(\cenv_1)(\cmap_1), \cenv_1) \in P_\fuel}
%{
%\begin{array}{c}
%\begin{array}{c c c}
%\cmap(\cn{\ell}{\cenv}) = \ctable & \ccsite \in \ctable & \pi_1(\ctable(\ccsite)) \not\in \{\bot, \cerr\} \\
%\cnode_x = \cvn{\cenv}{\ccsite}{x} & \cnode_f = \cvn{\cenv}{\ccsite}{f} & \cenv_1 = \cenv.x\!:\cnode_x.f\!:\cnode_f \\
%\end{array}\\
%\begin{array}{c}
%\pair{\ctable'_x}{\ctable'} = \cprop([\ccsite \mapsto \pair{\cmap(\cnode_x)}{\cmap(\cn{\cenv_1}{\ell_1})}], \ctable)\\
%\pair{\ctable''}{\ctable'_f} = \cprop(\ctable, \cmap(\cnode_f)) \ind[2] \pair{\cval'_x}{\cval'_1} = \ctable'x(\ccsite) \\
%\cmap_1 = \cmap[\cn{\cenv}{\ell} \mapsto \ctable' \cvjoin \ctable'', \cnode_x \mapsto \cval'_x, \cnode_f \mapsto \ctable'_f, \cn{\cenv_1}{\ell_1} \mapsto \cval'_1]\\
%(\ell, \cmap, \cenv) \in P_{\fuel + 1} \ind[4] (\ell_1, \cmap_1, \cenv_1) \in P_\fuel
%\end{array}
%\end{array}
%}
%
\end{gather*}
\end{itemize}
%
Given a program $e^\ell$, we define its \textit{strongest inductive invariant} $I$ as the smallest inductive property
of $e^\ell$ such that $(\ell, \cmap_\bot, \emptyset) \in I$.




==> proofs/c-semantics-properties.tex <==
% !TEX root = ../../thesis.tex
\paragraph{Additional Properties}
\label{sec:proofs-c-semantics-additional}

We now introduce and prove several interesting properties related to the concrete data flow semantics.


\paragraph{Finiteness}
\newcommand{\cfin}{\m{fin}}

We say a value $\cval$ is finite $\cfin(\cval)$ if it is either a ground value or a table
that has seen only a finite number of inputs.
%
\begin{align*}
\cfin(\cval) \Def= & (\cval \in \{\bot, \cerr\} \cup \consts) \vee (\cval \in \ctables \wedge |\setc{\ccsite}{\ccsite \in \cval}| \in \mathbb{N} \;\wedge\\
&\ind[11] \forall \ccsite \in \cval.\, \cfin(\pi_1(\cval(\ccsite))) \wedge \cfin(\pi_2(\cval(\ccsite))))
\end{align*}
%
It can be shown that $\cprop$ does not affect the finiteness of values. The same clearly holds for joins $\cvjoin$.
%
\begin{lemma}~\label{thm:c-val-finite-prop}
Let $\cval_1$, $\cval_2$, $\cval_3$, and $\cval_4$ be values. If $\cfin(\cval_1)$, $\cfin(\cval_2)$,
and $\pair{\cval_3}{\cval_4} = \cprop(\cval_1, \cval_2)$, then $\cfin(\cval_3)$ and $\cfin(\cval_4)$.
\end{lemma}
\begin{proof}
By structural induction on $\cval_1$ and $\cval_2$. The cases when either $\cval_1$ or $\cval_2$ are not
a table are trivial. For tables, the argument follows by i.h.\ and the simple fact that $\cprop$ does not
invent new call site nodes, yet only manipulates the existing ones, whose total number is finite by the lemma assumption.
\end{proof}
%
We say a map $\cmap$ is finite $\cfin(\cmap)$ if all of its values are finite and the set of reachable nodes is finite as well
$|\setc{\cnode}{\cmap(\cnode) \not= \bot}| \in \mathbb{N}$. It can be shown that $\ctransname$ preserves
the finiteness of maps.
%
\begin{lemma}~\label{thm:c-step-finite}
Let $\cmap$ and $\cmap'$ be maps, $\cenv$ an environment, and $e^\ell$ an expression. If $\cfin(\cmap)$,
$(e, \cenv)$ is well-formed, and $\ctrans[\fuel]{e^\ell}(\cenv)(\cmap) = \cmap'$, then $\cfin(\cmap')$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. The argument follows from the
Lemma~\ref{thm:c-val-finite-prop}. Note that in the case $e$ is a lambda abstraction and $\cmap(\cn{\cenv}{\ell}) = \ctable$, 
for some table $\ctable$, the set of $\ccsite$ in $\ctable$ is finite. Hence, the set $\overline{\cmap}$ is finite and by 
i.h.\ each $\cmap' \in \overline{\cmap}$ is finite as well. The result then follows from the basic properties of joins.
\end{proof}



\paragraph{Computation Range}

\newcommand{\cerange}{\m{erange}}
\newcommand{\crange}{\m{range}}

We define an \textit{expression range} of an expression node $\cn{\cenv}{\ell}$ subject to a program $p$ to be a set of
expression nodes whose location is a sublocation of $\ell$ in $p$ and whose environment is an extension of $\cenv$
%
\[\cerange_p(\cn{\cenv}{\ell}) \Def= \setc{\cn{\cenv'}{\ell'}}{\cenv \subseteq \cenv' \wedge \ell' \in \locs(p(\ell))}. \]
%
The corresponding \textit{range} is then defined as 
\[ \crange_p(\cn{\cenv}{\ell}) \Def= \cerange_p(\cn{\cenv}{\ell}) \cup \setc{\cvnode}{\cvnode \in \m{rng}(\cenv') \wedge \cn{\cenv'}{\_} \in \cerange_p(\cn{\cenv}{\ell}))} \]
%
Note that in the above definition we use the $\_$ pattern to existentially quantify a certain object instead of explicitly
writing down the quantifier. We do this to avoid clutter.


\newcommand{\domvalid}{\m{domvalid}}
Let domain validity $\domvalid(\ell, p, \cenv)$ of an environment $\cenv$ subject to program $p$ and a location
$\ell$ in $p$ holds iff $\m{dom}(\cenv)$ consists of exactly all variables bound above $\ell$ in $p$. We use this
definition to characterize the range of a computation performed by $\ctransname$.
%

\begin{lemma}~\label{thm:c-frame}
Let $\cmap$ and $\cmap'$ be maps, $\cenv$ an environment, and $e^\ell$ an expression of a program $p$. 
If $\domvalid(\ell, p, \cenv)$ and $\ctrans[\fuel]{e^\ell}(\cenv)(\cmap) = \cmap'$, then 
$\forall \cnode. \cmap(\cnode) \not = \cmap'(\cnode) \implies \cnode \in \crange_p(\cn{\cenv}{\ell})$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. The domain validity assumption
together with the uniqueness of locations in $p$ guarantees that environments are always extended, i.e., their contents
never get rewritten by environment updates done when analyzing the bodies of lambda abstraction, which is needed in order
to ensure that updated nodes are in the $\cerange$ of the current node.
\end{proof}

We now state few properties relating ranges. First, ranges of non-related expression do not share visited expression nodes.
\begin{lemma}~\label{thm:c-disjoint-1}
Let $\cenv$ be an environment, $p$ be a program, $\ell_1$ and $\ell_2$ two locations such that $\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$.
Then, $\crange_p(\cn{\cenv}{\ell_1}) \cap \crange_p(\cn{\cenv}{\ell_2}) \cap \cenodes = \emptyset$.
\end{lemma}
\begin{proof}
Follows directly from $\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$.
\end{proof}
%
Similarly, the ranges of nodes whose environments are non-related do not have any common expression nodes.
%
\begin{lemma}~\label{thm:c-disjoint-2}
Let $\cenv_1$ and $\cenv_2$ be two environments and $\ell$ a location of a program $p$.
If $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$ and $\cenv_1 \not= \cenv_2$, then 
$\crange_p(\cn{\cenv}{\ell_1}) \cap \crange_p(\cn{\cenv}{\ell_2}) \cap \cenodes = \emptyset$.
\end{lemma}
\begin{proof}
The argument follows from the fact that the extensions of $\cenv_1$ and $\cenv_2$ have to be different as
$\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$ and environments are modeled as functions.
\end{proof}


\paragraph{Refined Range}
\newcommand{\ceranger}{\m{eranger}}
\newcommand{\cranger}{\m{ranger}}
We can also give a more refined definition of a range.
%
\begin{align*}
\ceranger_p(\cn{\cenv}{\ell}) \Def={} & \mathbf{lfp}^{\subseteq}_{\{\cn{\cenv}{\ell}\}} \lambda L.\,L \cup \{\cn{\cenv'}{\ell'} \mid \ell' \in \locs(p(\ell)) \wedge \cenv \subseteq \cenv' \wedge \forall \cvnode \in \m{rng}(\cenv'{\setminus}\cenv).\\
&\ind[6] \exists \cnode'\in L.\, \nenv(\cvnode) = \nenv(\cnode') \wedge \nloc(\cvnode) \in \locs(p(\ell))\}
\end{align*}
%
The corresponding \textit{range} is then defined as expected
\[ \cranger_p(\cn{\cenv}{\ell}) \Def= \ceranger_p(\cn{\cenv}{\ell}) \cup \setc{\cvnode}{\cvnode \in \m{rng}(\cenv') \wedge \cn{\cenv'}{\_} \in \ceranger_p(\cn{\cenv}{\ell}))} \]
%
The same result about the range of computation can be shown.
\begin{lemma}~\label{thm:c-framer}
Let $\cmap$ and $\cmap'$ be maps, $\cenv$ an environment, and $e^\ell$ an expression of a program $p$. 
If $\domvalid(\ell, p, \cenv)$ and $\ctrans[\fuel]{e^\ell}(\cenv)(\cmap) = \cmap'$, then 
$\forall \cnode. \cmap(\cnode) \not = \cmap'(\cnode) \implies \cnode \in \cranger_p(\cn{\cenv}{\ell})$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-frame}.
\end{proof}
%
However, something stronger can be said about the disjointness.
\begin{lemma}~\label{thm:c-disjointr-1}
Let $\cenv$ be an environment, $p$ be a program, $\ell_1$ and $\ell_2$ two locations such that $\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$.
Then, $\crange_p(\cn{\cenv}{\ell_1}) \cap \crange_p(\cn{\cenv}{\ell_2}) = \rng(\cenv)$.
\end{lemma}
\begin{proof}
Expression nodes of both ranges are clearly different by $\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$.
The environment nodes $\cvnode$ not in $\rng(\cenv)$ must have the associated variable $\nloc(\cvnode)$ from 
$\locs(p(\ell_1))$ and $\locs(p(\ell_2))$, respectively. The result then again follows from 
$\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$.
\end{proof}
%
Similarly, the ranges of nodes whose environments are non-related have the same property.
%
\begin{lemma}~\label{thm:c-disjointr-2}
Let $\cenv_1$ and $\cenv_2$ be two environments and $\ell$ a location of a program $p$.
If $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$ and $\cenv_1 \not= \cenv_2$, then 
$\crange_p(\cn{\cenv}{\ell_1}) \cap \crange_p(\cn{\cenv}{\ell_2}) = \rng(\cenv_1) \cap \rng(\cenv_2)$.
\end{lemma}
\begin{proof}
The environment nodes $\cvnode$ in both ranges must have the associated environment $\nenv(\cvnode)$  equal to the
environment of some expression node in the corresponding range. These environments are by definition the extensions 
of $\cenv_1$ and $\cenv_2$, respectively, that have to be different as $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$ and 
environments are modeled as functions. Hence, the only shared nodes are those environment nodes that appear in
both $\cenv_1$ and $\cenv_2$.
\end{proof}








\paragraph{Environment Consistency}

\newcommand{\envcons}{\m{envcons}}
We next formalize the notion of environment consistency for a map that states
that no node can be visited with an environment holding a $\bot$ or $\cerr$ value.
%
\[\envcons(\cmap) \Def\iff \forall \cnode, \cnode_x \in \rng(\nenv(\cnode)).\,\cmap(\cnode)\not=\bot \implies  \cmap(\cnode_x) \not \in \{\bot, \cerr\}\]
%
Additionally, we also define consistency of an environment $\cenv$ subject to a map $\cmap$
%
\[\envcons_\cmap(\cenv) \Def\iff \forall \cnode_x \in \rng(\cenv).\, \cmap(\cnode_x) \not \in \{\bot, \cerr\}\]




\paragraph{Table IO Consistency}

\newcommand{\tiocons}{\m{tiocons}}
We next formalize the notion of input output consistency for tables.
%
\begin{align*}
\tiocons(\cval) \Def\iff & (\cval {\in} \{\bot, \cerr\} \cup \consts) \vee (\cval {\in} \ctables \wedge \forall \ccsite {\in} \cval.
\pi_1(\cval(\ccsite)){=}\bot {\implies} \pi_2(\cval(\ccsite)){=}\bot \\
&\ind[5]  \wedge\; \forall \ccsite \in \cval.\, \tiocons(\pi_1(\cval(\ccsite))) \wedge \tiocons(\pi_2(\cval(\ccsite))))
\end{align*}
%
As expected, a map is input-output consistent $\tiocons(\cmap)$ if all of its values are IO consistent.



\paragraph{Constant Consistency}

\newcommand{\constcons}{\m{constcons}}
We next formalize the notion of constant consistency that intuitively states that reachable nodes corresponding
to constant and lambda expression must be either constants and tables, respectively, or an error value. Let $p$ be a program.
A map $\cmap$ is constant consistent $\constcons_p(\cmap)$ if for every node $\cnode$, where $\cmap(\cnode) = \cval$ and
$\nloc(\cnode) = \ell$, it must be
%
\begin{align*}
\cval \in \{\cerr,\bot, \const\} && \text{if } p(\ell) = c \\
\cval \in \{\cerr,\bot\} \cup \ctables && \text{if } p(\ell) = \mu f. \lambda x.e
\end{align*}
%

\paragraph{Error Consistency}

\newcommand{\noerr}{\m{noerr}}
We continue by formalizing the notion of the error absence of values that intuitively states the a given value is not an error
and, if it is a table, it does not recursively contain errors.
%
\begin{align*}
\noerr(\cval) \Def\iff & (\cval \in \{\bot\} \cup \consts) \vee (\cval \in \ctables \wedge \forall \ccsite \in \cval.\\
& \ind[10] \noerr(\pi_1(\cval(\ccsite))) \wedge \noerr(\pi_2(\cval(\ccsite))))
\end{align*}
%

\newcommand{\errcons}{\m{errcons}}
\noindent A map $\cmap$ is error consistent $\errcons(\cmap)$ if either (1) $\cmap = \cmap_\cerr$ or 
(2) for every node $\cnode$ it must be that $\noerr(\cmap(\cnode))$.




\paragraph{Concrete Subtyping}

\newcommand{\csub}{{<:}^c}
Next, we introduce the notion of subtyping for our concrete values that resembles the subtyping on types.
%
\begin{align*}
\cval_1 \csub \cval_2 \Def\iff & (\cval_2 = \bot) \vee (\cval_1 = \cval_2 \wedge \cval_1 \in \{\cerr\}\cup \consts ) \vee 
(\cval_1 \in \ctables \wedge \cval_2 \in \ctables \;\wedge\\ 
& \forall \ccsite \in \cval_2.\,\pi_1(\cval_2(\ccsite)) \csub \pi_1(\cval_1(\ccsite)) \wedge \pi_2(\cval_1(\ccsite)) \csub \pi_2(\cval_2(\ccsite)))
\end{align*}
%
\newcommand{\cmsub}{\m{csub}}
A map $\cmap$ is subtype consistent $\cmsub_p(\cmap)$, subject to a program $p$, iff for every node $\cnode$, where $\nloc(\cnode) = \ell$, it must be that
%
\begin{align*}
\cmap(\nenv(\cnode)(x)) \csub \cmap(\cnode) \ind[4] \textbf{if } p(\ell) = x \textbf{ and } x \in \m{dom}(\nenv(\cnode))\\[1ex]
%
\cmap(\cn{\nenv(\cnode)}{\ell_1}) \csub [\cn{\nenv(\cnode)}{\ell_1} \mapsto \pair{\cmap(\cn{\nenv(\cnode)}{\ell_2})}{\cmap(\cnode)}] \ind[5]\\ 
\ind[3] \textbf{if } p(\ell) = (e_1^{\ell_1} e_2^{\ell_2}) \textbf{ and } \cmap(\cn{\nenv(\cnode)}{\ell_1}) \in \ctables \\[1ex]
%
%\cmap(\cn{\nenv(\cnode)}{\ell_1}) \csub \cmap(\cnode) \ind[19]\\ 
%\ind[3] \textbf{if } p(\ell) = (\ifte{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}}) \textbf{ and } \cmap(\cn{\nenv(\cnode)}{\ell_0}) = \btrue \\[1ex]
%
%\cmap(\cn{\nenv(\cnode)}{\ell_2}) \csub \cmap(\cnode) \ind[19]\\ 
%\ind[3] \textbf{if } p(\ell) = (\ifte{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}}) \textbf{ and } \cmap(\cn{\nenv(\cnode)}{\ell_0}) = \bfalse \\[1ex]
%
\cmap(\cnode) \csub \cmap(\cnode_f) \wedge [\ccsite \mapsto \pair{\cmap(\cnode_x)}{\cmap(\cn{\cenv_1}{\ell_1})}] \csub \cmap(\cnode) \ind[5]\\ 
\ind[3] \textbf{if } p(\ell) = (\mu f.\lambda x. e_1^{\ell_1}),\,\cmap(\cnode) \in \ctables\,,\ccsite \in \cmap(\cnode),\,\\
\ind[3] \cvnode_x = \cvn{\nenv(\cnode)}{\ccsite}{x},\,\cvnode_f = \cvn{\nenv(\cnode)}{\ccsite}{f}, \textbf{ and } \cenv_1 = \nenv(\cnode).x:\cvnode_x.f:\cvnode_f
\end{align*}

We can also show that propagation does not invalidate subtyping.
\begin{lemma}~\label{thm:c-prop-sub}
Let $\cval_1 \in \cvalues$, $\cval_2 \in \cvalues$, $\cval_3 \in \cvalues$, and $\cval_4 \in \cvalues$.
If $\cval_1 \csub \cval_2$ and $\pair{\cval_3}{\cval_4} = \cprop(\cval_1, \cval_2)$, then 
$\cval_3 \csub \cval_4$.
\end{lemma}
\begin{proof}
By structural induction on $\cval_1$ and $\cval_2$.
\end{proof}

\begin{lemma}~\label{thm:c-prop-sub-no-err-bot}
Let $\cval_1 \in \cvalues$, $\cval_2 \in \cvalues$, $\cval_3 \in \cvalues$, and $\cval_4 \in \cvalues$.
If $\cval_1 \csub \cval_2$ , $\cval_1 \not\in \{\bot, \cerr\}$, and
$\pair{\cval_3}{\cval_4} = \cprop(\cval_1, \cval_2)$, then $\cval_3 \not\in \{\bot, \cerr\}$
and $\cval_4 \not\in \{\bot, \cerr\}$.
\end{lemma}
\begin{proof}
Immediate from the definition of $\cprop$.
\end{proof}
%
We can even say something stronger.
\begin{lemma}~\label{thm:c-prop-sub-noerr}
Let $\cval_1 \in \cvalues$, $\cval_2 \in \cvalues$, $\cval_3 \in \cvalues$, and $\cval_4 \in \cvalues$.
If $\cval_1 \csub \cval_2$ , $\noerr(\cval_1)$, $\noerr(\cval_2)$, and
$\pair{\cval_3}{\cval_4} = \cprop(\cval_1, \cval_2)$, then $\noerr(\cval_3)$ and $\noerr(\cval_4)$.
\end{lemma}
\begin{proof}
By structural induction on $\cval_1$ and $\cval_2$. The base cases are trivial.
For the induction case where both $\cval_1$ and $\cval_2$ are tables, the argument follows
by the i.h.
\end{proof}

\paragraph{Dataflow Invariant}
\newcommand{\dfinv}{df}
We say a map $\cmap$ is data flow consistent subject to a program $p$ if it satisfies the invariant
$\dfinv_p(\cmap)$ iff
%
\[ \cfin(\cmap) \wedge \cmsub_p(\cmap) \wedge \errcons(\cmap) \wedge \tiocons(\cmap) \wedge \constcons_p(\cmap) \wedge \envcons(\cmap)\]
%

%\begin{lemma}~\label{thm:c-dfinv-inductive}
%Let $e^\ell$ be an expression of a program $p$, $\cmap' \in \cmaps$, $\cmap$ a map such that 
%$\dfinv_p(\cmap)$, $\fuel \in \fuels$, and $\cenv$ an environment where $\envcons_\cmap(\cenv)$, $(e, \cenv)$ is well-formed, and 
%$\domvalid(\ell, p, \cenv)$. If $\ctrans[\fuel]{e^\ell}(\cenv)(\cmap) = \cmap'$, then $\dfinv_p(\cmap')$
%and $\errcons_{\cmap'}(\cenv)$.
%\end{lemma}


\paragraph{Constant Compatibility}

\newcommand{\constcomp}{\m{ccomp}}
We next introduce formally the notion of constant compatibility between two concrete values
that intuitively states that the join of values does not introduce error values. 
%
\begin{align*}
\constcomp(\cval_1,  \cval_2) \Def\iff & (\cval_1 \in \{\bot, \cerr\}) \vee (\cval_2 \in \{\bot, \cerr\}) \vee (\cval_1 {\in} \consts \wedge \cval {\in} \consts \wedge \cval_1 {=} \cval_2) \\
& \vee (\cval_1 \in \ctables \wedge \cval_2 \in \ctables \wedge
 \forall \ccsite.\,\constcomp(\pi_1(\cval_2(\ccsite)), \pi_1(\cval_1(\ccsite))) \;\wedge\\ 
&\ind[3] \constcomp(\pi_2(\cval_1(\ccsite)), \pi_2(\cval_2(\ccsite))))
\end{align*}
%
We also raise the definition of constant compatibility to a set of values $V$ in the expected
way $\constcomp(V) \Def\iff \forall \cval_1, \cval_2 \in V.\,\constcomp(\cval_1, \cval_2)$.
Note that constant compatibility is a reflexive relation.
%
\begin{lemma}~\label{thm:const-comp-reflexive}
Let $\cval$ be a concrete value. Then, $\constcomp(\cval, \cval)$.
\end{lemma}
\begin{proof}
By structural induction on $\cval$.
\end{proof}
%
Next, we say that two maps $\cmap_1$ and $\cmap_2$ are constant compatible 
$\constcomp(\cmap_1, \cmap_2)$ iff $\forall \cnode.\,\constcomp(\cmap_1(\cnode), \cmap_2(\cnode))$.
Given a set of maps $\hat{M}$, we define its constant compatibility
$\constcomp(\hat{M})$ as $\forall \cmap_1 \in \hat{M}, \cmap_2 \in \hat{M}.\,\constcomp(\cmap_1, \cmap_2)$.

Constant compatibility preserves error consistency of maps over joins.
\begin{lemma}~\label{thm:const-comp-errcons}
Let $\cmap_1$ and $\cmap_2$ be two concrete maps such that $\constcomp(\cmap_1, \cmap_2)$,
$\errcons(\cmap_1)$, and $\errcons(\cmap_2)$. Then, $\errcons(\cmap_1 \cmjoin \cmap_2)$.
\end{lemma}
\begin{proof}
By the definition of $\constcomp(\cval_1, \cval_2)$ on values $\cval_1$ and $\cval_2$, the
join $\cval_1 \cvjoin \cval_2$ cannot introduce errors. That is, if $\noerr(\cval_1)$ and
$\noerr(\cval_2)$, then $\noerr(\cval_1 \cvjoin \cval_2)$. This can be easily shown by structural
induction on $\cval_1$ and $\cval_2$. The result then follows directly from the lemma assumptions.
\end{proof}

A similar result can be shown in the other direction.
\begin{lemma}~\label{thm:errcons-const-comp}
Let $\cmap$, $\cmap_1$, and $\cmap_2$ be concrete maps such that $\cmap = \cmap_1 \cmjoin \cmap_2$.
If $\errcons(\cmap)$ and $\cmap \not= \cmap_\cerr$, then $\constcomp(\cmap_1, \cmap_2)$, 
$\errcons(\cmap_1)$, and $\errcons(\cmap_2)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:const-comp-errcons}.
\end{proof}
%
Clearly, the above result can be lifted to an arbitrary finite join of maps.
%
\begin{lemma}~\label{thm:errcons-const-comp-maps}
Let $\hat{\cmap}$ be a finite set of concrete maps. If $\errcons(\cmjoin \hat{\cmap})$ and 
$\cmjoin \hat{\cmap} \not= \cmap_\cerr$, then $\constcomp(\hat{\cmap})$
and $\forall \cmap \in \hat{\cmap}.\,\errcons(\cmap)$.
\end{lemma}
\begin{proof}
By induction on $|\hat{\cmap}|$. The argument follows almost directly from 
Lemma~\ref{thm:errcons-const-comp}.
\end{proof}

We next show that constant compatibility is preserved by $\cprop$ of value chains.
\begin{lemma}\label{thm:sub-prop-ccomp}
Let $\cval_1 \in \cvalues$, $\cval_2 \in \cvalues$, $\cval_3 \in \cvalues$,
$\cval'_1 \in \cvalues$, $\cval'_2 \in \cvalues$, $\cval''_2 \in \cvalues$ , 
and $\cval'_3 \in \cvalues$.
If $\cval_1 \csub \cval_2$, $\cval_2 \csub \cval_3$,
$\pair{\cval'_1}{\cval'_2} = \cprop(\cval_1, \cval_2)$, and 
$\pair{\cval''_2}{\cval'_3} = \cprop(\cval_2, \cval_3)$, then $\constcomp(\cval'_2, \cval''_2)$. 
\end{lemma}
\begin{proof}
By structural induction on $\cval_2$. We first cover the base cases.
\begin{itemize}
\item $\cval_2 = \bot$. Then, $\cval_3 = \bot$ and hence $\cval''_2 = \bot$ by the def.\
      of $\cprop$.
\item $\cval_2 = \const$. By $\csub$, $\cval_1 = \const$ and $\cval_3 = \const \vee \cval_2 = \bot$.
       Therefore, $\cval'_2 = \cval''_2 = \const$.
\item $\cval_2 = \cerr$. By $\csub$, $\cval_1 = \cerr$ and $\cval_3 = \cerr \vee \cval_2 = \bot$.
       Therefore, $\cval'_2 = \cval''_2 = \cerr$.
\end{itemize}
%
Let us now consider the case when $\cval_2 \in \ctables$. By $\csub$, it must be that
$\cval_1 \in \ctables$. If $\cval_3 = \bot$, then $\cval''_2 = \cval_2$ and 
$\cval'_2 = \cval_2 \cvord \cval'_2$ by Lemma~\ref{thm:c-prop-increase}. The result then follows
trivially. Hence, we are left with the case where $\cval_3 \in \ctables$.
Let us focus on any call site $\ccsite$ and let 
$\cval_1(\ccsite) = \pair{\cval_{1i}}{\cval_{1o}}$,
$\cval_2(\ccsite) = \pair{\cval_{2i}}{\cval_{2o}}$, and
$\cval_3(\ccsite) = \pair{\cval_{3i}}{\cval_{3o}}$.
By the def.\ of $\cprop$, we have that $\cval'_1 \in \ctables$,
$\cval'_2 \in \ctables$, $\cval''_2 \in \ctables$, and $\cval'_3 \in \ctables$.
Let then
$\cval'_1(\ccsite) = \pair{\cval'_{1i}}{\cval'_{1o}}$,
$\cval'_2(\ccsite) = \pair{\cval'_{2i}}{\cval'_{2o}}$,
$\cval''_2(\ccsite) = \pair{\cval''_{2i}}{\cval''_{2o}}$, and
$\cval'_3(\ccsite) = \pair{\cval'_{3i}}{\cval'_{3o}}$. 
By the def.\ of $\cprop$, we have to only consider the cases of 
whether $\ccsite \in \cval_2$ and $\ccsite \in \cval_3$.
\begin{itemize}
\item $\ccsite \not\in \cval_2, \ccsite \not\in \cval_3$. By the def.\ of $\cprop$,
          we have $\cval'_{2i} = \cval''_{2i} = \cval_{2i}$ and
          $\cval'_{2o} = \cval''_{2o} = \cval_{2o}$. The argument is then straightforward.

\item $\ccsite \not\in \cval_2, \ccsite \in \cval_3$. By the def.\ of $\cprop$, we have 
          $\cval'_{2i} = \cval_{2i}$ and $\cval'_{2o} = \cval_{2o}$. By 
          Lemma~\ref{thm:c-prop-increase}, we have $\cval_{2i} \cvord \cval''_{2i}$ and 
          $\cval_{2o} \cvord \cval''_{2o}$. The argument then follows easily.

\item $\ccsite \in \cval_2, \ccsite \not\in \cval_3$. By the def.\ of $\cprop$, we have 
          $\cval''_{2i} = \cval_{2i}$ and $\cval''_{2o} = \cval_{2o}$. By 
          Lemma~\ref{thm:c-prop-increase}, we have $\cval_{2i} \cvord \cval'_{2i}$ and 
          $\cval_{2o} \cvord \cval'_{2o}$. The argument then follows easily.


\item $\ccsite \in \cval_2, \ccsite \in \cval_3$. First, by $\csub$ we have
          $\cval_{3i} \csub \cval_{2i}$ and $\cval_{2i} \csub \cval_{1i}$.
          Next, we also have $\cval_{1o} \csub \cval_{2o}$ and $\cval_{2o} \csub \cval_{3o}$.
          By the def.\ of $\cprop$, we next have 
          $\pair{\cval'_{2i}}{\cval'_{1i}} = \cprop(\cval_{2i}, \cval_{1i})$, 
          $\pair{\cval'_{3i}}{\cval''_{2i}} = \cprop(\cval_{3i}, \cval_{2i})$, 
          $\pair{\cval'_{1o}}{\cval'_{2o}} = \cprop(\cval_{1o}, \cval_{2o})$, and
          $\pair{\cval''_{2o}}{\cval'_{3o}} = \cprop(\cval_{2o}, \cval_{3o})$. 
          By the i.h., we then have $\constcomp(\cval'_{2i}, \cval''_{2i})$ 
          and $\constcomp(\cval'_{2o}, \cval''_{2o})$. The result then follows
          from the def.\ of $\constcomp$.
\end{itemize}
\end{proof}


\input{proofs/c-semantics-inductive-properties}


==> proofs/c-semantics.tex <==
% !TEX root = ../../thesis.tex
\subsection{Concrete Semantics Proofs}
\label{sec:proofs-c-semantics}

\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}


\begin{lemma}\label{thm:c-prop-increase}
$\cprop$ is increasing.
\end{lemma}
\begin{proof}
Let $\pair{\cval'_1}{\cval'_2} = \cprop(\cval_1, \cval_2)$. The proof goes by mutual structural induction on
$\cval_1$ and $\cval'_2$.

\noindent Base cases.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $\cval_1 = \bot$.
\begin{align*}
\cval'_1 = \bot, \cval'_2 = \cval_2 && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 = \cerr$.
\begin{align*}
\cval'_1 = \cval'_2 = \cerr && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 = c, \cval_2 = \bot$.
\begin{align*}
\cval'_1 = \cval'_2 = c && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 = c, \cval_2 = c$.
\begin{align*}
\cval'_1 = \cval'_2 = c && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 = c_1, \cval_2 = c_2, c_1 \not = c_2$.
\begin{align*}
\cval'_1 = \cval_1, \cval'_2 = \cerr && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 = c_1, \cval_2 = \cerr$.
\begin{align*}
\cval'_1 = \cval_1, \cval'_2 = \cerr && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 = c, \cval_2 \in \ctables$.
\begin{align*}
\cval'_1 = \cval_1, \cval'_2 = \cerr && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 \in \ctables, \cval_2 = \bot$.
\begin{align*}
\cval'_1 = \cval_1, \cval'_2 = \ctable_{\bot} && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 \in \ctables, \cval_2 = c$.
\begin{align*}
\cval'_1 = \cval_1, \cval'_2 = \cerr && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}

\item $\cval_1 \in \ctables, \cval_2 = \cerr$.
\begin{align*}
\cval'_1 = \cval'_2 = \cerr && \text{def. of } \cprop \\ 
\cval_1 \cvord \cval'_1, \cval_2 \cvord \cval'_2 && \text{def. of } \cvord 
\end{align*}
\end{itemize}
%
\noindent Induction case: $\cval_1 = \ctable_1, \cval_2 = \ctable_2$. By definition of $\cprop$, we need to consider
two cases of call-sites subject to the table $\ctable_2$.
%
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\item $\ccsite \not \in \ctable_2$.
\begin{align*}
\cval_{1i} = \cval'_{1i}, \cval_{2i} = \cval'_{2i}, \cval_{1o} = \cval'_{1o}, \cval_{20} = \cval'_{2o} && \text{def. of } \cprop \\ 
\cval_{1i} \cvord \cval'_{1i}, \cval_{2i} \cvord \cval'_{2i}, \cval_{1o} \cvord \cval'_{1o}, \cval_{20} \cvord \cval'_{2o} && \text{def. of } \cvord 
\end{align*}

\item $\ccsite \in \ctable_2$.
\begin{align}
\cval_{1i} \cvord \cval'_{1i}, \cval_{2i} \cvord \cval'_{2i}, \cval_{1o} \cvord \cval'_{1o}, \cval_{20} \cvord \cval'_{2o} && \text{def. of $\cprop$ and i.h.}
\end{align}
\end{itemize}
%
\end{proof}





\begin{lemma}\label{thm:c-step-increase}
$\ctransname$ is increasing.
\end{lemma}
\begin{proof}
By structural induction on program expressions. The result follows from the increasing property 
of the join $\cvjoin$ and Lemma~\ref{thm:c-prop-increase}.
\end{proof}





\begin{lemma}\label{thm:c-prop-monotone}
$\cprop$ is monotone.
\end{lemma}
\begin{proof}
Let $\pair{\cval'_1}{\cval'_2} = \cprop(\cval_1, \cval_2)$, $\pair{\cval'_3}{\cval'_4} = \cprop(\cval_3, \cval_4)$,
$\cval_1 \cvord \cval_3$, and $\cval_2 \cvord \cval_4$. We show that $\cval'_1 \cvord \cval'_3$ and $\cval'_2 \cvord \cval'_4$.
The proof goes by mutual structural induction on $\cval_3$ and $\cval_4$.

\noindent Base cases.
%
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\item $\cval_3 = \cerr$.
\begin{align*}
\cval'_3 = \cerr, \cval'_4 = \cerr && \text{def. of } \cprop \\ 
\cval'_1 \cvord \cval'_3, \cval'_2 \cvord \cval'_4 && \text{def. of } \cvord 
\end{align*}


\item $\cval_4 = \cerr$.
\begin{align*}
\cval'_4 =\cerr && \text{def. of } \cprop \\
\cval'_2 \cvord \cval'_4  && \text{by } \cvord 
\end{align*}
	\begin{itemize}
	\item $\cval_3 = c$
	\begin{align*}
	\cval_1 = \bot \vee \cval_1 = c   && \text{by } \cval_1 \cvord \cval_3\\ 
	\cval'_3 = c, \cval'_1 = \bot \vee \cval'_1 = c && \text{def. of } \cprop \\ 
	\cval'_1 \cvord \cval'_3 && \text{by } \cvord 
	\end{align*}

	\item $\cval_3 \in \ctables$
	\begin{align*}
	\cval'_3 = \cerr && \text{def. of } \cprop \\ 
	\cval'_1 \cvord \cval'_3 && \text{by } \cvord 
	\end{align*}
	\end{itemize}


\item $\cval_3 = \bot$.
\begin{align*}
\cval_1 = \bot  && \text{by } \cval_1 \cvord \cval_3\\ 
\cval'_4 =\cval_4, \cval'_2 = \cval_2, \cval'_3 = \cval_3, \cval'_1 = \cval_1 && \text{def. of } \cprop \\ 
\cval'_1 \cvord \cval'_3, \cval'_2 \cvord \cval'_4 && \text{def. of } \cvord 
\end{align*}


\item $\cval_4 = \bot$.
\begin{align*}
\cval_2 = \bot  && \text{by } \cval_2 \cvord \cval_4\\ 
\cval'_1 =\cval_1, \cval'_3 = \cval_3 && \text{def. of } \cprop \\
\cval'_1 \cvord \cval'_3  && \text{def. of } \cvord
\end{align*}
	\begin{itemize}
	\item $\cval_3 = c$
	\begin{align*}
	\cval_1 = \bot \vee \cval_1 = c   && \text{by } \cval_1 \cvord \cval_3\\ 
	\cval'_4 = c, \cval'_2 = \bot \vee \cval'_2 = c && \text{def. of } \cprop \\ 
	\cval'_2 \cvord \cval'_4 && \text{by } \cvord 
	\end{align*}

	\item $\cval_3 \in \ctables$
	\begin{align*}
	\cval_1 = \bot \vee \cval_1 \in \ctables   && \text{by } \cval_1 \cvord \cval_3\\ 
	\cval'_4 = \ctable_{\bot}, \cval'_2 = \bot \vee \cval'_2 = \ctable_{\bot} && \text{def. of } \cprop \\ 
	\cval'_2 \cvord \cval'_4 && \text{by } \cvord 
	\end{align*}
	\end{itemize}


\item $\cval_3 = c, \cval_4 = c$.
\begin{align*}
\cval'_4 = \cval_4 = \cval_3 = \cval'_3 = c && \text{def. of } \cprop \\ 
\cval_1 = \bot \vee \cval_1 = c, \cval_2 = \bot \vee \cval_2 = c  && \text{by } \cval_1 \cvord \cval_3, \cval_2 \cvord \cval_4\\ 
\cval'_1 = \bot \vee \cval'_1 = c, \cval'_2 = \bot \vee \cval'_2 = c  && \text{def. of } \cprop\\ 
\cval'_1 \cvord \cval'_3, \cval'_2 \cvord \cval'_4 && \text{def. of } \cvord 
\end{align*}


\item $\cval_3 = c_1, \cval_4 = c_2, c_1 \not = c_2$.
\begin{align*}
\cval'_4 = \cerr, \cval_3 = \cval'_3 = c_1 && \text{def. of } \cprop \\ 
\cval_1 = \bot \vee \cval_1 = c_1 && \text{by } \cval_1 \cvord \cval_3, \cval_2 \cvord \cval_4\\ 
\cval'_1 = \bot \vee \cval'_1 = c_1 && \text{def. of } \cprop\\ 
\cval'_1 \cvord \cval'_3, \cval'_2 \cvord \cval'_4 && \text{def. of } \cvord 
\end{align*}


\item $\cval_3 = c, \cval_4 \in \ctables$.
\begin{align*}
\cval'_4 = \cerr, \cval_3 = \cval'_3 = c && \text{def. of } \cprop \\ 
\cval_1 = \bot \vee \cval_1 = c && \text{by } \cval_1 \cvord \cval_3, \cval_2 \cvord \cval_4\\ 
\cval'_1 = \bot \vee \cval'_1 = c && \text{def. of } \cprop\\ 
\cval'_1 \cvord \cval'_3, \cval'_2 \cvord \cval'_4 && \text{def. of } \cvord 
\end{align*}


\item $\cval_3 \in \ctables, \cval_4 = c$.
\begin{align*}
\cval'_4 = \cerr, \cval_3 = \cval'_3 && \text{def. of } \cprop \\ 
\cval_1 = \bot \vee \cval_1 \in \ctables, \cval_2 = \bot \vee \cval_2 = c && \text{by } \cval_1 \cvord \cval_3, \cval_2 \cvord \cval_4\\ 
\cval'_1 = \cval_1  && \text{def. of } \cprop\\ 
\cval'_1 \cvord \cval'_3, \cval'_2 \cvord \cval'_4 && \text{def. of } \cvord 
\end{align*}
\end{itemize}


\noindent Induction case: $\cval_3 = \ctable_3$ and $\cval_4 = \ctable_4$. If $\cval_1 = \bot$, then $\cval'_1 = \bot$ and $\cval'_1 \cvord \cval'_3$
trivially follows. When $\cval_2 = \bot$, we have $\cval'_2 = \bot \vee \cval'_2 = \ctable_{\bot}$ and the argument follows
from Lemma~\ref{thm:c-prop-increase}.

We are hence left with the case when $\cval_1 = \ctable_1$ and $\cval_2 = \ctable_2$. First, we have that
$\ccsite \in \ctable_2 {\implies} \ccsite \in \ctable_4$ by the $\ctable_2 \cvord \ctable_4$ assumption.
We have three cases to consider.
%
\begin{itemize}
\item $\ccsite \not \in \ctable_2$ and $\ccsite \not \in \ctable_4$. Trivial, as there is no propagation.
\item $\ccsite \not \in \ctable_2$ and $\ccsite \in \ctable_4$. By $\cprop$, there is no propagation between 
      the pairs $\ctable_1(\ccsite)$ and $\ctable_2(\ccsite)$. The result then follows from Lemma~\ref{thm:c-prop-increase}.
\item $\ccsite \in \ctable_2$ and $\ccsite \in \ctable_4$. The result follows from the induction hypothesis.
\end{itemize}
\end{proof}




\begin{lemma}\label{thm:c-step-monotone}
$\ctransname$ is monotone.
\end{lemma}
\begin{proof}
Let $\cmap' \cmord \cmap''$. For any $\cenv$ and $e$, we show that $\cmap'_f \cmord \cmap''_f$ where
$\cmap'_f = \ctrans[\fuel]{e}(\cenv)(\cmap')$ and $\cmap''_f = \ctrans[\fuel]{e}(\cenv)(\cmap'')$. The proof goes
by structural induction on $e$.
%
\begin{itemize}
\item $e = c^{\ell}$. $\cmap'_f \cmord \cmap''_f$ follows from the monotonicity of $\cvjoin$.
\item $e = x^{\ell}$. Here, $\cmap'_f \cmord \cmap''_f$ follows from the monotonicity of $\cprop$ (Lemma~\ref{thm:c-prop-monotone}).
\item $e = (e_1^{\ell_1} e_2^{\ell_2})^{\ell}$. We do case analysis on the values computed for $e_1$ and $e_2$
      by $\ctrans[\fuel]{e}(\cenv)(\cmap')$ and $\ctrans[\fuel]{e}(\cenv)(\cmap'')$. 
	\begin{itemize}
		\item $\cval'_1 = \bot$. Then $\cmap'_f = \cmap'_1$ and the result holds by Lemma~\ref{thm:c-step-increase}.
		\item $\cval''_1 = \bot$. By i.h., $\cmap'_1 \cmord \cmap''_1$, hence $\cval'_1 = \bot$ and the argument
      			follows from the previous case.
		\item $\cval'_1 \not = \bot \wedge \cval'_1 \not \in \ctables$. By i.h., $\cmap'_1 \cmord \cmap''_1$
      			and hence $\cval''_1 \not = \bot \wedge \cval'' \not \in \ctables$. Therefore, $\cmap''_f = \cmap_{\cerr}$ and
      			the result follows trivially.
		\item $\cval'_1 \in \ctables, \cval''_1 \not \in \ctables$. The argument is trivial as $\cmap''_f = \cmap_{\cerr}$.
		\item $\cval'_1 \in \ctables, \cval''_1 \in \ctables$. By i.h., $\cval'_1 \cvord \cval''_1$. The cases for 
      			$\cval'_2$ and $\cval''_2$ are handled the same way as for $\cval'_1$ and $\cval''_1$. We are thus 
      			interested in the remaining case where $\cval'_2, \cval''_2 \not \in \{\bot, \cerr\}$ where by i.h. 
      			$\cval'_2 \cvord \cval''_2$. The result then follows by the monotonicity of $\cprop$ (Lemma~\ref{thm:c-prop-monotone}).
	\end{itemize}

\item $e = (\lambda x.e)^{\ell}$. The argument, similar to the case for function applications, follows
                                  from Lemmas~\ref{thm:c-prop-monotone},~\ref{thm:c-prop-increase}, and 
                                  basic properties of joins $\cvjoin$.
\end{itemize}
\end{proof}


\begin{zproof*}[of Lemma~\ref{prop-monotone}]\end{zproof*}
\begin{proof}
Follows directly from Lemma~\ref{thm:c-prop-increase} and Lemma~\ref{thm:c-prop-monotone}.
\end{proof}

\begin{zproof*}[of Lemma~\ref{step-monotone}]\end{zproof*}
\begin{proof}
Follows directly from Lemma~\ref{thm:c-step-increase} and Lemma~\ref{thm:c-step-monotone}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now introduce a more descriptive definition of the join $\cvjoin$ on concrete data flow values.
\begin{definition}[Join on Concrete Values]
\[\begin{array}{c c}
\bot \cvjoin \cval \Def= \cval \quad\quad \cval \cvjoin \bot \Def= \cval & c \cvjoin c \Def= c \\
\ctable_1 \cvjoin \ctable_2 \Def= \lambda \ccsite.\, \ctable_1(\ccsite) \;\vecop{\cvjoin}\; \ctable_2(\ccsite) 
& \quad\cval_1 \cvjoin \cval_2 \Def= \cerr \quad \text{(otherwise)}
\end{array}\]
\end{definition}
\newcommand{\cvdepth}{\m{depth}}
We next prove that our definitions of joins and meets are indeed correct.
The definition of a binary join on concrete values is raised to an arbitrary number of values in the 
expected way where $\cvjoin \emptyset \Def= \bot$ and $\cvjoin \{\cval\} \Def = \cval$. 
The meet $\cvmeet$ is defined similarly. We also define a depth of a concrete data flow value in 
the expected way. The depth of constants,
errors, and unreachable values is simply 0. The depths of tables is the maximum depth of any of 
the values stored for any call site, increased by 1.
%
\begin{definition}[Depth of Values]
\begin{gather*}
\cvdepth(\bot) \Def= \cvdepth(c) \Def= \cvdepth(\cerr) \Def= 0  \\
\cvdepth(\ctable) \Def = 1 + \m{max}(\bigcup_{\ccsite} \cvdepth(\pi_1(\ctable(\ccsite))) \cup \bigcup_{\ccsite} \cvdepth(\pi_1(\ctable(\ccsite))))
\end{gather*}
\end{definition}
%
\noindent Note that $\cvdepth$ is well-defined since, although there is an infinite number of
call sites in a table, the depth of every value stored at every call site in a table is bounded
by the table depth, as tables are defined inductively.
%
\begin{lemma}\label{thm:cvjoin}
Let $V \in \powerset(\cvalues)$. Then, $\cvjoin V = \mi{lub}(V)$ subject to $\cvord$.
\end{lemma}
\begin{proof}
We carry the proof by case analysis on elements of $V$ and induction on the minimum depth
thereof when $V$ consists of tables only. 

We first consider the trivial (base) cases where $V$ is not a set of multiple tables.
\begin{itemize}
\item $V = \emptyset$. By $\cvord$, $\mi{lub}(V) = \bot$ and $\cvjoin(V) = \bot$ by $\cvjoin$.
\item $V = \{\cval\}$. Trivial.
\item $c \in V, \ctable \in V$. By $\cvord$, lub of $\{c, \ctable\}$ is $\cerr$
        and since $\cerr$ is the top element, $\mi{lub}(V) = \cerr = \cvjoin V$.
\item $c_1 \not = c_2, c_1 \in V, c_2 \in V$. As in the previous case.
\item $\bot \in V$. By $\cvord$, $\mi{lub}(V) = \mi{lub}(V/\{\bot\})$ 
                     and $\cvjoin(V) = \cvjoin(V/\{\bot\})$ by $\cvjoin$. The set $V/\{\bot\}$
                     either falls into one of the above cases or consists of multiple tables,
                     which is the case we show next.
\end{itemize}
%
Let $V \subseteq \ctables$ and $|V| > 1$. Let $d$ be the minimum depth of any table in $V$.
By $\cvord$, lub of $V$ is a table $\ctable$ that for every call site $\ccsite$ has input (resp. output)
that is lub of the corresponding inputs (resp. outputs) of tables in $V$ for $\ccsite$.
We focus on inputs; the same argument goes for outputs.
Let $V_i = \setc{\pi_1(\cval(\ccsite))}{\ccsite \in \ccallsites \wedge \cval \in V}$.
By $\cvjoin$, $\pi_1(\ctable(\ccsite)) = \cvjoin V_i$. We hence need to show that $\cvjoin V_i = \mi{lub}(V_i)$.
The set $V_i$ either falls into one of the trivial cases, from which the argument easily follows, or 
$V_i \subseteq \ctables \wedge |V| > 1$. In the latter case, the minimum depth of any value in $V_i$
is smaller than $d$ by the definition of $\cvdepth$ and the result follows from the i.h.

The proof of correctness for the meet $\cvmeet$ is similar.
\end{proof}

\input{proofs/c-semantics-properties}

%\begin{lemma}\label{thm:cvmeet}
%Let $V \in \powerset(\cvalues)$. Then, $\cvmeet V = \mi{glb}(V)$ subject to $\cvord$.
%\end{lemma}
%\begin{proof}
%As in the proof of Lemma~\ref{thm:cvjoin}.
%\end{proof}



==> proofs/cl-semantics.tex <==
% !TEX root = ../../thesis.tex
\clearpage
\subsection{Collapsed Semantics Proofs}
\label{sec:proofs-cl-semantics}

We first provide a more descriptive definition of the join
$\pvjoin$ on collapsed data flow values.
%
\begin{definition}[Join on Collapsed Values]
\[\begin{array}{cc}
\pbot \pvjoin[] \pval \Def= \pval \quad\quad \pval \pvjoin[] \pbot \Def= \pval &
           \prel_1 \pvjoin[] \prel_2 \Def= \prel_1 \cup \prel_2 \\
\ptab{\pval_1}{\pval_2} \pvjoin[] \ptab{\pval_3}{\pval_4} \Def= 
	\ptab{\pval_1\pvjoin[]\pval_3}{\pval_2\pvjoin[]\pval_4} 
& \pval_1 \pvjoin[] \pval_2 \Def= \perr \quad \text{(otherwise)}
\end{array}\]
\end{definition}
%\pbot \pvjoin[] \pval \Def= \pval \quad\quad \pval \pvjoin[] \pbot \Def= \pval && \prel_1 \pvjoin[] \prel_2 \Def= \prel_1 \cup \prel_2 \\
%\ptab{\pval_1}{\pval_2} \pvjoin[] \ptab{\pval_3}{\pval_4} \Def= 
%	\ptab{\pval_1\pvjoin[]\pval_3}{\pval_2\pvjoin[]\pval_4} 
%&& \pval_1 \pvjoin[] \pval_2 \Def= \perr \quad \text{otherwise}
%\end{align*}
%\end{definition}
%
%\noindent The above definition of binary join is raised to an arbitrary number of collapsed
%values in the expected way where $\pvjoin[] \emptyset \Def= \pbot$ and $\pvjoin[] \{\pval\} \Def = \pval$. 
%The meet $\pvmeet[]$ is defined similarly. 

%Note that, as usual, we assume that the join and 
%meet operators are defined for values of the same abstract scope that is kept implicit.

%A depth of a collapsed value is defined in the similar way as for the concrete and
%relational values. We hence reuse the function $\cvdepth$ to denote the depth of collapsed values.
We next prove that our definitions of collapsed meet and join are correct.
A depth of a collapsed value is defined in the similar way as for the concrete and
relational values. We hence reuse the function $\cvdepth$ to denote the depth of collapsed values.
\begin{lemma}\label{thm:clvjoin}
Let $V \in \powerset(\pvalues)$. Then, $\pvjoin[] V = \mi{lub} (V)$ and 
$\pvmeet[] V = \mi{glb} (V)$ subject to $\pvord[]$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:rvjoin}, the proof is carried by case analysis on elements 
of $U$ and induction on the minimum depth thereof when $U$ consists of collapsed tables only. 
\end{proof}


The next proof shows that the concretization function for collapsed values is a complete meet-morphism.
%
\begin{theorem}[Complete Meet Morphism of $\pgamma$]\label{thm:cl-meet-morph-values}
Let $U \in \powerset(\pvalues)$ and let $\rscope$ be a concrete scope. 
Then $\pgamma[\delta](\pvmeet[] U) = \rvmeet_{\pval \in U} \pgamma[\delta](\pval)$ for $\delta \in \Delta(\pscope, \rscope)$.
\end{theorem}
\begin{proof}
We carry the proof by case analysis on elements of $U$ and induction on the minimum depth
thereof when $U$ consists of tables only. 

We first consider the trivial (base) cases where $U$ is not a set of multiple collapsed tables.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $U = \emptyset$. Here, $\pgamma[\delta](\pvmeet[] \emptyset) = \pgamma[\delta](\perr) = \perr = \rvmeet \emptyset$.
\item $U= \{\pval\}$. Trivial.
\item $\prel \in U, \ptable \in U$. We have $\pvmeet[] \{\prel, \ptable\} = \pbot$
        and since $\pbot$ is the bottom element, $\pvmeet[] U = \pbot$. Similarly,
	$\pgamma[\delta](\prel) \rvmeet \pgamma[\delta](\ptable) = \rbot = \pgamma(\pbot)$ so by the 
        definition of $\rvmeet$ we have $\rvmeet_{\pval \in U} \pgamma[\delta](\pval) = \rbot$.

\item $U \subseteq \prels$. Here,
{\footnotesize \begin{gather*}
\pgamma[\delta](\pvmeet[] U) = \pgamma[\delta](\pvmeet[] \setc{\prel_{\pscope}}{\prel \in U}) = \pgamma[\delta](\bigcap_{\prel \in U} \prel) \\
\ind[21] \textbf{\scriptsize [by def. of $\pvmeet[]$]} \\
= \setc{\dmap}{\pdmap \in (\bigcap_{\prel \in U}\,\prel)) \wedge \pdmap(\nu) = \dmap(\nu) \wedge \forall \pnode \in \pscope.\,\dmap(\delta(\pnode)) = \pdmap(\pnode)}\\
\ind[21] \textbf{\scriptsize [by def. of $\pgamma[\delta]$]} \\
= \bigcap_{\prel \in U} \setc{\dmap}{\pdmap \in \prel \wedge \pdmap(\nu) = \dmap(\nu) \wedge \forall \pnode \in \pscope.\,\dmap(\delta(\pnode)) = \pdmap(\pnode)}\\
=  \bigcap_{\prel \in U} \pgamma[\delta](\prel) = \rvmeet_{\prel \in U} \pgamma[\delta](\prel)
\ind[10] \textbf{\scriptsize [by def. of $\pgamma$ and $\rvmeet$]}
\end{gather*}}%


\item $\perr \in U$. Here, $ \pvmeet[] U = \pvmeet[] (U/\{\perr\})$ and $\rvmeet_{\pval \in U} \pgamma[\delta](\pval) = \rvmeet_{\pval \in U, \pval \not = \perr} \pgamma[\delta](\pval)$ since $\pgamma(\perr) = \rerr$. The set $U/\{\perr\}$ either falls into one of the above cases or consists of multiple tables, which is the case we show next.
\end{itemize}


Let $U \subseteq \ptables$ and $|U| > 1$. Let $d$ be the minimum depth of any table in $U$.
{\footnotesize
\begin{gather*}
\pgamma[\delta](\pvmeet[] U) = \pgamma[\delta](\ptab{\pvmeet[] \setc{\pi_1(\ptio(\ptable))}{\ptable \in U}}{\pvmeet \setc{\pi_2(\ptio(\ptable))}{\ptable \in U}}) \\
\ind[15] \textbf{\scriptsize [by def. of $\pvmeet[]$]} \\
= \lambda \ccsite. \pair{\pgamma[\delta](\pvmeet[] \setc{\pi_1(\ptio(\ptable))}{\ptable \in U})}{\pgamma[{\delta[\absn \mapsto \ccsite]}](\pvmeet[] \setc{\pi_2(\ptio(\ptable))}{\ptable \in U})} \\
\ind[15] \textbf{\scriptsize [by def. of $\pgamma[]$]} \\
= \lambda \ccsite. \pair{\rvmeet \setc{\pgamma[\delta](\pi_1(\ptio(\ptable)))}{\ptable \in U}}{\rvmeet \setc{\pgamma[{\delta[\absn \mapsto \ccsite]}](\pi_2(\ptio(\ptable)))}{\ptable \in U}} \\
\textbf{\scriptsize [by i.h. on the min. depth of $\setc{\pi_1(\ptio(\ptable)))}{\ptable \in U}$ and $\setc{\pi_2(\ptio(\ptable)))}{\ptable \in U}$]} \\
= \rvmeet_{\pval \in U} \pgamma[\delta](\pval) \ind[9] \textbf{\scriptsize [by def. of $\rvmeet$]}
\end{gather*}}%
\end{proof}

We can now state the monotonicity of functions constituting the Galois connection between
collapsed and relational values.
%
\begin{lemma}\label{thm:cl-alpha-gamma-monotone}
For any abstract scope $\pscope$, concrete scope $\rscope$, and $\delta \in \Delta(\pscope, \rscope)$, 
both $\palpha[\delta]$ and $\pgamma[\delta]$ are monotone.
\end{lemma}
\begin{proof}
The argument follows from the fact that $\palpha[\delta]$ and $\pgamma[\delta]$ constitute a Galois connection (Prop.\ref{prop:galois-connections}), 
as evidenced by Theorem~$\ref{thm:cl-meet-morph-values}$.
\end{proof}

The meet morphism requirement is also satisfied by the concretization function defined over
collapsed maps.
\begin{theorem}[Complete Meet Morphism of $\pmgamma$]\label{thm:cl-meet-morph-maps}
Let $m^{\pdesignation} \in \powerset(\pmaps)$. Then $\pmgamma(\pmmeet m^{\pdesignation}) = \rmmeet_{\pmap \in m^{\pdesignation}} \pmgamma(\pmap)$.
\end{theorem}
\begin{proof}
\begin{align*}
\pmgamma (\pmmeet m^{\pdesignation}) =\,& \Lambda \cnode.\, \rvmeet \setc{\pgamma[\delta](\pvmeet[]\setc{\pmap(\rho(\cnode))}{\pmap \in m^{\pdesignation}}}{\delta \in \Delta(\rscope_{\rho(\cnode)}, \pscope_{\cnode})} \\
& \ind[15] \textbf{\scriptsize [by def. of $\pvmeet[]$ and $\pmgamma$]} \\
=\,& \Lambda \cnode.\, \rvmeet \setc{\rvmeet \setc{\pgamma[\delta](\pmap(\rho(\cnode)))}{\pmap \in m^{\pdesignation}}}{\delta \in \Delta(\rscope_{\rho(\cnode)}, \pscope_{\cnode})} \\
& \ind[15] \textbf{\scriptsize [by Theorem~\ref{thm:cl-meet-morph-values}]} \\
=\,& \Lambda \cnode.\, \rvmeet \setc{\rvmeet \setc{\pgamma[\delta](\pmap(\rho(\cnode)))}{\delta \in \Delta(\rscope_{\rho(\cnode)}, \pscope_{\cnode})}}{\pmap \in m^{\pdesignation}} \\
& \ind[15] \textbf{\scriptsize [by assoc. of meets ($\pvmeet[]$)]} \\
=\,& \rmmeet_{\pmap \in m^{\pdesignation}} \pmgamma(\pmap) \ind[8] \textbf{\scriptsize [by def. of $\pvmeet[]$ and $\pmgamma$]} \\
\end{align*}
\end{proof}

Moreover, $\palpha[\delta]$ is surjective and $\pgamma[\delta]$ is injective for any $\delta \in \Delta(\pscope, \rscope)$
given a concrete scope $\rscope$. Hence, the Galois connection on collapsed values is in fact a Galois insertion.
\begin{lemma}\label{thm:cl-alpha-gamma-id}
Let $\delta \in \Delta(\pscope, \rscope)$ for some abstract scope $\pscope$ and concrete scope $\rscope$.
Then, $\palpha[\delta]$ is surjective and $\pgamma[\delta]$ is injective.
\end{lemma}
\begin{proof}
We show the injectivity of $\pgamma[\delta]$. The surjective nature of $\palpha[\delta]$ then follows
from Proposition~\ref{prop:galois-connections-2}. Suppose $\pgamma[\delta]$ is not surjective. Then,
there exist $\pval_1 \in \pvalues$ and $\pval_2 \in \pvalues$ s.t. $\pval_1 \not = \pval_2$ (modulo
variable renaming) and $\pgamma[\delta](\pval_1) = \pgamma[\delta](\pval_2)$. We arrive at contradiction
by structural induction on $\pval_1$ and $\pval_2$. Let $\pgamma[\delta](\pval_1) = \rval_1$ and 
$\pgamma[\delta](\pval_2) = \rval_2$.

Base cases.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $\pval_1 = \pbot$ or $\pval_2 = \pbot$. Assume $\pval_1 = \pbot$ w.l.g. Then,
      $\rval_1 = \rbot$. By def. of $\pgamma[\delta]$, $\rval_2 = \rbot$ iff $\pval_2 = \pbot$, contradiction.

\item $\pval_1 = \perr$ or $\pval_2 = \perr$. Assume $\pval_1 = \perr$ w.l.g. Then,
      $\rval_1 = \rerr$. By def. of $\pgamma[\delta]$, $\rval_2 = \rerr$ iff $\pval_2 = \perr$, contradiction.

\item $\pval_1 \in \prels, \pval_2 \in \ptables$ or $\pval_1 \in \ptables, \pval_1 \in \prels$.
      Assume $\pval_1 = \prels$ and $\pval_2 \in \ptables$ w.l.g. Then,
      $\rval_1 \in \rels$ and $\rval_2 \in \rtables$. Hence, $\rval_1 \not = \rval_2$.

\item $\pval_1 \in \prels, \pval_2 \in \prels$. By def. of $\pgamma[\delta]$ and
      $\delta$ being a function it follows $\rval_1 \not = \rval_2$. Essentially,
      $\pgamma[\delta]$ simply \textit{renames} dependency variables in dep. vectors using $\delta$. 
\end{itemize}

\noindent Induction case. Let $\pval_1 = \ptab{\pval_{1i}}{\pval_{1o}}$ and $\pval_2 = \ptab{\pval_{2i}}{\pval_{2o}}$.
By $\pval_1 \not = \pval_2$, we have $\pval_{1i} \not = \pval_{2i}$ or $\pval_{1o} \not = \pval_{2o}$. The result
then follows from the i.h.
\end{proof}





\subsubsection{Domain Operations}

In this subsection, we state the basic properties and the corresponding proofs of
strengthening operations on collapsed values.


\paragraph{Soundness, Strengthening, Idempotency, and Monotonicity}

We start by showing soundness of the domain operations of the collapsed semantics
subject to the relational semantics. We first show the proof for strengthening
by imposing equality between two abstract nodes.

\begin{lemma}\label{thm:cl-neq-strengthening-sound}
Let $\delta_1 \in \Delta(\pscope, \rscope)$ for some abstract scope $\pscope$ and concrete scope $\rscope$,
$\rval \in \rvalues$, $\pval \in \pvalues$, $\pnode_1 \in \pnodes$, and $\pnode_2 \in \pnodes$. 
If $\rval \rvord \pgamma[\delta_1](\pval)$, then 
$\requality{\rval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)} \rvord \pgamma[\delta_1](\requality{\pval}{\pnode_1}{\pnode_2})$.
\end{lemma}
\begin{proof}
We recall $\requality{\pval}{\pnode_1}{\pnode_2} = \pvjoinb[] \pset{\palphac_{\delta}(\requality{\pgammac_{\delta}(\pval)}{\delta(\pnode_1)}{\delta(\pnode_2)})}{\rscope \subseteq \cnodes \wedge \delta \in \Delta(\pscope,\rscope)}$ for a given concrete scope $\rscope$.
 
\begin{align*}
\requality{\rval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)} \rvord \requality{\pgamma[\delta](\pval)}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)} && 
\text{by Lemma~\ref{thm:r-neq-strengthening}}\\  
\palpha[\delta_1](\requality{\rval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)}) \rvord \palpha[\delta_1](\requality{\pgamma[\delta](\pval)}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)}) &&
\text{by Lemma~\ref{thm:cl-alpha-gamma-monotone}}\\  
\palpha[\delta_1](\requality{\rval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)}) \rvord \requality{\pval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)} &&
\text{by def. of $\requality{\pval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)}$}\\  
\requality{\rval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)} \rvord \pgamma[\delta_1](\requality{\pval}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)}) &&
\text{by Prop.~\ref{prop:galois-connections}}
\end{align*}
\end{proof}

\noindent The above result can be made more general.
\begin{lemma}~\label{thm:cl-strengthenings-sound}
Strengthening operations on collapsed values are sound.
\end{lemma}
\begin{proof}
The proof closely follows that of Lemma~\ref{thm:cl-neq-strengthening-sound}: the proof
relies on the properties of monotonicity of abstraction and concretization functions
and monotonicity of the corresponding strengthening operation defined over relational values.
\end{proof}

We next show that the strengthening operations on collapsed values indeed perform
strengthening.
\begin{lemma}\label{thm:cl-n-strengthening}
Let $\pval_1 \in \pvalues$, $\pval \in \pvalues$, $\pnode_1 \in \pnodes$ and $\pnode_2 \in \pnodes$. 
Then $\requality{\pval}{\pnode_1}{\pnode_2} \pvord \pval$.
\end{lemma}
\begin{proof}
Again, recall $\requality{\pval}{\pnode_1}{\pnode_2} = \pvjoinb[] \pset{\palphac_{\delta}(\requality{\pgammac_{\delta}(\pval)}{\delta(\pnode_1)}{\delta(\pnode_2)})}{\rscope \subseteq \cnodes \wedge \delta \in \Delta(\pscope,\rscope)}$ for a given concrete scope $\rscope$.
Let $\delta_1 \in \Delta(\pscope, \rscope)$ for any concrete scope $\rscope$.
%
\begin{align*}
\requality{\pgammac_{\delta_1}(\pval)}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)} \rvord \pgamma[\delta_1](\pval) 
&& \text{by Lemma~\ref{thm:r-neq-strengthening}}\\
\palpha[\delta_1](\requality{\pgammac_{\delta_1}(\pval)}{\delta_1(\pnode_1)}{\delta_1(\pnode_2)}) \rvord \pval 
&& \text{by prop. of Galois conn.}\\
\end{align*}
%
The result then follows from the glb property of the join $\pvjoin[]$ operator (Theorem~\ref{thm:clvjoin}).
\end{proof}

\noindent The above result and the proof can be applied to all strengthening operations on collapsed values.
\begin{lemma}\label{thm:cl-strengthenings}
Strengthening operations on collapsed values are indeed strengthening.
\end{lemma}
\begin{proof}
The argument closely follows that of Lemma~\ref{thm:cl-n-strengthening}.
\end{proof}


As expected, strengthening operations are also monotone.
\begin{lemma}\label{thm:cl-strengthenings-monotone}
Strengthening operation on collapsed values are monotone.
\end{lemma}
\begin{proof}
The argument follows directly from the monotonicity of strengthening operations
on relational values and monotonicity of the join operator $\pvjoin[]$ on collapsed values.
\end{proof}


In order to prove the idempotency of a strengthening of a collapsed value with another
collapsed value, we first prove the following result.
%
\begin{lemma}\label{thm:cl-strength-idempotent-h}
Let $\pscope$ and $\pscope_1$ be abstract scopes, $\rscope$ and $\rscope_1$ concrete scopes,
$\pnode \in \pnodes$, $\pval \in \pvalues$, $\pval_1 \in \pvalues[\pscope_1]$, $\rval \in \rvalues$, 
$\delta \in \Delta(\pscope, \rscope)$, and $\delta_1 \in \Delta(\pscope_1, \rscope_1)$. 
Then, $\palpha[\delta](\rupdate{\rval}{\delta(\pnode)}{\pgamma[\delta_1](\pval_1)}) \pvord[] \rupdate{\palpha[\delta](\rval)}{\pnode}{\pval_1}$.
\end{lemma}
\begin{proof}
We recall
% 
\[\rupdate{\palpha[\delta](\rval)}{\pnode}{\pval_1} = \pvjoinb[] \pset{\palphac_{\delta}(\rupdate{\pgammac_{\delta}(\palpha[\delta](\rval))}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)}\]
%
By basic properties of Galois connections, monotonicity of joins and strengthening operations on relational values
(Theorem~\ref{thm:r-n-strength-monotone}), $\rupdate{\palpha[\delta](\rval)}{\pnode}{\pval_1}$ is larger than
%
\[\pval' = \pvjoinb[] \pset{\palphac_{\delta}(\rupdate{\rval}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)}\]
%
By definition of $\pval'$, we have $\palpha[\delta](\rupdate{\rval}{\delta(\pnode)}{\pgamma[\delta_1](\pval_1)}) \pvord[] \pval' \pvord[] \rupdate{\palpha[\delta](\rval)}{\pnode}{\pval_1}$. 
\end{proof}
%
We can now prove the idempotency of strengthening using a value.
%
\begin{lemma}\label{thm:cl-strength-idempotent}
Let $\pscope$ and $\pscope_1$ be abstract scopes, $\rscope$ and $\rscope_1$ concrete scopes,
$\pnode \in \pnodes$, $\pval \in \pvalues$, $\pval_1 \in \pvalues[\pscope_1]$. 
%$\delta \in \Delta(\pscope, \rscope)$, and $\delta_1 \in \Delta(\pscope_1, \rscope_1)$. 
Then, $\rupdate{\pval}{\pnode}{\pval_1} = \rupdate{\rupdate{\pval}{\pnode}{\pval_1}}{\pnode}{\pval_1}$.
\end{lemma}
\begin{proof}
We first recall
% 
\[\rupdate{\pval}{\pnode}{\pval_1} = \pvjoinb[] \pset{\palphac_{\delta}(\rupdate{\pgammac_{\delta}(\pval)}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)}\]
%
By Theorem~\ref{thm:cl-strengthenings}, we know $\rupdate{\rupdate{\pval}{\pnode}{\pval_1}}{\pnode}{\pval_1} \rvord \rupdate{\pval}{\pnode}{\pval_1}$.
We thus need to show $\rupdate{\pval}{\pnode}{\pval_1} \rvord \rupdate{\rupdate{\pval}{\pnode}{\pval_1}}{\pnode}{\pval_1}$.

{\small
\begin{align*}
\rupdate{\pval}{\pnode}{\pval_1} =\\ 
\text{\scriptsize [by def of $\rupdate{\cdot}{\cdot}{\cdot}$]}\\
\pvjoinb[] \pset{\palphac_{\delta}(\rupdate{\pgammac_{\delta}(\pval)}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)} =\\
\text{\scriptsize [by Lemma~\ref{thm:r-n-strength-idempotent}]}\\
\pvjoinb[] \pset{\palphac_{\delta}(\rupdate{\rupdate{\pgammac_{\delta}(\pval)}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)}}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)} \rvord\\
\text{\scriptsize [by Lemma~\ref{thm:cl-strength-idempotent-h}]}\\
\pvjoinb[] \pset{\rupdate{\palphac_{\delta}(\rupdate{\pgammac_{\delta}(\pval)}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\pnode}{\pval_1}}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)} \rvord\\
\text{\scriptsize [by glb property of $\pvjoin[]$]}\\
\rupdate{(\pvjoinb[] \pset{\rupdate{\palphac_{\delta}(\pgammac_{\delta}(\pval)}{\delta_1(\pnode)}{\pgamma[\delta_1](\pval_1)})}{\delta \in \Delta(\pscope,\rscope), \delta_1 \in \Delta(\pscope_1,\rscope_1)})}{\pnode}{\pval_1} =\\
\text{\scriptsize [by def of $\rupdate{\cdot}{\cdot}{\cdot}$]}\\
\rupdate{\rupdate{\pval}{\pnode}{\pval_1}}{\pnode}{\pval_1}
\end{align*}}%
\end{proof}


\input{proofs/cl-structural}

\subsubsection{Propagation and Transformer}

\begin{zproof*}[of Lemma~\ref{thm:p-prop-increasing-monotone}]\end{zproof*}
\begin{proof}
For the increasing property, the proof goes by structural induction on both 
collapsed value arguments of $\pprop$ and it closely
follows the proof of Theorem~\ref{thm:c-prop-increase}.
Regarding monotonicity, the proof again goes by structural induction 
on the collapsed arguments of $\pprop$, closely
follows the proof of Theorem~\ref{thm:c-prop-monotone}, and relies on
Lemma~\ref{thm:cl-strengthenings-monotone} (introduced later).
\end{proof}


We next show that propagation in collapsed semantics is an abstraction of the propagation
in relational semantics.
\begin{theorem}\label{thm:cl-prop-sound}
Let $\pval_1 \in \pvalues$, $\pval_2 \in \pvalues$, $\pscope$ an abstract scope, $\rscope$ a concrete scope, and
$\delta \in \Delta(\pscope, \rscope)$. Further, let $\pair{\rval'_1}{\rval'_2} = \rprop(\rval_1, \rval_2)$
where $\rval_1 \rvord \pgamma[\delta](\pval_1)$ and $\rval_2 \rvord \pgamma[\delta](\pval_2)$. Lastly, let
$\pair{\pval'_1}{\pval'_2} = \pprop(\pval_1, \pval_2)$. Then, $\rval'_1 \rvord \pgamma[\delta](\pval'_1)$
and $\rval'_2 \rvord \pgamma[\delta](\pval'_2)$. 
\end{theorem}
\begin{proof}
The proof is carried by structural induction on $\pval_1$ and $\pval_2$.

Base cases.
%
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $\pval_1 = \pbot$.
\begin{align*}
\pval'_1 = \pbot, \pval'_2 = \pval_2 && \text{by } \pprop \\ 
\rval_1 = \rbot && \text{by } \pgamma[\delta] \\ 
\rval'_1 = \rbot, \rval'_2 = \rval_2 && \text{by } \rprop \\
\pgamma[\delta](\pval'_1) = \rbot, \pgamma[\delta](\pval'_2) = \rval'_2 && \text{by } \pgamma[\delta] \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 \in \prels$ and $\pval_2 = \pbot$.
\begin{align*}
\pval'_1 = \pval_1, \pval'_2 = \pval_1 && \text{by } \pprop \\ 
\rval'_2 = \rbot && \text{by } \pgamma[\delta] \\
\rval'_1 = \rval_1, \rval'_2 = \rval_1 && \text{by } \rprop \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 \in \ptables$ and $\pval_2 = \pbot$.
\begin{align*}
\pval'_1 = \pval_1, \pval'_2 = \ptable_{\pbot} && \text{by } \pprop \\ 
\rval'_1 = \rval_1, \rval'_2 = \rtable_{\rbot} \vee \rval'_2 = \rbot && \text{by } \rprop \\
\rtable_{\rbot} = \pgamma[\delta](\ptable_{\pbot}) && \text{by } \pgamma[\delta] \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 = \perr$.
\begin{align*}
\pval'_1 = \perr, \pval'_2 = \perr && \text{by } \pprop \\ 
\pgamma[\delta](\pval'_1) = \perr, \pgamma[\delta](\pval'_2) = \perr && \text{by } \pgamma[\delta] \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 \in \prels$ and $\pval_2 = \perr$.
\begin{align*}
\pval'_1 = \pval_1, \pval'_2 = \pval_2 && \text{by } \pprop \\ 
\rval'_1 = \rval_1 && \text{by } \rprop \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 \in \ptables$ and $\pval_2 = \perr$.
\begin{align*}
\pval'_1 = \perr, \pval'_2 = \pval_2 = \perr && \text{by } \pprop \\ 
\pgamma[\delta](\pval'_1) = \rerr, \pgamma[\delta](\pval'_2) = \rerr && \text{by } \pgamma[\delta] \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 \in \ptables$ and $\pval_2 \in \prels$.
\begin{align*}
\pval'_1 = \pval_1, \pval'_2 = \perr && \text{by } \pprop \\ 
\rval'_1 = \rval_1 && \text{by } \rprop \\
\rval'_1 \rvord \pgamma[\delta](\pval'_1), \rval'_2 \rvord \pgamma[\delta](\pval'_2)
\end{align*}

\item $\pval_1 \in \prels$ and $\pval_2 \in \ptables$. Similar to the previous case.
\end{itemize}

For the induction case, let $\pval_1 = \ptab{\pval_{1i}}{\pval_{1o}}$ and $\pval_1 = \ptab{\pval_{2i}}{\pval_{2o}}$.
By $\pgamma[\delta]$, the only interesting case is when $\rval_1 \in \rtables$ and $\rval_2 \in \rtables$ per
Theorem~\ref{thm:p-prop-increasing-monotone}. For any $\ccsite$, let $\rval_1(\ccsite) = \pair{\rval_{1i}}{\rval_{1o}}$ 
and $\rval_2(\ccsite) = \pair{\rval_{2i}}{\rval_{2o}}$. By $\rval_1 \rvord \pgamma[\delta](\pval_1)$ and 
$\rval_2 \rvord \pgamma[\delta](\pval_2)$ we have $\rval_{1i} \rvord \pgamma[\delta](\pval_{1i})$,
$\rval_{1o} \rvord \pgamma[{\delta[\absn \mapsto \ccsite]}](\pval_{1o})$, $\rval_{2i} \rvord \pgamma[\delta](\pval_{2i})$, and
$\rval_{2o} \rvord \pgamma[{\delta[\absn \mapsto \ccsite]}](\pval_{2o})$. By i.h., we have 
$\rval'_{1i} \rvord \pgamma[\delta](\pval'_{1i})$ and $\rval'_{2i} \rvord \pgamma[\delta](\pval'_{2i})$.
By monotonicity (Lemmas~\ref{thm:r-n-strengthening} and~\ref{thm:cl-strengthenings-monotone}) and 
Lemma~\ref{thm:cl-strength-idempotent-h},
$\rupdate{\rval_{1o}}{\ccsite}{\rval_{2i}}\rvord \pgamma[{\delta[\absn \mapsto \ccsite]}](\rupdate{\pval_{1o}}{\absn}{\pval_{2i}})$ and
$\rupdate{\rval_{2o}}{\ccsite}{\rval_{2i}}\rvord \pgamma[{\delta[\absn \mapsto \ccsite]}](\rupdate{\pval_{2o}}{\absn}{\pval_{2i}})$. 
By i.h. and monotonicity of joins, we have
$\rval'_{1o} \rvord \pgamma[\delta](\pval'_{1o})$ and $\rval'_{2o} \rvord \pgamma[\delta](\pval'_{2o})$.
Since the resulting relational tables $\rval'_1$ and $\rval'_2$ can be expressed as respective joins $\rvjoin$ of singleton relational
tables $[\ccsite \mapsto \pair{\rval'_{1i}}{\rval'_{1o}}]$ and $[\ccsite \mapsto \pair{\rval'_{2i}}{\rval'_{1o}}]$
for every call site $\ccsite$, the result follows from the fact that the join $\rvjoin$ over relational
values is lub (Lemma~\ref{thm:rvjoin}).
\end{proof}


\begin{zproof*}[of Lemma~\ref{thm:p-step-increasing-monotone}]\end{zproof*}
\begin{proof}
The increasing property of $\Ptrans{\cdot}$ is obvious.
The proof goes by structural induction on program expressions and it closely
follows the proof of Theorem~\ref{thm:c-step-monotone}. The proof relies on
Theorem~\ref{thm:p-prop-increasing-monotone} as well as 
Lemma~\ref{thm:cl-strengthenings-monotone}.
\end{proof}





\begin{theorem}\label{thm:cl-step-soundness}
For all programs e, $\rcoll\llbracket e \rrbracket \rmord \pmgamma(\ccoll\llbracket e \rrbracket)$.
\end{theorem}
\begin{proof}
First, observe that $\rmap_{\rbot} \rmord \pmgamma(\pmap_{\pbot})$. The remainder of the proof
is carried by structural induction on $e$ showing that if $\rmap \rmord \pmgamma(\pmap)$ then
$\rmap_1 \rmord \pmgamma(\pmap_1)$ where $\rmap_1 = \rtrans{e}(\cenv)(\rmap)$, 
$\pmap_1 = \ptrans{e}(\rho(\cenv))(\pmap)$, and $\rho$ function is raised to environments in
the expected way. 
We focus on the lambda abstraction rule; other rules are even more trivial. 
For any $\ccsite$, let $\rmap_{\ccsite} = \overline{\rmap}(\ccsite)$. It follows in an almost
straightforward fashion by 
Theorems~\ref{thm:cl-strengthenings-sound} and~\ref{thm:cl-prop-sound} that
$\rmap_{\ccsite} \rmord \pmgamma(\pmap_1)$. Since $\rmjoin$ is a glb 
(by def. of $\rmjoin$ and Theorem~\ref{thm:rvjoin}), 
$\rmjoin_{\ccsite \in \rtable} \overline{\rmap}(\ccsite) \rmord \rmgamma(\rmap_1)$.
\end{proof}


\newcommand{\scopevars}{\m{scope\_vars}}
\newcommand{\prange}{\m{arange}}
\newcommand{\aenv}{\m{aenv}}
We now switch to proving Lemma~\ref{lem:finite-nodes} that states that only a finite
number of nodes is reachable by the collapsed semantics.
Given a program $e$ and a location $\elabel$ in $e$, let $\scopevars_e(l)$ denote
the sequence of program variable pairs ($f, x$) that are (1) bound by some lambda abstraction
strictly above $l$ in the abstract syntax tree (AST) of $e$ and (2) ordered top-bottom
based on their binding appearance in $e$. As an example,
given a program $e = \mu f_1.\lambda x_1.(\mu f_2.\lambda x_2.e^{\ell})^{\ell_1}$, we have
for instance $\scopevars_e(\ell) = \langle (f_1, x_1), (f_2, x_2) \rangle$ and
$\scopevars_e(\ell_1) = \langle (f_1, x_1) \rangle$.
The function $\scopevars_e$ can be simply computed based on the abstract syntax of $e$. 
Given an environment $\penv$ and pair of variables $(f, x)$, 
let $\penv[f, x] = \penv.x{:}\cn{\penv}{x}.f{:}\cn{\penv}{f}$. Given a sequence $s$ of
variable pairs $(f_1, x_1) \cdots (f_j, x_j)$, 
let $\aenv(s) = \emptyset[f_1, x_1] \cdots [f_j, x_j]$. We can thus define an abstract
environment for a location $\ell$ in a program $e \in \Exp$ as 
$\aenv_{e}(\ell) \Def= \aenv(\scopevars_e(\ell))$.  
Given a program $e$, we denote its abstract range 
$\prange(e) = \setc{\cn{\penv}{\elabel}}{\elabel \in \locs(e) \wedge s = \scopevars_e(l) \wedge \penv = \aenv(s)}$.  

\begin{zproof*}[of Lemma~\ref{lem:finite-nodes}]\end{zproof*}
\begin{proof}
The proof follows from a straightforward inductive argument on $e$. Either
$\pcoll[e](\pnode) =\pmap_{\perr}$ or the nodes updated by $\ptrans[k]{e}$ belong to the
set $\prange(e) \cup \setc{\pvnode}{\pnode' \in \prange(e) \wedge \pnode \in \m{rng}(\nenv(\pnode'))}$ 
that is finite since (1) there are only a finite number of locations and lambda expressions
in $e$, (2) program variables are unique, (3) and environments are finite partial functions.
\end{proof}




==> proofs/cl-structural.tex <==
\paragraph{Structural Strengthening}

We also here provide a structural definition of strengthening on
collapsed values and argue its soundness.
First, whenever $\absn \not \in \pscope$, then 
$\supdate{\pval_{\pscope}}{\absn}{\pval} \Def= \pval$. 
Otherwise, 
%
\[\begin{array}{l l}
\supdate{\pval}{\pnode}{\pbot} & \Def= \pbot \\[1ex]
\supdate{\pval}{\pnode}{\pval'} & \Def= \pval \ind[3] \text{if } \pval \in \{\pbot, \perr\} \text{ or } \pval' \in \{\perr\} \cup \ptables[]\\[1ex]
%
\supdate{\prel_1}{\pnode}{\prel_2} &\Def= \rupdate{\prel_1}{\pnode}{\prel_2} \\[1ex]
% 
\supdate{\ptab{\pval_i}{\pval_o}}{\pnode}{\pval} &\Def=  \ptab{
\supdate{\pval_i}{\pnode}{\pval}}{\supdate{\pval_o}{\cnode}{\exists \absn.\,\pval}} \ind[1]\;\; \pval \in \prels[]
\end{array}\]
%
It can be shown that the structural strengthening is sound.
\begin{lemma}~\label{thm:cl-structural-soundness}
Structural strengthening is sound. Let $\pval \in \pvalues$, $\pval' \in \pvalues[\pscope_1]$,
$\pnode \in \pnodes$, $\rval \in \rvalues$, $\rval' \in \rvalues[\rscope_1]$,
$\delta \in \Delta(\pscope, \rscope)$, and $\delta_1 \in \Delta(\pscope_1, \rscope_1)$. 
If $\rval \rvord \pgamma[\delta](\pval)$ and $\rval' \rvord \pgamma[\delta_1](\pval')$,
then $\rupdate{\rval}{\delta(\pnode)}{\rval'} \rvord \supdate{\pval}{\pnode}{\pval'}$.
\end{lemma}
\begin{proof}
The proof is carried by structural induction on $\pval$. The proof in fact shows
that structural strengthening on collapsed values overapproximates the structural strengthening
on relational values. The argument then follows from Lemma~\ref{thm:r-structural-soundness} and Lemma~\ref{thm:cl-strengthenings-sound}.
\end{proof}



==> proofs/lq-semantics.tex <==
% !TEX root = ../../thesis.tex
\clearpage
\subsection{Liquid Types Semantics Proofs}
\label{sec:proofs-lq-semantics}


For the rest of this section, we assume the set of Liquid types $\tvalues$
is defined as described in \S~\ref{sec:liquid-types-ai}.



\subsubsection{Domain Operations}
We next show the basic results regarding the strengthening operations on Liquid Types.

\begin{lemma}~\label{thm:lq-v-strengthening}
The strengthening operations on Liquid types are sound and strengthening.
\end{lemma}
\begin{proof}
The results follow from the soundness and strengthening properties of the refinement
domain (follow from the semantics of logical conjunction), 
Lemma~\ref{thm:t-v-strengthening}, and Lemma~\ref{thm:t-structural-soundness}.
\end{proof}


We can also show that strengthening operations are idempotent. Here, we
assume that the strengthening of the liquid types refinement domain is idempotent.
This is true in practice as strengthening amounts to adding equality conjuncts.
\[ \rupdate{\paramelem}{\absn}{\paramelem_1} = \rupdate{\rupdate{\paramelem}{\absn}{\paramelem_1}}{\absn}{\paramelem_1} \quad\quad \text{idempotency}\]
%
\begin{lemma}~\label{thm:lq-v-strengthen-idempotent}
Let $\tval \in \tvalues$, $\tval_1 \in \tvalues$, and $\absn \in \absns$. 
Then, $\rupdate{\tval}{\absn}{\tval_1} = \rupdate{\rupdate{\tval}{\absn}{\tval_1}}{\absn}{\tval_1}$. 
\end{lemma}
\begin{proof}
The proof goes by the structural induction on $\tval$.
First, observe that if $\absn \not\in \pscope$, the argument is trivial.
Otherwise, if  $\tval_1 = \tbot$ then 
$\rupdate{\tval}{\absn}{\tbot} = \tbot = \rupdate{\rupdate{\tval}{\absn}{\tbot}}{\absn}{\tbot}$.
Next, if $\tval_1 \in \{\terr\} \cup \ttables[]$, then
$\rupdate{\tval}{\absn}{\tval_1} = \tval = \rupdate{\rupdate{\tval}{\absn}{\tval_1}}{\absn}{\tval_1}$.
We can thus just focus on the case where
$\tval \in \tyrels[]$. Let $\tval = \tyrel[\basetype_1]{\paramelem_1}$. 
We cover the base cases first.
\begin{itemize}
\item $\tval = \tbot$. Here, $\rupdate{\tbot}{\absn}{\tval_1} = \tbot = \rupdate{\rupdate{\tbot}{\absn}{\tval_1}}{\absn}{\tval_1}$.
\item $\tval = \terr$. Similar to the above case, $\rupdate{\terr}{\absn}{\tval_1} = \terr = \rupdate{\rupdate{\terr}{\absn}{\tval_1}}{\absn}{\tval_1}$.
\item $\tval = \tyrel{\paramelem}$. In this case,
$\rupdate{\tyrel{\paramelem}}{\absn}{\tval_1} = \tyrel{\rupdate{\paramelem}{\absn}{\paramelem_1}}$
and $\rupdate{\rupdate{\tyrel{\paramelem}}{\absn}{\tval_1}}{\absn}{\tval_1} = 
\rupdate{\tyrel{\rupdate{\paramelem}{\absn}{\paramelem_1}}}{\absn}{\tval_1} = 
\tyrel{\rupdate{\rupdate{\paramelem}{\absn}{\paramelem_1}}{\absn}{\paramelem_1}}$.
The result then follows from the idempotency of the refinement strengthening.
\end{itemize}
For the induction case where $\tval \in \ttables[]$, the result holds by the i.h.
\end{proof}


\begin{lemma}~\label{thm:lq-strengthenings-idempotent}
Strengthening operations on the liquid abstract domain of refinement are idempotent.
\end{lemma}
\begin{proof}
Follows the proof of Lemma~\ref{thm:lq-v-strengthen-idempotent}.
\end{proof}

\subsubsection{Data Propagation}


We can now prove that the sutbyping between types implies fixpoint in data propagation established
between those types.
\begin{zproof*}[of Lemma~\ref{thm:liq-subtyping-prop-fixpoint}]\end{zproof*}
\begin{proof}
The proof goes by an induction on the maximum depth of types $d = \mi{max}(\cvdepth(\tval_1), \cvdepth(\tval_2))$.
We first cover the base cases where $d = 1$. We only need to consider few cases based on the definition of $\liqsub$.
\begin{itemize}
%\item $\tval_1 = \tbot$. Then, $\tprop(\tbot, \tval_2) = \pair{\tbot}{\tval_2}$.
%\item $\tval_1 = \terr$. Then also $\tval_2 = \terr$ and we have $\tprop(\terr, \terr) = \pair{\terr}{\terr}$.
\item $\tval_1 = \tyrel{\paramelem_1}, \tval_2 = \tyrel{\paramelem_2}$, and 
$\paramelem_1 \paramord[] \paramelem_2$. We have 
$\tprop(\tyrel{\paramelem_1}, \tyrel{\paramelem_2}) = \pair{\tyrel{\paramelem_1}}{\tyrel{\paramelem_1 \paramjoin[] \paramelem_2}} = \pair{\tyrel{\paramelem_1}}{\tyrel{\paramelem_2}}$.
\end{itemize}

Let us now consider the induction case for $d > 1$ where $\tval_1 \in \ttables[]$ and $\tval_2 \in \ttables[]$. Let $\tprop(\tval_1, \tval_2) = \pair{\tval_3}{\tval_4}$.
Observe that the maximum depth of input and output types of $\tval_1$ and $\tval_2$ and 
their arbitrary strengthening is smaller than $d$ by the definition of $\cvdepth$ and 
Lemma~\ref{thm:lq-v-strengthening}.
Let $\tval_1= \ttab{\tval_{1i}}{\tval_{1o}}$ and $\tval_2 = \ttab{\tval_{2i}}{\tval_{2o}}$. 
By definition of $\liqsub$, we have that (1) $\tval_{2i} \,\liqsub\, \tval_{1i}$ and (2) 
$\rupdate{\tval_{1o}}{\absn}{\tval_{2i}} \,\liqsub\, \rupdate{\tval_{2o}}{\absn}{\tval_{2i}}$.
By i.h., we thus have $\tprop(\tval_{2i}, \tval_{1i}) = \pair{\tval_{2i}}{\tval_{1i}}$
and $\tprop(\rupdate{\tval_{1o}}{\absn}{\tval_{2i}}, \rupdate{\tval_{2o}}{\absn}{\tval_{2i}}) = 
\pair{\rupdate{\tval_{1o}}{\absn}{\tval_{2i}}}{\rupdate{\tval_{2o}}{\absn}{\tval_{2i}}}$.
By Lemma~\ref{thm:lq-v-strengthening}, we have 
$\rupdate{\tval_{2o}}{\absn}{\tval_{2i}} \tvord[] \tval_{2o}$ and
$\rupdate{\tval_{1o}}{\absn}{\tval_{2i}} \tvord[] \tval_{1o}$. Therefore, by the definition
of $\tprop$ it follows $\tval_3 = \ttab{\tval_{1i}}{\tval_{1o}} = \tval_1$ and
$\tval_4 = \ttab{\tval_{2i}}{\tval_{2o}} = \tval_2$.
\end{proof}



\subsubsection{Connection to Liquid Types}

%We first show that when $\ttrans{\cdot}$ reaches a fixpoint for a certain expression, the same
%is true for the subexpressions.
%
%\begin{lemma}~\label{thm:lq-fixpoint-subexpressions}
%Let $\tmap \in \tmaps$, $e^{\ell} \in \Exp$, and $\penv \in \penvironments$. If 
%$\ttrans{\cdot}$ reaches a fixpoint $\ttrans{e^{\ell}}(\tmap)(\penv) = \tmap$, the same
%is true for recursive calls to $\ttrans{\cdot}$ for the subexpressions of $e$.
%\end{lemma}
%\begin{proof}
%The proof goes by structural induction on $e$.
%\begin{itemize}
%\item $e=x^{\ell}$ or $e=c^{\ell}$. Trivial.
%\item $e = (e_1^{\ell_1}e_2^{\ell_2})^{\ell}$. By Lemma~\ref{thm:t-step-increasing}
%and Lemma~\ref{thm:tprop-increasing}, 
%$\tmap \tvecord \tmap_1 \tvecord \tmap_2 \tvecord \tmap$. Hence, $\tmap_1 = \tmap$ and 
%$\tmap_2 = \tmap$, concluding $\ttrans{e_1^{\ell_1}}(\tmap)(\penv) = \tmap$ as well as
%$\ttrans{e_2^{\ell_2}}(\tmap)(\penv) = \tmap$.
%
%\item $e = (\mu f.\lambda x.e_1^{\ell_1})^{\ell}$ or $e = \ifte{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}}$. 
%Similar.
%\end{itemize}
%\end{proof}


%To prove the formal connection between our model of Liquid type inference and the original
%work, we first provide a formal definition of $\kappa_e$ for a program, an injective mapping
%variables to their unique variable nodes created by $\tcoll[e]$. 
%We first define $\kappa_e \Def= \Lambda x \in \vars(e).\,\cn{\aenv(\scopevars_e(\m{lam\_loc}_{e,x}))}{x}$
%where $\m{lam\_loc(e, x)}$ is the location of the body of the lambda abstraction one of whose
%binding variables is $x$. In other words, $\kappa_e$ assigns to each program variable in $e$
%the abstract variable node created for that variable. That is, it is not hard to inductively 
%see that that every $x \in \vars(e)$, $\tcoll[e]$ creates a unique variable node $\kappa_e(x)$.
%This follows from Lemma~\label{thm:rt-finite-nodes}.

%\newcommand{\penve}{\emptyset}
%\newcommand{\tconstcons}{\m{tconst\_cons}}
%First, we say that a type map $\tmap$ is \textit{constant consistent}, denoted by 
%$\tconstcons_e(\tmap)$, subject to a program $e$ a iff for all abstract nodes $\pnode$
%
%\begin{itemize}
%\item $e(\nloc(\pnode)) = c \implies \tmap(\penv) \in \{\tbot, \terr\} \vee \tmap(\penv)=\tconst$
%\item $e(\nloc(\pnode)) \mu\_.\lambda\_.\_ \implies \tmap \in \{\tbot, \terr\} \cup \ttables[]$
%\end{itemize}
%
%Note that we use above the underscore pattern notation to existentially quantify out mathematical
%objects whose meta-level types should be obvious from the context. We use this notation to avoid 
%notational clutter that would otherwise be introduced by existential quantification.
%
%The above property is inductive
%\begin{lemma}~\label{thm:t-const-cons-inductive}
%Let $e$ be a program, $e^{\ell}_1 \in e$, $\tmap \in \tmaps$, and $\tmap_1 \in \tmaps$, and
%$\penv \in \penvironments$. If $\tconstcons_e(\tmap)$ and $\tmap_1 = \ttrans{e^{\ell}_1}(\penv)(\tmap)$,
%then $\tconstcons_e(\tmap_1)$. Also, $\tconstcons_e(\tmap_{\tbot})$.
%\end{lemma}
%\begin{proof}
%By structural induction on $e$. The result follows from the basic properties of $\tprop$
%and $\tvjoin[]$.
%\end{proof}
%
%\begin{zproof*}[of Theorem~\ref{thm:liquid-types}]\end{zproof*}
%\begin{proof}
%Note that the theorem only states the connection for the top level program expression where
%the environment is $\emptyset$. Hence, $\kappa_e = \emptyset$ as well.
%
%We carry the proof by case analysis on $e$.
%\begin{itemize}
%\item $e = c^{\ell}$. Since $\kappa_e = \emptyset$, we have that 
%$\tconst[\liqenv]^{\kappa} = \tconst$. Now, since $\tmap$ is safe, it must be 
%by Lemma~\ref{thm:t-const-cons-inductive} that $\tmap(\cn{\penve}{\ell}) = \tconst$.
%
%\item $e = (e_1^{\ell_1} e_2^{\ell_2})^{\ell}.$ Let $\tmap_1(\cn{\penve}{\ell_1}) \in \ttables[]$
%and $\tmap_2(\cn{\penve}{\ell_2}) \not \in \{\tbot, \terr\}$. By the fixpoint assumption,
%$\tprop(\tval_1, [\cn{\penve}{\ell_2} \mapsto \pair{\tmap_2(\cn{\penve}{\ell_2})}{\tmap_2(\cn{\penve}{\ell})}]) = \pair{\tval_1}{[\cn{\penve}{\ell_2} \mapsto \pair{\tmap_2(\cn{\penve}{\ell_2})}{\tmap_2(\cn{\penve}{\ell})}]}$. The result then follows from Lemma~\ref{thm:liq-subtyping}.
%
%\item $e = x^{\ell}$. Since $e$ is a program, this case cannot occur.
%
%\item Conditional. Similar.
%
%\end{itemize}
%\end{proof}

\newcommand{\liqtypm}[1][\kappa]{\vdash^{#1}_{\mathsf{m}}}
First, we define a typing relation $\liqtypm : \liqenvs^\kappa \times \Exp \times \tvalues[] \times \tmaps$ that
mimics the earlier typing relation $\liqtyp$, but also produces a type map that accumulates the results deduced
in the typing derivation. To this end, given a $\kappa$ and $\liqenv \in \liqenvs^\kappa$, we define 
$\tmap_{\kappa, \liqenv}$ to be a type map that holds $\liqenv(x)$ for all nodes 
$\pnode \in \m{rng}(\kappa)$ where $\kappa(x) = \pnode$; otherwise, it returns $\tbot$.
%
\begin{figure}[h!]
\[\begin{array}{c}
\infer{\liqenv \liqtypm x^{\ell} : \tval, \tmap_{\liqenv, \kappa}[\cn{\kappa(\liqenv)}{\ell} \mapsto \tval]}
{
\begin{array}{c}
x \in \m{dom}(\liqenv) \ind[2] \liqenv(x) \;\liqsub\; \tval \\ 
\tval = \liqenv(x)[\nu=\kappa(x)][\liqenv]^\kappa
\end{array}
}
\ind[3]
%
%
\infer{\liqenv \liqtypm \const^\ell :\tval, \tmap_{\liqenv, \kappa}[\cn{\kappa(\liqenv)}{\ell} \mapsto \tval]}{\tval= \tconst[\liqenv]^{\kappa}} \\[2ex]
%
%
\infer{\tmap, \liqenv \liqtypm (e_1^{\ell_1} e_2^{\ell_2})^\ell: \tval, (\tmap_1 \;\tmjoin\; \tmap_2)[\cn{\kappa(\liqenv)}{\ell} \mapsto \tval]}
{\begin{array}{c c}
\liqenv \liqtypm e_1^{\ell_1}: \tval_1, \tmap_1 & \liqenv \liqtypm e_2^{\ell_2}: \tval_2, \tmap_2 \\
\tval_1 \in \ttables[] & \tval_1 \;\liqsub\; \ptvar(\tval_1)\!:\tval_2 \to \tval
\end{array}
}\\[2ex]
%
%
\infer{\liqenv \liqtypm (\mu f. \lambda x.\,e_1^{\ell_1})^\ell : \tval, \tmap_1[\cn{\kappa(\liqenv)}{\ell} \mapsto \tval]}
{\begin{array}{c c c}
& \ptvar(\tval)\!:\tval_x \to \tval_1 \;\liqsub\; \tval \ind \tval \;\liqsub\; \tval_f & \\
\liqenv_1 = \liqenv.x:\!\tval_x.f\!:\tval_f & \kappa_1 = \kappa.x:\!\cn{\kappa(\liqenv)}{x}.f:\!\cn{\kappa(\liqenv)}{f}  & \liqenv_1 \liqtypm[\kappa_1] e_1^{\ell_1}: \tval_1, \tmap_1 \\[0.5ex]
\end{array}
}
%
%
\more{\\[2ex]
\infer{\liqenv \liqtypm (\ite{x}{e_1^{\ell_1}}{e_2^{\ell_2}})^\ell: \tval, (\tmap_0 \;\tmjoin\; \tmap_1 \;\tmjoin\; \tmap_2)[\cn{\kappa(\liqenv)}{\ell} \mapsto \tval]}
{\begin{array}{c c}
\liqenv \liqtypm x: \tval_0, \tmap_0 \quad\quad \tval_0 \;\liqsub\; \tbools & \tval_1 \,\liqsub\, \tval \quad \tval_2 \,\liqsub\, \tval\\
\liqenv_1 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \ttrue}
&  \liqenv_1 \liqtypm e_1: \tval_1, \tmap_1 \\
\liqenv_2 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \tfalse} & \liqenv_2 \liqtypm e_2: \tval_2, \tmap_2
\end{array}}
}
\end{array}\]
\end{figure}
%
\begin{lemma}~\label{thm:liqtyp-equiv}
Let $e$ be a program, $\kappa$ an injective mapping from variables to abstract nodes, $\tval \in \tvalues[]$, and $\liqenv \in \liqenvs^\kappa$. 
Then, $\liqenv \liqtyp e : \tval$ iff $\liqenv \liqtypm e: \tval, \tmap$ for some $\tmap \in \tmaps$. 
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. The result follows directly from the fact that $\liqtypm$ simply collects a type map $\tmap$,
without basing the rule premises on the contents of $\tmap$.
\end{proof}


\indent We now show several interesting but rather obvious properties of $\liqtypm$. 
%
\begin{lemma}~\label{thm:liqtypm-top}
Let $e$ be a program, $\kappa$ an injective mapping from variables to abstract nodes, $\tval \in \tvalues[]$, and $\liqenv \in \liqenvs^\kappa$. 
If $\liqenv \liqtypm e: \tval, \tmap$ for some $\tmap \in \tmaps$, then $\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval$. 
\end{lemma}
\begin{proof}
The proof is carried trivially by structural induction on $e$. 
\end{proof}
%

%\newcommand{\domvalid}{\m{\dom\_valid}}
Let domain validity $\domvalid(\ell, p, \liqenv)$ of a type environment $\liqenv$ subject to program $p$ and a location
$\ell$ in $p$ holds iff $\m{dom}(\liqenv)$ consists of exactly all variables bound above $\ell$ in $p$.
%
\begin{lemma}~\label{thm:liqtypm-env-agree}
Let $e^\ell$ be an expression of a program $p$, $\kappa$ and injective mapping from variables to abstract nodes, $\tval \in \tvalues[]$,
$\liqenv \in \liqenvs^\kappa$, and $\domvalid(\ell, p, \liqenv)$. 
If $\liqenv \liqtypm e: \tval, \tmap$ for some $\tmap \in \tmaps$, then $\forall x \in \m{dom}(\liqenv).\,\tmap(\kappa(x)) = \liqenv(x)$. 
\end{lemma}
\begin{proof}
The proof is carried by structural induction on $e$. First, we note that programs $p \in \Exp$ have unique variables. Due to this, 
domain validity is preserved for updates to typing environments when typing the bodies of recursive functions. Further, every typing
derivation has leaves at either variable or constant expressions where the environment assumptions are directly pushed to the maps.
Finally, $\liqenv_1$ and $\liqenv_2$ are smaller than $\liqenv$ when analyzing conditionals, due to strengthening, so the join of 
$\tmap_1$ and $\tmap_2$ with $\tmap_0$ ensures that the result holds since by i.h.\ $\forall x \in \m{dom}(\liqenv).\,\tmap_0(\kappa(x)) = \liqenv(x)$.
\end{proof}
%
%
%
%
\begin{lemma}~\label{thm:t-e-frame}
Let $e \in \Exp$, $\kappa$ an injective mapping from variables to abstract nodes, 
$\tval \in \tvalues[]$, $\liqenv \in \liqenvs^\kappa$, and $\tmap \in \tmaps$ such that $\liqenv \liqtypm e : \tval, \tmap$.
Then for every $\pnode \in \penodes$, if $\tmap(\pnode) \not= \tbot$ then $\nloc(\pnode) \in \locs(e)$.
\end{lemma}
\begin{proof}
By structural induction on $e$.
\end{proof}
%
\newcommand{\trange}{\m{trange}}
Let $\trange(\tmap) \Def= \setc{\pnode}{\tmap(\pnode) \not= \tbot}$ be a set of non-$\tbot$ nodes of $\tmap$.
%
\begin{lemma}~\label{thm:t-v-frame}
Let $p$ be a program, $\ell_1$ and $\ell_2$ locations in $p$ such that $\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$, 
$\kappa$ an injective mapping from variables to abstract nodes, $\tval_1 \in \tvalues[]$, $\tval_2 \in \tvalues[]$, 
$\liqenv \in \liqenvs^\kappa$, $\tmap_1 \in \tmaps$, $\tmap_2 \in \tmaps$, and $\domvalid(\ell_1, p, \liqenv)$ as well 
as $\domvalid(\ell_2, p, \liqenv)$. Suppose $\liqenv \liqtypm p(\ell_1): \tval_1, \tmap_1$ and 
$\liqenv \liqtypm p(\ell_2): \tval_2, \tmap_2$. Then, $\trange(\tmap_1) \cap \trange(\tmap_2) = \rng(\kappa)$.
\end{lemma}
\begin{proof}
The argument follows from Lemma~\ref{thm:t-e-frame}. Also, since $p$ is a program, the program variables of lambda
abstractions are unique. Therefore, the updates to $\liqenv$ in the derivation for $p(\ell_1)$ and $p(\ell_2)$ are
unique. Also, by domain validity of $\liqenv$, we have that $\kappa$ and $\liqenv$ are always extended (rather than
being updated, i.e., some bindings being rewritten). Therefore, only the variable nodes associated with $\liqenv$,
and hence in $\m{\rng}(\kappa)$, will and must appear in both $\tmap_1$ and $\tmap_2$. 
\end{proof}


%
\begin{lemma}~\label{thm:liqtypm-safe}
Let $e^\ell$ be an expression, $\kappa$ an injective mapping from variables to abstract nodes, $\tval \in \tvalues[]$, 
$\liqenv \in \liqenvs^\kappa$ a valid typing environment, $\tmap \in \tmaps$, and $\domvalid(\ell, p, \liqenv)$. Suppose 
$\liqenv \liqtypm e^\ell: \tval, \tmap$. Then, $\tmap$ is safe and $\tval \not= \terr$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. By $\liqenv$ being valid and the definition of $\liqsub$, further updates 
to the environment are also safe. Also, direct updates to the maps are safe by the definition of $\liqsub$. Finally, 
joins do not introduce errors by Lemma~\ref{thm:t-v-frame} and~\ref{thm:liqtypm-env-agree}. The fact that $\tval \not = \terr$ 
can be established then by Lemma~\ref{thm:liqtypm-top}.
\end{proof}

%\begin{lemma}~\label{thm:liqtypm-env-agree}
%Let $p$ be a program, $\ell_1$ and $\ell_2$ locations in $p$ such that $\locs(p(\ell_1)) \cap \locs(p(\ell_2)) = \emptyset$, 
%$\kappa$ an injective mapping from variables to abstract nodes, $\tval \in \tvalues[]$, $\liqenv \in \liqenvs^\kappa$, 
%$\tmap_1 \in \tmaps$, $\tmap_2 \in \tmaps$, and $\domvalid(\ell_1, p, \liqenv)$ as well as $\domvalid(\ell_2, p, \liqenv)$. 
%Suppose $\liqenv \liqtypm p(\ell_1): \tval_1, \tmap_1$ and $\liqenv \liqtypm p(\ell_2): \tval_2, \tmap_2$
% for some $\tmap \in \tmaps$, then $\forall x \in \m{dom}(\liqenv).\,\tmap(\kappa(x)) = \liqenv(x)$. 
%\end{lemma}
%\begin{proof}
%The proof is carried by structural induction on $e$. First, we note that programs $p \in \Exp$ have unique variables. Due to this, 
%domain validity is preserved for updates to typing environments when typing the bodies of recursive functions. Further, every typing
%derivation has leaves at either variable or constant expressions where the environment assumptions are directly pushed to the maps.
%Finally, $\liqenv_1$ and $\liqenv_2$ are smaller than $\liqenv$ when analyzing conditionals, due to strengthening, so the join of 
%$\tmap_1$ and $\tmap_2$ with $\tmap_0$, where by i.h.\ $\forall x \in \m{dom}(\liqenv).\,\tmap_0(\kappa(x)) = \liqenv(x)$, so the
%result follows from the basic properties of joins.
%\end{proof}

\newcommand{\liqtypc}[1][\kappa]{\vdash^{#1}_{\mathsf{c}}}
We next define a typing relation $\liqtypc: \tmap \times \liqenv^\kappa \times \Exp \times \tval$ that checks if a given type map
satisfies our Liquid typing relation. 
%
\begin{figure}[h!]
\[\begin{array}{c}
\infer{\tmap, \liqenv \liqtypc x^{\ell} : \tval}
{\begin{array}{c c}
x \in \m{dom}(\liqenv) & \liqenv(x)\;\liqsub\;\tval \\[0.5ex]
\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval & \tval = \liqenv(x)[\nu=\kappa(x)][\liqenv]^\kappa
\end{array}
} \ind[3]
%
\infer{\tmap, \liqenv \liqtypc \const^\ell : \tval}{\tval= \tconst[\liqenv]^{\kappa} & \tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval} \\[1ex]
%
\infer{\tmap, \liqenv \liqtypc (e_1^{\ell_1} e_2^{\ell_2})^\ell: \tval}
{\begin{array}{c c c}
\tmap, \liqenv \liqtypc e_1^{\ell_1}: \tval_1 & \tmap, \liqenv \liqtypc e_2^{\ell_2}: \tval_2 & \tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval\\[0.5ex] 
& \tval_1 \in \ttables[] \quad\quad \tval_1 \;\liqsub\; \ptvar(\tval_1)\!:\tval_2 \to \tval
\end{array}
}\\[1ex]
%
\infer{\tmap, \liqenv \liqtypc (\mu f. \lambda x.\,e_1^{\ell_1})^\ell : \tval}
{\begin{array}{c c c}
 & \ptvar(\tval)\!:\tval_x \to \tval_1 \;\liqsub\; \tval \quad\quad\quad \tval \;\liqsub\; \tval_f & \\
\liqenv_1 = \liqenv.x\!:\tval_x.f\!:\tval_f & \kappa_1 = \kappa.x\!:\cn{\kappa(\liqenv)}{x}.f\!:\cn{\kappa(\liqenv)}{f}  & \tmap, \liqenv_1 \liqtypc[\kappa_1] e^{\ell_1}:\tval_1\\
\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval & \tmap(\kappa_1(x)) = \tval_x \ind \tmap(\kappa_1(f)) = \tval_f & \tmap(\cn{\kappa_1(\liqenv_1)}{\ell_1}) = \tval_1
\end{array}
}
%
\more{\\[1ex]
\infer{\tmap, \liqenv \liqtyp (\ite{x^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}})^{\ell}: \tval}
{\begin{array}{c c}
\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval \ind[2] \tmap, \liqenv \liqtyp x: \tval_0 \quad \tval_0 \;{\liqsub}\; \tbools & \tval_1 \,\liqsub\, \tval \quad \tval_2 \,\liqsub\, \tval\\[0.5ex]
\liqenv_1 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \ttrue}
&  \tmap_{\liqenv_2, \kappa}, \liqenv_1 \liqtyp e_1: \tval_1 \\[0.5ex] 
\liqenv_2 = \Lambda x \in \m{dom}(\liqenv).\,\rupdate{\liqenv(x)}{\kappa(x)}{\tval_0 \tvmeet[] \tfalse} & \tmap_{\liqenv_1, \kappa}, \liqenv_2 \liqtyp e_2: \tval_2
\end{array}}
}
\end{array}\]
\end{figure}
%
%
\newcommand{\tmagree}{\m{tmagree}}
We say that two type maps $\tmap_1$ and $\tmap_2$ agree, denoted $\tmagree(\tmap_1, \tmap_2)$ iff
$\forall \pnode. \tmap_1(\pnode) \not= \tbot \wedge \tmap_2(\pnode) \not= \tbot \implies \tmap_1(\pnode) = \tmap_2(\pnode)$.
%
\begin{lemma}~\label{thm:t-split}
Let $e^\ell$ be an expression of $p$ be a program, $\kappa$ an injective mapping from variables to abstract nodes, 
$\tval \in \tvalues[]$, $\liqenv \in \liqenvs^\kappa$, $\tmap \in \tmaps$, $\tmap_0 \in \tmaps$, and $\domvalid(\ell, p, \liqenv)$.
If $\tmagree(\tmap, \tmap_0)$ and $\liqenv \liqtypm e: \tval, \tmap$, then $\tmap_0, \liqenv \liqtypc e: \tval$.
\end{lemma}
\begin{proof}
By structural induction on $e$.
\begin{itemize}
\item $e^\ell = c^\ell$. Trivial.

\item $e^\ell = x^\ell$. Also straightforward.

\item $e^\ell = (e_1^{\ell_1} e_2^{\ell_2})^\ell$. By Lemma~\ref{thm:t-v-frame} and~\ref{thm:liqtypm-env-agree}, we have that
$\tmagree(\tmap_1, \tmap_0)$ and $\tmagree(\tmap_2, \tmap_0)$. The result then follows from the induction hypothesis.

\item $e^\ell = (\mu f.\lambda x. e_1^{\ell_1})^\ell$. Similar to the previous case.

%\item $e^\ell = (\ite{x^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}})^\ell$. Similar, the argument again relies on Lemma~\ref{thm:t-v-frame} and~\ref{thm:liqtypm-env-agree}.
\end{itemize}
\end{proof}




We can now easily show an important connection between $\liqtypm$ and $\liqtypc$.
\begin{lemma}~\label{thm:t-liqtypm-m-c}
Let $e^\ell$ be an expression of $p$ be a program, $\kappa$ an injective mapping from variables to abstract nodes, 
$\tval \in \tvalues[]$, $\liqenv \in \liqenvs^\kappa$, $\tmap \in \tmaps$, and $\domvalid(\ell, p, \liqenv)$.
If  $\liqenv \liqtypm e: \tval, \tmap$, then $\tmap, \liqenv \liqtypc e: \tval$.
\end{lemma}
\begin{proof}
Direct corollary of Lemma~\ref{thm:t-split}.
\end{proof}


We say a triple $(\liqenv, \tmap, \kappa)$ \textit{matches} if $\forall x \in \m{dom}(\liqenv).\, \liqenv(x) = \tmap(\kappa(x))$. 
%
\begin{theorem}~\label{thm:liqtypc-fixpoint}
Let $e^{\ell}$ be an expression, $\kappa$ an injective encoding of abstract variable nodes,
$\liqenv \in \liqenvs^\kappa$, $\tmap$ a safe type map, and $\tval \in \tvalues[\pscope_\kappa]$. 
If $\tmap, \liqenv \liqtypc e^{\ell}: \tval$ and $(\liqenv, \tmap, \kappa)$ match, 
then $\Ttrans{e^\ell}(\cn{\kappa(\liqenv)}{\ell})(\tmap)= \tmap$ and $\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tval$. 
\end{theorem}
\begin{proof}
The proof goes by structural induction on $e$.
%
\begin{itemize}
\item $e = x^\ell$. By matching $(\liqenv, \tmap, \kappa)$, we have that 
$\kappa(\liqenv)(x) = \kappa(x)$ and $\tmap(\kappa(\liqenv)(x)) = \liqenv(x)$.
Hence, $\tmap(\kappa(\liqenv)(x)) \;\liqsub\; \tmap(\cn{\kappa(\liqenv)}{\ell})$.
Then by the definition of $\liqtypc$, we have that 
$\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tmap(\kappa(\liqenv)(x))[\nu=\kappa(x)][\liqenv]^\kappa$ 
and hence by matching $(\liqenv, \tmap, \kappa)$ we have 
$\tmap(\cn{\kappa(\liqenv)}{\ell}) = \tmap(\kappa(\liqenv)(x))[\nu=\kappa(\liqenv)(x)][\tmap]$.
Therefore, $\tmap(\kappa(\liqenv)(x))[\nu=\kappa(\liqenv)(x)] \;\liqsub\; \tmap(\cn{\kappa(\liqenv)}{\ell})$ 
by the structural definition of strengthening. The result then follows from 
Lemma~\ref{thm:liq-subtyping-prop-fixpoint} and Lemma~\ref{thm:lq-strengthenings-idempotent}.


\item $e = c^\ell$. The result follows from the definition of $\tconst[\liqenv]^{\kappa}$.
That is, $\tconst[\liqenv]^{\kappa} = \tconst[\tmap]$ by matching $(\liqenv, \tmap, \kappa)$. 


\item $e = (e_1^{\ell_1} e_2^{\ell_2})^{\ell}$. By i.h., we have that
$\Ttrans{e_1^{\ell_1}}(\kappa(\liqenv))(\tmap) = \tmap$ and $\tmap(\cn{\kappa(\liqenv)}{\ell_1}) = \tval_1$ where $\tval_1 \in \ttables[]$. Similarly,
$\Ttrans{e_2^{\ell_2}}(\kappa(\liqenv))(\tmap) = \tmap$ and  
$\tmap(\cn{\kappa(\liqenv)}{\ell_2}) = \tval_2$ where $\tval_2 \not \in \{\tbot, \terr\}$ by the definition of $\liqsub$.
Then by the definition of $\Ttrans{\cdot}$, we thus have that $\tmap_1 = \tmap_2 = \tmap$ and
the result then follows from Lemma~\ref{thm:liq-subtyping-prop-fixpoint}.

\item $e = (\mu f. \lambda x.\,e^{\ell_1})^\ell$. First, by the definition of $\liqsub$,
it must be that $\pi_1(\ptio(\ttable)) \not \in \{\tbot, \terr\}$. Further, by the definition 
of $\Ttrans{\cdot}$ and Lemma~\ref{thm:liq-subtyping-prop-fixpoint}, we have that $\ttable = \ttable_1 = \ttable_2$,
$\tval_x = \tval'_x$, $\tval_f = \tval'_f$, and $\tval_1 = \requality{\tval'_1}{\pnode_x}{\ptvar(\ttable)}$ since
$\ptvar(\ttable)$ is not initially in the scope of $\tval_1$ ($\pnode_x$ and $\ptvar(\ttable)$ are simply used as synonym variables).
Next, by $\domvalid(\ell, p, \liqenv)$ 
it follows that $(\liqenv_1, \kappa_1, \tmap)$ is matching and that domain validity is preserved $\domvalid(\ell_1, p, \liqenv_1)$ .
Also, by $\Ttrans{\cdot}$ we have that $\kappa(\liqenv_1) = \penv_1$. Hence, $\tmap_1 = \tmap$ by the induction hypothesis. 

%\begin{comment}
%\item $e = (\ifte{x^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}})^\ell$. First, observe that by definition of $\liqsub$,
%if $\tval_0 \liqsub \tbools$, then $\tval_0 \not= \tbot$ and $\tval_0 \tvord[] \tbools$. Next, by i.h.,
%we have that $\tmap_0 = \tmap$ and $\tval_0$ in $\liqtypc$ and $\Ttrans{\cdot}$ are the same. Now, $\Ttrans{\cdot}$
%strengthens the environment nodes of $\kappa(\liqenv)$ in $\tmap_0$, using the node $\cn{\penv}{\ell_0}$, while
%the typing relation $\liqtypc$ uses $\kappa(x)$. However, by the typing rule of $\liqtypc$ for variable nodes, we 
%know that $\liqenv(x) \;\liqsub\; \tval_0$ where $\tval_0 = \requality{\liqenv(x)}{\nu}{\kappa(x)}[\tmap_0]$. By
%matching $(\liqenv, \kappa, \tmap_0)$ (that is implied by matching $(\liqenv, \kappa, \tmap)$ and $\tmap_0 = \tmap$),
%we have $\tval_0 = \requality{\tmap_0(\kappa(\liqenv)(x))}{\nu}{\kappa(\liqenv)(x)}[\tmap_0]$.
%%By the definition of $\tbools$, it must be that $\tmap_0(\kappa(\liqenv)(x)) = \tyrel[\tbool]{\paramelem_1}$ 
%%for some $\paramelem_1$ and $\tval_0 = \tyrel[\tbool]{\paramelem_1}[\nu = \kappa(\liqenv)(x)][\tmap_0]$.
%By the definition of the liquid abstract domain, $\tval_0$ implies that $\kappa(\liqenv)(x) = \cn{\penv}{\ell_0}$
%and thus $\kappa(x) = \cn{\penv}{\ell_0}$.
%%By the definition of $\liqsub$ and Lemma~\ref{thm:lq-v-strengthening}, we have that 
%%$\tmap(\kappa(\liqenv)(x)) = \tval_0$ (modulo implicit rescoping).
%%By the definition 
%%of $\liqsub$, we have that $\paramelem_1 \paramord[] \paramelem_2$. As we can think  of liquid domain elements 
%%as conjunctions of logical formulas, we have that $\paramelem_1 {\implies} \paramelem_2$ and 
%%$\paramelem_2 {\implies} \kappa(x) = \nu$ by $\tval_0 = \tval_0[\nu=\kappa(x)]$. Similarly, 
%%$\paramelem_2 {\implies} \paramelem_1[\nu/\kappa(x)]$ by $\tval_0 = \tval_0[\liqenv]^\kappa$. 
%%Therefore, $\paramelem_1$ and $\paramelem_2$ are equivalent (modulo implicit rescoping). 
%Since $\cn{\penv}{\ell_0}$ is not in the scope of any node in $\pscope_{\cn{\penv}{\ell_0}}$, we have 
%$\tmap_i = \rupdate{\tmap_0}{\cn{\penv}{\ell_0}}{\ttrue \tvmeet[] \tval_0} = \rupdate{\tmap_0}{\kappa(x)}{\ttrue \tvmeet[] \tval_0} = \tmap_{\liqenv_1, \kappa}$ and
%$\tmap_j = \rupdate{\tmap_0}{\cn{\penv}{\ell_0}}{\tfalse \tvmeet[] \tval_0} = \rupdate{\tmap_0}{\kappa(x)}{\tfalse \tvmeet[] \tval_0} = \tmap_{\liqenv_2, \kappa}$. 
%Therefore, $(\liqenv_1, \kappa_1, \tmap_i)$ is matching and so is $(\liqenv_2, \kappa_2, \tmap_j)$. By i.h.\ then,
%we have $\tmap_1 = \tmap_i$ and $\tmap_2 = \tmap_j$. By Lemma~\ref{thm:liq-subtyping-prop-fixpoint}, we thus have
%that $\tval = \tval' = \tval''$, $\tval_1 = \tval'_1$, and $\tval_2 = \tval'_2$. The result then follows from the 
%fact that both $\tmap_i$ and $\tmap_j$, and consequently $\tmap_1$ and $\tmap_2$, are smaller than $\tmap_0$ that is equal to $\tmap$.
%\end{comment}
\end{itemize}
\end{proof}

\begin{zproof*}[of Theorem~\ref{thm:liquid-types}]\end{zproof*}
\begin{proof}
Our implicit assumption is that $e^{\ell}$ is an expression of a program $p$ such
that $\domvalid(\ell, p, \liqenv)$. Then
by Lemma~\ref{thm:liqtyp-equiv}, there exists a type map $\tmap$ such that $\liqenv \liqtyp e: \tval$
iff $\liqenv \liqtypm e : \tval, \tmap$. Let $\tmap$ be such map. We know this map is safe
by Lemma~\ref{thm:liqtypm-safe} and that it satisfies $\tmap, \liqenv \liqtypc e : \tval$.
We also know by Lemma~\ref{thm:liqtypm-env-agree} that $(\liqenv, \tmap, \kappa)$ is matching.
The result then follows from Theorem~\ref{thm:liqtypc-fixpoint}.
\end{proof}





==> proofs/path-semantics.tex <==
\clearpage
\subsubsection{Path Data Flow Semantics}

In this section, we introduce an alternative definition of the concrete
data flow semantics that, besides data flow values, also keeps track
of paths the data flow values take. This semantics can be thought of as
accumulating ghost information of the data flow semantics. We will use
this ghost information to show several useful properties of the original
data flow semantics.

\paragraph{Semantic Domains}

We define paths $\wpath \in \wpaths$ as a sequence of nodes
$\cnodes^{+}$. The path data flow
values are defined in a similar way as are the data flow values 
except that path information is maintained as well.
%
\begin{align*}
\wval \in \wvalues \; ::= {} & \; \wbot \mid \werr \mid \cw{\const}{\wpath} \mid \cw{\wtable}{\wpath} & \text{path (data flow) values}\\
\wtable \in \wtables \; \Def= {} & \; \wpaths \to \wvalues \times \wvalues & \text{path tables}\\
\wmap \in \wmaps \; \Def= {} & \; \cnodes \to \wvalues & \text{path execution maps}
\end{align*}
%
The set $\wconsts \Def= \consts \times \wpaths$ denotes the set of all constant path values
that also Boolean path values $\wbools \Def= \{\btrue, \bfalse\} \times \wpaths$.

The computational partial ordering on path values is defined similarly to the ordering
on the ordinary the data flow values. In addition, we require that corresponding
paths are related by the prefix relation $\wpord$.
\begin{align*}
\wval_1 \wvord \wval_2 {\Def\iff} & \wval_1 = \wbot \;\vee\; \wval_2 = \werr
   \;\vee \\ 
   & (\wval_1 = \cw{\const}{\wpath_1} \wedge \wval_2 = \cw{\const}{\wpath_2} \wedge \const \in \consts \wedge \wpath_1, \wpath_2 \in \wpaths \wedge \wpath_1 \wpord \wpath_2) \;\vee\\
  & \wval_1{=}\cw{\wtable_1}{\wpath_1} \wedge \wval_2{=}\cw{\wtable_2}{\wpath_2} \wedge \wtable_1, \wtable_2 {\in} \wtables \wedge \wpath_1,\wpath_2 \in \wpaths \wedge \wpath_1 \wpord \wpath_2 \\
  & \;\wedge \forall \ccsite.\, \wtable_1(\ccsite) \mathrel{\vecop{\wvord}} \wtable_2(\ccsite)
\end{align*}
%
The join on the path values is defined as follows.
\begin{align*}
%
\cw{\const}{\wpath_1} \wvjoin \cw{\const}{\wpath} \Def= \cw{\const}{\wpath} \ind[2]
\text{if } \wpath_1 \wpord \wpath_2 \vee \wpath_2 \wpord \wpath_1 \text{ and }\\
\wpath = \ite{\wpath_1 \wpord \wpath_2}{\wpath_2}{\wpath_1}\\
%
\cw{\wtable_1}{\wpath_1} \wvjoin \cw{\wtable_2}{\wpath_2} \Def= \cw{\Lambda \ccsite.\, \ptable_1(\ccsite) \dot{\wvjoin} \ptable_2(\ccsite)}{\wpath} \ind[2]
\text{if } \wpath_1 \wpord \wpath_2 \vee \wpath_2 \wpord \wpath_1 \text{ and }\\
\wpath = \ite{\wpath_1 \wpord \wpath_2}{\wpath_2}{\wpath_1}\\
%
\wbot \wvjoin \wval \Def= \wval \quad\quad  \wval \wvjoin \wbot \Def= \wval \quad\quad \wval_1 \wvjoin \wval_2 \Def= \werr \quad \text{(otherwise)}
\end{align*}
%
The meet on path values is defined similarly, as expected.
\begin{lemma}~\label{thm:w-v-join-meet-sound}
The join $\wvjoin$ and $\wvmeet$ on path values are lub and glb operators subject to the $\wvord$ ordering. 
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:cvjoin}.
\end{proof}
%
An empty table that maps every call site to the pair of $\wbot$ values is denoted by $\wtable_\wbot$.
We reuse the notation for denoting singleton tables from the data flow semantics. The same applies for
the notation $\ccsite \in \wtable$ denoting if some non-$\wbot$ input has been seen for the call 
site $\ccsite$ in a given table $\wtable$.
A path value map $\wmap \in \wmaps \Def= \cnodes \to \wvalues$ is a function from nodes to path 
values, as expected. Path maps $\wmap_\wbot$ and $\wmap_\werr$ assign to each node the $\wbot$
and $\werr$ value, respectively.

We also define a function $\allpaths$ that collects paths of a value
\begin{align*}
\allpaths(\wbot) \Def= & \emptyset \ind[2] \allpaths(\werr) \Def={} \emptyset \ind[2] \allpaths(\cw{\const}{\wpath}) \Def= {} \{\wpath\} \\
\allpaths(\cw{\wtable}{\wpath}) \Def= & \{\wpath\} \cup \bigcup_{\wpath' \in \wtable} \{\wpath'\} \cup \allpaths(\pi_1(\wtable(\wpath'))) \cup \allpaths(\pi_2(\wtable(\wpath')))
\end{align*}
%
All paths $\allpaths(\wmap)$ of path map $\wmap$ are defined as the
union of all paths of values in the map, as expected.

\subsubsection{Data Propagation}

The data propagation $\wprop:\wvalues\times\wvalues\to\wvalues\times\wvalues$ on path values 
closely resembles the data propagation on the plain data flow values. The main difference is 
that a meaningful propagation only happens in the case when the paths of the given values 
match by the $\wpord$ relation. Otherwise, the propagation just sets both values to top $\werr$.
As we shall see shortly, such cases never happen during the computation.
%
\begin{figure}[h!]
\[
\begin{array}{r l}
%\cprop(\const, \bot) \Def=& \pair{\const}{\const} \ind[4] \cprop(\ctable, \bot) \Def= \;\pair{\ctable}{\ctable_{\bot}} \ind[4] \cprop(\cerr, \bot) \Def= \;\pair{\cerr}{\cerr}  \\[1.25ex]
\wprop(\cw{\wtable_1}{\wpath_1}, \cw{\wtable_2}{\wpath_2}) \Def=&  \ind[15] \text{if } \wpath_1 \wpord \wpath_2 \\ [1ex]
\multicolumn{2}{l}{\;\; \Mlet \ctable' = \Lambda \wpath. } \\[1ex]
\multicolumn{2}{l}{\ind[1]\Mif \wpath \not\in \wtable_2 \;\Mthen \pair{\wtable_1(\wpath)}{\wtable_2(\wpath)} \;\Melse} \\[1ex]
\multicolumn{2}{l}{\ind[1]\Mlet \pair{\wval_{1i}}{\wval_{1o}} = \wtable_1(\ccsite) \Mend \pair{\wval_{2i}}{\wval_{2o}} = \wtable_2(\ccsite)} \\ [1ex]
\multicolumn{2}{l}{\ind[2]\;\;\pair{\wval'_{2i}}{\wval'_{1i}} = \wprop(\wval_{2i}, \wval_{1i}) \Mend \pair{\wval'_{1o}}{\wval'_{2o}} = \wprop(\wval_{1o}, \wval_{2o})} \\[1ex]
%&\ind[2] \;\; \pair{\cval'_{1o}}{\cval'_{2o}} = \Mif \cval'_{1i} = \cval'_{2i} \;\Mthen \cprop(\cval_{1o}, \cval_{2o}) \;\Melse \pair{\cval_{1o}}{\cval_{2o}} \\[0.5ex]
\multicolumn{2}{l}{\ind[1] \Min (\pair{\wval'_{1i}}{\wval'_{1o}}, \pair{\wval'_{2i}}{\wval'_{2o}}) \quad\quad\quad \ind[4]} \\[1ex]
\multicolumn{2}{l}{\;\; \Min \pair{\Lambda \wpath.\; \pi_1(\ctable'(\wpath))}{\Lambda \wpath.\; \pi_2(\ctable'(\wpath))}} \\[2ex]
%
\wprop(\cw{\wtable}{\wpath}, \wbot) \Def= &  (\cw{\wtable}{\wpath}, \cw{\wtable_{\wbot}}{\wpath}) \ind[2] \wprop(\cw{\wtable}{\wpath}, \werr) \Def=  \pair{\werr}{\werr} \\[2ex]
%
\wprop(\cw{\wtable_1}{\wpath_1}, \cw{\wtable_2}{\wpath_2}) \Def=& \pair{\werr}{\werr} \ind[12]\; \text{if } \wpath_1 \not\wpord \wpath_2 \\ [3ex]


\wprop(\cw{\const}{\wpath_1}, \cw{\const}{\wpath_2}) \Def=& (\cw{\const}{\wpath_1}, \cw{\const}{\wpath_2}) \ind[8]\;\; \text{if } \wpath_1 \wpord \wpath_2 \\ [2ex]
%
\wprop(\cw{\const}{\wpath_1}, \cw{\const}{\wpath_2}) \Def=& \pair{\werr}{\werr} \ind[12]\; \text{if } \wpath_1 \not\wpord \wpath_2 \\ [3ex]

%\cprop(\cval_1, \cval_2) \Def= &  \pair{\cval_1}{\cval_2} \ind[3] \textbf{(otherwise)}
\wprop(\wval_1, \wval_2) \Def= &  \pair{\wval_1}{\wval_1 \wvjoin \wval_2} \ind[8] \textbf{(otherwise)}
\end{array}\]
\end{figure}
%
\begin{lemma}~\label{thm:w-prop-increasing-monotone}
$\wprop$ is increasing and monotone.
\end{lemma}
\begin{proof}
By structural induction on the arguments of $\wprop$. The argument for the increasing property is rather
straightforward. Regarding monotonicity, arguably the most interesting case is that of constants.
Suppose $\wval_1 = \cw{\const}{\wpath_1}$, $\wval_2 = \cw{\const}{\wpath_2}$, $\wval_3 = \cw{\const}{\wpath_3}$,
and $\wval_4 = \cw{\const}{\wpath_4}$. Let $\wval_1 \wvord \wval_3$ and $\wval_2 \wvord \wval_4$.
First, if $\wpath_1 \not\wpord \wpath_2$ then $\wpath_3 \not\wpord \wpath_4$ since by the definition
of $\wvord$ it must be that $\wpath_1 \wpord \wpath_3$ and $\wpath_2 \wpord \wpath_4$. In this case,
the argument is trivial. If $\wpath_1 \wpord \wpath_2$ the argument is again simple as the values
$\wval_1$ and $\wval_2$ do not get updated. Assume now that $\wval_2 = \wbot$ and $\wval_4 = \wbot$. 
The argument is again straightforward. Lastly, assume that only $\wval_2 = \wbot$ (note that we cannot 
have the case when only $\wval_4 = \wbot$ since we assume for the purpose of showing monotonicity 
that $\wval_2 \wvord \wval_4$). The propagation will result in an updated value $\wval'_2 = \wval_1$. 
If $\wpath_3 \not \wvord \wpath_4$, the argument is easy. Otherwise, since $\wpath_1 \wpord \wpath_3$ 
and $\wpath_3 \wpord \wpath_4$, then it also must be that $\wpath_1 \wpord \wpath_4$. The same
reasoning, together with the induction hypothesis, applies to the case of tables.
\end{proof}
%
It can be also shown that the propagation does not invent new paths. That is, propagation between two values
results in two values where each resulting value is either top $\werr$ or a new path values that has the same
path as the original path value.
\begin{lemma}~\label{thm:w-prop-paths}
Let $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ for some path values $\wval_1, \wval'_1, \wval_2$, and $\wval'_2$.
Then, if $\wval_1 = \pair{\_}{\wpath}$ for some path $\wpath$, then $\wval'_1 = \werr$ or $\wval'_2 = \pair{\_}{\wpath}$.
The same hold for $\wval_2$ and $\wval'_2$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\wval_1$ and $\wval_2$. 
\end{proof}


\subsubsection{Transformer}

The transformer $\wtransname:\Exp \to \cenvironments \to \wmaps \to \wmaps$
of the paths semantics works similarly as the transformer for the original data flow semantics.
The only difference is that the path information needs to be properly handled when creating
new values. For that purpose, we introduce a function for extending path information in path
values with nodes.
%
\begin{align*}
\ext(\wpath, \cnode) \Def= \wpath \ind[2]\text{if } \ptop(\wpath) = \cnode && 
\ext(\wpath, \cnode) \Def= \wpath\cdot\cnode \ind[2]\text{(otherwise)}\\[1ex]
%
\ext(\cw{\wtable}{\wpath}, \cnode) \Def= \cw{\wtable}{\ext(\wpath, \cnode)} &&
\ext(\cw{\const}{\wpath}, \cnode) \Def= \cw{\const}{\ext(\wpath, \cnode)}\\
\ext(\werr, \cnode) \Def= \werr && \ext(\wbot, \cnode) \Def= \wbot
\end{align*} 
%
Here, we use $\ptop$ to denote the top/final node of a path. Further, $\cdot$ operation
concatenates two given paths. Note that we also consider a node as a path. Finally,
observe that the operation $\ext$ on paths is idempotent. Also, let $\ppath$ be a partial
function on path values that returns a path associated with the value, if such a path exists.
\begin{figure}[h!]
  \centering
\[\begin{array}{l}
% base case
\more{\wtrans[0]{e}(\cenv)(\wmap) \Def= \wmap \quad\quad\quad} \\[1.5ex]

%constant
%\ctrans{c^\elabel}(\cenv)(\cmap) \Def= \Mif \cmap(\cn{\cenv}{\elabel}) = \bot \;\Mthen \cmap[\cn{\cenv}{\elabel} \mapsto c]  \;\Melse \cmap\\[2.5ex]
\wtrans{c^\elabel}(\cenv)(\wmap) \Def= \wmap[\cn{\cenv}{\elabel} \to \wmap(\cn{\cenv}{\elabel}) \cvjoin \cw{\const}{\cn{\cenv}{\elabel}}] \\[1.5ex]

% var
\wtrans{x^\elabel}(\cenv)(\wmap) \Def= \\[0.5ex]
\sind 	\Mlet \pair{\wval_x'}{\wval'} = \wprop(\wmap(\cenv(x)),
    \wmap(\cn{\cenv}{\elabel})) \\[0.5ex]
\sind    \Min \wmap[\cenv(x) \mapsto \wval_x', \cn{\cenv}{\elabel} \mapsto \ext(\wval',\cn{\cenv}{\elabel})] \\[1.5ex]

%function application
\wtrans{(e_1^{\elabel_1} e_2^{\elabel_2})^\elabel}(\cenv)(\wmap) \Def=  \\[0.5ex] 
\sind 	\Mlet \wmap_1 = \wtrans[k]{e_1}(\cenv)(\wmap) \Mend \wval_1 =_{\wmap_1} \wmap_1(\cn{\cenv}{\elabel_1}) \;\Min \\[0.5ex]
%\ind	\Mif \cval_1 = \bot \;\Mthen \cmap_1 \;\Melif \cval_1 \not \in \ctables \;\Mthen \cmap_{\cerr} \;\Melse \\[0.5ex]
\sind	\Mif \wval_1 \not \in \wtables \;\Mthen \wmap_{\werr} \;\Melse \\[0.5ex]
\sind[2]	\Mlet \wmap_2 = \wtrans[k]{e_2}(\cenv)(\wmap_1) \Mend \wval_2 =_{\wmap_2} \wmap_2(\cn{\cenv}{\elabel_2}) \;\Min \\[0.5ex]
%\ind[2]	\Mif \cval_2 = \bot \;\Mthen \cmap_2 \;\Melif \cval_2 = \cerr \;\Mthen \cmap_{\cerr} \;\Melse\\[0.5ex]
%    \ind[3]	\Mlet \cval = \cmap_2(\cn{\cenv}{\elabel})\\[0.75ex]
%    \ind[4] \;\ctable = \ctable_{\bot}[\pair{\cn{\cenv}{\elabel_2}}{\cn{\cenv}{\elabel}} \mapsto \pair{\cval_2}{\cval}]\\[0.5ex]
 %   \ind[4] \;\pair{\cval'_1}{\ctable'} = \cprop(\cval_1, \ctable_{\bot}[\cn{\cenv}{\elabel_2} \mapsto \pair{\cval_2}{\cval}])\\[0.5ex]
    \sind[2] \Mlet \pair{\wval'_1}{\wtable} = \wprop(\wval_1, [\ppath(\wval_1) \mapsto \pair{\wval_2}{\wmap_2(\cn{\cenv}{\elabel})}])\\[0.5ex]
    \sind[7] \pair{\wval'_2}{\wval'} = \wtable(\ppath(\wval_1)) \\[0.5ex]
\sind[2]	\Min \wmap_2[\cn{\cenv}{\elabel_1} \mapsto \wval'_1,
\cn{\cenv}{\elabel_2} \mapsto \wval'_2, \cn{\cenv}{\elabel} \mapsto \ext(\wval', \cn{\cenv}{\ell})] \\[1.5ex]


%%lambda abstraction
%\ctrans{(\mu f. \lambda x^.e^{\elabel_1})^{\elabel}}(\cenv)(\cmap) \Def= \\[0.75ex]  
%\ind	\Mlet \ctable = \Mif \cmap(\cn{\cenv}{\elabel}) = \bot \;\Mthen \ctable_{\bot} \;\Melse \cmap(\cn{\cenv}{\elabel}) \Min \\[0.75ex]
%\ind	\Mlet \cmap' = \Lambda \cenode_i, \cenode_o.\; \\[0.75ex]
%\ind[2]	\Mlet \pair{\cval_i}{\cval_o} = \ctable(\cenode_i, \cenode_o) \Min \\[0.75ex]	
%\ind[2] \Mif \cval_i = \bot \;\Mthen \cmap \;\Melse \\[0.75ex]
%\ind[3]	\Mlet \cvnode_x = \cvn{\cenv}{\pair{\cenode_i}{\cenode_o}}{\vlabel} \Mand \cvnode_f = \cvn{\cenv}{\pair{\cenode_i}{\cenode_o}}{\vlabel[f]}  \Min \\[0.75ex]
%\ind[3]  \Mlet \pair{\cval'_i}{\cval'_x} = \cprop(\cval_i, \cmap(\cvnode_x)) \Mand \pair{\ctable'}{\cval'_f} = \cprop(\ctable, \cmap(\cvnode_f)) \Min \\[0.75ex]
%\ind[3]	\Mlet \cenv_1 = \cenv[x \mapsto \cvnode_x][f \mapsto \cvnode_f] \Min \\[0.75ex]
%\ind[3]	\Mlet \cmap_1 = \ctrans{e^{\elabel_1}}(\cenv_1)(\cmap[\cvnode_x \mapsto \cval'_x][\cvnode_f \mapsto \cval'_f]) \Min \\[0.75ex]
%\ind[3]	\Mlet \pair{\cval'_b}{\cval'_o} = \cprop(\cmap_1(\cn{\cenv_1}{\elabel_1}), \cval_o) \Min \\[0.75ex]
%\ind[4] \cmap_1[\cn{\cenv_1}{\elabel_1} \mapsto \cval'_b][\cn{\cenv}{\elabel} \mapsto \ctable[\pair{\cenode_i}{\cenode_o} \mapsto \pair{\cval'_i}{\cval'_o}]] \Min\\[1ex]
%\ind[2] \cmjoinb \setc{\cmap'(\cenode_1, \cenode_2)}{\cenode_1 \in \cenodes \wedge \cenode_2 \in \cenodes} \\[2ex]

%lambda abstraction
\wtrans{(\mu f. \lambda x.e_1^{\elabel_1})^{\elabel}}(\cenv)(\wmap) \Def= \\[0.5ex]  
\sind	\Mlet T_w =_{\wmap} \cw{\wtable_{\wbot}}{\cn{\cenv}{\ell}} \wvjoin \wmap(\cn{\cenv}{\elabel}) \;\Min \\[0.5ex]
%\ind	\Mif \ctable = \cerr \;\Mthen \cmap_{\cerr} \;\Melse \\[0.5ex]
%\sind	\Mlet \overline{\cmap} = \Lambda \ccsite.\, \Mif \pi_1(\ctable(\ccsite)) = \bot \;\Mthen \cmap \;\Melif \pi_1(\ctable(\ccsite)) = \cerr \;\Mthen \cmap_{\cerr} \;\Melse  \\[0.5ex] 
\sind	\Mlet \overline{\wmap} = \Lambda \wpath \in T_w.\, \Mif \pi_1(\wtable(\ccsite)) = \werr \;\Mthen \wmap_{\werr} \;\Melse  \\[0.5ex] 
%\ind[2]	\Mlet \pair{\cval_i}{\cval_o} = \ctable(\cenode_i, \cenode_o) \Min \\[0.5ex]	
%\ind[2] \Mif \cval_i = \bot \;\Mthen \cmap \;\Melse \\[0.5ex]
\sind[2]	\Mlet \cnode_x {=} \cvn{\cenv}{\ptop(\wpath)}{x} \Mend \cnode_f
{=} \cvn{\cenv}{\ptop(\wpath)}{f} \Mend \cenv_1 {=} \cenv[x {\mapsto} \cnode_x, f {\mapsto} \cnode_f]\\[0.5ex]
%\ind[3]	\;\pair{\ctable'_x}{\ctable'} = \cprop(\ctable_{\bot}[\ccsite \mapsto \pair{\cmap(\cnode_x)}{\cmap(\cn{\cenv_1}{\elabel_1})}], \ctable) \\[0.5ex]
\sind[3]	\;\pair{\wtable_x}{\wtable_0} = \wprop([\wpath \mapsto \pair{\wmap(\cnode_x)}{\wmap(\cn{\cenv_1}{\elabel_1})}], T_w) \\[0.5ex]
%\ind[3]	\;\pair{\ctable''}{\ctable'_f} = \cprop(\ctable, \cmap(\cnode_f)) \\[0.5ex]
%\ind[3]	\;\pair{\cval'_x}{\cval'_1} = \ctable'_x(\ccsite) \\[0.5ex]
\sind[3]	\;\pair{\wtable_2}{\wtable_f} = \wprop(T_w, \wmap(\cnode_f)) \Mend \pair{\wval'_x}{\wval'_1} = \wtable_x(\wpath) \\[0.5ex]
\sind[3] \;\wmap_1 = \wmap[\cn{\cenv}{\elabel} {\mapsto}
\wtable_1 \wvjoin \wtable_2, \cnode_f {\mapsto} \ext(\wtable_f, \cnode_f), \cnode_x {\mapsto} \ext(\wval'_x, \cnode_x) ,\cn{\cenv_1}{\elabel_1} {\mapsto} \wval'_1] \\[0.5ex]
    \sind[2] \Min \wtrans[k]{e_1}(\cenv_1)(\wmap_1)\\[0.5ex]
%\sind    \Min \cmjoinb_{\ccsite \in \ccallsites} \;\overline{\cmap}(\ccsite)\\[2ex]
\sind    \Min \wmap[\cn{\cenv}{\ell} \mapsto \wtable] \;\wmjoin\; \wmjoinb_{\wpath \in \wtable} \;\overline{\cmap}(\wpath)

\more{\\[1.5ex]
\wtrans{(\ifte{e_0^{\elabel_0}}{e_1^{\elabel_1}}{e_2^{\elabel_2}})^{\elabel}}(\cenv)(\wmap) \Def= \\[0.5ex]
\sind	\Mlet \wmap_0 = \wtrans[k]{e_0}(\cenv)(\wmap) \Mend \wval_0 =_{\wmap_0} \wmap_0(\cn{\cenv}{\elabel_0}) \;\Min \\[0.5ex]
%\ind	\Mif \cval_0 = \bot \;\Mthen \cmap_0 \;\Melif \cval_0 \not \in \bools \;\Mthen \cmap_{\cerr} \;\Melse \\[0.5ex]
\sind	\Mif \wval_0 \not \in \wbools \;\Mthen \wmap_{\cerr} \;\Melse \\[0.5ex]
\sind[2]	\Mlet b =  \Mif \wval_0 = \cw{\btrue}{\_}\;\Mthen 1 \;\Melse 2 \;\Min  \\[0.5ex]
\sind[2]	\Mlet \wmap_b = \wtrans[k]{e_b}(\cenv)(\wmap_0) \Mend \wval_b =_{\wmap_b} \wmap_b(\cn{\cenv}{\elabel_b})  \;\Min\\[0.5ex]
%    \ind[2] \Min \\[0.75ex]
%    \ind[2] \Mif \cval_b = \bot \; \Mthen \cmap_b \;\Melif \cval_b = \cerr \;\Mthen \cmap_{\cerr} \;\Melse \\[0.5ex]
\sind[2]	\Mlet \pair{\wval'_b}{\wval'} = \wprop(\wval_b, \wmap_b(\cn{\cenv}{\elabel}))\\[0.5ex]
\sind[2]	\Min \wmap_b[\cn{\cenv}{\elabel} \mapsto \ext(\wval', \cn{\cenv}{\ell}), \cn{\cenv}{\elabel_b} \mapsto \wval'_b] 
}
\end{array}\]
\end{figure}
%
Note that path semantics models call sites as paths rather than nodes, but the variable nodes are created only using the top
of the call site path. As we shall see later, the actual paths observed during the computation that have unique top nodes.
%
\begin{lemma}~\label{thm:w-step-increasing-monotone}
$\wtransname$ is increasing and monotone.
\end{lemma}
\begin{proof}
The increasing property follows from the increasing property of $\wprop$ (Lemma~\ref{thm:w-prop-increasing-monotone}).
The proof of monotonicity closely follows that of Lemma~\ref{thm:c-prop-monotone}.
\end{proof}

\paragraph{Additional Properties}

We next introduce several useful properties related to the path semantics.

\paragraph{Computation Range}

The results regarding the computation range are the same as for the ordinary 
data flow semantics.
%
\begin{lemma}~\label{thm:w-framer}
Let $\wmap$ and $\wmap_0$ be path maps, $\cenv$ an environment, $e^\ell$ an expression of a program $e'$ 
where $(e, \cenv)$ is well-formed. 
If $\domvalid(\ell, e', \cenv)$ and $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$ then 
$\forall \cnode. \wmap(\cnode) \not = \wmap_0(\cnode) \implies \cnode \in \cranger_{e'}(\cn{\cenv}{\ell})$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-framer}.
\end{proof}
%
\begin{lemma}~\label{thm:w-disjointr-1}
Let $\cenv$ be an environment, $e'$ be a program, $\ell_1$ and $\ell_2$ two locations such that $\locs(e'(\ell_1)) \cap \locs(e'(\ell_2)) = \emptyset$.
Then, $\crange_{e'}(\cn{\cenv}{\ell_1}) \cap \crange_{e'}(\cn{\cenv}{\ell_2}) = \rng(\cenv)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-disjointr-1}.
\end{proof}
%
\begin{lemma}~\label{thm:w-disjointr-2}
Let $\cenv_1$ and $\cenv_2$ be two environments and $\ell$ a location of a program $e'$.
If $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$ and $\cenv_1 \not= \cenv_2$, then 
$\crange_{e'}(\cn{\cenv}{\ell_1}) \cap \crange_{e'}(\cn{\cenv}{\ell_2}) = \rng(\cenv_1) \cap \rng(\cenv_2)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-disjointr-2}.
\end{proof}


\paragraph{Finiteness}

We say a value $\wval$ is finite $\cfin(\wval)$ if it is either a ground value or a table
that has seen only a finite number of inputs, just as in the case of regular data flow semantics.
%
\begin{align*}
\cfin(\wval) \Def= & (\wval \in \{\wbot, \werr\} \cup \wconsts) \vee (\exists \wtable.\, \wval = \cw{\wtable}{_} \in \wtables \wedge |\setc{\wpath}{\wpath \in \wtable}| \in \mathbb{N} \;\wedge\\
&\ind[11] \forall \wpath \in \wtable.\, \cfin(\pi_1(\wtable(\wpath))) \wedge \cfin(\pi_2(\wtable(\wpath))))
\end{align*}
%
As expected, $\wprop$ does not affect the finiteness of values. The same clearly holds for joins $\cvjoin$.
%
\begin{lemma}~\label{thm:w-val-finite-prop}
Let $\wval_1$, $\wval_2$, $\wval_3$, and $\wval_4$ be path values. If $\cfin(\wval_1)$, $\cfin(\wval_2)$,
and $\pair{\wval_3}{\wval_4} = \wprop(\wval_1, \wval_2)$, then $\cfin(\wval_3)$ and $\cfin(\wval_4)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-val-finite-prop}.
\end{proof}
%
We say a path map $\wmap$ is finite $\cfin(\wmap)$ if all of its values are finite and the set of reachable nodes is finite as well
$|\setc{\cnode}{\wmap(\cnode) \not= \wbot}| \in \mathbb{N}$. It can be shown that $\wtransname$ preserves
the finiteness of maps.
%
\begin{lemma}~\label{thm:w-step-finite}
Let $\wmap$ and $\wmap_0$ be maps, $\cenv$ an environment, and $e^\ell$ an expression where $(e, \cenv)$ is well-formed. 
If $\cfin(\wmap)$ and $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\cfin(\wmap_0)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-step-finite}.
\end{proof}

\paragraph{Top of the Path Consistency}

We say a path map $\wmap$ is consistent subject to the top of the paths $\tpcons(\wmap)$ iff for every node
$\cnode$ it is the case that $\wmap(\cnode) \in \{\wbot, \werr\}$ or $\wmap(\cnode) = \cw{\_}{\wpath}$ for 
some path $\wpath$ where $\ppath(\wpath) = \cnode$.

The consistency of maps subject to the top of paths is an preserved by the path semantics transformer.
%
\begin{lemma}~\label{thm:w-step-tpcons}
Let $\wmap \in \wmaps$ where $\tpcons(\wmap)$, $\wmap_0 \in \wmaps$, $e^\ell$ an expression, 
and $\cenv$ an environment where $(e, \cenv)$
is well-formed. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\tpcons(\wmap_0)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. The argument follows from the basic properties
of the join on path values, Lemma~\ref{thm:w-prop-paths}, and the idempotency of $\ext$ operation.
\end{proof}

Top of the path consistency can be used to establish an interesting
and useful property of the concrete transformer $\wtransname$. Once
path has been inferred for some value in the map, then after
applying the transformer, the updated value is either top $\werr$
or a new path value but with the same associated path.
%
\begin{lemma}~\label{thm:w-step-path-stable}
Let $\cnode \in \cnodes$, $\wmap \in \wmaps$ where $\tpcons(\wmap)$, 
$\wmap_0 \in \wmaps$, $e^\ell$ an expression,
and $\cenv$ an environment where $(e, \cenv)$ is well-formed. 
Suppose $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$.
If $\wmap(\cnode) = \cw{\_}{\wpath}$ for some path $\wpath$,
then $\wmap(\cnode_0) = \cw{\_}{\wpath}$ or $\wmap_0(\cnode) = \werr$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. 
The argument follows from the basic properties
of the join on path values and Lemma~\ref{thm:w-prop-paths}.
The top of the path consistency property together with 
Lemma~\ref{thm:w-step-tpcons} is needed to prove
that the calls to $\ext$ on existing paths do not create new paths.
\end{proof}


\paragraph{Call Site Path Consistency}

We next define the notion of call site path consistency intuitively capturing
the idea that a table can be called at call site path that refers to the future points reached by the table,
i.e., call site paths must be an extension of the path associated with the
table. A path value $\wval$ is call site path consistent $\pcscons(\wval)$ iff
%
\begin{align*}
(\wval \in \{\wbot, \werr\} \cup \wconsts) \;\vee \ind[11] \\
\exists \wtable, \wpath.
\wval = \cw{\wtable}{\wpath} \wedge \forall \wpath' \in \wtable.\,\wpath \wpord \wpath' \wedge
\pcscons(\pi_1(\wtable(\wpath'))) \wedge \pcscons(\pi_2(\wtable(\wpath')))
\end{align*}
%
We raise the definition of call site path consistency to the maps.
That is, a path map $\wmap$ is said to be call site path consistent 
$\pcscons(\wmap)$ iff for every node $\cnode$ we have $\pcscons(\wmap(\cnode))$.

It can be shown that the data propagation does not invalidate the
call site path consistency.
%
\begin{lemma}~\label{thm:w-prop-pcscons}
Let $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ for path values $\wval_1, \wval'_1, \wval_2$, and $\wval'_2$. 
If $\pcscons(\wval_1)$ and $\pcscons(\wval_2)$, then
$\pcscons(\wval'_1)$ and $\pcscons(\wval'_2)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\wval_1$ and $\wval_2$.
The base cases are trivial and so is the the induction case when both 
$\wval_1$ and $\wval_2$ are path tables but the path associated with 
$\wval_1$ is not a prefix of the one associated with $\wval_2$.
Otherwise, the argument follows from the i.h.\ and
the fact that any call site path seen in $\wval_2$ has to also be an extension
of the path associated with $\wval_1$.
\end{proof}

The call site path consistency is preserved by the
transformer of the path semantics.
%
\begin{lemma}~\label{thm:w-step-pcscons}
Let $\wmap \in \wmaps$ where $\pcscons(\wmap)$, $\wmap_0 \in \wmaps$, $e^\ell$ an expression, 
 and $\cenv$ an environment where $(e, \cenv)$
is well-formed. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\pcscons(\wmap_0)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. The argument follows from the basic properties
of the join on path values, Lemma~\ref{thm:w-prop-paths}, 
Lemma~\ref{thm:w-prop-pcscons}, and Lemma~\ref{thm:w-step-path-stable}.
\end{proof}



\paragraph{Root Path Consistency}

A path $\wpath$ is called to be root consistent $\rootcons_e(\wpath)$, 
subject to some program $e$, iff its root node corresponds to a constant 
or lambda expression of the program.
%
\[\rootcons_e(\wpath) \Def\iff \exists \const. e(\nloc(\proot(\wpath))) = \const \vee \exists f,x,e'.\, e(\nloc(\proot(\wpath))) = \mu f.\lambda x.e'\]
%
Note that we use $\proot(\wpath)$ to denote the starting/root node of a path $\wpath$.
A map $\wmap$ is root consistent if all of its paths in $\allpaths(\wmap)$
are root consistent.
%
\begin{lemma}~\label{thm:w-prop-rootcons}
Let $e$ be a program, $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ for path values $\wval_1, \wval'_1, \wval_2$, and $\wval'_2$. 
If $\rootcons_e(\wval_1)$ and $\rootcons_e(\wval_2)$, then
$\rootcons(\wval'_1)$ and $\rootcons(\wval'_2)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\wval_1$ and $\wval_2$.
\end{proof}

The root path consistency is preserved by the transformer of the path semantics.
%
\begin{lemma}~\label{thm:w-step-pcscons}
Let $\wmap \in \wmaps$ where $\pcscons(\wmap)$, $\wmap_0 \in \wmaps$, $e^\ell$ an expression, 
and $\cenv$ an environment where $(e, \cenv)$
is well-formed. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\pcscons(\wmap_0)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. 
The argument follows from the basic properties
of the join on path values, Lemma~\ref{thm:w-prop-paths}, 
and Lemma~\ref{thm:w-prop-rootcons}.
\end{proof}



\paragraph{Table IO Consistency}

We next formalize the notion of input-output consistency for tables
that is the same as for the standard data flow semantics.
%
\begin{align*}
\tiocons(\wval) {\Def\iff} & (\wval \in \{\wbot, \werr\} \cup \wconsts) \vee (\exists \wtable.\,\wval=\cw{\wtable}{\_} \wedge \forall \wpath \in \wtable.\\
& \pi_1(\wtable(\wpath)) = \wbot \implies \pi_2(\wtable(\wpath)) = \wbot \;\wedge \\
& \tiocons(\pi_1(\wtable(\wpath))) \wedge \tiocons(\pi_2(\wtable(\wpath))))
\end{align*}
%
As expected, a map is input-output consistent $\tiocons_e(\cmap)$, subject
to a program $e$, iff all of its values are IO consistent and for every node
$\cnode$
%
\begin{align*}
\wmap(\cn{\nenv(\cnode)}{\ell_1}) {=} \wbot {\implies} \wmap(\cn{\nenv(\cnode)}{\ell_2}) {=} \bot \;\wedge && \\
\wmap(\cn{\nenv(\cnode)}{\ell_2}) {=} \wbot {\implies} \wmap(\cn{\nenv(\cnode)}{\ell}) {=} \bot && \\
&&\textbf{if } \exists e_1, e_2, \ell_1, \ell_2.\, e(\nloc(\cnode)) = e_1^{\ell_1} e_2^{\ell_2} \\[1ex]
%
\pi_1(\wmap(\cnode)(\wpath)) {=} \wbot {\implies} \wmap(\cnode_f) {=} \wbot \;\wedge &&\\
\pi_1(\wmap(\cnode)(\wpath)) {=} \wbot {\implies} \wmap(\cnode_x) {=} \wbot \;\wedge &&\\
\pi_1(\wmap(\cnode_x)) {=} \wbot {\implies} \wmap(\cn{\cenv_1}{\ell_1}) {=} \wbot  &&\\
\textbf{if } \cmap(\cnode) \in \wtables \textbf{ and } \exists x, f, e_1, \ell_1, \cnode_x, \cnode_f, \wpath. && \wpath \in \wmap(\cnode) \wedge 
\cnode_x {=} \cvn{\nenv(\cnode)}{\ptop(\wpath)}{x} \\
\wedge\; \cnode_f {=} \cvn{\nenv(\cnode)}{\ptop(\wpath)}{f} \wedge
\cenv_1 = \cenv.x\!{:}\cnode_x.f\!{:}\cnode_f
\end{align*}
%
The input-output consistency of values is not violated by data propagation.
\begin{lemma}~\label{thm:w-prop-tiocons}
Let $e$ be a program, $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ for path values $\wval_1, \wval'_1, \wval_2$, and $\wval'_2$. 
If $\tiocons_e(\wval_1)$ and $\tiocons_e(\wval_2)$, then
$\tiocons(\wval'_1)$ and $\tiocons(\wval'_2)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\wval_1$ and $\wval_2$.
\end{proof}
%
The input-output consistency is preserved by $\wtransname$.
%
\begin{lemma}~\label{thm:w-step-tiocons}
Let $\wmap \in \wmaps$ where $\tiocons(\wmap)$, $\wmap_0 \in \wmaps$, $e^\ell$ an expression, 
and $\cenv$ an environment where $(e, \cenv)$
is well-formed. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\tiocons(\wmap_0)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. 
The argument follows from the fact that the join on 
path values does not invalidate input output consistency
and Lemma~\ref{thm:w-prop-tiocons}.
\end{proof}


\paragraph{Table Input Consistency}

A path value $\wval$ is input consistent $\inpcons_e(\wval)$, 
subject to some program $e$, iff the path associated with every input of 
a table has to come from a function application expression in $e$.
%
\begin{align*}
\inpcons_e(\wval) \Def\iff & (\wval \in \{\wbot, \werr\} \cup \wconsts) \vee
\exists \wtable.\,\wval = \cw{\wtable}{\_} \wedge \forall \wpath \in \wtable.\\
& \inpcons_e(\pi_1(\wtable(\wpath))) \wedge \inpcons_e(\pi_2(\wtable(\wpath)))  \wedge \exists e_1, e_2, \ell_2, \wpath'.\\
& e_1^{\nloc(\ptop(\wpath))} e_2^{\ell_2} \in e
\wedge (\pi_1(\wtable(\wpath)) \in \{\wbot, \werr\} \vee
\pi_1(\wtable(\wpath)) = \cw{\_}{\wpath'} \\
&\wedge \ptop(\wpath') = \cn{\nenv(\ptop(\wpath))}{\ell_2})
\end{align*}
%
A map $\wmap$ is input consistent $\inpcons_e(\wmap)$ iff all of its 
values are input consistent.

%
\begin{lemma}~\label{thm:w-prop-inpcons}
Let $e$ be a program, $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ for path values $\wval_1, \wval'_1, \wval_2$, and $\wval'_2$. 
If $\inpcons_e(\wval_1)$ and $\inpcons_e(\wval_2)$, then
$\inpcons(\wval'_1)$ and $\inpcons(\wval'_2)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\wval_1$ and $\wval_2$
and it relies on Lemma~\ref{thm:w-prop-paths}.
\end{proof}

The input consistency of path maps is preserved by $\wtransname$.
%
\begin{lemma}~\label{thm:w-step-inpcons}
Let $\wmap \in \wmaps$ where $\inpcons(\wmap)$, $\wmap_0 \in \wmaps$, $e^\ell$ an expression, 
and $\cenv$ an environment where $(e, \cenv)$
is well-formed. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\inpcons(\wmap_0)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $e$. 
The argument follows from the fact that join on paths values
does not invalidate input consistency and Lemma~\ref{thm:w-prop-inpcons}.
\end{proof}



\paragraph{Table Output Consistency}

A path value $\wval$ is output consistent $\outcons_e(\wval)$, 
subject to some program $e$, iff the path associated with every input of 
a table has to come from a function application expression in $e$.
%
\begin{align*}
\outcons_e(\wval) {\Def\iff} & (\wval \in \{\wbot, \werr\} \cup \wconsts) \vee
\exists \wtable, \wpath, f, x, e_1, \ell_1.\,\wval = \cw{\wtable}{\wpath} \;\wedge\\
& e(\nloc(\proot(\wpath))) = \mu f. \lambda x.\,e_1^{\ell_1} \wedge 
\forall \wpath' \in \wtable.\, \outcons_e(\pi_1(\wtable(\wpath'))) \;\wedge \\
& \outcons_e(\pi_2(\wtable(\wpath'))) \wedge 
(\exists \cenv, \wpath''.\,\pi_2(\wtable(\wpath')) \in \{\wbot, \werr\} \;\vee\\
& \pi_2(\wtable(\wpath')) = \cw{\_}{\wpath''} \wedge \ptop(\wpath'') = 
\cn{\cenv}{\ell_1} \wedge \cenv=\\
&\nenv(\proot(\wpath)).x\!:\cvn{\nenv(\proot(\wpath))}{\ptop(\wpath')}{x}.f\!:\cvn{\nenv(\proot(\wpath))}{\ptop(\wpath')}{f})
\end{align*}
%
A map $\wmap$ is output consistent $\outcons_e(\wmap)$ iff all of its 
values are output consistent.


\begin{lemma}~\label{thm:w-prop-outcons}
Let $e$ be a program, $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ for path values $\wval_1, \wval'_1, \wval_2$, and $\wval'_2$. 
If $\outcons_e(\wval_1)$ and $\outcons_e(\wval_2)$, then
$\outcons(\wval'_1)$ and $\outcons(\wval'_2)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\wval_1$ and $\wval_2$.
\end{proof}

The output consistency of path maps is preserved by $\wtransname$.
%
\begin{lemma}~\label{thm:w-step-outcons}
Let $\wmap \in \wmaps$ where $\outcons(\wmap)$, $\wmap_0 \in \wmaps$, $e^\ell$ an expression, 
and $\cenv$ an environment where $(e, \cenv)$
is well-formed. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_0$, then $\outcons(\wmap_0)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction $e$. 
The argument follows from the fact that join on paths values
does not invalidate input consistency and Lemma~\ref{thm:w-prop-inpcons}.
\end{proof}


\paragraph{Constant Consistency}

We next formalize the notion of constant consistency for path maps
that is identical to the notion of constant consistency for regular maps.
A path map $\wmap$ is constant consistent $\constcons_e(\wmap)$, subject
to a program $e$, iff for every node $\cnode$, where $\wmap(\cnode) = \wval$ for
some path value $\wval$ and $\nloc(\cnode) = \ell$ for some location $\ell$, it must be
%
\begin{align*}
\wval \in \{\werr, \wbot, \cw{\const}{\cnode}\} && \text{if } e(\ell) = c \\
\wval \in \{\werr,\wbot\} \cup \setc{\cw{\wtable}{\cn{\cenv}{\ell}}}{\wtable \in \wtables} && \text{if } e(\ell) = \mu f. \lambda x.e_1 \text{ for some $x$, $f$, and $e_1$} 
\end{align*}



\paragraph{Concrete Path Subtyping}

The notion of subtyping for path values resembles the one on the regular data flow values.
Additionally, we also require that a table cannot see a call site path (coming from the future) 
unless the future table has seen it as well.
%
\begin{align*}
\wval_1 \wsub \wval_2 \Def\iff & (\wval_2 = \wbot) \vee 
(\wval_1 = \cw{\const}{\wpath_1} \wedge \wval_2=\cw{\const}{\wpath_2} \wedge \const \in \consts 
\wedge \wpath_1, \wpath_2 \in \wpaths ) \\
& \vee (\wval_1 = \wval_2 = \werr) \vee (\wval_1=\cw{\wtable_1}{\wpath_1} \wedge 
\wval_2=\cw{\wtable_2}{\wpath_2} \wedge \wtable_1, \wtable_2 \in \wtables \\
& \wedge\; \wpath_1, \wpath_2 \in \wpaths \wedge \wpath_1 \wpord \wpath_2 \wedge 
(\forall \wpath \in \wtable_1.\, \wpath_2 \wpord \wpath {\implies} \wpath \in \wtable_2) \;\wedge\\
& \forall \wpath \in \wtable_2. \pi_1(\wtable_2(\wpath)) \;\wsub\; \pi_1(\wtable_1(\wpath)) 
\wedge \pi_2(\wtable_1(\wpath)) \;\wsub\; \pi_2(\wtable_2(\wpath)))
\end{align*}
%
Unlike the subtyping relation on the ordinary data flow values, the above subtyping relation
for path values is transitive, given certain simple assumptions on the values.
\begin{lemma}~\label{thm:w-sub-transitive}
Let $\wval_1 \in \wvalues$, $\wval_2 \in \wvalues$, and $\wval_3 \in \wvalues$
such that $\tiocons(\wval_1)$, $\tiocons(\wval_2)$, $\tiocons(\wval_3)$,
$\pcscons(\wval_1)$, $\pcscons(\wval_2)$, and $\pcscons(\wval_3)$.
If $\wval_1 \;\wsub\; \wval_2$ and $\wval_2 \;\wsub\; \wval_3$, then $\wval_1 \;\wsub\; \wval_3$.
\end{lemma}
\begin{proof}
By structural induction on $\wval_2$. We first cover the base cases.
%
\begin{itemize}
\item $\wval_2=\wbot$
\begin{align*}
\wval_3 = \wbot && \text{by def.\ of }\wsub\\
\wval_1 \wsub \wbot &&
\end{align*}


\item $\wval_2=\werr$
\begin{align*}
\wval_3 = \wbot \vee \wval_3 = \wbot && \text{by def.\ of }\wsub\\
\wval_1 = \werr && \text{by def.\ of }\wsub\\
\werr \wsub \werr \wedge \werr \wsub \wbot &&
\end{align*}

\item $\wval_2=\cw{\const}{\wpath_2}$
\begin{align*}
\wval_1 = \cw{\const}{\wpath_1}, \wpath_1 \wpord \wpath_2 && \text{by def.\ of }\wsub\\
\wval_3 = \wbot \vee \wval_3 = \cw{\const}{\wpath_3} \wedge \wpath_2 \wpord \wpath_3 && \text{by def.\ of }\wsub\\
\cw{\const}{\wpath_1} \wsub \wbot \wedge \cw{\const}{\wpath_1} \wsub \cw{\const}{\wpath_3} &&
\text{by trans.\ of }\wpord 
\end{align*}
\end{itemize}

For the induction case, suppose $\wval_2 = \cw{\wtable_2}{\wpath_2}$ for some $\wtable_2$
and $\wpath_2$. If $\wval_3 = \wbot$, the argument is trivial. We are thus left with the case
where $\wval_1 = \cw{\wtable_1}{\wpath_1}$ and $\wval_3 = \cw{\wtable_3}{\wpath_3}$ for some
$\wtable_1$, $\wtable_3$, $\wpath_1$, and $\wpath_3$ where $\wpath_1 \wpord \wpath_2$ and
$\wpath_2 \wpord \wpath_3$. Hence, $\wpath_1 \wpord \wpath_3$. Let us first argue
that $\forall \wpath \in \wtable_1.\,\wpath_3 \wpord \wpath {\implies} \wpath \in \wtable_3$.
Suppose not, i.e., there exists a path $\wpath \in \wtable_1$ such that $\wpath_3 \wpord \wpath$
and $\wpath \not \in \wtable_3$. By $\wpath_2 \wpord \wpath_3$, we have that 
$\wpath_2 \wpord \wpath$ and hence $\wpath \in \wtable_2$ by $\wval_1 \wsub \wval_2$. 
Therefore, it also must be that $\wpath \in \wtable_3$ by $\wval_2 \wsub \wval_3$.

Consider next any call site path 
$\wpath$. Let $\wtable_1(\wpath) = \pair{\wval_{1i}}{\wval_{1o}}$, 
$\wtable_2(\wpath) = \pair{\wval_{2i}}{\wval_{2o}}$, and 
$\wtable_3(\wpath) = \pair{\wval_{3i}}{\wval_{3o}}$.
If $\wpath \not \in \wtable_3$, the argument is trivial. Hence, we can only focus on 
the case where $\wpath \in \wtable_3$. We branch on the occurrence of $\wpath$ in $\wtable_2$. 

Suppose $\wpath \not \in \wtable_2$. 
Hence, $\wval_{2i}=\wbot$ and by $\tiocons(\wval_2)$ it must be that $\wval_{2o}=\wbot$.
Next, it cannot be the case where both $\wpath \in \wtable_1$ and 
$\wpath \in \wtable_3$ when $\wpath \not\in \wtable_2$. To see this, suppose
this is not the case, i.e., $\wpath \in \wtable_1$. By $\pcscons(\wval_3)$, we 
have that $\wpath_3 \wpord \wpath$.
Since $\wpath_2 \wpord \wpath_3$, then also $\wpath_2 \wpord \wpath$. Then,
$\wpath_2 \in \wtable_2$ by $\wval_1 \wsub \wval_2$, a contradiction.
Hence, $\wpath \not \in \wtable_1$. By $\tiocons(\wval_1)$ we have 
$\wval_{1i} = \wval_{1o} = \wbot$ . The result
then follows by $\wtable_1(\wpath) = \wtable_2(\wpath)$.

Suppose now $\wpath \in \wtable_2$. Then, we have 
$\wval_{3i} \wsub \wval_{2i}$ and $\wval_{2i} \wsub \wval_{1i}$ as well as
$\wval_{1o} \wsub \wval_{2o}$ and $\wval_{2o} \wsub \wval_{3o}$ and the result follows
by i.h.
\end{proof}

We next prove several results stating how the propagation between values affect the
subtyping relation between the values. We start with the expected result that the 
propagation preserves subtyping between path values.
\begin{lemma}~\label{thm:w-prop-sub}
Let $\wval_1 \in \wvalues$, $\wval_2 \in \wvalues$, $\wval_3 \in \wvalues$, and 
$\wval_4 \in \wvalues$. If $\wval_1 \wsub \wval_2$ and 
$\pair{\wval_3}{\wval_4} = \wprop(\wval_1, \wval_2)$, then $\wval_3 \wsub \wval_4$.
\end{lemma}
\begin{proof}
By structural induction on $\wval_1$ and $\wval_2$. The proof argument is similar
to the one of Lemma~\ref{thm:c-prop-sub}.
\end{proof}
%
The propagation between two values reserves the subtyping relation
not only between the two values, but also on the whole subtyping chain containing these 
two values. 
\begin{lemma}~\label{thm:w-sub-prop-chain}
Let $\wval_1 \in \wvalues$, $\wval_2 \in \wvalues$, $\wval_3 \in \wvalues$,
$\wval'_1 \in \wvalues$, $\wval'_2 \in \wvalues$, and $\wval'_3 \in \wvalues$.
Suppose $\wval_1 \wsub \wval_2$, $\wval_2 \wsub \wval_3$, $\tiocons(\wval_1)$, 
$\tiocons(\wval_2)$, $\tiocons(\wval_3)$, $\pcscons(\wval_1)$, $\pcscons(\wval_2)$, 
and $\pcscons(\wval_3)$. If $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ 
then $\wval'_2 \wsub \wval_3$. Similarly, if $\pair{\wval'_2}{\wval'_3} = 
\wprop(\wval_2, \wval_3)$ then $\wval_1 \wsub \wval'_2$. 
\end{lemma}
\begin{proof}
The proof goes by structural induction on $\wval_2$ and follows the structure
of the proof of Lemma~\ref{thm:w-sub-transitive}. Also, the proof relies on
Lemma~\ref{thm:w-prop-tiocons} and Lemma~\ref{thm:w-prop-pcscons} to trigger
the induction hypothesis.
\end{proof}
%
It can also be shown that updated versions, by means of propagation, of value 
lying on the subtyping chain can be joined while retaining the subtyping property of the chain. 
\begin{lemma}~\label{thm:w-sub-prop-join-chain}
Let $\wval_1 \in \wvalues$, $\wval_2 \in \wvalues$, $\wval_3 \in \wvalues$,
$\wval'_1 \in \wvalues$, $\wval'_2 \in \wvalues$, $\wval''_2 \in \wvalues$,
 and $\wval''_3 \in \wvalues$.
Suppose $\wval_1 \wsub \wval_2$, $\wval_2 \wsub \wval_3$, $\tiocons(\wval_1)$, 
$\tiocons(\wval_2)$, $\tiocons(\wval_3)$, $\pcscons(\wval_1)$, $\pcscons(\wval_2)$, 
and $\pcscons(\wval_3)$. Next, suppose 
$\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$ and
$\pair{\wval''_2}{\wval''_3} = \wprop(\wval_2, \wval_3)$ such that
$\wval'_1 \wsub \wval'_2 \wsub \wval_3$ and $\wval_1 \wsub \wval''_2 \wsub \wval''_3$.  
Then, $\wval'_1 \;\wsub\; \wval_2 \wvjoin \wval''_2 \;\wsub\; \wval'_3$.
\end{lemma}
\begin{proof}
By structural induction on $\wval_1$, $\wval_2$, and $\wval_3$.
\end{proof}

We now finally define the subtyping consistency of path maps.
A map $\wmap$ is subtyping consistent $\cmsub_e(\wmap)$, subject to a program $e$, 
iff for every node $\cnode$, where $\nloc(\cnode) = \ell$, it must be that
%
\begin{align*}
%
\wmap(\cn{\nenv(\cnode)}{\ell_2}) \;\wsub\; \pi_1(\wmap(\cn{\nenv(\cnode)}{\ell_1})(\wpath)) \wedge \pi_2(\wmap(\cn{\nenv(\cnode)}{\ell_1})(\wpath)) \;\wsub\; \wmap(\cnode) \\
\ind[3] \textbf{if }\exists e_1, e_2, \ell_1, \ell_2, \wtable, \wpath.\, e(\ell) = (e_1^{\ell_1} e_2^{\ell_2}) \textbf{ and } \wmap(\cn{\nenv(\cnode)}{\ell_1}) = \cw{\wtable}{\wpath} \\[1ex]
%
\pi_1(\wmap(\cnode)(\wpath)) \;\wsub\; \wmap(\cnode_x) \wedge \wmap(\cn{\cenv_1}{\ell_1}) \;\wsub\; \pi_2(\wmap(\cnode)(\wpath)) \\
\textbf{if }\exists x, f, e_1, \ell_1, \wtable, \wpath, \cvnode_x, \cvnode_f.\, e(\ell) = (\mu f.\lambda x. e_1^{\ell_1}),\,\wmap(\cnode) =\cw{\wtable}{\_}\,,\wpath \in \wmap(\cnode),\,\\
\cvnode_x = \cvn{\nenv(\cnode)}{\ptop(\wpath)}{x},\,\cvnode_f = \cvn{\nenv(\cnode)}{\ptop(\wpath)}{f}, \textbf{ and } \cenv_1 = \nenv(\cnode).x\!:\cvnode_x.f\!:\cvnode_f
\end{align*}
%
and $\forall \wpath \in \allpaths(\wmap), \pair{\cnode_1}{\cnode_2} \in \wpath.\, \wmap(\cnode_1) \;\wsub\; \wmap(\cnode_2)$.


\paragraph{Path Consistency}

We next introduce a path consistency, a property of maps similar to subtyping but providing
more information about paths of values related to subtyping. A path map $\wmap$ is called
path consistent $\pvcons(\wmap)$, subject to a program $e$, iff 
$\forall \wpath \in \allpaths(\wmap).\,\wmap(\ptop(\wpath)) = \wpath \wedge 
\forall \pair{\cnode_1}{\cnode_2} \in \wpath.\, \wagree_{\cnode_2}(\wmap(\cnode_1),\wmap(\cnode_2))$
where 
\[\wagree_\cnode(\wval_1, \wval_2) {\Def\iff} \exists \wpath_1, \wpath_2.\, \wpath_2 = \wpath_1 \cdot \cnode \wedge \wval_1=\cw{\_}{\wpath_1} \wedge \wval_2=\cw{\_}{\wpath_2}. \]
%
That is, the values associated with neighbouring nodes cannot be bottom $\wbot$ or top $\werr$ and
associated paths have to be an extension of each other.

We next prove several interesting properties of path consistent maps. We use
$\wprefix(\wpath, i)$ to denote a prefix of $\wpath$ up to and including the node at position $i$
in $\wpath$. We also use $\cnode \in^i \wpath$ to denote that $\cnode$ appears in $\wpath$ at 
the position $i$.
\begin{lemma}~\label{thm:w-pvcons-prefix}
Let $\wmap$ be a path map, $\wpath \in \allpaths(\wmap)$, and $\cnode \in^i \wpath$.
If $\pvcons(\wmap)$, then $\wmap(\cnode) = \pair{\_}{\wprefix(\wpath, i)}$. 
\end{lemma}
\begin{proof}
Follows from the definition of $\pvcons$ and $\wagree$.
\end{proof}
%
If two values agree, the data propagation between these two values is preserved.
\begin{lemma}~\label{thm:w-prop-pvcons}
Let $e$ be a program, $\cnode$ a node, and $\pair{\wval_3}{\wval_4} = \wprop(\wval_1, \wval_2)$ 
for path values $\wval_1, \wval_2, \wval_3$, and $\wval_4$. If $\wagree_\cnode(\wval_1, \wval_2)$, 
then $\wagree_\cnode(\wval_3, \wval_4)$.
\end{lemma}
\begin{proof}
The argument follows from Lemma~\ref{thm:w-prop-paths}.
\end{proof}


\paragraph{Path Determinism}

We next introduce another useful property of paths taken by data flow values in our semantics.
That is, every taken path is deterministic in the sense that for every node in a path there
is always a unique predecessor node. For this purpose, we define the predecessor relation
$\wpred^e_{\wmap}(\cnode_1, \cnode_2)$ to hold between nodes $\cnode_1$ and $\cnode_2$, subject
to a path map $\wmap$ and program $e$, iff one of the following six cases hold
\begin{enumerate}[leftmargin=1.5em]
\item 
\begin{align*}
\cnode_1 \in \cvnodes \wedge \cnode_2 \in \cenodes \wedge \exists x.\,e(\nloc(\cnode_1))=x 
\wedge x \in \m{dom}(\nenv(\cnode_1)) \wedge \cnode_2 = \nenv(\cnode_1)(x)
\end{align*}
%
\item
\begin{align*}
\cnode_1 \in \cenodes \wedge \cnode_2 \in \cvnodes \wedge \exists \cnode, \cenv_0, e_1, e_2,
\ell_1, \ell_2, x, \wtable, \wpath.\,\cnode_2 {=} \cvn{\cenv_0}{\cnode}{x} \wedge 
\cnode_1 {=} \cn{\nenv(\cnode)}{\ell_2} \\
\wedge\; e_1^{\nloc(\cnode)} e_2^{\ell_2} \in e 
\wedge \wmap(\cn{\nenv(\cnode)}{\ell_2}) \not\in \{\wbot, \werr\} \wedge 
\wmap(\cnode) = \cw{\wtable}{\wpath} \;\wedge \\
\nenv(\proot(\wpath)) = \cenv_0 \wedge e(\nloc(\proot(\wpath))) = \mu \_.\lambda x.\_
\end{align*}
%
\item
\begin{align*}
\cnode_1 \in \cenodes \wedge \cnode_2 \in \cvnodes \wedge \exists \cnode, \cenv_0, e_1, e_2,
\ell_1, \ell_2, f, \wtable, \wpath.\,\cnode_2 {=} \cvn{\cenv_0}{\cnode}{f} \wedge 
\cnode_1 {=} \proot(\wpath) \\
\wedge\; e_1^{\nloc(\cnode)} e_2^{\ell_2} \in e 
\wedge \wmap(\cn{\nenv(\cnode)}{\ell_2}) \not\in \{\wbot, \werr\} \wedge 
\wmap(\cnode) = \cw{\wtable}{\wpath} \;\wedge \\
\nenv(\proot(\wpath)) = \cenv_0 \wedge e(\nloc(\proot(\wpath))) = \mu f.\lambda \_.\_
\end{align*}
%
\item
\begin{align*}
\cnode_1 \in \cenodes \wedge \cnode_2 \in \cenodes \wedge \exists \cnode, \cenv_0, \cenv_b, 
e_1, e_2, e_b, \ell_1, \ell_2, \ell_b, f, x,\wtable, \wpath. \\
\nenv(\cnode_2) {=} \nenv(\cnode) \wedge
\cnode_1 {=} \cn{\cenv_b}{\ell_b} \wedge e(\nloc(\cnode_2)) = e_1^{\nloc(\cnode)} e_2^{\ell_2} 
\wedge \wmap(\cnode) = \cw{\wtable}{\wpath} \;\wedge \\
\wmap(\cn{\nenv(\cnode)}{\ell_2}) \not\in \{\wbot, \werr\} \wedge \nenv(\proot(\wpath)) = \cenv_0
\wedge e(\nloc(\proot(\wpath))) = \mu f.\lambda x.e_b^{\ell_b} \;\wedge\\ 
\cenv_b = \cenv_0.x\!:\cvn{\cenv_0}{\cnode}{x}.f\!:\cvn{\cenv_0}{\cnode}{f}
\end{align*}
%
%\item
%\begin{align*}
%\cnode_1 \in \cenodes \wedge \cnode_2 \in \cenodes \wedge \exists  
%e_0, e_1, e_2, \ell_0. \\
%e(\nloc(\cnode_2)) = \ifte{e_0^{\ell_0}}{e_1^{\nloc(\cnode_1)}}{e_2} \wedge
%\wmap(\cn{\nenv(\cnode_2)}{\ell_0}) = \cw{\btrue}{\_} \wedge \nenv(\cnode_1)=\nenv(\cnode_2)
%\end{align*}
%%
%\item
%\begin{align*}
%\cnode_1 \in \cenodes \wedge \cnode_2 \in \cenodes \wedge \exists  
%e_0, e_1, e_2, \ell_0. \\
%e(\nloc(\cnode_2)) = \ifte{e_0^{\ell_0}}{e_1}{e_2^{\nloc(\cnode_1)}} \wedge
%\wmap(\cn{\nenv(\cnode_2)}{\ell_0}) = \cw{\bfalse}{\_} \wedge \nenv(\cnode_1)=\nenv(\cnode_2)
%\end{align*}
\end{enumerate}
%
Note that we again use the $\_$ pattern to quantify out certain mathematical objects to avoid
clutter.


The first interesting property of the predecessor relation is that there is no predecessor
of a node that corresponds to the constant expression or lambda expression.
\begin{lemma}~\label{thm:w-pred-nopred}
Let $\cnode_2$ be a node, $\wmap$ a path map, and $e$ a program. If
$e(\nloc(\cnode_2))$ is a constant or a lambda expression, then there does not exist
a node $\cnode_1$ such that $\wpred^e_{\wmap}(\cnode_1, \cnode_2)$.
\end{lemma}
\begin{proof}
Follows from the definition of the $\wpred$ relation.
\end{proof}
%
A node cannot be its predecessor, i.e., the $\wpred$ relation is not reflexive.
\begin{lemma}~\label{thm:w-pred-not-reflexive}
Let $\cnode$ be a node, $\wmap$ a path map, and $e$ a program. Then, it cannot
be the case that $\wpred^e_{\wmap}(\cnode, \cnode)$.
\end{lemma}
\begin{proof}
Follows from the definition of the $\wpred$ relation.
\end{proof}
%
%
Next, the predecessor relation is deterministic.
\begin{lemma}~\label{thm:w-pred-det}
Let $\cnode$, $\cnode_1$, and $\cnode_2$ be nodes, $\wmap$ a path map, and $e$ a program. 
If $\wpred^e_{\wmap}(\cnode, \cnode_1)$ and  $\wpred^e_{\wmap}(\cnode, \cnode_2)$, then
$\cnode_1 = \cnode_2$.
\end{lemma}
\begin{proof}
Follows from the definition of the $\wpred$ relation, the fact that environments and path maps
are modeled as functions, and uniqueness of locations in $e$.
\end{proof}
%
Although the predecessor relation is deterministic, two different nodes can share their predecessor.
\begin{lemma}~\label{thm:w-pred-branch}
Let $\cnode$, $\cnode_1$, and $\cnode_2$ be nodes where $\cnode_1 \not= \cnode_2$, 
$\wmap$ a path map, and $e$ a program. 
If $\wpred^e_{\wmap}(\cnode, \cnode_1)$ and $\wpred^e_{\wmap}(\cnode, \cnode_2)$, then
$\cnode \in \cvnodes$ or $e(\nloc(\cnode))$ is a lambda expression.
\end{lemma}
\begin{proof}
Follows from the definition of the $\wpred$ relation.
\end{proof}
%

We say that path $\wpath$ is deterministic $\wdet^e_{\wmap}(\wpath)$, subject to a program
$e$ and path map $\wmap$, iff 
$\forall \pair{\cnode_1}{\cnode_2} \in \wpath.\,\wpred^e_{\wmap}(\cnode_1, \cnode_2)$.
A map $\wmap$ is deterministic $\wdet^e(\wmap)$ subject to a program $e$ iff
$\forall \wpath \in \allpaths(\wmap).\,\wdet^e_{\wmap}(\wpath)$.

\paragraph{Error Consistency}

Similar to data flow semantics, we introduce the notion of the error absence of values 
that intuitively states the a given value is not an error and, if it is a table, it does not recursively contain errors.
%
\begin{align*}
\noerr(\wval) \Def\iff & (\wval \in \{\wbot\} \cup \wconsts) \vee (\exists \wtable.\,\wval = \cw{\wtable}{\_} \wedge \forall \wpath \in \wtable.\\
& \ind[7] \noerr(\pi_1(\wtable(\wpath))) \wedge \noerr(\pi_2(\wtable(\wpath))))
\end{align*}
%
\noindent A path map $\wmap$ is error consistent $\errcons(\wmap)$ if either (1) $\wmap = \wmap_\werr$ or 
(2) for every node $\cnode$ it must be that $\noerr(\wmap(\cnode))$.

Data propagation does not invalidate the absence of error property of path values, given
that these values are related by the concrete subtyping relation on path values.
\begin{lemma}~\label{thm:w-prop-sub-noerr}
Let $\wval_1 \in \wvalues$, $\wval_2 \in \wvalues$, $\wval_3 \in \wvalues$, and 
$\wval_4 \in \wvalues$. If $\wval_1 \wsub \wval_2$ , $\noerr(\wval_1)$, $\noerr(\wval_2)$, 
and $\pair{\wval_3}{\wval_4} = \wprop(\wval_1, \wval_2)$, then $\noerr(\wval_3)$ and 
$\noerr(\wval_4)$.
\end{lemma}
\begin{proof}
By structural induction on $\wval_1$ and $\wval_2$. The proof argument is almost identical
to the one of Lemma~\ref{thm:c-prop-sub-noerr}.
\end{proof}


\paragraph{Environment Consistency}

The notion of environment consistency for a path map is identical to the one for regular data flow maps.
%
\[\envcons(\wmap) \Def\iff \forall \cnode, \cnode_x \in \rng(\nenv(\cnode)).\,\wmap(\cnode)\not=\wbot \implies \wmap(\cnode_x) \not \in \{\wbot, \werr\}.\]
%
Consistency of an environment $\cenv$ subject to a path map $\wmap$ is defined as follows
%
\[\envcons_\wmap(\cenv) \Def\iff \forall \cnode_x \in \rng(\cenv).\, \wmap(\cnode_x) \not \in \{\wbot, \werr\}\]


\paragraph{Consistency}

We can now define a general consistency $\wcons_e(\wmap)$ of a path map $\wmap$ subject 
to a program $e$ as follows
\begin{align*}
\wcons_e(\wmap) {\Def\iff} & \tpcons(\wmap) \wedge \pcscons(\wmap) \wedge \rootcons_e(\wmap) 
 \wedge \inpcons_e(\wmap) \;\wedge\\
& \outcons_e(\wmap) \wedge \wdet_e(\wmap) \wedge \cmsub_e(\wmap) \wedge \tiocons_e(\wmap) \wedge \cfin(\wmap)\\
& \wedge\; \constcons_e(\wmap) \wedge \errcons(\wmap) \wedge \envcons(\wmap) \wedge \pvcons(\wmap)
\end{align*}


We now prove several interesting properties of general consistency of maps.
\begin{lemma}~\label{thm:w-cons-bot-err}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$.
Then, $\forall \wpath \in \allpaths(\wmap), \cnode \in \wpath.\,\wmap(\cnode) \not \in \{\wbot, \werr\}$.
\end{lemma}
\begin{proof}
Follows from the definition of $\pvcons$.
\end{proof} 
%
The next result states that the observed paths in a consistent map can be
uniquely identified by their top nodes.
\begin{lemma}~\label{thm:w-cons-top-unique}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$.
Then, $\forall \wpath_1, \wpath_2 \in \allpaths(\wmap). \wpath_1 \not= \wpath_2{\implies}
\ptop(\wpath_1) \not= \ptop(\wpath_2)$.
\end{lemma}
\begin{proof}
By the induction on both $|\wpath_1|$ and $|\wpath_2|$. By $\pvcons(\wmap)$, prefixes of
both $\wpath_1$ and $\wpath_2$ are in $\allpaths(\wmap)$. The argument then follows from
$\wdet_e(\wmap)$, $\rootcons_e(\wmap)$, Lemma~\ref{thm:w-pred-det}, and Lemma~\ref{thm:w-pred-nopred}.
\end{proof} 
%
Further, a node cannot appear at two different location in any path of a consistent map.
That is, individual paths do not constitute cycles.
\begin{lemma}~\label{thm:w-cons-node-norepeat}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$ and
$\wpath \in \allpaths(\wmap)$. For any given node $\cnode$, suppose $\cnode \in^i \wpath$
and $\cnode \in^j \in \wpath$. Then, it must be that $i = j$.
\end{lemma}
\begin{proof}
Suppose not, $i \not= j$. Let $\wpath_i = \wprefix(\wpath, i)$ and $\wpath_j = \wprefix(\wpath, j)$.
Clearly, $\wpath_i \not= \wpath_j$. However, by Lemma~\ref{thm:w-pvcons-prefix} it must be that
$\wmap(\cnode) = \cw{\_}{\wpath_i} = \cw{\_}{\wpath_j}$. Hence, $\wpath_i = \wpath_j$. Contradiction.
\end{proof} 
%
Moreover, a node is always visited from the same predecessor node.
\begin{lemma}~\label{thm:w-cons-agree}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$.
Also, let $\cnode_1$ and $\cnode_2$ be nodes such that $\wpred^e_{\wmap}(\cnode_1, \cnode_2)$.
Then, $\wmap(\cnode_2) = \wbot \vee \wmap(\cnode_2) = \werr \vee 
\wagree_{\cnode_2}(\wmap(\cnode_1), \wmap(\cnode_2))$.
\end{lemma}
\begin{proof}
Let $\wmap(\cnode_2) = \cw{\_}{\wpath}$ for some $\wpath$. First, consider the
case $|\wpath|=1$.
\begin{align*}
\wpath \in \allpaths(\wmap) && \text{by def.\ of }\allpaths\\
e(\nloc(\cnode_2)) \text{ is a constant or lambda} && \text{by def.\ of }\rootcons\\
\neg \wpred^e_{\wmap}(\cnode_1, \cnode_2) && \text{by Lemma~\ref{thm:w-pred-nopred}}
\end{align*}
%
Next, consider the case $|\wpath| > 1$.
\begin{align*}
\wpath = \wpath' \cdot \cnode_2 && \text{by }\tpcons_e(\wmap) \text{ for some } \wpath'\\
\wmap(\cnode_1) = \cw{\_}{\wpath'} && \text{by Lemma~\ref{thm:w-pvcons-prefix} and Lemma~\ref{thm:w-cons-node-norepeat}} 
\end{align*}
\end{proof} 
%
We next show that propagation among values from a consistent map cannot invalidate
subtyping on branching points in the subtyping chains.
\begin{lemma}~\label{thm:w-cons-csub-branch}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$.
Also, let $\cnode$, $\cnode_1$, and $\cnode_2$ be nodes such that 
$\cnode_1 \not= \cnode_2$, $\wpred^e_{\wmap}(\cnode, \cnode_2)$, and $\wpred^e_{\wmap}(\cnode, \cnode_2)$.
Suppose $\wmap(\cnode) \;\wsub\; \wmap(\cnode_1)$, $\wmap(\cnode) \;\wsub\; \wmap(\cnode_2)$,
and $\pair{\wval'}{\wval'_1} = \wprop(\wmap(\cnode), \wmap(\cnode_1))$.
Then, $\wval' \;\wsub\; \wmap(\cnode_2)$.
\end{lemma}
\begin{proof}
Let $\wmap(\cnode)=\wval$, $\wmap(\cnode_1) = \wval_1$, and $\wmap(\cnode_2) = \wval_2$.
First, observe that if $\wval_1 = \wbot$ then $\wval' = \wval$ and the result follows
immediately. Otherwise, the proof goes by a case analysis on $\wmap(\cnode_2)$.
\begin{itemize}
\item $\wval_2 = \wbot$. Trivial, by the def.\ of $\wsub$.
\item $\wval_2 = \cw{\const}{\wpath_2}$. Then $\wval = \cw{\const}{\wpath}$ so that $\wpath \wpord \wpath_2$ 
and $\wval_1 = \wbot$ or $\wval_1 = \cw{\const}{\wpath_1}$ where $\wpath \wpord \wpath_1$.
Then, by the def.\ of $\wprop$ it follows that $\wval' = \cw{\const}{\wpath}$.
\item $\wval_2 = \werr$. Then, $\wval = \wval'=\wval'_1 = \wval_2 = \werr$.
\end{itemize}
%
Next, suppose $\wval = \cw{\wtable_2}{\wpath_2}$ for some $\wtable_2$ and $\wpath_2$.
Then it must be that $\wval_1 = \cw{\wtable_1}{\wpath_1}$ for some $\wtable_1$ and $\wpath_1$.
Also, it is the case that $\wval = \cw{\wtable}{\wpath}$ for some $\wtable$ and $\wpath$.
First, observe that
\begin{align*}
\ptop(\wpath) = \cnode, \ptop(\wpath_1) = \cnode_1, \ptop(\wpath_2) = \cnode_2 && \text{by }\tpcons(\wmap)\\
\wpath_1 \not= \wpath_2  &&
\end{align*}
We next show that $\wpath_1 \not\wpord \wpath_2$; the case $\wpath_2 \not\wpord \wpath_1$ is
handled similarly. Suppose $\wpath_1 \wpord \wpath_2$. By $\pvcons(\wmap)$ and $\wdet_e(\wmap)$, 
we know that $\wpath_2 = \wpath \cdot \cnode_2$ and $\wpath_1 = \wpath \cdot \cnode_1$.
Hence, there exist $i$ and $j$ such that $i \not= j$, $\cnode \in^i \wpath_2$, $\cnode \in^j \in \wpath_2$.
However, this is a contradiction by Lemma~\ref{thm:w-cons-node-norepeat}. Thus,
$\wpath_1 \not= \wpath_2$, $\wpath_1 \not\wpord \wpath_2$, and $\wpath_2 \not\wpord \wpath_1$.
By $\pcscons(\wmap)$, the set of observed call site paths in $\wtable_1$ and $\wtable_2$
is different. The result then follows immediately from the definition of $\wprop$.
\end{proof}

We next show that output values in tables must agree, via concrete subtyping, with the value
of the lambda body used to initially populate the table.
\begin{lemma}~\label{thm:w-cons-vouts}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$, $\wval$ a path value, 
$\cnode$ a node, and $\wpath_c$ as well as $\wpath'$ paths.
Suppose $\cw{\wtable}{\wpath} = \wmap(\cnode)$, for some $\wtable$ and $\wpath$, and let
$\pi_2(\wtable(\wpath_c)) = \wval$.
If $\wval = \cw{\_}{\wpath'}$, then $\wmap(\ptop(\wpath')) \;\wsub\; \wval$ and $\wmap(\ptop(\wpath')) = \cw{\_}{\wpath'}$.
\end{lemma}
\begin{proof}
\begin{align*}
\wpath, \wpath_c, \wpath' \in \allpaths(\wmap) && \text{by def.\ of } \allpaths\\
e(\nloc(\proot(\wpath))) = \mu f.\lambda x.e_1^{\ell_1} && \text{for some $f, x, e_1, \ell_1$ by } \rootcons_e(\wmap)\\
            \cnode_x = \cvn{\nenv(\proot{\wpath})}{\ptop(\wpath_c)}{x}, && \text{assume}\\
            \cnode_f = \cvn{\nenv(\proot{\wpath})}{\ptop(\wpath_c)}{f}, && \\
            \cenv_1 = \nenv(\proot(\wpath)).x\!:\cnode_x.f\!:\cnode_f  && \\
\ptop(\wpath') = \cn{\cenv_1}{\ell_1} && \text{by } \outcons_e(\wmap)\\
\wmap(\proot(\wpath)) \;\wsub\; \wmap(\cnode) && \text{by } \cmsub_e(\wmap), \tiocons{\wmap}, \pcscons_e(\wmap), \\
&& \text{and Lemma~\ref{thm:w-sub-transitive}}\\
\wmap(\proot(\wpath)) = \cw{\wtable_r}{\_} && \text{for some $\wtable_r$ by def.\ of } \wsub\\
\wmap(\cn{\cenv_1}{\ell_1}) \;\wsub\; \pi_2(\wtable_r(\wpath_c)) && \text{by } \cmsub_e(\wmap) \\
\wmap(\cn{\cenv_1}{\ell_1}) \;\wsub\; \wval && \text{by } \cmsub_e(\wmap), \tiocons{\wmap}, \pcscons_e(\wmap), \\
&& \text{and Lemma~\ref{thm:w-sub-transitive}}\\
\wmap(\cn{\cenv_1}{\ell_1})= \cw{\_}{\wpath'} && \text{by $\tpcons(\wmap)$ and Lemma~\ref{thm:w-cons-top-unique}} 
\end{align*}
\end{proof}
%
A similar result holds for inputs of tables that are pushed to tables at the execution points 
corresponding to function application expressions.
%
\begin{lemma}~\label{thm:w-cons-vins}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$, $\wval$ a path value, 
$\cnode$ a node, and $\wpath_c$ as well as $\wpath'$ paths.
Suppose $\cw{\wtable}{\wpath} = \wmap(\cnode)$, for some $\wtable$ and $\wpath$, and let
$\pi_1(\wtable(\wpath_c)) = \wval$.
If $\wval = \cw{\_}{\wpath'}$, then $\wmap(\ptop(\wpath')) \;\wsub\; \wval$ and $\wmap(\ptop(\wpath')) = \cw{\_}{\wpath'}$.
\end{lemma}
\begin{proof}
\begin{align*}
\wpath, \wpath_c, \wpath' \in \allpaths(\wmap) && \text{by def.\ of } \allpaths\\
\wpath \wpord \wpath_c && \text{by } \pcscons(\wmap)\\
e_1^{\nloc(\ptop(\wpath_c))} e_2^{\nloc(\ptop(\wpath'))} \in e, && \text{for some $e_1, e_2$ by } \inpcons_e(\wmap)\\
\nenv(\ptop(\wpath_c)) = \nenv(\ptop(\wpath')) && \\ 
\wmap(\cnode) \;\wsub\; \wmap(\ptop(\wpath_c)) && \text{by } \cmsub_e(\wmap), \tiocons{\wmap}, \pcscons_e(\wmap), \\
&& \text{and Lemma~\ref{thm:w-sub-transitive}}\\
\wmap(\ptop(\wpath_c)) = \cw{\wtable_c}{\_} && \text{by def.\ of } \wsub \text{ and } \pvcons(\wmap)\\
\pi_1(\wtable_c(\wpath_c)) \;\wsub\; \wval && \text{by def.\ of } \wsub \\
\wmap(\ptop(\wpath')) \;\wsub\; \pi_1(\wtable_c(\wpath_c)) && \text{by } \cmsub_e(\wmap) \\
\wmap(\ptop(\wpath')) \;\wsub\; \wval && \text{by } \cmsub_e(\wmap), \tiocons{\wmap}, \pcscons_e(\wmap), \\
&& \text{and Lemma~\ref{thm:w-sub-transitive}}\\
\wmap(\ptop(\wpath'))= \cw{\_}{\wpath'} && \text{by $\tpcons(\wmap)$ and Lemma~\ref{thm:w-cons-top-unique}} 
\end{align*}
\end{proof}

We next show that the concrete transformer does not change the structure of the paths, i.e., the $\wpred$ relation.
\begin{lemma}~\label{thm:w-cons-parallel-paths}
Let $\wmap$, $\wmap_1$, and $\wmap_2$ be path maps such that $\wcons_e(\wmap_1)$, $\wcons_e(\wmap_2)$, and 
$\wcons_e(\wmap)$ for some program $e$. Given an expression $e_0^\ell \in e$, and two environments 
$\cenv_1$ and $\cenv_2$ such that $\cenv_1 \not= \cenv_2$, $\domvalid(\ell, e, \cenv_1,$, $\domvalid(\ell, e, \cenv_2)$, 
and $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$, assume that $\wtrans[k]{e_0^\ell}(\cenv_1)(\wmap) = \wmap_1$ and $\wtrans[k]{e_0^\ell}(\cenv_2)(\wmap) = \wmap_2$. Then,
$\forall \wpath_1, \wpath_2 \in \allpaths(\wmap_1) \cup \allpaths(\wmap_2), i, j, \cnode.\, \cnode \in^i \wpath_1 \wedge \cnode \in^j \wpath_2
{\implies} \wprefix(\wpath_1, i) = \wprefix(\wpath_2, j)$.
\end{lemma}
\begin{proof}
Let $\wpath' = \wprefix(\wpath_1, i)$ and $\wpath'' = \wprefix(\wpath_2, j)$.
Clearly, $\ptop(\wpath') = \cnode = \ptop(\wpath'')$ by the definition of $\wprefix$.
First, if $\wpath_1 \in \allpaths(\wmap_1)$ and $\wpath_2 \in \allpaths(\wmap_1)$, then
by Lemma~\ref{thm:w-pvcons-prefix} we have that $\wpath', \wpath'' \in \allpaths(\wmap_1)$
and the result thus follows from Lemma~\ref{thm:w-cons-top-unique}. The same argument 
applies for the case when $\wpath_1 \in \allpaths(\wmap_2)$ and $\wpath_2 \in \allpaths(\wmap_2)$.

We are therefore left with the case when $\wpath_1 \in \allpaths(\wmap_1)$ and $\wpath_2 \in \allpaths(\wmap_2)$
but $\wpath_1 \not\in \allpaths(\wmap_2)$ and $\wpath_2 \not\in \allpaths(\wmap_1)$. (The same
argument that follows also applies for the case where we invert the memberships of $\wpath_1$ and $\wpath_2$.)
By Lemma~\ref{thm:w-pvcons-prefix}, we have that $\wpath' \in \allpaths(\wmap_1)$ and $\wpath'' \in \allpaths(\wmap_2)$.
We thus have $\wdet^e_{\wmap_1}(\wpath')$ and $\wdet^e_{\wmap_2}(\wpath'')$. The argument follows
by a mutual induction on $|\wpath'|$ and $|\wpath''|$. If $|\wpath'| = |\wpath''| = 1$, the argument
is trivial. Next, observe that by $\rootcons_e(\wmap_1)$ and $\rootcons_e(\wmap_2)$ and Lemma~\ref{thm:w-pred-nopred}
it cannot be the case that $|\wpath'| > 1$ and $|\wpath''| = 1$ (and similarly $|\wpath''| > 1$ and $|\wpath'| = 1$).
Hence, both $\wpath'$ and $\wpath''$ have a predecessor of a top node $\cnode$; let those predecessor
node be $\cnode'$ and $\cnode''$, respectively. We next show that $\cnode' = \cnode''$. The argument
then inductively follows by Lemma~\ref{thm:w-pvcons-prefix}. We consider all the possible cases of $\cnode$
by inspecting the definition of $\wpred$.
Observe that we have $\wpred^e_{\wmap_1}(\cnode', \cnode)$ and $\wpred^e_{\wmap_2}(\cnode'', \cnode)$.
\begin{itemize}
\item $e(\nloc(\cnode)) = x$.
\begin{align*}
x \in \m{dom}(\nenv(\cnode))  && \text{by def.\ of }\wpred\\
\forall \wmap, \cnode_0.\,\wpred^e_{\wmap}(\cnode_0, \cnode){\implies} \cnode_0 = \nenv(\cnode)(x) && \text{by def.\ of } \wpred\\                         
\wpred^e_{\wmap_1}(\nenv(\cnode)(x), \cnode), \wpred^e_{\wmap_2}(\nenv(\cnode)(x), \cnode) && \\
\cnode' = \cnode'' = \nenv(\cnode)(x)
\end{align*}

\item $\cnode = \cvn{\cenv}{\cnode_c}{x}$ for some $\cenv$, $\cnode_c$, and $x$.
\begin{align*}
\bullet\, \cnode_c \not\in \cranger(\cn{\cenv_1}{\ell}), \cnode_c \not\in \cranger(\cn{\cenv_2}{\ell}) && \textbf{assume}\\
\quad \wmap(\cnode_c) = \wmap_1(\cnode_c) = \wmap_2(\cnode_c) && \text{by Lemma~\ref{thm:w-framer} and Lemma~\ref{thm:w-disjointr-1}}\\
\quad \cnode' = \cnode'' && \text{by def.\ of } \wpred\\[1ex]
%
\bullet\, \cnode_c \in \cranger(\cn{\cenv_1}{\ell}), \cnode_c \in \cranger(\cn{\cenv_2}{\ell}) && \textbf{assume}\\
\quad \text{impossible} && \text{by Lemma~\ref{thm:w-framer} and Lemma~\ref{thm:w-disjointr-1}}\\[1ex]
%
\bullet\, \cnode_c \in \cranger(\cn{\cenv_1}{\ell}), \cnode_c \not\in \cranger(\cn{\cenv_2}{\ell}) && \textbf{assume}\\
\quad \wmap_2(\cnode_c)= \wmap(\cnode_c) && \text{by Lemma~\ref{thm:w-framer} and Lemma~\ref{thm:w-disjointr-1}}\\
\quad \wmap(\cnode_c) \not= \wbot && \text{by def.\ of } \wpred\\
\quad \wmap_1(\cnode_c) \not= \werr && \text{by } \errcons(\wmap_1)\\
\quad \wmap(\cnode_c) = \cw{\_}{\wpath_c}, \wmap_1(\cnode_c) = \cw{\_}{\wpath_c},  && \text{for some $\wpath_c$ by Lemma~\ref{thm:w-step-path-stable}}\\
\quad \wmap_2(\cnode_c) = \cw{\_}{\wpath_c} &&\\
\quad \cnode' = \cnode'' && \text{by def.\ of } \wpred\\[1ex]
%
\bullet\, \cnode_c \not\in \cranger(\cn{\cenv_1}{\ell}), \cnode_c \in \cranger(\cn{\cenv_2}{\ell}) && \textbf{assume}\\
\quad\text{similar to above} &&
\end{align*}
%
\item Similar for other cases of $\cnode$.
\end{itemize}
\end{proof}



We also show that the join of two consistent path maps, obtained by parallel applications of the concrete
transformer, is subtype consistent.
\begin{lemma}~\label{thm:w-cons-sub-parallel}
Let $\wmap$, $\wmap_1$, and $\wmap_2$ be path maps such that $\wcons_e(\wmap_1)$, $\wcons_e(\wmap_2)$, and 
$\wcons_e(\wmap)$ for some program $e$. Assume we are also given an expression $e_0^\ell \in e$, and two environments 
$\cenv_1$ and $\cenv_2$ such that $\cenv_1 \not= \cenv_2$, $\domvalid(\ell, e, \cenv_1)$, $\domvalid(\ell, e, \cenv_2)$, 
and $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$. If $\wtrans[k]{e_0^\ell}(\cenv_1)(\wmap) = \wmap_1$ 
and $\wtrans[k]{e_0^\ell}(\cenv_2)(\wmap) = \wmap_2$, then $\cmsub_e(\wmap_1 \wmjoin \wmap_2)$.
\end{lemma}
\begin{proof}
Let $\wpath \in \allpaths(\wmap_1 \wmjoin \wmap_2)$ and $\pair{\cnode_1}{\cnode_2}$. 
We show that 
\[\wmap_1(\cnode_1) \wvjoin \wmap_2(\cnode_1) \wsub \wmap_2(\cnode_1) \wvjoin \wmap_1(\cnode_2)\]
For the remainder of the definition of $\cmsub_e$, the argument follows from Lemma~\ref{thm:w-framer} 
and Lemma~\ref{thm:w-disjointr-1}. Let $\wval_1 = \wmap_1(\cnode_1) \wvjoin \wmap_2(\cnode_1)$
and $\wval_2 = \wmap_1(\cnode_2) \wvjoin \wmap_2(\cnode_2)$.

First, observe that $\wpath \in \allpaths(\wmap_1)$ or $\wpath \in \allpaths(\wmap_2)$ by the definition of
$\wmjoin$. Also, note that $\wmap_1(\cnode_1) \not=\werr, \wmap_2(\cnode_1) \not= \werr, \wmap_2(\cnode_1) \not= \werr$, and
$\wmap_1(\cnode_2) \not=\werr$. Suppose not. By $\errcons(\wmap_1)$ and $\errcons(\wmap_2)$ we have that
$\wmap_1 = \wmap_\werr$ or $\wmap_2 = \wmap_\werr$, in which case $\wmap_1 \wmjoin \wmap_2 = \wmap_\werr$ 
and thus $\allpaths(\wmap_1 \wmjoin \wmap_2) = \emptyset$, a contradiction. Further, note that 
$\wval_1 \not= \wbot$ and $\wval_2 \not= \wbot$ by $\wcons_e(\wmap_1)$, $\wcons_e(\wmap_2)$, and Lemma~\ref{thm:w-cons-bot-err}. 

We proceed with the proof by structural induction on $\wval_1$ and $\wval_2$ where we focus on the cases where 
$\wval_1\not=\wbot$ and $\wval_2\not=\wbot$. Suppose first $\wval_1 = \werr$. There are two cases possible. 
First, $\wmap_1(\cnode_1) = \cw{\const_1}{\wpath_1}$
and $\wmap_2(\cnode_1) = \cw{\const_2}{\wpath_2}$ where either $\const_1 \not= \const_2$ or 
$\wpath_1 \not\wpord \wpath_2 \wedge \wpath_2 \not\wpord \wpath_1$. 
%
\begin{align*}
\wpath_1 = \wpath_2 && \text{by Lemma~\ref{thm:w-cons-parallel-paths}}\\
\wmap_1(\proot(\wpath_1)) = \cw{\const}{\_}, \wmap_2(\proot(\wpath_2)) = \cw{\const}{\_} && \text{by }\rootcons_e(\wmap_1), \rootcons_e(\wmap_2),\\
&& \constcons(\wmap_1)\text{, and }\constcons(\wmap_2)\\
\wmap_1(\ptop(\wpath_1)) = \cw{\const}{\_}, \wmap_2(\ptop(\wpath_2)) = \cw{\const}{\_} && \text{by }\cmsub_e(\wmap_1), \cmsub_e(\wmap_2),\\
&& \text{Lemma~\ref{thm:w-sub-transitive}, and def.\ of }\wsub\\
\text{contradiction} &&
\end{align*}
%
The other case is when $\wmap_1(\cnode_1)$ is a constant path value and $\wmap_2(\cnode_1)$ is table path value, or vice versa. 
The argument is then exactly the same. Moreover, the same reasoning steps are sufficient to show that $\wval_2 \not= \werr$.
In conclusion, $\wval_1 \not= \werr$ and $\wval_2 \not= \werr$.

Next, suppose that $\wval_1 = \cw{\const_1}{\wpath_1}$ and $\wval_2 = \cw{\const_2}{\wpath_2}$ where either 
$\const_1 \not= \const_2$ or $\wpath_1 \not\wpord \wpath_2 \wedge \wpath_2 \not\wpord \wpath_1$. 
%
\begin{align*}
(\wmap_1(\cnode_1) = \cw{\const_1}{\wpath_1} \wedge \wmap_1(\cnode_2) = \cw{\const_1}{\wpath_2}) \;\vee && \text{by }\wcons_e(\wmap_1), \wcons_e(\wmap_2),\\
(\wmap_2(\cnode_1) = \cw{\const_1}{\wpath_1} \wedge \wmap_2(\cnode_2) = \cw{\const_1}{\wpath_2}) && \text{and Lemma~\ref{thm:w-cons-bot-err}}\\
\wpath_1 \wpord \wpath_2 && \text{by $\cmsub_e(\wmap_1)$ and $\cmsub_e(\wmap_2)$}\\
\const_1 = \const_2 && \text{by }\rootcons_e(\wmap_1), \rootcons_e(\wmap_2),\\
&& \constcons(\wmap_1), \constcons(\wmap_2),\\
&& \cmsub_e(\wmap_1), \cmsub_e(\wmap_2),\\
&& \text{Lemma~\ref{thm:w-sub-transitive}, and def.\ of }\wsub\\
\text{contradiction} &&
\end{align*}
%
The same reasoning steps apply for the other base cases of $\wval_1\in\wconsts \wedge \wval_2\in\wtables$ and $\wval_1\in\wtables \wedge \wval_2\in\wconsts$.
When $\wval_1 \in \wtables$ and $\wval_2\in\wtables$, for every call site path $\wpath$ the  
inputs of $\wval_1$ and $\wval_2$, and outputs respectively, at $\wpath$ must agree on the top nodes by $\inpcons_e(\wmap_1)$, $\inpcons_e(\wmap_2)$,
$\outcons_e(\wmap_1)$, and $\outcons_e(\wmap_2)$. The same reasoning as above then inductively applies by Lemma~\ref{thm:w-cons-vins}, 
Lemma~\ref{thm:w-cons-vouts}, and the definition of $\wsub$.
\end{proof}


\begin{lemma}~\label{thm:w-cons-pvcons-parallel}
Let $\wmap$, $\wmap_1$, and $\wmap_2$ be path maps such that $\wcons_e(\wmap_1)$, $\wcons_e(\wmap_2)$, and 
$\wcons_e(\wmap)$ for some program $e$. Given an expression $e_0^\ell \in e$, and two environments 
$\cenv_1$ and $\cenv_2$ such that $\cenv_1 \not= \cenv_2$, $\domvalid(\ell, e, \cenv_1)$, $\domvalid(\ell, e, \cenv_2)$, 
and $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$, assume that $\wtrans[k]{e_0^\ell}(\cenv_1)(\wmap) = \wmap_1$ 
and $\wtrans[k]{e_0^\ell}(\cenv_2)(\wmap) = \wmap_2$. Then, $\pvcons(\wmap_1 \wmjoin \wmap_2)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:w-cons-sub-parallel}.
\end{proof}

\begin{lemma}~\label{thm:w-cons-errcons-parallel}
Let $\wmap$, $\wmap_1$, and $\wmap_2$ be path maps such that $\wcons_e(\wmap_1)$, $\wcons_e(\wmap_2)$, and 
$\wcons_e(\wmap)$ for some program $e$. Given an expression $e_0^\ell \in e$,  and two environments 
$\cenv_1$ and $\cenv_2$ such that $\cenv_1 \not= \cenv_2$, $\domvalid(\ell, e, \cenv_1)$, $\domvalid(\ell, e, \cenv_2)$, 
and $\m{dom}(\cenv_1) = \m{dom}(\cenv_2)$, assume that $\wtrans[k]{e_0^\ell}(\cenv_1)(\wmap) = \wmap_1$ 
and $\wtrans[k]{e_0^\ell}(\cenv_2)(\wmap) = \wmap_2$. Then, $\errcons(\wmap_1 \wmjoin \wmap_2)$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:w-cons-sub-parallel}.
\end{proof}


The above results are used to show that the general consistency of path maps is preserved by $\wtransname$.
\begin{theorem}~\label{thm:w-cons-inductive}
Let $\wmap, \wmap_f \in \wmaps$, $\wmap_f \in \wmaps$, $e^\ell$ an expression of a
program $m$,  and $\cenv$ an environment where $(e, \cenv)$
is well-formed, $\domvalid(\ell, m, \cenv)$, and $\envcons_\wmap(\cenv)$. 
If $\wcons_m(\wmap)$ and $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_f$, then $\wcons_m(\wmap_f)$ and $\envcons_{\wmap_f}(\cenv)$.
\end{theorem}
\begin{proof}
The proof goes by structural induction on $e$. We need to show
that $\envcons(\wmap)$, $\cmsub_m(\wmap_f)$, $\pvcons_m(\wmap_f)$, $\errcons(\wmap_f)$,
$\constcons_m(\wmap_f)$, $\wdet_m(\wmap_f)$. When $k=0$, the argument is trivial.
We consider the cases for $e$ when $k>1$.
\begin{itemize}
\item $e=c$. Let $\wmap(\cn{\cenv}{\ell}) = \wval$. By $\constcons_m(\wmap_f)$, we have that
             $\wval \in \{\wbot, \werr, \cw{\const}{\ell}\}$. If $\wval = \cw{\const}{\ell}$,
             then $\wmap = \wmap_f$ and the argument is trivial. If $\wval = \werr$, then by 
             $\errcons(\wmap)$, we have $\wmap = \wmap_\werr$ and hence $\wmap_f = \wmap_\werr = \wmap$,
             from which the argument directly follows. If $\wval = \wbot$, then $\wmap_f = \wmap[\cn{\cenv}{\ell} \mapsto \cw{\const}{\cn{\cenv}{\ell}}]$,
             from which $\wdet_e(\wmap_f)$, $\errcons(\wmap_f)$,  $\envcons(\wmap_f)$, and $\constcons_m(\wmap_f)$ immediately follow.
             Lastly, $\pvcons(\wmap_f)$ and $\cmsub_m(\wmap_f)$ hold by Lemma~\ref{thm:w-cons-bot-err}.
	     Note that $\envcons_{\wmap_f}(\cenv)$ holds trivially.

\item $e=x$. Let $\wval_x = \wmap(\cenv(x))$ and $\wval = \wmap(\cn{\cenv}{\ell})$. 
             If $\wval_x = \werr \vee \wval = \werr$, then $\wmap = \wmap_{\werr}$ and
	     by Lemma~\ref{thm:w-prop-increasing-monotone} it follows that $\wmap_f = \wmap_\werr$
	     and $\wcons_m(\wmap_f)$ trivially. Also note that  $\constcons_m(\wmap_f)$ holds trivially. 
	     
	     Next, note that by the def.\ of $\wpred$,
             we have $\wpred^m_{\wmap}(\cenv(x), \cn{\cenv}{\ell})$. By Lemma~\ref{thm:w-cons-agree},
	     it is the case that
	     $\wval = \wbot$ or $\wagree_{\cn{\cenv}{\ell}}(\wval_x, \wval)$.
	     In case $\wval=\wbot$, $\wdet^m(\wmap_f)$ follows by $\wpred^m_{\wmap}(\cenv(x), \cn{\cenv}{\ell})$ 
	     and Lemma~\ref{thm:w-cons-bot-err} whereas $\pvcons(\wmap_f)$ follows by the
	     def.\ of $\wprop$ and $\ext$. In the other case, $\wdet^m(\wmap_f)$ and $\pvcons(\wmap_f)$
	     follow by Lemma~\ref{thm:w-step-path-stable}.

	     Since $\wval = \wbot$ or $\wagree_{\cn{\cenv}{\ell}}(\wval_x, \wval)$,
	     by $\wcons_m(\wmap)$ and the definition of $\wsub$, we have that $\wval_x \wsub \wval$.
	     Then by Lemma~\ref{thm:w-prop-sub-noerr} it follows that $\errcons(\wmap_f)$.
	     This lemma and Lemma~\ref{thm:w-prop-increasing-monotone} imply $\envcons(\wmap_f)$ 
	     and $\envcons_{\wmap_f}(\cenv)$.

	     We now turn to proving that $\cmsub_m(\wmap_f)$. 
	     By Lemma~\ref{thm:w-prop-sub}, we have that $\wval'_x \wsub \wval'$. For any path at
	     which the pair $\pair{\cenv(x)}{\cn{\cenv}{\ell}}$ lies, the subtyping across the whole path
	     is not invalidated by Lemma~\ref{thm:w-sub-prop-chain} and $\wcons_m(\wmap_f)$. As paths
	     can branch on variable nodes by Lemma~\ref{thm:w-pred-branch}, the subtyping between $\cenv(x)$
	     and successive nodes in other paths on which $\cenv(x)$ lies holds by Lemma~\ref{thm:w-cons-csub-branch}.
	     Next, suppose $e_1^{\ell_1} x^{\ell} \in m$ for some $e_1$ and $\ell_1$. If $\wmap(\cn{\cenv}{\ell_1}) = \cw{\wtable}{\wpath_1}$,
	     for some $\wtable \in \wtables$ and path $\wpath_1$, then we need to show 
	     that $\wval' \wsub \pi_2(\wtable(\wpath_1))$. We know by the def.\ of $\cmsub_m$ that
	     $\wval \wsub \pi_1(\wtable(\wpath_1))$ and, from earlier, that $\wval \wsub \wval'_x$.
	     Then, the argument follows by Lemma~\ref{thm:w-sub-prop-chain}. The similar reasoning applies
	     for other places where $x$ can appear in $m$.

\item $e = e_1^{\ell_1} e_2^{\ell_2}$. Clearly $(e_1, \cenv)$ is well-formed and $\domvalid(\ell_1, m, \cenv)$ so 
             by the i.h., we have that $\wcons_m(\wmap_1)$ and $\envcons_{\wmap_1}(\cenv)$. Also, $(e_2, \cenv)$ is 
	     well-formed and $\domvalid(\ell_2, m, \cenv)$ so we have by the i.h.\ that $\wcons_m(\wmap_2)$ and $\envcons_{\wmap_2}(\cenv)$.
	     By Lemma~\ref{thm:w-framer} and Lemma~\ref{thm:w-disjointr-1} we have that $\wval_1 = \wmap_2(\cn{\cenv}{\ell_1})$.
	     Hence, we have that $\wval_1 \wsub [\ppath(\wval_1) \mapsto \pair{\wval_2}{\wval}]$, where $\wval = \wmap_2(\cn{\cenv}{\ell})$,
	     by the def.\ of $\cmsub_m(\wmap_2)$. Then, $\envcons(\wmap_f)$ and $\envcons_{\wmap_f}(\cenv)$ hold
	     trivially, $\errcons(\wmap_f)$ follows by Lemma~\ref{thm:w-prop-sub-noerr}, and $\constcons(\wmap_f)$
	     holds by the def.\ of $\wprop$. That is, suppose $m(\ell_1)$ is a lambda expression.  Then 
	     by Lemma~\ref{thm:w-prop-increasing-monotone}, $\wval'_1 \in \wtables \cup \{\werr\}$. However,
	     $\wval'_1 \not= \werr$ by Lemma~\ref{thm:w-prop-sub-noerr}.

	     We next show that $\cmsub_m(\wmap_f)$.
	     First, let $\wval_o = \pi_2(\wtable(\ppath(\wval_1)))$. We know that $\wval_o \wsub \wval$.
	     If $\wval_o = \wbot$, then $\wval = \wbot$. A more interesting case is when $\wval_o=\cw{\_}{\wpath_o}$.
	     By $\outcons_m(\wmap_2)$, we have that $\ptop(\wpath_o) = \cn{\cenv_b}{\ell_b}$ where
	     $\cenv_b = \cenv_0.x\!:\cvn{\cenv_0}{\cnode_c}{x}.f\!:\cvn{\cenv_0}{\cnode_c}{f}$,
             $\cenv_0 = \nenv(\proot(\ppath(\wval_1)))$, $\cenv_c = \ptop(\ppath(\wval_1))$, and
	     $m(\nloc(\proot(\ppath(\wval_1)))) = \mu f. \lambda x.e_b^{\ell_b}$ for some $e_b$, $f$, $x$, and $\ell_b$.
	     Hence, $\wpred^m_{\wmap_2}(\cn{\cenv_b}{\ell_b}, \cn{\cenv}{\ell})$ by the def.\ of $\wpred$. By Lemma~\ref{thm:w-cons-agree},
	     it is the case that $\wval = \wbot$ or $\wagree_{\cn{\cenv}{\ell}}(\wmap_2(\cn{\cenv_b}{\ell_b}), \wval)$.

	     We next need to show that $\wmap_f(\cn{\cenv_b}{\ell_b}) \wsub \wval'$. Note that 
	     $\wmap_f(\cn{\cenv_b}{\ell_b}) = \wmap_2(\cn{\cenv_b}{\ell_b})$. We know that $\wval_o \wsub \wval$
	     by $\cmsub_m(\wmap_2)$ and hence $\wval'_o \wsub \wval'$ by Lemma~\ref{thm:w-prop-sub}. 
	     By Lemma~\ref{thm:w-cons-vouts}, we have that $\wmap_2(\cn{\cenv_b}{\ell_b}) \wsub \wval_o$.
	     Therefore, by Lemma~\ref{thm:w-sub-prop-chain} we have $\wmap_2(\cn{\cenv_b}{\ell_b}) \wsub \wval'_o$  and 
	     thus by Lemma~\ref{thm:w-sub-transitive} it must be that $\wmap_2(\cn{\cenv_b}{\ell_b}) \wsub \wval'$.
	     The same argument applies for the updated input of $\wval'_1$. The remaining argument for $\cmsub_m(\wmap_f)$
	     as well as $\wdet_m(\wmap_f)$, $\pvcons(\wmap_f)$, is the same as in the case of program variables.


\item $e = \mu f. \lambda x.\, e_1^{\ell_1}$. First, observe that for any $\wpath_1, \wpath_2 \in \wtable$ where
             $\wpath_1 \not= \wpath_2$, we have that $\ptop(\wpath_1) \not= \ptop(\wpath_2)$ by Lemma~\ref{thm:w-cons-top-unique}.
	     Hence, for any $\wpath \in \wtable$, we have unique $\cnode_x$, $\cnode_f$, and $\cenv_1$.
	     By $\cmsub_m(\wmap)$, we know that $\wtable \;\wsub\; \wmap(\cnode_f)$ and 
	     $[\wpath \mapsto \pair{\wmap(\cnode_x)}{\wmap(\cn{\cenv_1}{\ell_1})}] \;\wsub\; \wtable$.
	     Since $\pi_1(\wtable(\wpath)) \not= \wbot$, we have by the definition of $\wpred$ and $\inpcons_m(\wmap)$
	     that $\wpred^m_{\wmap}(\ptop(\ppath(\pi_1(\wtable(\wpath)))), \cnode_x)$ and by the def.\ of $\wpred$
	     we also have $\wpred^m_{\wmap}(\cn{\cenv}{\ell}, \cnode_f)$. The argument then goes as usual
	     to show that $\wcons_m(\wmap_1)$. Note that in order to show that $\cmsub_m(\wmap_1)$ we also
	     additionally use Lemma~\ref{thm:w-sub-prop-join-chain} to show that the join $\wtable_1 \wvjoin \wtable_2$
	     does not invalidate the subtyping on the paths at which $\cnode_f$ appears.

	     Finally, we switch to proving that the join of all such $\wmap_1$, resulting in $\wmap_f$, is consistent. 
	     First, $\errcons(\wmap_f)$ follows by Lemma~\ref{thm:w-step-finite} and Lemma~\ref{thm:w-cons-errcons-parallel}. 
	     Next, $\envcons(\wmap_f)$ and $\envcons_{\wmap_f}(\cenv)$ simply follows by the def.\ of $\wmjoin$. Similarly,
	     $\wdet_m(\wmap_f)$ follows from the def.\ of $\wmjoin$. Finally, $\cmsub_m(\wmap_f)$ and $\pvcons(\wmap_f)$
	     follows by Lemma~\ref{thm:w-step-finite}, Lemma~\ref{thm:w-cons-sub-parallel}, and Lemma~\ref{thm:w-cons-pvcons-parallel}.

%\item $e = \ifte{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}}$. Similar to the earlier cases.
\end{itemize} 
\end{proof}


\input{proofs/path-to-data-flow}


==> proofs/path-to-data-flow.tex <==
\subsubsection{Connection to Data Flow Semantics}

In this subsection, we make the formal connection between path data flow semantics
and the regular data flow semantics without the path information. To that end, we
first introduce the notion on uniqueness $\tpcsuniq(\wval)$ of a value $\wval$ in terms of the uniqueness of 
paths subject to their top nodes. 
%
\begin{align*}
\tpcsuniq(\wval) \Def\iff & (\wval \in \{\wbot, \werr\} \cup \wconsts) \vee
(\exists \wtable.\, \wval = \cw{\wtable}{\_} \wedge (\forall \wpath_1, \wpath_2 \in \wtable.\\
& \ptop(\wpath_1) = \ptop(\wpath_2){\implies}\wpath_1 = \wpath_2) \wedge
\forall \wpath \in \wtable.\\
& \tpcsuniq(\pi_1(\wtable(\wpath))) \wedge \tpcsuniq(\pi_2(\wtable(\wpath))))
\end{align*}
%
We first prove the results stating that two paths drawn from a set
of root consistent and deterministic paths must have unique top nodes.
\begin{lemma}~\label{thm:w-strip-paths-unique}
Let $P$ be a set of paths such that for every $\wpath \in P$ we have
$\rootcons_e(\wpath)$ and $\wdet^e_{\wmap}(\wpath)$ for some program
$e$ and a path map $\wmap$. Then, for any $\wpath_1, \wpath_2 \in P$,
$\ptop(\wpath_1) = \ptop(\wpath_2)$ implies $\wpath_1 = \wpath_2$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:w-cons-top-unique}.
\end{proof}
%
Data propagation does not invalidate the $\tpcsuniq$ property.
\begin{lemma}~\label{thm:w-prop-tpcsuniq}
Let $\wval_1$ and $\wval_2$ be path values s.t. $\tpcsuniq(\wval_1)$,
$\tpcsuniq(\wval_2)$, and $P = \allpaths(\wval_1) \cup \allpaths(\wval_2)$ 
where for every $\wpath \in P$ we have
$\rootcons_e(\wpath)$ and $\wdet^e_{\wmap}(\wpath)$ for some program
$e$ and a path map $\wmap$. Further, let $\wval_3$ and $\wval_4$ be
values such that $\pair{\wval_3}{\wval_4} = \wprop(\wval_1, \wval_2)$.
Then, $\tpcsuniq(\wval_3)$ and $\tpcsuniq(\wval_4)$.
\end{lemma}
\begin{proof}
By structural induction on $\wval_1$ and $\wval_2$. The base cases
are trivial.
For the inductive case, let $\wval_1 = \cw{\wtable_1}{\wpath_1}$ and
$\wval_2 = \cw{\wtable_2}{\wpath_2}$ where $\wpath_1 \wpord \wpath_2$.
Let $\wpath \in \wtable_2$ for some $\wpath$. By Lemma~\ref{thm:w-strip-paths-unique},
there is no different $\wpath' \in \wtable_2$ such that  $\ptop(\wpath) = \ptop(\wpath')$. Also, for every $\wpath' \in \wtable_1$ s.t. $\ptop(\wpath') = \ptop(\wpath)$, we have by Lemma~\ref{thm:w-strip-paths-unique} that
$\wpath = \wpath'$. In other words, by Lemma~\ref{thm:w-strip-paths-unique} 
the call site paths both in $\wval_1$ and $\wval_2$ can be uniquely and
consistently identified with their top nodes. The argument then follows by i.h.
\end{proof}

Next, we present the conversion function $\wstrip:\wvalues \rightharpoonup \cvalues$
from path data flow values to regular data flow values that simply strips
the path information.
%
\begin{align*}
\wstrip(\wbot) \Def= \bot & \ind[4]\wstrip(\werr) \Def= \cerr && \wstrip(\cw{\const}{\wpath}) \Def= \const\\
\wstrip(\cw{\wtable}{\wpath}) \Def= & \;\Lambda \ccsite.\,\Mif \exists \wpath' \in \wtable.\, \ptop(\wpath') = \ccsite && \text{if } \tpcsuniq(\cw{\wtable}{\wpath})\\
& \quad\Mthen \pair{\wstrip(\pi_1(\wtable(\wpath')))}{\wstrip(\pi_2(\wtable(\wpath')))} &&\\
& \quad\Melse \cw{\bot}{\bot} &&
\end{align*}
%
The strip function on maps $\wstrip: \wmaps \rightharpoonup \cmaps$ is defined in the expected way.

Using the $\wstrip$ function, we next connect the subtyping relation between path values and plain data flow values.
%
\begin{lemma}~\label{thm:w-strip-sub}
Let $\wval_1$ and $\wval_2$ be path values and $P = \allpaths(\wval_1) \cup \allpaths(\wval_2)$ 
where for every $\wpath \in P$ we have
$\rootcons_e(\wpath)$ and $\wdet^e_{\wmap}(\wpath)$ for some program
$e$ and a path map $\wmap$. Further, assume that $\tpcsuniq(\wval_1)$ and 
$\tpcsuniq(\wval_2)$. Then, $\wval_1 \;\wsub\; \wval_2$ implies 
$\wstrip(\wval_1) \;\csub\; \wstrip(\wval_2)$.
\end{lemma}
\begin{proof}
First, note that $\tpcsuniq(\wval_1)$ implies $\wval_1 \in \m{dom}(\wstrip)$.
The same holds for $\wval_2$.
The proof goes by structural induction on $\wval_1$ and $\wval_2$.
We first cover the base cases.
\begin{itemize}
\item $\wval_1 = \wbot$, $\wval_1 \in \wvalues$. The result immediately
         follows by the def.\ of $\csub$ since $\wstrip(\wbot) = \bot$.

\item $\wval_1 = \werr$.
\begin{align*}
\wval_2 = \werr && \text{by def.\ of } \wsub\\
\wstrip(\wval_1) = \wstrip(\wval_2) = \cerr && \text{by def.\ of }\wstrip
\end{align*}

\item $\wval_1 = \cw{\const}{\wpath_1}, \wval_2 = \cw{\const}{\wpath_2}, \wpath_1 \wpord \wpath_2$.
\begin{align*}
\wstrip(\wval_1) = \wstrip(\wval_2) = \const && \text{by def.\ of }\wstrip
\end{align*}
\end{itemize}
%
For the inductive case, let $\wval_1 = \cw{\wtable_1}{\wpath_1}$ and
$\wval_2 = \cw{\wtable_2}{\wpath_2}$ where $\wpath_1 \wpord \wpath_2$.
Let $\wpath \in \wtable_2$ for some $\wpath$. By Lemma~\ref{thm:w-strip-paths-unique},
there is no different $\wpath' \in \wtable_2$ such that  $\ptop(\wpath) = \ptop(\wpath')$. 
Also, for every $\wpath' \in \wtable_1$ s.t. $\ptop(\wpath') = \ptop(\wpath)$, we 
have by Lemma~\ref{thm:w-strip-paths-unique} that $\wpath = \wpath'$. The argument 
then follows by i.h.
\end{proof}

We next show that the propagation between path values and their stripped counterparts
in the data flow semantics yields values that are again related by the $\wstrip$ function.
\begin{lemma}~\label{thm:w-prop-strip-parallel}
Let $\wval_1$ and $\wval_2$ be path values such that $\wval_1 \wsub \wval_2$ and 
$P = \allpaths(\wval_1) \cup \allpaths(\wval_2)$ where for every $\wpath \in P$ we have 
$\rootcons_e(\wpath)$ and $\wdet^e_{\wmap}(\wpath)$ for some program $e$ and a path map $\wmap$. 
Further, assume that $\tpcsuniq(\wval_1)$, $\tpcsuniq(\wval_2)$, and $\pair{\wval'_1}{\wval'_2} = \wprop(\wval_1, \wval_2)$
for some path values $\wval'_1$ and $\wval'_2$. Lastly, let $\pair{\cval'_1}{\cval'_2} = \cprop(\wstrip(\wval_1), \wstrip(\wval_2))$.
Then, $\wval'_1 \in \m{dom}(\wstrip), \wval'_2 \in \m{dom}(\wstrip), \wstrip(\wval'_1) = \cval'_1,$ and $\wstrip(\wval'_2) = \cval'_2$.
\end{lemma}
\begin{proof}
By Lemma~\ref{thm:w-prop-tpcsuniq}, we have $\tpcsuniq(\wval'_1)$ and $\tpcsuniq(\wval'_2)$. By the def.\ of
$\wstrip$, it must also be that $\wval_1 \in \m{dom}(\wstrip)$ and $\wval_1 \in \m{dom}(\wstrip)$.
The proof continues by the structural induction on $\wval_1$ and $\wval_2$. We cover the base cases first.
\begin{itemize}
\item $\wval_1 = \wbot, \wval_2 = \wbot$.
\begin{align*}
\wval'_1 = \wval'_2 = \wbot && \text{by def.\ of }\wprop\\
\wstrip(\wval_1) = \wbot, \wstrip(\wval_2) = \wbot && \text{by def.\ of }\wstrip\\
\cval'_1 = \cval'_2 = \wbot && \text{by def.\ of }\cprop
\end{align*}


\item $\wval_1 = \cw{\const}{\wpath}, \wval_2 = \wbot$.
\begin{align*}
\wval'_1 = \cw{\const}{\wpath}, \wval'_2 = \cw{\const}{\wpath} && \text{by def.\ of }\wprop\\
\wstrip(\wval_1) = \const, \wstrip(\wval_2) = \wbot && \text{by def.\ of }\wstrip\\
\cval'_1 = \const, \cval'_2 = \const && \text{by def.\ of }\cprop
\end{align*}


\item $\wval_1 = \cw{\wtable}{\wpath}, \wval_2 = \wbot$.
\begin{align*}
\wval'_1 = \wval_1, \wval'_2 = \cw{\wtable_{\wbot}}{\wpath} && \text{by def.\ of }\wprop\\
\cval'_1 = \wstrip(\wval_1), \cval'_2 = \ctable_{\bot} && \text{by def.\ of }\cprop
\end{align*}

\item $\wval_1 = \cw{\const}{\wpath_1}, \wval_2 = \cw{\const}{\wpath_2}, \wpath_1 \wpord \wpath_2$.
\begin{align*}
\wval'_1 = \cw{\const}{\wpath_1}, \wval'_2 = \cw{\const}{\wpath_2} && \text{by def.\ of }\wprop\\
\wstrip(\wval_1) = \const, \wstrip(\wval_2) = \const && \text{by def.\ of }\wstrip\\
\cval'_1 = \const, \cval'_2 = \const && \text{by def.\ of }\cprop
\end{align*}


\item $\wval_1 = \werr, \wval_2 = \werr$.
\begin{align*}
\wval'_1 = \werr, \werr && \text{by def.\ of }\wprop\\
\wstrip(\wval_1) = \cerr, \wstrip(\wval_2) = \cerr && \text{by def.\ of }\wstrip\\
\cval'_1 = \cerr, \cval'_2 = \cerr && \text{by def.\ of }\cprop
\end{align*}
\end{itemize}
%
For the inductive case, let $\wval_1 = \cw{\wtable_1}{\wpath_1}$ and
$\wval_2 = \cw{\wtable_2}{\wpath_2}$ where $\wpath_1 \wpord \wpath_2$.
Let $\wpath \in \wtable_2$ for some $\wpath$. By Lemma~\ref{thm:w-strip-paths-unique},
there is no different $\wpath' \in \wtable_2$ such that  $\ptop(\wpath) = \ptop(\wpath')$.
Also, for every $\wpath' \in \wtable_1$ s.t. $\ptop(\wpath') = \ptop(\wpath)$, we 
have by Lemma~\ref{thm:w-strip-paths-unique} that $\wpath = \wpath'$. Hence,
the call site paths seen in $\wtable_1$ and $\wtable_2$ are uniquely identified by their top nodes.
The argument then follows by def.\ of $\allpaths$,
$\tpcsuniq$, and i.h.
\end{proof}
%
\begin{lemma}~\label{thm:w-join-strip-parallel}
Let $\wval_1$ and $\wval_2$ be path values such that $P = \allpaths(\wval_1) \cup \allpaths(\wval_2)$ 
where for every $\wpath_, \wpath_2 \in P$ we have $\ptop(\wpath_1) = \ptop(\wpath_2){\implies} \wpath_1=\wpath_2$. 
Further, assume that $\tpcsuniq(\wval_1)$, $\inpcons_e(\wval_1)$, $\outcons_e(\wval_1)$, $\tiocons(\wval_1)$,  
$\tpcsuniq(\wval_2)$, $\inpcons_e(\wval_2)$, $\outcons_e(\wval_2)$, and $\tiocons(\wval_2)$.
Further, assume $\wval_1 \in \m{dom}(\wstrip)$, $\wval_2 \in \m{dom}(\wstrip)$, $\wstrip(\wval_1) = \cval_1$,
and $\wstrip(\wval_2) = \cval_2$. Lastly, we assume that $\wval_1$ and $\wval_2$ agree on the paths.
Then, $\wval_1 \wvjoin \wval_2 \in \m{dom}(\wstrip)$ and $\wstrip(\wval_1 \wvjoin \wval_2) = \cval_1 \cvjoin \cval_2$.
\end{lemma}
\begin{proof}
We carry the proof by structural induction on $\wval_1$ and $\wval_2$. We first cover the base cases.
\begin{itemize}
\item $\wval_1 = \wbot$.
\begin{align*}
\wval_1 \wvjoin \wval_2 = \wval_2 && \text{by def.\ of }\wvjoin \\
\cval_1 = \bot && \text{by def.\ of }\wstrip\\
\cval_1 \cvjoin \cval_2 = \cval_2 = \wstrip(\wval_2) = \wstrip(\wval_1 \wvjoin \wval_2) && \text{by def.\ of }\cvjoin
\end{align*}

\item $\wval_2 = \wbot$. Similar to the previous case.

\item $\wval_1 = \werr$.
\begin{align*}
\wval_1 \wvjoin \wval_2 = \werr && \text{by def.\ of }\wvjoin\\
\cval_1 = \cerr && \text{by def.\ of }\cvjoin\\
\cval_1 \cvjoin \cval_2 = \cerr && \text{by def.\ of }\cvjoin\\
\wstrip(\werr) = \cerr && \text{by def.\ of }\wstrip
\end{align*}

\item $\wval_1 = \cw{\const_1}{\wpath}, \wval_2 = \cw{\const_2}{\wpath}, \const_1 \not= \const_2$.
\begin{align*}
\wval_1 \wvjoin \wval_2 = \werr && \text{by def.\ of }\wvjoin\\
\cval_1 = \const_1, \cval_2 = \const_2 && \text{by def.\ of }\wstrip \\
\cval_1 \cvjoin \cval_2 = \cerr && \text{by def.\ of }\cvjoin\\
\wstrip(\werr) = \cerr && \text{by def.\ of }\wstrip
\end{align*}

\item $\wval_1 = \cw{\const}{\wpath}, \wval_2 = \cw{\const}{\wpath}$.
\begin{align*}
\wval_1 \wvjoin \wval_2 = \cw{\const}{\wpath} && \text{by def.\ of }\wvjoin\\
\cval_1 = \const, \cval_2 = \const && \text{by def.\ of }\wstrip \\
\cval_1 \cvjoin \cval_2 = \const && \text{by def.\ of }\cvjoin\\
\wstrip(\cw{\const}{\wpath}) = \const && \text{by def.\ of }\wstrip
\end{align*}

\item $\wval_1 = \cw{\const}{\wpath}, \wval_2 = \cw{\wtable}{\wpath}$.
\begin{align*}
\wval_1 \wvjoin \wval_2 = \werr && \text{by def.\ of }\wvjoin\\
\cval_1 = \const, \cval_2 \in \ctables && \text{by def.\ of }\wstrip \\
\cval_1 \cvjoin \cval_2 = \cerr && \text{by def.\ of }\cvjoin\\
\wstrip(\werr) = \cerr && \text{by def.\ of }\wstrip
\end{align*}

\item \textit{Other}. Similar for the other cases.
\end{itemize}


For the inductive case, let $\wval_1 = \cw{\wtable_1}{\wpath_1}$ and
$\wval_2 = \cw{\wtable_2}{\wpath_2}$ where $\wpath_1 \wpord \wpath_2$.
Let $\wpath \in \wtable_2$ for some $\wpath$. By Lemma~\ref{thm:w-strip-paths-unique},
there is no different $\wpath' \in \wtable_2$ such that  $\ptop(\wpath) = \ptop(\wpath')$.
Also, for every $\wpath' \in \wtable_1$ s.t. $\ptop(\wpath') = \ptop(\wpath)$, we 
have by Lemma~\ref{thm:w-strip-paths-unique} that $\wpath = \wpath'$. Hence,
the call site paths seen in $\wtable_1$ and $\wtable_2$ are uniquely identified by their top nodes.
\begin{itemize}
\item $\wpath \in \wtable_1, \wpath \in \wtable_2$. Let $\wtable_1(\wpath) = \pair{\wval_{1i}}{\wval_{1o}}$
           and $\wtable_2(\wpath) = \pair{\wval_{2i}}{\wval_{2o}}$. If $\wval_{1i}, \wval_{2i} \not\in \{\wbot, \werr\}$,
	   then $\ppath(\wval_{2i}) = \ppath(\wval_{1i})$ by $\ppath(\wval_{2i}), \ppath(\wval_{1i}) \in P$ (by def.\ of $\allpaths$),
	   Lemma~\ref{thm:w-strip-paths-unique}, and $\ptop(\ppath(\wval_{2i})) = \ptop(\ppath(\wval_{1i}))$ which
	   follows by the def.\ of $\inpcons$. The same property holds for the outputs by the same reasoning and def.\ of $\outcons$. 
	   The argument then follows from the i.h.

\item $\wpath \in \wtable_1, \wpath \not\in \wtable_2$. By $\tiocons(\wtable_2)$, we then have that
           $\wtable_2(\wpath) = \pair{\wbot}{\wbot}$. The argument then follows trivially since $\wstrip(\wval_2)(\ptop(\wpath)) = \cw{\bot}{\bot}$.

\item \textit{Other cases}. Handled similarly.

\end{itemize}
\end{proof}

We can now establish a result connecting the path based data flow semantics and plain data flow semantics.
For that purpose, we first state an almost obvious result.
\begin{lemma}~\label{thm:w-cons-strip}
Let $\wmap$ be a consistent map $\wcons_e(\wmap)$ subject to a program $e$. Then, $\wmap \in \m{dom}(\wstrip)$.
\end{lemma}
\begin{proof}
The result follows from Lemma~\ref{thm:w-cons-top-unique}.
\end{proof}
%
We can now state our main theorem.
%
\begin{theorem}~\label{thm:path-to-data-flow}
Let $e^\ell$ be an expression of a program $m$, $\wmap$ a consistent map $\wcons_m(\wmap)$, $\cenv$ an environment
where $\domvalid(\ell, m, \cenv)$, $\envcons_{\wmap}(\cenv)$, and $(e, \cenv)$ is well-formed. Further, let $\cmap$ be 
a concrete map such that $\cmap = \wstrip(\wmap)$. If $\wtrans[\fuel]{e^\ell}(\cenv)(\wmap) = \wmap_f$ 
and $\ctrans[\fuel]{e^\ell}(\cenv)(\cmap) = \cmap_f$, 
for some maps $\wmap_f$ and $\cmap_f$, then $\wmap_f \in \m{dom}(\wstrip)$ and $\wstrip(\wmap_f) = \cmap_f$.
\end{theorem}
\begin{proof}
The proof goes by structural induction on $e$. 
Otherwise, the proof branches on $e$.
\begin{itemize}
\item $e = \const$. Let $\wval = \wmap(\cn{\cenv}{\ell})$, $\wval_f = \wmap_f(\cn{\cenv}{\ell})$, 
                    $\cval = \cmap(\cn{\cenv}{\ell})$, and $\cval_f = \cmap_f(\cn{\cenv}{\ell})$.
                    By $\wcons_m(\wmap)$, $\wval \in \{\wbot, \werr, \cw{\const}{\cn{\cenv}{\ell}}\}$.
                    If $\wval = \wbot$, then $\wval_f = \cw{\const}{\cn{\cenv}{\ell}}$, $\cval = \bot$,
                    $\cval_f = \const$, and the result follows from the definition of $\wstrip$.
                    If $\wval = \cw{\const}{\cn{\cenv}{\ell}}$, then $\wval_f = \wval$ and $\cval_f = \cval$,
                    from which the result follows immediately. Lastly, if $\wval = \werr$, then by
                    $\errcons(\wmap)$ (implied by $\wcons_e(\wmap)$) we have $\wmap = \wmap_{\werr}$
                    and hence $\wmap_f = \wmap_{\werr}$, $\cmap = \cmap_{\cerr}$, as well as $\cmap_f = \cmap_{\cerr}$.
                    The result then follows simply from the definition of $\wstrip$. 

\item $e = x$. Let $\wval_x = \wmap(\cenv(x))$, $\wval = \wmap(\cn{\cenv}{\ell})$, $\cval_x = \cmap(\cenv(x))$, and 
               $\cval = \cmap(\cn{\cenv}{\ell})$. By $\cmsub_m(\wmap)$ (implied by $\wcons_m(\wmap)$) and Lemma~\ref{thm:w-cons-agree},
               we have $\wval_x \;\wsub\;\wval$. Further, by $\wcons_m(\wmap)$, we have $\tpcsuniq(\wval_1)$,
               $\tpcsuniq(\wval_2)$, and that all paths in $\allpaths(\wval_1) \cup \allpaths(\wval_2)$ are deterministic
               and root consistent. The result then follows from Lemma~\ref{thm:w-prop-strip-parallel}.

\item $e = e_1^{\ell_1} e_2^{\ell_2}$. Clearly, we have $\domvalid(\ell_1, m, \cenv)$ and so by i.h.\ $\wmap_1 \in \m{dom}(\wstrip)$
               and $\cmap_1 = \wstrip(\wmap_1)$. By Theorem~\ref{thm:w-cons-inductive} it is the case that $\envcons_{\wmap_1}(\cenv)$
               and $\wcons_m(\wmap_1)$. As $\domvalid(\ell_2, m, \cenv)$ trivially, we have by i.h. that $\wmap_2 \in \m{dom}(\wstrip)$
               and $\cmap_2 = \wstrip(\wmap_2)$. Also, again by Theorem~\ref{thm:w-cons-inductive} we have $\envcons_{\wmap_2}(\cenv)$
               and $\wcons_m(\wmap_2)$.

               By Lemmas~\ref{thm:w-framer} and~\ref{thm:w-disjointr-1}, we have $\wval_1 = \wmap_2(\cn{\cenv}{\ell_1})$ and so by 
               $\cmsub_m(\wmap_2)$ (implied by $\wcons_m(\wmap_2)$) it must be 
               $\wval_1 \;\wsub\; \wval'$ where $\wval' = \cw{[\ppath(\wval_1) \mapsto \pair{\wval_2}{\wmap_2(\cn{\cenv}{\ell_2})}]}{\ppath(\wval_1)}$. 
               Note that by the def.\ of $\wstrip$ and $\cmap_2 = \wstrip(\wmap_2)$, we have 
               $\wstrip(\wval') = [\ptop(\ppath(\wval_1)) \mapsto \pair{\cval_2}{\cmap_2(\cn{\cenv}{\ell_2})}]$. Further, by $\wcons_m(\wmap)$, 
               we have $\tpcsuniq(\wval_1)$, $\tpcsuniq(\wval')$, and that all paths in $\allpaths(\wval_1) \cup \allpaths(\wval')$ are deterministic
               and root consistent. The result then follows from Lemma~\ref{thm:w-prop-strip-parallel}.


\item $e = \mu f. \lambda x. e_1^{\ell_1}$. Let $\wval = \wmap(\cn{\cenv}{\ell})$ and $\cval = \cmap(\cn{\cenv}{\ell})$.
               By $\wcons_m(\wmap)$, $\wval \in \{\wbot, \werr, \cw{\wtable}{\cn{\cenv}{\ell}}\}$ for some $\wtable \in \wtables$. 
               If $\wval = \wbot$, then $T_w = \cw{\wtable_{wbot}}{\cn{\cenv}{\ell}}$, $\cval = \bot$, $\ctable = \ctable_\bot$.
               In that case, $\wmap_f = \wmap[\cn{\cenv}{\ell} \mapsto T_w]$, $\cmap_f = \cmap[\cn{\cenv}{\ell} \mapsto \ctable]$, 
               the result follows from the definition of $\wstrip$. If $\wval = \werr$, then by $\errcons(\wmap)$ (implied by 
               $\wcons_e(\wmap)$) we have $\wmap = \wmap_{\werr}$ and hence $\wmap_f = \wmap_{\werr}$ by Lemma~\ref{thm:w-step-increasing-monotone}, 
               $\cmap = \cmap_{\cerr}$ and thus $\cmap_f = \cmap_{\cerr}$ by Lemma~\ref{thm:c-step-increase}.
               The result then follows simply from the definition of $\wstrip$. Lastly, if $\wval = \cw{\wtable}{\cn{\cenv}{\ell}}$, 
               then $T_w = \wval$ and $\ctable = \cval$. The argument then goes as follows.

               By Lemma~\ref{thm:w-cons-top-unique} and def.\ of $\wstrip$, we have $\setc{\ccsite}{\ccsite \in \ctable} = \setc{\ptop(\wpath)}{\wpath \in \wtable}$.
               That is, for every $\wpath \in \wtable$ there is a unique $\ccsite \in \ctable$ such that $\ptop(\wpath) = \ccsite$, and vice versa.
               Then, by $\cmsub_m(\wmap)$ (implied by $\wcons_m(\wmap)$) it is that $\cw{[\wpath \mapsto \pair{\wmap(\cnode_x)}{\wmap(\cn{\cenv_1}{\ell_1})}]}{\wpath} \wsub T_w$.
               Similarly, by $\cmsub_m(\wmap)$ and Lemma~\ref{thm:w-cons-agree} we have $T_w \;\wsub\; \wmap(\cnode_f)$. Also, by 
               $\wcons_m(\wmap)$ we have $\tpcsuniq(\wmap(\cnode_x))$, $\tpcsuniq(\wmap(\cn{\cenv_1}{\ell_1}))$, $\tpcsuniq(T_w)$, $\tpcsuniq(\wmap(\cnode_f))$,
               and all paths in $\allpaths(\wmap(\cnode_x)) \cup \allpaths(\wmap(\cnode_f)) \cup \allpaths(T_w) \cup \allpaths \wmap(\cn{\cenv_1}{\ell_1})$ are
               deterministic and root consistent. Then by Lemma~\ref{thm:w-prop-strip-parallel} and Lemma~\ref{thm:w-join-strip-parallel} we have
               $\wmap_1 \in \m{dom}(\wstrip)$ and $\wstrip(\wmap_1) = \cmap_1$. By Lemmas~\ref{thm:w-prop-increasing-monotone} and~\ref{thm:w-prop-sub-noerr}
               as well as $\envcons_{\wmap}(\cenv)$ we have $\envcons_{\wmap_1}(\cenv_1)$. Also, $\domvalid(\ell_1, m, \cenv_1)$ holds by the definition of $\cenv_1$
               and $\domvalid(\ell, m, \cenv)$. Then by the i.h., $\wtrans[k]{e_1}(\cenv_1)(\wmap_1) \in \m{dom}(\wstrip)$ and 
               $\wstrip(\wtrans[k]{e_1}(\cenv_1)(\wmap_1)) = \ctrans[k]{e_1}(\cenv_1)(\cmap_1)$.

               Finally, observe that for each two different $\wmap_1, \wmap_2 \in \vec{\wmap}$, $\wmap_1$ and $\wmap_2$ agree on all nodes except
               possibly those in $\m{rng}(\cenv)$ by Lemma~\ref{thm:w-disjointr-2}. By $\envcons_{\wmap}(\cenv)$, for every node $\cnode$ in $\m{rng}(\cenv)$
               we have $\wmap(\cnode) \not\in \{\wbot, \werr\}$. Then by Lemma~\ref{thm:w-step-path-stable} we have $\ppath(\wmap(\cnode)) = \ppath(\wmap_1(\cnode))$,
               $\ppath(\wmap(\cnode)) = \ppath(\wmap_2(\cnode))$, for every node $\cnode$ in $\m{rng}(\cenv)$, which clearly implies $\ppath(\wmap_2(\cnode)) = \ppath(\wmap_1(\cnode))$.
               The result then follows from $\cfin(\wmap)$, which implies $|\setc{\ptop(\wpath)}{\wpath \in \wtable}|$ is finite, and Lemma~\ref{thm:w-join-strip-parallel}.

%\item $e = \ifte{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}}$. Similar to the earlier cases. 
\end{itemize}
\end{proof}

We additionally show that consistency of a path map implies that its stripped plain data flow map
has the data flow invariant property.
\begin{lemma}~\label{thm:w-cons-dataflow-inv}
Let $\wmap$ be consistent map $\wcons_e(\wmap)$ subject to a program $e$. Then, $\dfinv(\wstrip(\wmap))$.
\end{lemma}
\begin{proof}
First, observe that by Lemma~\ref{thm:w-cons-strip} we have $\wmap \in \m{dom}(\wstrip)$. Next,
let $\cmap = \wstrip(\wmap)$. Then, $\errcons(\cmap)$ follows by $\errcons(\wmap)$ (implied by $\wcons_e(\wmap)$)
and the definition of $\wstrip$. The same argument can be given to show $\cfin(\cmap)$, $\tiocons(\cmap)$, $\constcons_e(\cmap)$,
and $\envcons(\cmap)$. Finally, $\cmsub_e(\cmap)$ follows from $\cmsub_e(\wmap)$, $\rootcons_e(\wmap)$, $\tpcons(\wmap)$, and $\wdet_e(\wmap)$.
To see this in more detail, first observe that the set of reachable (non-$\bot$) nodes of $\wmap$ and $\cmap$ is the same by the def.\ of $\wstrip$.
For every reachable node $\cnode$ that corresponds to a non-leaf expression of $e$, we have that $\wmap(\cnode) = \cw{\_}{\wpath}$ for some
path $\wpath$. By $\tpcons(\wmap)$, $\ptop(\wpath) = \cnode$ and by $\rootcons_e(\wmap)$ as well as Lemma~\ref{thm:w-pred-nopred} we have 
that $|\wpath| > 1$. Then, for the predecessor $\cnode'$ of $\cnode$ in $\wpath$, we have that $\wmap(\cnode') \;\wsub\; \wmap(\cnode)$ 
by $\cmsub_e(\wmap)$ and $\wpred^e_{\wmap}(\cnode', \cnode)$ by $\wdet_e(\wmap)$. The result then follows from the definition of
$\wpred$, Lemma~\ref{thm:w-strip-sub}, and the fact that $\wcons_e(\wmap)$ implies $\tpcsuniq(\wmap(\cnode')) \wedge \tpcsuniq(\wmap(\cnode))$. 
\end{proof}





 


==> proofs/r-semantics-soundness.tex <==
\subsubsection{Soundness}

We first provide several useful results used to argue soundness of relational semantics.


\begin{lemma}~\label{thm:r-choose-dep-f}
Let $\cmap \in \cmaps$, $\cval \in \cvalues$, $\cnode \in \cnodes$, and $\rval \in \rvalues$.
Suppose $\pair{\cmap}{\cval} \in \rgamma(\rval)$ and $\cmap(\cnode) \in \ctables$.
Then, for any $\ctable \in \ctables$, $\pair{\cmap[\cnode \mapsto \ctable]}{\cval} \in \rgamma(\rval)$.
\end{lemma}
\begin{proof}
When $\cnode \not\in \rscope$, the argument follows by Lemma~\ref{thm:r-gamma-out-of-scope}.
If $\rval \in \{\rbot, \rerr\}$, the argument is trivial. For other cases, the result follows
by the definition of $\rgamma$, specifically $\dgamma$ ($\dgamma(\rdf) = \ctables$).
\end{proof}

\begin{lemma}~\label{thm:r-v-meaning-up}
Let $\cmap \in \cmaps$, $\cmap' \in \cmaps$, $\cval \in \cvalues$, and $\rval \in \rvalues$.
Suppose $\cmap \cmord \cmap'$, $\pair{\cmap}{\cval} \in \rgamma(\rval)$, and 
$\forall \cnode \in \rscope.\,\cmap(\cnode) \not= \cerr \implies \cmap'(\cnode) \not = \cerr$.
Then $\pair{\cmap'}{\cval} \in \rgamma(\rval)$.
\end{lemma}
\begin{proof}
The argument goes by structural induction on $\rval$. By Lemma~\ref{thm:r-gamma-out-of-scope},
the proof analysis can focus only on the nodes $\rscope$ of $\cmap'$. The cases when
$\rval \in \{\rbot, \rerr\}$ are trivial. The other cases follow by the definition of $\rgamma[]$. 
For instance, suppose $\cnode \in \rscope$ and $\cmap(\cnode) = \const$.
Then, $\cmap'(\cnode) = \const$. Otherwise, suppose $\cmap(\cnode) \in \ctables$. 
The argument then follows from Lemma~\ref{thm:r-choose-dep-f}.
\end{proof}


\paragraph{Data Propagation}

\newcommand{\scopecons}{\m{scopecons}}

We start proving the soundness of the relational semantics by formalizing and showing that
relational propagation abstracts the concrete one.
We begin by introducing the notion of scope consistency that closely resembles the environment
consistency.
%
\[\scopecons_\rscope(\cmap) \Def\iff \forall \cnode \in \rscope.\,\cmap(\cnode) \not\in \{\bot, \cerr\}\]
%
\begin{lemma}~\label{thm:r-prop-sound}
Let $\cval_1$, $\cval_2$, $\cval_3$, and $\cval_4$ be values, $\cmap_1$ and $\cmap_2$ maps, 
$\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, $\rval_3 \in \rvalues$, and $\rval_4 \in \rvalues$. 
Let $\cval_1 \csub \cval_2$, $\noerr(\cval_1)$, $\noerr(\cval_2)$, 
$\pair{\cmap_1}{\cval_1} \in \rgamma(\rval_1)$, $\pair{\cmap_2}{\cval_2} \in \rgamma(\rval_2)$, 
$\cmap_1 \cmord \cmap_2$, 
$\scopecons_\rscope(\cmap_1)$, and $\scopecons_\rscope(\cmap_2)$. 
%be equal to $\cmap_2$ for all nodes except those in $\rscope$ where $\cmap_1(\cnode) \cvord \cmap_2(\cnode)$
If $\pair{\cval_3}{\cval_4} = \cprop(\cval_1, \cval_2)$ and $\pair{\rval_3}{\rval_4} = \rprop(\rval_1, \rval_2)$, 
then $\pair{\cmap_1}{\cval_3} \in \rgamma(\rval_3)$ and $\pair{\cmap_2}{\cval_4} \in \rgamma(\rval_4)$.
\end{lemma}
\begin{proof}
By structural induction on both $\cval_1$ and $\cval_2$.
\begin{itemize}
   \item $\cval_1 = \bot, \cval_2 = \bot$.
%
\begin{align*}
\cval_3 = \bot, \cval_4 = \bot && \text{by def. of $\cprop$}\\
\forall \rval.\,\cmaps \times \{\bot\} \in \rgamma(\rval) && \text{by def. of $\rgamma$}
\end{align*}
%
   \item $\cval_1 = \const, \cval_2 = \bot$.
%
\begin{align*}
\cval_3 = \const, \cval_4 = \const && \text{by def. of $\cprop$}\\
\pair{\cmap_2}{\cval_4} \in \rgamma(\rval_1) && \text{by $\scopecons_{\cmap_2}(\rscope)$ and Lemma~\ref{thm:r-v-meaning-up}}\\
\rval_1 \in \rels \cup \{\rerr\} && \text{by def. of $\rgamma$}\\
\rval_3 = \rval_1, \rval_1 \rvord \rval_4 && \text{by def. of $\rprop$}
\end{align*}
%
   \item $\cval_1 = \ctable, \cval_2 = \bot$, $\rval_2 \not \in \rtables$.
%
\begin{align*}
\cval_3 = \cval_1, \cval_4 = \ctable_\bot && \text{by def. of $\cprop$}\\
\rval_1 \in \rtables \cup \{\rerr\} && \text{by def. of $\rgamma$}\\
\rval_3 = \rval_1 \vee \rval_3 = \rerr, \rval_4 = \rtable_{\rbot} \vee \rval_4 = \rerr && \text{by def. of $\rprop$}\\
\pair{\cmap_2}{\ctable_\bot} \in \rgamma(\rval_4) && \text{by def. of $\rgamma$}
\end{align*}
%
   \item $\cval_1 = \ctable, \cval_2 = \bot$, $\rval_2 \in \rtables$.
%
\begin{align*}
\cval_3 = \cval_1, \cval_4 = \ctable_\bot && \text{by def. of $\cprop$}\\
\rval_1 \in \rtables \cup \{\rerr\} && \text{by def. of $\rgamma$}\\
\rval_3 = \rval_1 \vee \rval_3 = \rerr, \rval_2 \rvord \rval_4 && \text{by def. of $\rprop$ and Lemma~\ref{thm:r-prop-increasing-monotone}}\\
\rgamma(\rtable_{\rbot}) \subseteq \rgamma(\rval_4) && \text{by def. of $\rgamma$}\\
\pair{\cmap_2}{\ctable_\bot} \in \rgamma(\rtable_{\rbot}) && \text{by def. of $\rgamma$} \\
\pair{\cmap_2}{\ctable_\bot} \in \rgamma(\rval_4) && 
\end{align*}

   \item $\cval_1 = \const, \cval_2 = \const$.
%
\begin{align*}
\cval_3 = \const, \cval_4 = \const && \text{by def. of $\cprop$}\\
\rval_1 \rvord \rval_3, \rval_2 \rvord \rval_4 && \text{by def. of $\rprop$ and Lemma~\ref{thm:r-prop-increasing-monotone}}
\end{align*}
%
%   \item $\cval_1 = \cerr, \cval_2 = \cerr$.
%
%\begin{align*}
%\rval_1 = \rerr, \rval_2 = \rerr && \text{by def. of $\rgamma$}\\
%\rval_3 = \rerr, \rval_4 = \rerr && \text{by def. of $\rprop$}
%\end{align*}
\end{itemize}

For the induction case, let $\cval_1 = \ctable_1$ and $\cval_2 = \ctable_2$.
By definition of $\rgamma$, it must be that $\rval_1 \in \rtables \cup \{\rerr\}$ 
and $\rval_2 \in \rtables \cup \{\rerr\}$. If $\rval_1 = \rerr$ or $\rval_2 = \rerr$, 
the argument is trivial as $\rval_3 = \rval_4 = \rerr$ by the def.\ of $\rprop$. 
We thus focus on the case
when $\rval_1 = \rtable_1$ and $\rval_2 = \rtable_2$. First, observe that
$\ccsite \in \ctable_2 \implies \ccsite \in \rtable_2$ by the def. of $\rgamma$.
If $\ccsite \in \rtable_2$ but $\ccsite \not \in \ctable_2$, the argument follows
from Lemma~\ref{thm:r-prop-increasing-monotone}.

We are left with the case where $\ccsite \in \rtable_2$ and $\ccsite \in \ctable_2$.
Let $\pair{\cval_{1i}}{\cval_{1o}} = \ctable_1(\ccsite)$, 
$\pair{\cval_{2i}}{\cval_{2o}} = \ctable_1(\ccsite)$, 
$\pair{\rval_{1i}}{\rval_{1o}} = \rtable_1(\ccsite)$, and
$\pair{\rval_{2i}}{\rval_{2o}} = \rtable_2(\ccsite)$. 
By definition of $\csub$, we have that $\cval_{2i} \csub \cval_{1i}$ and $\cval_{1o} \csub \cval_{2o}$.


Suppose first that
$\pair{\cval'_{2i}}{\cval'_{1i}} = \cprop(\cval_{2i}, \cval_{1i})$ and 
%$\pair{\cval'_{1o}}{\cval'_{2o}} = \cprop(\cval_{1o}, \cval_{2o})$, 
$\pair{\rval'_{2i}}{\rval'_{1i}} = \rprop(\rval_{2i}, \rval_{1i})$.
%$\pair{\rval'_{1o}}{\rval'_{2o}} = \rprop(\rval_{1o}, \rval_{2o})$.
We have $\noerr(\cval_{1i})$, $\noerr(\cval_{2i})$, $\noerr(\cval_{1o})$,
$\noerr(\cval_{2o})$ by the definition of $\noerr$. Also, it trivially follows
that $\scopecons_{\cmap_1}(\rscope\setminus\{\ccsite\})$ and 
$\scopecons_{\cmap_2}(\rscope\setminus\{\ccsite\})$.
By definition of $\rgamma[]$, the fact that $\ccsite$ is not in the scope of
$\cval_{2i}$, $\cval_{1i}$, $\rval_{2i}$, $\rval_{1i}$, and Lemma~\ref{thm:r-gamma-out-of-scope},
we have $\pair{\cmap_1}{\cval_{1i}} \in \rgamma[\rscope\setminus\{\ccsite\}](\rval_{1i})$
and $\pair{\cmap_2}{\cval_{2i}} \in \rgamma[\rscope\setminus\{\ccsite\}](\rval_{2i})$.
It then follows from induction hypothesis that $\pair{\cmap_1}{\cval'_{1i}} \in \
\rgamma[\rscope\setminus\{\ccsite\}](\rval'_{1i})$ and 
$\pair{\cmap_2}{\cval'_{2i}} \in \rgamma[\rscope\setminus\{\ccsite\}](\rval'_{2i})$.


Next, $\pair{\cmap_1[\ccsite \mapsto \cval_{1i}]}{\cval_{1o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval_{1o})$ and
$\pair{\cmap_2[\ccsite \mapsto \cval_{2i}]}{\cval_{2o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval_{2o})$. 
Since $\ccsite \in \cval_2$, we know $\cval_{2i} \not= \bot$. Also, we know by $\noerr(\cval_{2i})$
that $\cval_{2i} \not= \cerr$. Hence, if $\cval_{2i} = \const$, then by $\cval_{2i} \csub \cval_{1i}$
we have that $\cval_{1i} = \const$. Further, if $\cval_{2i} \in \ctables$, then 
$\pair{\cmap_1[\ccsite \mapsto \cval_{2i}]}{\cval_{1o}}$ by Lemma~\ref{thm:r-choose-dep-f}. 
It also holds that 
$\pair{\cmap_1[\ccsite \mapsto \cval_{2i}]}{\cval_{1o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval_{1o})$ and
$\pair{\cmap_2[\ccsite \mapsto \cval_{2i}]}{\cval_{2o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval_{2o})$. By definition of strengthening, one then also has
$\pair{\cmap_1[\ccsite \mapsto \cval_{2i}]}{\cval_{1o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rupdate{\rval_{1o}}{\ccsite}{\rval_{2i}})$ and
$\pair{\cmap_2[\ccsite \mapsto \cval_{2i}]}{\cval_{2o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rupdate{\rval_{2o}}{\ccsite}{\rval_{2i}})$.  

Let $\pair{\cval'_{1o}}{\cval'_{2o}} = \cprop(\cval_{1o}, \cval_{2o})$ and
$\pair{\rval'_{1o}}{\rval'_{2o}} = \rprop(\rupdate{\rval_{1o}}{\ccsite}{\rval_{2i}}, \rupdate{\rval_{2o}}{\ccsite}{\rval_{2i}})$. 
As $\cmap_1[\ccsite \mapsto \cval_{2i}] \rmord \cmap_2[\ccsite \mapsto \cval_{2i}]$,
$\scopecons_{\cmap_1[\ccsite \mapsto \cval_{2i}]}(\rscope\cup\{\ccsite\})$, and
$\scopecons_{\cmap_2[\ccsite \mapsto \cval_{2i}]}(\rscope\cup\{\ccsite\})$,
we have by induction hypothesis that 
$\pair{\cmap_1[\ccsite \mapsto \cval_{2i}]}{\cval'_{1o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval'_{1o})$ and
$\pair{\cmap_2[\ccsite \mapsto \cval_{2i}]}{\cval'_{2o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval'_{2o})$. 

By Lemma~\ref{thm:c-prop-sub} and Lemma~\ref{thm:c-prop-sub-no-err-bot}, we have 
$\cval'_{2i} \csub \cval'_{1i}$ and, if $\cval_{2i} = \const$, 
$\cval_{2i} = \cval'_{2i} = \cval_{1i} = \cval'_{1i} = \const$. In that case,
$\pair{\cmap_1[\ccsite \mapsto \cval'_{1i}]}{\cval'_{1o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval'_{1o})$ and
$\pair{\cmap_1[\ccsite \mapsto \cval'_{2i}]}{\cval'_{2o}} \in \rgamma[\rscope\cup\{\ccsite\}](\rval'_{2o})$.
In the case $\cval'_{2i} \in \ctables$, then also $\cval'_{1i} \in \ctables$ and the same result
follows by Lemma~\ref{thm:r-choose-dep-f}.
\end{proof}






\paragraph{Joins}

We next show several results showing the soundness of the relational join subject to to the
concrete one.
%
\begin{lemma}~\label{thm:r-join-sound}
Let $\cval_1$, $\cval_2$, be values, $\cmap$ a concrete map, $\rval_1 \in \rvalues$, and 
$\rval_2 \in \rvalues$. 
If $\noerr(\cval_1)$, $\noerr(\cval_2)$, $\constcomp(\cval_1, \cval_2)$, $\pair{\cmap}{\cval_1} \in \rgamma(\rval_1)$, $\pair{\cmap}{\cval_2} \in \rgamma(\rval_2)$, 
then $\pair{\cmap}{\cval_1 \cvjoin \cval_2} \in \rgamma(\rval_1 \rvjoin \rval_2)$.
\end{lemma}
\begin{proof}
By structural induction on both $\cval_1$ and $\cval_2$. Let $\cval = \cval_1 \cvjoin \cval_2$
and $\rval = \rval_1 \rvjoin \rval_2$.
\begin{itemize}
   \item $\cval_1 = \bot$ or $\cval_1 = \bot$. Trivial, as $\cval = \const$ and the argument then
follows by monotonicity of $\rgamma$.
%
%   \item $\cval_1 = \cerr$ or $\cval_2 = \cerr$. Also straightforward as $\rval_1 = \rerr$ or
%$\rval_2 = \rerr$, and hence $\rval = \rerr$. The result then follows from the def.\ of $\rgamma$.
%
   \item $\cval_1 = \const, \cval_2 = \const$. Again, by monotonicity of $\rgamma$.
\end{itemize}


For the induction case, let $\cval_1 = \ctable_1$ and $\cval_2 = \ctable_2$.
By definition of $\rgamma$, it must be that $\rval_1 \in \rtables \cup \{\rerr\}$ 
and $\rval_2 \in \rtables \cup \{\rerr\}$. If $\rval_1 = \rerr$ or $\rval_2 = \rerr$, 
the argument is trivial as $\rval_3 = \rerr$ by the def.\ of $\rvjoin$. 
We thus focus on the case
when $\rval_1 = \rtable_1$ and $\rval_2 = \rtable_2$. Consider any call site $\ccsite$.
Let $\pair{\cval_{1i}}{\cval_{1o}} = \ctable_1(\ccsite)$, 
$\pair{\cval_{2i}}{\cval_{2o}} = \ctable_1(\ccsite)$, 
$\pair{\rval_{1i}}{\rval_{1o}} = \rtable_1(\ccsite)$, and
$\pair{\rval_{2i}}{\rval_{2o}} = \rtable_2(\ccsite)$. 
Let us first consider the case for inputs. We have $\pair{\cmap}{\cval_{1i}} \in \rgamma(\rval_{1i})$,
$\pair{\cmap}{\cval_{2i}} \in \rgamma(\rval_{2i})$, $\noerr(\cval_{2i})$, $\noerr(\cval_{1i})$,
and $\constcomp(\cval_{1i}, \cval_{2i})$. By i.h., we then have 
$\pair{\cmap}{\cval_{1i} \cvjoin \cval_{2i}} \in \rgamma[](\rval_{1i} \rvjoin \rval_{2i})$.

Next, we have that $\pair{\cmap[\ccsite \mapsto \cval_{1i}]}{\cval_{1o}} \in \rgamma(\rval_{1o})$,
$\pair{\cmap[\ccsite \mapsto \cval_{2i}]}{\cval_{2o}} \in \rgamma(\rval_{2o})$, 
$\noerr(\cval_{2o})$, $\noerr(\cval_{1o})$, and
$\constcomp(\cval_{1o}, \cval_{2o})$. Now, if $\cval_{1i} = \bot$, 
then $\cval_{1o} = \bot$ by the def.\ of $\rgamma[]$ and $\noerr(\cval_{1o})$. Hence, 
$\pair{\cmap[\ccsite \mapsto \cval_{2i}]}{\cval_{1o}} \in \rgamma(\rval_{1o})$ as well
again by the definition of $\rgamma$. 
The same holds in the other direction.
For the remaining cases, if $\cval_{1i} = \const$
then by $\constcomp(\cval_{1i}, \cval_{2i})$ we have $\cval_{1i} = \cval_{2i}$, hence clearly
$\pair{\cmap[\ccsite \mapsto \cval_{2i}]}{\cval_{1o}} \in \rgamma(\rval_{1o})$.
Lastly, if $\cval_{1i} \in \ctables$
then by $\constcomp(\cval_{1i}, \cval_{2i})$ we have $\cval_{2i} \in \ctables$, 
and by Lemma~\ref{thm:r-choose-dep-f}
$\pair{\cmap[\ccsite \mapsto \cval_{2i}]}{\cval_{1o}} \in \rgamma(\rval_{1o})$.
By the induction hypothesis, we then have 
$\pair{\cmap[\ccsite \mapsto \cval_{2i}]}{\cval_{2o} \cvjoin \cval_{1o}} \in
\rgamma(\rval_{1o} \rvjoin \rval_{2o})$. Again, if $\cval_{2i} \in \ctables$
then by $\constcomp(\cval_{1i}, \cval_{2i})$ and Lemma~\ref{thm:r-choose-dep-f}
$\pair{\cmap[\ccsite \mapsto \cval_{2i} \cvjoin \cval_{1i}]}{\cval_{2o} \cvjoin \cval_{1o}} \in \rgamma(\rval_{1o} \rvjoin \rval_{2o})$. Similar reasoning applies for the cases when
$\cval_{2i} \in \{\bot\} \cup \consts$.
\end{proof}

\begin{lemma}~\label{thm:r-K-join-sound}
Let $K \geq 2$, $\cval_1$ to $\cval_K$ be values where $\constcomp(\{\cval_1, \dots, \cval_K\})$
and $\forall 1 \leq i \leq K.\,\noerr(\cval_i)$, $\rval_1$ to $\rval_K$ relational values in
$\rvalues$, and $\forall 1 \leq i \leq K.\, \pair{\cmap}{\cval_i} \in \rgamma(\rval_i)$.
Then, $\pair{\cmap}{\cvjoin_{1\leq i \leq K} \cval_i} \in \rgamma(\rvjoin_{1\leq i \leq K}\rval_i)$.
\end{lemma}
\begin{proof}
The argument goes by induction on $K$. The result follows from the 
Lemma~\ref{thm:r-join-sound} and the fact that join $\cvjoin$
does not invalidate the constant compatibility of values.
\end{proof}

\begin{lemma}~\label{thm:r-K-map-join-sound}
Let $K \geq 2$, $\hat{M} = \{\cmap_1, \dots, \cmap_K\}$ be a set of concrete maps where 
$\constcomp(\hat{M})$ and $\forall \cmap \in \hat{M}.\,\errcons(\cmap)$, 
$\hat{M_r} = \{\rmap_1, \dots, \rmap_K\}$ a set of relational maps, and 
$\forall 1 \leq i \leq K.\, \cmap_i \in \rmgamma(\rmap_i)$.
Then, $\cmjoin \hat{M} \in \rmgamma(\rmjoin \hat{M_r})$.
\end{lemma}
\begin{proof}
First, let
\[ \cmap_u  = \cmjoin \hat{M} = \Lambda \cnode. \cvjoin \setc{\cmap(\cnode)}{\cmap \in \hat{M}} \]
and
\[ \rmap_u  = \rmjoin \hat{M} = \Lambda \cnode. \rvjoin \setc{\rmap(\cnode)}{\rmap \in \hat{M_r}} \]
%

First, suppose there exists a map $\cmap_i \in \hat{M}$ s.t.\ exists a node $\cnode$ where
it is not the case that $\noerr(\cmap_i(\cnode))$. By $\errcons(\cmap_i)$, it must be that
$\cmap_i = \cmap_\cerr$, in which case $\cmap_u = \cmap_\cerr$. Also, it then must be that
$\rmap_i = \rmap_{\rerr}$ and clearly $\rmap_u = \rmap_{\rerr}$. The result then trivially follows
by the definition of $\rmgamma$.

Otherwise, we have the following. As a reminder, by the definition of $\rmgamma$ one has 
that $\cmap \in \rmgamma(\rmap)$ implies that 
$\forall \cnode. \pair{\cmap}{\cmap(\cnode)} \in \rgamma[](\rmap(\cnode))$. 
Also, by Lemma~\ref{thm:const-comp-errcons} and $\cmap_u \not= \cmap_\cerr$, 
we have $\errcons(\cmap_u)$. Hence,
%
\begin{align*}
\forall 1 \leq i \leq K.\, \forall \cnode. \pair{\cmap_i}{\cmap_i(\cnode)} \in \rgamma[](\rmap_i(\cnode)) && \text{by def. of $\rmgamma$}\\
\forall 1 \leq i \leq K.\, \forall \cnode. \pair{\cmap_u}{\cmap_i(\cnode)} \in \rgamma[](\rmap_i(\cnode)) && \text{by Lemma~\ref{thm:r-v-meaning-up}}\\
\forall \cnode. \pair{\cmap_u}{\cvjoin \setc{\cmap_i(\cnode)}{\cmap_i \in \hat{M}}} \in \rgamma[](\rvjoin \setc{\rmap_i(\cnode)}{\rmap_i \in \hat{M_r}}) && \text{by Lemma~\ref{thm:r-K-join-sound}}\\
\forall \cnode. \pair{\cmap_u}{\cmap_u(\cnode)} \in \rgamma[](\rmap_u(\cnode)) && \text{by def.\ of $\rmjoin$ and $\cmjoin$}\\
\cmap_u \in \rmgamma(\rmap_u) && \text{by def.\ of $\rmgamma$}
\end{align*}
\end{proof}




\paragraph{Constants}

We now prove the soundness of relational abstraction for constants.
%
\begin{lemma}~\label{thm:r-constant-sound}
Let $\cmap \in \cmaps$, $\rscope$ a scope, and $\const \in \consts$.
If $\scopecons_\cmap(\rscope)$, then $\pair{\cmap}{\const} \in \rgamma(\rconst)$.
\end{lemma}
\begin{proof}
By definition, we have $\rconst_\rscope \pset{\dmap \in \dmaps_\rscope}{\dmap(\nu) = c}$.
By $\rgamma$, we also have  
%
\begin{align*}
\rgamma(\rconst) = \rgamma(\pset{\dmap \in \dmaps_\rscope}{\dmap(\nu) = c})  = \\
\setc{\pair{\cmap}{c}}{\dmap \in \dmaps_\rscope \wedge \dmap(\nu) = c \land
\forall \cnode \in \rscope.\; \cmap(\cnode) \in \dgamma(\dmap(\cnode))} \cup \rgamma[](\rbot) =\\
\setc{\pair{\cmap}{c}}{\dmap(\nu) = c \land
\forall \cnode \in \rscope.\; \cmap(\cnode) \not\in \{\bot, \cerr\}} \cup \rgamma[](\rbot)
\end{align*}
%
The result then follows from the definition of $\scopecons$.
\end{proof}


\paragraph{Strengthening}

We now prove the soundness of several strengthening operations.
%
\begin{lemma}~\label{thm:r-update-sound}
Let $\cmap \in \cmaps$, $\cval_1 \in \cvalues$, $\cnode \in \cnodes$,
$\rval \in \rvalues$, and $\rval' \in \rvalues[]$. If $\pair{\cmap}{\cval_1} \in \rgamma(\rval)$
and $\pair{\cmap}{\cmap(\cnode)} \in \rgamma[](\rval')$, then 
$\pair{\cmap}{\cval_1} \in \rgamma(\rupdate{\rval}{\cnode}{\rval'})$.
\end{lemma}
\begin{proof}

\begin{align*}
\rgamma(\rupdate{\rval_{\rscope}}{\cnode}{\rval'}) =
\rgamma(\ralpha(\rgamma[](\rval_\rscope) \;\cap \setc{ \pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma[](\rval')})) \supseteq \\
\rgamma[](\rval_\rscope) \;\cap \setc{ \pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma[](\rval')} \supseteq \\
\{\pair{\cmap}{\cval_1}\} \;\cap \setc{ \pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma[](\rval')} \supseteq\\
\{\pair{\cmap}{\cval_1}\} \;\cap \setc{ \pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap}{\cval'} \in \{\pair{\cmap}{\cmap(\cnode)}\}} = \\
\{\pair{\cmap}{\cval_1}\} \;\cap \setc{ \pair{\cmap[\cnode \mapsto \cmap(\cnode)]}{\cval}}{\cval \in \cvalues} = \\
\{\pair{\cmap}{\cval_1}\} \;\cap \setc{ \pair{\cmap}{\cval}}{\cval \in \cvalues} = \\
\{\pair{\cmap}{\cval_1}\} 
\end{align*}

\end{proof}
%
We can generalize the above result.
%
\begin{lemma}~\label{thm:r-scope-map-updates-sound}
Let $\cmap \in \cmaps$, $\cval \in \cvalues$, $\rscope$ a scope, $\rmap \in \rmaps$, 
$\rval \in \rvalues$. If $\pair{\cmap}{\cval} \in \rgamma(\rval)$ and $\cmap \in \rmgamma(\rmap)$, 
then $\pair{\cmap}{\cval} \in \rstrengthen{\rval}{\rmap}$.
\end{lemma}
\begin{proof}
Consider any $\cnode \in \rscope$. By $\cmap \in \rmgamma(\rmap)$, we have that
$\pair{\cmap}{\cmap(\cnode)} \in \rgamma[](\rmap(\cnode))$. Then by 
Lemma~\ref{thm:r-update-sound}, $\pair{\cmap}{\cval} \in \rgamma(\rupdate{\rval}{\cnode}{\rmap(\cnode)})$.
Hence, $\pair{\cmap}{\cval} \in \bigcap_{\cnode \in \rscope} \rgamma(\rupdate{\rval}{\cnode}{\rmap(\cnode)})$. 
Then by Lemma~\ref{thm:r-meet-morph-values} we have
$\pair{\cmap}{\cval} \in \rgamma(\rvmeet_{\cnode \in \rscope} \rupdate{\rval}{\cnode}{\rmap(\cnode)})$.
\end{proof}

Next, we present a results showing that updates to a relational map with sound information
yields a sound map.
\begin{lemma}~\label{thm:r-map-simple-update}
Let $\cmap \in \cmaps$, $\rmap \in \rmaps$, $\cnode \in \cnodes$, $\cval \in \cvalues$, and 
$\rval \in \rvalues[]$. If $\pair{\cmap}{\cval} \in \rgamma[](\rval)$ and
$\cmap \in \rmgamma(\rmap)$, then
$\cmap \in \rmgamma(\rmap[\cnode \mapsto \rval])$.
\end{lemma}
\begin{proof}
Clearly, as $\forall \cnode'. \pair{\cmap}{\cmap(\cnode')} \in \rgamma[](\rmap[\cnode \mapsto \rval](\cnode'))$. 
\end{proof}


Our rescoping operations are also sound.
\begin{lemma}~\label{thm:r-rescoping-up-sound}
Let $\cmap \in \cmaps$, $\cval_1 \in \cvalues$, $\rval \in \rvalues$, and 
$N' \subseteq \powerset(\cnodes)$ such that $\scopecons_\cmap(N')$.
If $\pair{\cmap}{\cval_1} \in \rgamma(\rval)$, 
then $\pair{\cmap}{\cval_1} \in \rgamma[\rscope \cup N'](\rrescope{\rval}{\rscope \cup N'})$ 
\end{lemma}
\begin{proof}
\begin{align*}
\rrescope{\rval_{\rscope}}{\rscope \cup N'} = \ralpha[\rscope \cup N'](\rgamma[](\rval_\rscope) 
\cap \setc{\pair{\cmap}{\cval}}{\forall n \in \rscope' {\setminus} \rscope. \cmap(n) \notin \set{\bot,\cerr}}) \\
{}\sqsupseteq^{\rdesignation} \ralpha[\rscope \cup N'](\{\pair{\cmap}{\cval_1})\} 
\cap \setc{\pair{\cmap}{\cval}}{\forall n \in \rscope' {\setminus} \rscope. \cmap(n) \notin \set{\bot,\cerr}}) \\
= \ralpha[\rscope \cup N'](\{\pair{\cmap}{\cval_1})\})
\end{align*}
%
\end{proof}
%
\begin{lemma}~\label{thm:r-rescoping-down-sound}
Let $\cmap \in \cmaps$, $\cval_1 \in \cvalues$, $\rval \in \rvalues$, and 
$N' \subseteq \rscope$.
If $\pair{\cmap}{\cval_1} \in \rgamma(\rval)$, 
then $\pair{\cmap}{\cval_1} \in \rgamma[N'](\rrescope{\rval}{N'})$ 
\end{lemma}
\begin{proof}
Straightforward as $N'\setminus \rscope = \emptyset$.
\end{proof}
%
Strengthening of a relational value with the information not in the scope
is sound as well.
%

\paragraph{Maps}


We next show the soundness of updates to the relational maps subject to their concretizations.
\begin{lemma}~\label{thm:r-map-update}
Let $\cmap \in \cmaps$, $\rmap \in \rmaps$, $\cnode \in \cnodes$, $\cval \in \cvalues$, and 
$\rval \in \rvalues[]$. If $\pair{\cmap}{\cval} \in \rgamma[](\rval)$, 
$\cmap \in \rmgamma(\rmap)$, $\cmap(\cnode) \cvord \cval$, and $\cval \not= \cerr$,
then $\cmap[\cnode \mapsto \cval] \in \rmgamma(\rmap[\cnode \mapsto \rval])$.
\end{lemma}
\begin{proof}
Suppose not. Let $\cmap_0 = \cmap[\cnode \mapsto \cval]$ and $\rmap_0 = \rmap[\cnode \mapsto \rval]$.
There must be a node $\cnode'$ such that $\pair{\cmap_0}{\cmap_0(\cnode')} \not \in \rgamma[](\rmap_0(\cnode'))$.
We branch on several cases:
\begin{itemize}
\item $\cnode \not \in \rscope_{\cnode'}$. If $\cnode = \cnode'$, the argument is trivial. 
Otherwise we know that $\pair{\cmap}{\cmap(\cnode')} \in \rgamma[](\rmap(\cnode'))$,
$\rmap(\cnode') = \rmap_0(\cnode')$, and $\cmap(\cnode') = \cmap_0(\cnode')$. Then by 
Lemma~\ref{thm:r-gamma-out-of-scope} also 
$\pair{\cmap_0}{\cmap_0(\cnode')} \in \rgamma[](\rmap_0(\cnode'))$.

\item $\cnode \in \rscope_{\cnode'}$. Again, we know that 
$\pair{\cmap}{\cmap(\cnode')} \in \rgamma[](\rmap(\cnode'))$,
$\rmap(\cnode') = \rmap_0(\cnode')$, and $\cmap(\cnode') = \cmap_0(\cnode')$. 
Since $\cmap \cmord \cmap'$, $\cmap =_{\setminus \{\cnode\}} \cmap'$, and $\cmap'(\cnode) \not= \cerr$,
then by Lemma~\ref{thm:r-v-meaning-up}
$\pair{\cmap_0}{\cmap_0(\cnode')} \in \rgamma[](\rmap(\cnode'))$ and hence
$\pair{\cmap_0}{\cmap_0(\cnode')} \in \rgamma[](\rmap_0(\cnode'))$.

\end{itemize}
\end{proof}


\paragraph{Transformer}

We next show that the relational transformer abstracts the concrete transformer
given certain invariants on the concrete maps. %
\begin{lemma}~\label{thm:r-transformer-soundness}
First, assume that $P$ is an inductive invariant family of a program $m$ where
$\forall k, \ell, \cenv.\,(\ell, \cmap, \cenv) \in P_{k} {\implies} \dfinv_m(\cmap) \wedge \envcons_{\cmap}(\cenv)$. Now,
let $e^\ell$ be an expression of $m$, $\cmap_f \in \cmaps$, 
$\cmap \in \cmaps$, and $\cenv$ an environment where 
$(e, \cenv)$ is well-formed, $\domvalid(\ell, m, \cenv)$, and $(\ell, \cmap, \cenv) \in P$. 
Also, let $\rmap_f \in \rmaps$ and $\rmap \in \rmaps$ such that $\cmap \in \rmgamma(\rmap)$. 
If $\ctrans[\fuel]{e^\ell}(\cenv)(\cmap) = \cmap_f$ and 
$\Rtrans[\fuel]{e^\ell}(\cenv)(\rmap) = \rmap_f$, then $\cmap_f \in \rmgamma(\rmap_f)$.
\end{lemma}
\begin{proof}
We carry the proof by structural induction on $e$. 
We note that $\Rtrans[\fuel]{e^\ell}(\cenv)(\rmap) = \rmap \rmjoin 
\rtrans[\fuel]{e^\ell}(\cenv)(\rmap)$, hence we focus on $\rtrans[\fuel]{e^\ell}$ and
consider all the cases for $e$. Also observe that $\dfinv(\cmap)$ and 
$\envcons_{\cmap}(\cenv)$ by $P$ and $(\ell, \cmap, \cenv) \in P$.

\paragraph{$e = \const^\ell$.} 
Let $\cval = \cmap(\cn{\cenv}{\ell})$ and $\rval = \rmap(\cn{\cenv}{\ell})$. 
By $\dfinv_m(\cmap)$, we have that $\constcons_m(\cmap)$ which implies 
$\cval \in \{\bot, \cerr, \const\}$. If $\cval = \cerr$ then by $\dfinv_n(\cmap)$
we have $\errcons(\cmap)$ and thus $\cmap = \cmap_\cerr$. Then it must be that 
$\rmap = \rmap_{\rerr}$ and the argument is trivial. 

Otherwise, $\cval \in \{\bot, \const\}$. By $\envcons_\cmap(\cenv)$ we have 
$\scopecons_\cmap(N)$ where $N = \rscope_{\cn{\cenv}{\ell}}$. Then by 
Lemma~\ref{thm:r-constant-sound} it follows $\pair{\cmap}{\const} \in \rgamma(\rconst)$
and by Lemma~\ref{thm:r-scope-map-updates-sound} it must be that
$\pair{\cmap}{\const} \in \rgamma(\rstrengthen{\rconst}{\rmap})$. Since
$\noerr(\const)$, $\noerr(\cval)$, $\constcomp(\cval, \const)$, and 
$\pair{\cmap}{\cval} \in \rgamma[](\rval)$,
by Lemma~\ref{thm:r-join-sound} it must be that 
$\pair{\cmap}{\cval \cvjoin \const} \in \rgamma(\rval \rvjoin \rstrengthen{\rconst}{\rmap})$.
The result then follows by Lemma~\ref{thm:r-map-update}.


\paragraph{$e = x^\ell$.} 
Let $\cmap(\cn{\cenv}{\ell}) = \cval$, $\cmap(\cenv(x)) = \cval_x$, 
$\rmap(\cn{\cenv}{\ell}) = \rval$, and $\rmap(\cenv(x)) = \rval_x$.
If $\cval_x = \cerr$ or $\cval=\cerr$, then by $\errcons(\cmap)$ it must
be that $\cmap = \cmap_\cerr$ and hence $\rmap = \rmap_{\rerr}$. In this case,
the argument is trivial.

Otherwise, we know that $\pair{\cmap}{\cval} \in \rgamma[](\rval)$,
and $\pair{\cmap}{\cval_x} \in \rgamma[](\rval_x)$. 
Let $\rval_0$ be $\rval_x$ implicitly rescoped with $N_{\cenv(x)} \cup N_{\cn{\cenv}{\ell}}$.
Let also $\rval_1$ be $\rval$ be rescoped with $N_{\cenv(x)} \cup N_{\cn{\cenv}{\ell}}$.
By $\envcons_\cmap(\cenv)$ and $\envcons(\cmap)$
and Lemma~\ref{thm:r-rescoping-up-sound}, we have $\pair{\cmap}{\cval_x} \in \rgamma[](\rval_0)$.  
$\pair{\cmap}{\cval} \in \rgamma[](\rval_1)$.
As $\cenv(x)$ was not initially in the scope of $\cenv(x)$, then also
$\pair{\cmap}{\cval_x} \in \rgamma[](\requality{\rval_0}{\cenv(x)}{\nu})$.

Next, by $\dfinv_m(\cmap)$ we have that $\cval_x \csub \cval$. As by
$\errcons(\cmap)$ we have $\noerr(\cval)$, $\noerr(\cval_x)$, and
$\scopecons_\cmap(\rscope)$ (via $\envcons_\cmap(\cenv)$), then by 
Lemma~\ref{thm:r-prop-sound} we have that $\pair{\cmap}{\cval'_x} \in \rgamma[](\rval'_x)$
and $\pair{\cmap}{\cval'} \in \rgamma[](\rval')$. As $\rval'_x$
is rescoped back to $N_{\cenv(x)}$ as $\rval_2$ and $\rval'$ is rescoped
back to $N_{\cn{\cenv}{\ell}}$ as $\rval_3$, by Lemma~\ref{thm:r-rescoping-down-sound}
we have $\pair{\cmap}{\cval'_x} \in \rgamma[](\rval_2)$
and $\pair{\cmap}{\cval'} \in \rgamma[](\rval_3)$. By Lemma~\ref{thm:r-scope-map-updates-sound},
we have $\pair{\cmap}{\cval'} \in \rgamma[](\rstrengthen{\rval_3}{\rmap})$.

Let $\cmap_1 = \cmap[\cenv(x) \mapsto \cval'_x]$, $\cmap_2 = \cmap_1[\cn{\cenv}{\ell} \mapsto \cval']$,
$\rmap_1 = \rmap[\cenv(x) \mapsto \rval_2]$, and $\rmap_2 = \rmap_1[\cn{\cenv}{\ell} \mapsto \rval_3]$.
By Lemma~\ref{thm:r-map-update}, $\cmap_1 \in \rgamma(\rmap_1)$. By the increasing property of $\cprop$ (Lemma~\ref{thm:r-prop-increasing-monotone}),
we have $\cmap \cmord \cmap_1$. Also, $\cmap =_{\setminus \{\cenv(x)\}} \cmap_1$ and $\cval'_x \not= \cerr$
by $\cval_x \csub \cval$ and Lemma~\ref{thm:c-prop-sub-no-err-bot}. Hence, $\envcons_{\cmap_1}(\cenv)$ and $\scopecons_{\cmap_1}(\rscope)$.
Then by Lemma~\ref{thm:r-v-meaning-up} we have $\pair{\cmap_1}{\cval'} \in \rgamma(\rval_3)$.
Finally, we then have by Lemma~\ref{thm:r-map-update} that $\cmap_2 \in \rmgamma(\rmap_2)$.


\paragraph{$e = (e_1^{\ell_1} e_2^{\ell_2})^\ell$.}
By i.h., $\cmap_1 \in \rmgamma(\rmap_1)$. By the inductiveness of $P$,
we have $\dfinv_m(\cmap_1)$ and $\envcons_{\cmap_1}(\cenv)$.   
If $\cval_1 = \bot$, then $\cmap_f = \cmap_1$ and $\rmap_1 \rmord \rmap_f$
by the obvious increasing property of $\Rtrans{\cdot}$ and $\rprop$ (Lemma~\ref{thm:r-prop-increasing-monotone});
the result thus follows by the monotonicity of $\rmgamma$. If $\cval_1 = \cerr$, then
by $\errcons(\cmap_1)$ it must be that $\cmap_1 = \cmap_\cerr$ and hence $\rmap = \rmap_{\rerr}$,
in which case the result follows immediately. If $\cval_1 \not \in \ctables$, then by the
definition of $\rgamma[]$ also $\rval_1 \not \in \rtables$. In that case, $\cmap_f = \cmap_\cerr$
and $\rmap = \rmap_{\rerr}$ and the argument is straightforward. If $\cval_1 \in \ctables$,
but $\rval_1 \not\in \rtables$, then $\rval_1 = \rerr$ and hence $\rmap_f = \rmap_{\rerr}$.
Otherwise, by i.h.\ $\cmap_2 \in \rmgamma(\rmap_2)$. Again by the inductive property of $P$,
we have $\dfinv_m(\cmap_2)$ and $\envcons_{\cmap_2}(\cenv)$. The cases when 
$\cval_2 \in \{\bot, \cerr\}$ are handled identically as for $\cval_1$.    

By $\domvalid(\ell, m, \cenv)$, $\domvalid(\ell_1, m, \cenv)$, and $\domvalid(\ell_2, m, \cenv)$,
Lemma~\ref{thm:c-frame}, and Lemma~\ref{thm:c-disjoint-1}, we have that 
$\cval_1 = \cmap_2(\cn{\cenv}{\ell_1})$. Similarly, by Lemma~\ref{thm:r-frame} it also
holds $\rval_1 = \rmap_2(\cn{\cenv}{\ell_1})$. Let $\cval = \cmap_2(\cn{\cenv}{\ell})$
and $\rval = \rmap_2(\cn{\cenv}{\ell})$. Then by $\cmap_2 \in \rmgamma(\rmap_2)$,
we have $\pair{\cmap_2}{\cval_1} \in \rgamma[](\rval_1)$, $\pair{\cmap_2}{\cval_2} \in \rgamma[](\rval_2)$,
and $\pair{\cmap_2}{\cval} \in \rgamma[](\rval)$. As $\rval$ is implicitly rescoped
with $\rscope_{\cn{\cenv}{\ell}} \cup \{\cn{\cenv}{\ell_1}\}$ to $\rval_0$, then by
Lemma~\ref{thm:r-rescoping-up-sound}, $\pair{\cmap_2}{\cval_2} \in \rgamma[](\rval_0)$.

If any of $\cval_1$, $\cval_2$, or $\cval_3$ is $\cerr$, then $\cmap_2 = \cmap_\cerr$ and
the argument goes as usual. Otherwise, we have $\noerr(\cval_1)$, $\noerr(\cval_2)$,
$\noerr(\cval_3)$ and by $\dfinv_m(\cmap_2)$ also 
$\cval_1 \csub [\cn{\cenv}{\ell_1} \mapsto \pair{\cval_2}{\cval}]$. Since
$\pair{\cmap_2}{[\cn{\cenv}{\ell_1} \mapsto \pair{\cval_2}{\cval_2}]} \in \rgamma([\cn{\cenv}{\ell_1} \mapsto \pair{\rval_2}{\rval_0}])$
by def.\ of $\rgamma[]$ and $\envcons_{\cmap_2}(\cenv)$, we have by Lemma~\ref{thm:r-prop-sound}
that $\pair{\cmap_2}{\cval'_1} \in \rgamma(\rval'_1)$ and
$\pair{\cmap_2}{[\cn{\cenv}{\ell_1} \mapsto \pair{\cval'_2}{\cval'}]} \in \rgamma([\cn{\cenv}{\ell_1} \mapsto \pair{\rval'_2}{\rval'_0}])$
and hence by def.\ of $\rgamma[]$ we have $\pair{\cmap_2}{\cval'_1} \in \rgamma[](\rval'_1)$, $\pair{\cmap_2}{\cval'_2} \in \rgamma[](\rval'_2)$,
and $\pair{\cmap_2}{\cval'} \in \rgamma[](\rval'_0)$. As $\rval'_0$ is implicitly rescoped back
with $\rscope_{\cn{\cenv}{\ell}}$ to $\rval''_0$, by Lemma~\ref{thm:r-rescoping-down-sound} we have
$\pair{\cmap_2}{\cval'} \in \rgamma[](\rval''_0)$. The argument for storing the results to maps
$\cmap_2$ and $\rmap_2$ then follows by Lemma~\ref{thm:c-prop-sub-no-err-bot},~\ref{thm:r-v-meaning-up}, 
and~\ref{thm:r-map-update} as earlier.

%\begin{comment}
%\paragraph{$(\ite{e_0^{\ell_0}}{e_1^{\ell_1}}{e_2^{\ell_2}})^\ell$.}
%By i.h., we have that $\cmap_0 \in \rgamma(\rmap_0)$. By the inductiveness of $P$,
%we have $\dfinv_m(\cmap_0)$ and $\envcons_{\cmap_0}(\cenv)$. The cases
%when $\cval_0 \in \{\bot, \cerr\}$ are handled as expected. If $\cval_0 \in \bools$ and
%$\rval_0 \not \in \rbools$, then $\rval_0 = \rerr$ by the definition of $\rgamma[]$
%and $\rmap_f = \rmap_{\rerr}$.
%
%Otherwise, the argument is as follows. Suppose $\cval_0 = \btrue$; the argument for
%the case when $\cval_0 = \bfalse$ is identical. Since $\envcons_{\cmap_0}(\cenv)$
%implies $\scopecons_{\cmap_0}(N_{\cn{\cenv}{\ell}})$, by Lemma~\ref{thm:r-constant-sound}
%we have that $\pair{\cmap_0}{\btrue} \in \rgamma[](\rtrue)$. Since 
%$\pair{\cmap_0}{\btrue} \in \rgamma[](\rval_0)$ by $\cmap_0 \in \rgamma(\rmap_0)$,
%we have that $\pair{\cmap_0}{\btrue} \in (\rgamma[](\rtrue) \cap \rgamma[](\rval_0))$.
%Then by Lemma~\ref{thm:r-meet-morph-values}, it also holds 
%$\pair{\cmap_0}{\btrue} \in \rgamma[](\rtrue \rvmeet \rval_0)$. Now, let
%$\cnode' \in N_{\cn{\cenv}{\ell_0}}$. By $\cmap_0 \in \rmgamma(\rmap_0)$,
%we have that $\pair{\cmap_0}{\cmap_0(\cnode')} \in \rgamma[](\rmap_0(\cnode'))$.
%As $\pair{\cmap_0}{\btrue} = \pair{\cmap_0}{\cmap_0(\cn{\cenv}{\ell_0})}$,
%we have that 
%$\pair{\cmap_0}{\cmap_0(\cnode')} \in \rgamma[](\rupdate{\rmap_0(\cnode')}{\cn{\cenv}{\ell_0}}{\rtrue \rvmeet \rval_0})$ by Lemma~\ref{thm:r-update-sound}.
%Hence, by Lemma~\ref{thm:r-map-simple-update} it is the case that
%$\cmap_0 \in \rmgamma(\rmap_0[\cnode' \mapsto \rupdate{\rmap_0(\cnode')}{\cn{\cenv}{\ell_0}}{\rtrue \rvmeet \rval_0}])$.
%Further, by Lemma~\ref{thm:r-meet-morph-maps} it is also the
%case that $\cmap_0 \in \rmgamma(\rmmeet_{\cnode' \in N_{\cn{\cenv}{\ell_0}}} \rmap_0[\cnode' \mapsto \rupdate{\rmap_0(\cnode')}{\cn{\cenv}{\ell_0}}{\rtrue \rvmeet \rval_0}])$.
%Therefore, $\cmap_0 \in \rmgamma(\rupdate{\rmap_0}{\cn{\cenv}{\ell_0}}{\rtrue \rvmeet \rval_0})$.
%
%It follows then by i.h.\ that $\cmap_1 \in \rgamma(\rmap_1)$ and by 
%the inductiveness of $P$, we have $\dfinv_m(\cmap_1)$ and $\envcons_{\cmap_1}(\cenv)$.
%The argument continues as usual by Lemma~\ref{thm:c-prop-sub-no-err-bot},~\ref{thm:r-v-meaning-up}, 
%and~\ref{thm:r-map-update} as before.
%\end{comment}

\paragraph{$e = (\mu f.\lambda x.e_1^{\ell_1})^{\ell}$.}
Let $\cval = \cmap(\cn{\cenv}{\ell})$. By $\dfinv_m(\cmap)$ it follows that
$\constcons_m(\cmap)$ which implies that $\cval \in \{\bot, \cerr\} \cup \ctables$.
If $\cval = \bot$, then $\ctable = \ctable_\bot$ and 
$\cmap_f = \cmap[\cn{\cenv}{\ell} \mapsto \ctable_\bot]$. By the definition of 
$\rgamma$, then either (1) $\rval =\rbot$ in which case 
$\rmap_f = \rmap[\cn{\cenv}{\ell} \mapsto \rtable_{\rbot}]$, (2) $\rval \in \rels[]$
in which case $\rmap_f = \rmap_{\rerr}$, (3) $\rval \in \rtables[]$ and the result
follows by the obvious increasing property of $\Rtrans{\cdot}$ and $\rprop$ 
(Lemma~\ref{thm:r-prop-increasing-monotone}), or (4) $\rval = \rerr$ in which case $\rmap_f = \rmap_{\rerr}$.
If $\cval = \cerr$ then by $\errcons(\cmap)$ it must be that $\cmap = \cmap_f = \cmap_\cerr$
and hence $\rmap = \rmap_f = \rmap_{\rerr}$. If $\cval \in \ctables$ but $\rval \not\in \rtables[]$,
then $\rval = \rerr$ and hence $\rmap_f = \rmap_{\rerr}$.

We are left with the case where $\ctable \in \ctables$ and $\rtable \in \rtables[]$
where $\cval = \ctable$ and $\rval = \rtable$. By $\rgamma[]$, $\ccsite \in \ctable$
implies $\ccsite \in \rtable$. For the case where $\ccsite \not\in \ctable$
and $\ccsite \not\in \rtable$, the argument is trivial. When $\ccsite \not\in \ctable$
but $\ccsite \in \rtable$, the result follows by the obvious increasing property of 
$\Rtrans{\cdot}$ and $\rprop$. We are thus left with the case when $\ccsite \in \ctable$
and $\ccsite \in \rtable$. The case when $\pi_1(\ctable(\ccsite)) \in \{\bot, \cerr\}$
are handled as expected. 

We thus continue assuming $\pi_1(\ctable(\ccsite)) \not\in \{\bot, \cerr\}$.
First, we have by $\dfinv_m(\cmap)$ that 
$[\ccsite \mapsto \pair{\cmap(\cnode_x)}{\cmap(\cn{\cenv_1}{\ell_1})}] \csub \ctable$
and $\ctable \csub \cmap(\cnode_f)$. By the def.\ of $\csub$, $\cmap(\cnode_x) \not\in \{\bot, \cerr\}$.
Next, $\pair{\cmap}{\cmap(\cn{\cenv_1}{\ell_1})} \in \rgamma[](\rmap(\cn{\cenv_1}{\ell_1}))$
by $\cmap \in \rgamma(\rmap)$. Since $\rmap(\cn{\cenv_1}{\ell_1})$ is first implicitly rescoped with
$N_{\cn{\cenv}{\ell_1}} \cup \{\ccsite\}$ to $\rval_0$ and $\cmap(\cnode_x) \not\in \{\bot, \cerr\}$,
by Lemma~\ref{thm:r-rescoping-up-sound} we have 
$\pair{\cmap}{\cmap(\cn{\cenv_1}{\ell_1})} \in \rgamma[](\rval_0)$. As 
$\ccsite \not\in N_{\cn{\cenv}{\ell_1}}$, then it must be that 
$\pair{\cmap}{\cmap(\cn{\cenv_1}{\ell_1})} \in \rgamma[](\requality{\rval_0}{\ccsite}{\cnode_x})$.
Then, $\rval_0$ is implicitly rescoped to the same scope but without $\cnode_x$ and
then by Lemma~\ref{thm:r-rescoping-down-sound} we have 
$\pair{\cmap}{\cmap(\cn{\cenv_1}{\ell_1})} \in \rgamma[](\rval_1)$.
We hence have 
$[\ccsite \mapsto \pair{\cmap(\cnode_x)}{\cmap(\cn{\cenv_1}{\ell_1})}] \in \rgamma[]
[\ccsite \mapsto \pair{\rmap(\cnode_x)}{\rval_1}$, $\ctable \in \rgamma[](\rtable)$,
and $\cmap(\cnode_f) \in \rgamma(\rmap(\cnode_f))$. As $\scopecons_\cmap(N_{\cn{\cenv}{\ell}})$
by $\envcons_\cmap(\cenv)$, $\noerr(\ctable)$, $\noerr(\cmap(\cnode_x))$, 
$\noerr(\cmap(\cnode_f))$, and $\noerr(\cmap(\cn{\cenv_1}{\ell_1}))$, by 
Lemma~\ref{thm:r-prop-sound} we have that $\pair{\cmap}{\ctable'} \in \rgamma(\rtable_1)$,
$\pair{\cmap}{\ctable''} \in \rgamma(\rtable_2)$, $\pair{\cmap}{\ctable'_x} \in \rgamma(\rtable_x)$,
and $\pair{\cmap}{\ctable'_f} \in \rgamma[](\rtable_f)$. By Lemma~\ref{thm:c-prop-sub-no-err-bot},
we have $\noerr(\ctable'')$ and $\noerr(\ctable')$. By Lemma~\ref{thm:sub-prop-ccomp} we have
that $\constcomp(\ctable', \ctable'')$ and thus 
$\pair{\cmap}{\ctable' \cvjoin \ctable''} \in \rgamma[](\rtable_1 \rvjoin \rtable_2)$ by Lemma~\ref{thm:r-join-sound}.

Note that by Lemma~\ref{thm:c-prop-sub-noerr} it must be that $\noerr(\ctable'_x)$
and hence $\cval'_x \not=\cerr$. By this and $\envcons_{\cmap}(\cenv)$ it must be that
$\envcons_{\cmap_1}(\cenv_1)$. It follows then by i.h.\ that $\cmap_1 \in \rgamma(\rmap_1)$ and by 
inductiveness of $P$ we have $\dfinv_m(\cmap_1)$ and $\envcons_{\cmap_1}(\cenv_1)$.
The argument continues as usual by Lemma~\ref{thm:c-prop-sub-no-err-bot},~\ref{thm:r-v-meaning-up}, 
and~\ref{thm:r-map-update} as before. Also, the soundness argument for implicit rescoping and 
strengthening of $\rval'_1$ goes as usual and relies on the fact that 
$\cnode_x$ is not in the scope of $\rval'_1$.

Remember that for every $\ccsite \in \m{dom}(\bar{\cmap})$ we have $\ccsite \in \m{dom}(\bar{\rmap})$ and
$\bar{\cmap}(\ccsite) \in \rmgamma(\bar(\rmap)(\ccsite))$. Given $\cfin(\cmap)$ implied
by $\dfinv_m(\cmap)$, we have $|\m{dom}(\bar{\cmap})| = K$
where $K \in \mathbb{N}$. By the inductiveness of $P$, we have that 
$\dfinv_m(\cmap_f)$ and hence $\errcons(\cmap_f)$.
If $\cmap_f = \cmap_\cerr$ then there exists $\ccsite$ such that $\bar{\cmap}(\ccsite) = \cmap_\cerr$
in which case $\bar{\rmap}(\ccsite) = \rmap_{\rerr}$ and hence $\rmap_f = \rmap_{\rerr}$.
Otherwise, by the definition of $\cmjoin$ 
we have that $\forall \cmap \in \bar{\cmap}.\, \cmap \not = \cmap_\cerr$. By 
Lemma~\ref{thm:errcons-const-comp-maps} we have $\constcomp(\bar{\cmap})$
and $\forall \cmap \in \bar{\cmap}.\,\errcons(\cmap)$. The result then follows from
Lemma~\ref{thm:r-K-join-sound}.
\end{proof}



We can now prove that relational semantics abstract the concrete one.
\begin{zproof*}[of Theorem~\ref{thm:relational-soundness}]\end{zproof*}
\begin{proof}
We assume a fixed program $e^{\ell_m}$. We first define a set 
$P \in \powerset(\locs \times \cmaps \times \cenvironments)$ 
as the smallest set satisfying the following. 
Initially, $(\ell_m, \cmap_\bot, \emptyset) \in P$.
Second, $(\ell, \cmap, \cenv) \in P$ if
(1) $\ell \in \locs(e)$, (2) $(e(\ell), \cenv)$ is well-formed,
(3) $\domvalid(\ell, e, \cenv)$, (4) there exists a path map $\wmap$
such that $\wcons_m(\wmap)$, $\wmap \in \m{dom}(\wstrip)$,
$\cmap = \wstrip(\wmap)$, and $\envcons_{\wmap}(\cenv)$. 
Lastly, for every $(\ell, \cmap, \cenv) \in P$,
if $\wtrans[\fuel]{e(\ell)}(\cenv)(\wmap) = \wmap_1$, $\wcons_m(\wmap)$, $\wcons_m(\wmap_1)$,
$\wmap \in \m{dom}(\wstrip)$, $\wmap_1 \in \m{dom}(\wstrip)$, 
$\cmap = \wstrip(\wmap)$, and $\cmap_1 = \wstrip(\wmap_1)$, then 
$(\ell, \cmap_1, \cenv) \in P$. 

By Theorem~\ref{thm:w-cons-inductive}, Theorem~\ref{thm:path-to-data-flow},
$\wcons_m(\wmap_{\wbot})$, $\wmap_\wbot \in \m{dom}(\wstrip)$, and
$\cmap_\bot = \wstrip(\wmap_\wbot)$, we have that $P$ is an inductive
invariant family of $m$. By Lemma~\ref{thm:w-cons-dataflow-inv}
and the definition of $\envcons$ for path maps, we have that
$(\ell, \cmap, \cenv) \in P$ 
implies $\dfinv_m(\cmap)$ and $\envcons_\cmap(\cenv)$.
Since $(\ell_m, \cmap_\bot, \emptyset) \in P$,
we have that the strongest inductive invariant $I$ of $m$ is 
subsumed by $P$, i.e, $S \subseteq P$. The result then
follows from the definition of $\ccoll|[\cdot|]$ and 
Lemma~\ref{thm:r-transformer-soundness}. 
\end{proof}


==> proofs/r-semantics.tex <==
% !TEX root = ../../thesis.tex
\clearpage
\subsection{Relational Semantics Proofs}
\label{sec:proofs-r-semantics}
We first provide a more direct definition of meets and joins
over relational values and show its correctness.
%
\begin{definition}[Join on Relational Values]
\[\begin{array}{cc}
\rbot \rvjoin \rval \Def= \rval \quad\quad \rval \rvjoin \rbot \Def= \rval & \rel_1 \rvjoin \rel_2 \Def= \rel_1 \cup \rel_2 \\
\rtable_1 \rvjoin \rtable_2 \Def= \lambda \ccsite.\, \rtable_1(\ccsite) \;\vecop{\rvjoin}\; \rtable_2(\ccsite) 
& \quad \rval_1 \rvjoin \rval_2 \Def= \rerr \quad \text{(otherwise)}
\end{array}\]
\end{definition}
%
\begin{lemma}\label{thm:rvjoin}
Let $V \in \powerset(\rvalues)$. Then, $\rvjoin V = \mi{lub} (V)$ and 
$\rvmeet V = \mi{glb} (V)$ subject to $\rvord$.
\end{lemma}
\begin{proof}
A depth of a relational value is defined in the same was as for the concrete values. We hence
reuse the function $\cvdepth$ to denote the depth of relational values.
We carry the proof by case analysis on elements of $V^r$ and induction on the minimum depth
thereof when $V^r$ consists of tables only. 

We first consider the trivial (base) cases where $V^r$ is not a set of multiple relational tables.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $V^r = \emptyset$. By $\rvord$, $\mi{lub}(V^r) = \rbot$ and $\rvjoin(V^r) = \rbot$ by $\rvjoin$.
\item $V^r = \{\rval\}$. Trivial.
\item $\rel \in V^r, \rtable \in V^r$. By $\rvord$, lub of $\{\rel, \rtable\}$ is $\rerr$
        and since $\rerr$ is the top element, $\mi{lub}(V^r) = \rerr = \rvjoin V^r$.
\item $V^r \subseteq \rels$. The lub of $V^r$ by $\rvord$ is the smallest set of dependency vectors
        containing each $\rel \in V^r$, which is exactly union of all $\rel \in V^r$. Hence, by def. of
	$\rvjoin$ we have that $\m{lub}V^r = \rvjoin V^r$.
\item $\rbot \in V^r$. By $\rvord$, $\mi{lub}(V^r) = \mi{lub}(V^r/\{\rbot\})$ and $\rvjoin(V^r) = \rvjoin(V^r/\{\rbot\})$ 
        by $\rvjoin$. The set $V^r/\{\rbot\}$ either falls into one of the above cases or consists of multiple tables, which is the case we show next.
\end{itemize}
%
Let $V^r \subseteq \rtables$ and $|V^r| > 1$. Let $d$ be the minimum depth of any table in $V^r$.
By $\rvord$, lub of $V^r$ is a table $\rtable$ that for every call site $\ccsite$ has input (resp. output)
that is lub of the corresponding inputs (resp. outputs) of tables in $V^r$ for $\ccsite$.
We focus on inputs; the same argument goes for outputs. Let $V^r_i = \setc{\pi_1(\rval(\ccsite))}{\ccsite \in \ccallsites \wedge \rval \in V^r}$.
By $\rvjoin$, $\pi_1(\rtable(\ccsite)) = \rvjoin V^r_i$. We hence need to show that $\rvjoin V^r_i = \mi{lub}(V^r_i)$.
The set $V^r_i$ either falls into one of the trivial cases, from which the argument easily follows, or $V^r_1 \subseteq \rtables \wedge |V^r| > 1$. 
In the latter case, the minimum depth of any value in $V^r_i$ is smaller than $d$ by the def. of $\cvdepth$ and the result follows from the i.h.
\end{proof}

%\begin{theorem}\label{thm:rvmeet}
%Let $V \in \powerset(\rvalues)$. Then, $\rvmeet V^r = \mi{glb} (V^r)$ subject to $\rvord$.
%\end{theorem}
%\begin{proof}
%Similar to Lemma~\ref{thm:rvjoin}. 
%\end{proof}


We next prove the monotonicity of the concretization function for relational values.
%
\begin{lemma}\label{thm:r-gamma-monotone}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, and $\rval_1 \rvord \rval_2$. Then, $\rgamma(\rval_1) \subseteq \rgamma(\rval_2)$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $\rval_2$. We first cover the base cases.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $\rval_2 = \rbot$. Then $\rval_1=\rbot$ and the result follows trivially.

\item $\rval_2 = \rerr$. Trivially by the def. of $\rgamma(\rerr)$.

\item $\rval_2 = \rel_2$. Then either $\rval_1 = \rbot$ or $\rval_1 = \rel_1$ s.t. $\rel_1 \subseteq \rel_2$. Since the former
               case is trivial due to $\forall \rval.\, \rgamma(\rbot) \subseteq \rgamma(\rval)$ by the def. of $\rgamma$, we focus on the latter case.
		Here,
\begin{gather*}
\rel_1 \subseteq \rel_2 {\implies} \setc{\pair{\cmap}{c}}{\dmap \in \rel_1 \wedge \dmap(\nu) = c} \subseteq \setc{\pair{\cmap}{c}}{\dmap \in \rel_2 \wedge \dmap(\nu) = c} \implies \\
\setc{\pair{\cmap}{c}}{\dmap \in \rel_1 \wedge \dmap(\nu) = c \wedge \forall \cnode \in \rscope.\cmap(\cnode) \in \dgamma(\cmap(\cnode))} \subseteq \\
\quad\quad\setc{\pair{\cmap}{c}}{\dmap \in \rel_2 \wedge \dmap(\nu) = c \wedge \forall \cnode \in \rscope.\cmap(\cnode) \in \dgamma(\cmap(\cnode))} \implies \\
\rgamma(\rval_1) \subseteq \rgamma(\rval_2).
\end{gather*}
\end{itemize}

For the induction step $\rval = \rtable_2$, if $\rval_1 = \rbot$ the argument is trivial. We hence focus on the case where $\rval_1 = \rtable_1$.
Let $\rtable_1(\ccsite) = \pair{\rval_{1i}}{\rval_{1o}}$ and $\rtable_2(\ccsite) = \pair{\rval_{2i}}{\rval_{2o}}$ for any call site $\ccsite$.
By $\rtable_1 \rvord \rtable_2$, we have $\rval_{1i} \rvord \rval_{2i}$ and $\rval_{1o} \rvord \rval_{2o}$. By i.h. on $\rval_{2i}$ and $\rval_{2o}$,
it follows $\rgamma(\rval_{1i}) \subseteq \rgamma(\rval_{2i})$ and $\rgamma(\rval_{1o}) \subseteq \rgamma(\rval_{2o})$, which implies 
$\rgamma(\rtable_1) \subseteq \rgamma(\rtable_2)$ by the def. of $\rgamma$.
\end{proof}
%

It can be also shown that the concretization of relational values does not impose any constraints on the values
for nodes not in the given scope.
%
\begin{lemma}~\label{thm:r-gamma-out-of-scope}
For any $\cnode \not \in \rscope$, $\cnode$ is unconstrained in $\rgamma(\rval_{\rscope})$ for any relational value $\rval$.
That is, $\forall \cnode \not \in \rscope, \cval, \cval', \cmap. \pair{\cmap}{\cval} \in \rgamma(\rval_{\rscope}) {\implies} 
\pair{\cmap[\cnode \to \cval']}{\cval} \in \rgamma(\rval_{\rscope})$.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $\rval$. The base cases are trivial. The induction case for tables follows from the
i.h. and the fact that for any table $\rtable$ and call site $\ccsite$, $\ccsite$ is not in the scope of $\pi_i(\rtable(\ccsite))$.
\end{proof}


The next proof shows that the concretization function satisfies the meet-morphism requirement.
%
\begin{theorem}[Complete Meet Morphism on Rel. Values]\label{thm:r-meet-morph-values}
Let $V^r \in \powerset(\rvalues)$. Then $\rgamma(\rvmeet V^r) = \bigcap_{\rval \in V^r} \rgamma(\rval)$.
\end{theorem}
\begin{proof}
We carry the proof by case analysis on elements of $V^r$ and induction on the minimum depth
thereof when $V^r$ consists of tables only. 

We first consider the trivial (base) cases where $V^r$ is not a set of multiple relational tables.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $V^r = \emptyset$. Here, $\rgamma(\rvmeet \emptyset) = \rgamma(\rerr) = \cmaps \times \cvalues = \bigcap \emptyset$.
\item $V^r = \{\rval\}$. Trivial.
\item $\rel \in V^r, \rtable \in V^r$. We have $\rvmeet \{\rel, \rtable\} = \rbot$
        and since $\rbot$ is the bottom element, $\rvmeet V^r = \rbot$. Similarly,
	$\rgamma(\rel) \cap \rgamma(\rtable) = \rgamma(\rbot)$ and since $\forall \rval.\, \rgamma(\rbot) \subseteq \rgamma(\rval)$,
	it follows $\bigcap_{\rval \in V^r} \rgamma(\rval) = \rgamma(\rbot) = \rgamma(\rvmeet V^r)$.

\item $V^r \subseteq \rels$. Here,
{\footnotesize \begin{gather*}
\rgamma(\rvmeet V^r) = \rgamma(\bigcap_{\rel \in V^r}\,\rel) \\
= \setc{\pair{\cmap}{c}}{\dmap \in (\bigcap_{\rel \in V^r}\,\rel)) \wedge \dmap(\nu) = c \wedge \forall \cnode \in \rscope.\cmap(\cnode) \in \dgamma(\cmap(\cnode))} \cup \rgamma(\rbot) \\
\ind[15] \textbf{\scriptsize [by def. of $\rgamma$]} \\
= \bigcap_{\rel \in V^r}  (\setc{\pair{\cmap}{c}}{\dmap \in \rel \wedge \dmap(\nu) = c \wedge \forall \cnode \in \rscope.\cmap(\cnode) \in \dgamma(\cmap(\cnode))} \cup \rgamma(\rbot)) \\
\ind[12] \textbf{\scriptsize [by uniqueness/non-overlapping of $\dgamma$]} \\
=  \bigcap_{\rel \in V^r} \rgamma(\rel)
\ind[13] \textbf{\scriptsize [by def. of $\rgamma$]}
\end{gather*}}%


\item $\rerr \in V^r$. Here, $ \rvmeet V^r = \rvmeet (V^r/\{\rerr\})$ and $\bigcap_{\rval \in V^r} \rgamma(\rval) = \bigcap_{\rval \in V^r, \rval \not = \rerr} \rgamma(\rval)$ since $\rgamma(\rerr) = \cmaps \times \cvalues$. The set $V^r/\{\rerr\}$ either falls into one of the above cases or consists of multiple tables, which is the case we show next.
\end{itemize}


Let $V^r \subseteq \rtables$ and $|V^r| > 1$. Let $d$ be the minimum depth of any table in $V^r$.
{\footnotesize
\begin{gather*}
\bigcap_{\rtable \in V^r} \rgamma(\rtable) = \{ \pair{\cmap}{\ctable}\;|\; \forall \ccsite.\;
  \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \pair{\cmap_i}{\cval_i} \in \bigcap_{\rtable \in V^r} \rgamma[](\pi_1(\rtable(\ccsite))) \;\wedge \\
   \pair{\cmap_o}{\cval_o} \in \bigcap_{\rtable \in V^r} \rgamma[](\pi_2(\rtable(\ccsite))) \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i]\} \cup \rgamma(\rbot) \\
\ind[10] \textbf{\scriptsize [by def. of $\rgamma$ and $\ccsite$ not in the scope of $\pi_1(\rtable(\ccsite))$]} \\
= \{ \pair{\cmap}{\ctable}\;|\; \forall \ccsite.\;
  \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \pair{\cmap_i}{\cval_i} \in \rgamma(\rvmeet_{\rtable \in V^r} \pi_1(\rtable(\ccsite))) \;\wedge \\
   \pair{\cmap_o}{\cval_o} \in \rgamma(\rvmeet_{\rtable \in V^r} \pi_2(\rtable(\ccsite))) \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i]\} \cup \rgamma(\rbot) \\
\textbf{\scriptsize [by i.h. on the min. depth of $\setc{\pi_1(\rtable(\ccsite)))}{\rtable \in V^r}$ and $\setc{\pi_2(\rtable(\ccsite)))}{\rtable \in V^r}$]} \\
= \rgamma(\rvmeet_{\rtable \in V^r} \rtable) \ind[20] \textbf{\scriptsize [by def. of $\rgamma$]}
\end{gather*}}%
\end{proof}

We can now state the monotonicity of abstraction function for the relational domain.
\begin{lemma}\label{thm:r-v-alpha-monotone}
$\ralpha$ is monotone.
\end{lemma}
\begin{proof}
The result follows from the properties of Galois connections.
\end{proof}

The meet morphism requirement is also satisfied by the concretization function defined over
relational maps.
\begin{theorem}[Complete Meet Morphism on Rel. Maps]\label{thm:r-meet-morph-maps}
Let $m^r \in \powerset(\rmaps)$. Then $\rmgamma(\rmmeet m^r) = \bigcap_{\rmap \in m^r} \rmgamma(\rmap)$.
\end{theorem}
\begin{proof}
\begin{align*}
 \bigcap_{\rmap \in m^r} \rmgamma(\rmap) = \setc{\cmap}{\forall \cnode.\, \pair{\cmap}{\cmap(\cnode)} \in \bigcap_{\rmap \in m^r} \rgamma(\rmap(\cnode))} && \\
  = \setc{\cmap}{\forall \cnode.\, \pair{\cmap}{\cmap(\cnode)} \in \rgamma(\rvmeet_{\rmap \in m^r} \rmap(\cnode))} && \textbf{\scriptsize [by Lemma~\ref{thm:r-meet-morph-values}]}\\
 = \rmgamma(\rmmeet m^r) && \textbf{\scriptsize [by def. of $\rmgamma$ and $\rmmeet$]}
 \end{align*}
\end{proof}












\paragraph{Domain Operations}

In this subsection, we state the basic properties and the corresponding proofs of
strengthening operations on relational values.

\paragraph{Strengthening} 
We first show that our strengthening operations indeed perform
strengthening.
\begin{lemma}\label{thm:r-n-strengthening}
Let $\rval_1 \in \rvalues$, $\rval \in \rvalues$, and $\cnode \in \cnodes$. 
Then $\rupdate{\rval}{\cnode}{\rval_1} \rvord \rval$.
\end{lemma}
\begin{proof}
In the below calculational proof, let $S = \setc{\pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma(\rval_1)}$.
%
{\small
\begin{align*}
\ralpha(\rgamma(\rval)) \rvord \rval && \text{by prop. of Galois conn.}\\
\ralpha(\rgamma(\rval) \cap S) \rvord \ralpha(\rgamma(\rval)) && \text{by Lemma~\ref{thm:r-v-alpha-monotone}}\\
\ralpha(\rgamma(\rval) \cap S) \rvord \rval && \text{by transitivity}\\
\rupdate{\rval}{\cnode}{\rval_1} \rvord \rval && \text{by def. of $\rupdate{\cdot}{\cdot}{\cdot}$}
\end{align*}}%
\end{proof}

\begin{lemma}\label{thm:r-neq-strengthening}
Let $\rval \in \rvalues$, $\cnode_1 \in \cnodes$, and $\cnode_2 \in \cnodes$. 
Then $\requality{\rval}{\cnode_1}{\cnode_2} \rvord \rval$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:r-n-strengthening}.
\end{proof}

\begin{lemma}\label{thm:r-veq-strengthening}
Let $\rval \in \rvalues$ and $\cnode \in \cnodes$. 
Then $\requality{\rval}{\nu}{\cnode_2} \rvord \rval$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:r-n-strengthening}.
\end{proof}

\begin{lemma}\label{thm:r-map-strengthening}
Let $\rval \in \rvalues$ and $\rmap \in \rmaps$. 
Then $\rstrengthen{\rval}{\rmap} \rvord \rval$.
\end{lemma}
\begin{proof}
Follows from the properties of meets and Lemma~\ref{thm:r-n-strengthening}.
\end{proof}

We can also show that strengthening operations are idempotent. We show the
proof of idempotency for strengthening by a relational value.
%
\begin{lemma}\label{thm:r-n-strength-idempotent}
Let $\rval_1 \in \rvalues$, $\rval \in \rvalues$, and $\cnode \in \cnodes$. 
Then $\rupdate{\rval}{\cnode}{\rval_1} = \rupdate{\rupdate{\rval}{\cnode}{\rval_1}}{\cnode}{\rval_1}$.
\end{lemma}
\begin{proof}
In the below calculational proof, let $S = \setc{\pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma(\rval_1)}$ 
and $\rval' = \rupdate{\rval}{\cnode}{\rval_1} = \ralpha(\rgamma(\rval) \cap S)$.
%
{\small
\begin{align*}
\rupdate{\rval'}{\cnode}{\rval_1} = \ralpha(\rgamma(\rval') \cap S) && \text{by def. of $\rupdate{\cdot}{\cdot}{\cdot}$}\\
\rgamma(\rval) \cap S \subseteq \rgamma(\rval')  && \text{by prop. of Galois conn.}\\
\rgamma(\rval) \cap S \subseteq \rgamma(\rval') \cap S  && \text{by def. of $\cap$}\\
\ralpha(\rgamma(\rval) \cap S) \rvord \ralpha(\rgamma(\rval') \cap S)  && \text{by Lemma~\ref{thm:r-v-alpha-monotone}}\\
\rupdate{\rval}{\cnode}{\rval_1} \rvord \rupdate{\rval'}{\cnode}{\rval_1}  && \text{by def. of $\rupdate{\cdot}{\cdot}{\cdot}$}\\
\rupdate{\rval}{\cnode}{\rval_1} \rvord \rupdate{\rupdate{\rval}{\cnode}{\rval_1}}{\cnode}{\rval_1} && \text{by def. of $\rval'$}\\
\rupdate{\rupdate{\rval}{\cnode}{\rval_1}}{\cnode}{\rval_1} \rvord \rupdate{\rval}{\cnode}{\rval_1} && \text{by Lemma~\ref{thm:r-n-strengthening}}\\
\rupdate{\rupdate{\rval}{\cnode}{\rval_1}}{\cnode}{\rval_1} = \rupdate{\rval}{\cnode}{\rval_1} &&
\end{align*}
}%
\end{proof}

\paragraph{Monotonicity} 

All of the strengthening operations on relational values are monotone.
\begin{lemma}\label{thm:r-n-strength-monotone}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, $\rval \in \rvalues$, and $\cnode \in \cnodes$. 
Then $\rval_1 \rvord \rval_2 \implies \rupdate{\rval_1}{\cnode}{\rval} \rvord \rupdate{\rval_2}{\cnode}{\rval}$.
\end{lemma}
\begin{proof}
In the below calculational proof, let $S = \setc{\pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma(\rval)}$.
%
{\small
\begin{align*}
\rval_1 \rvord \rval_2 & \implies \rgamma(\rval_1) \subseteq \rgamma(\rval_2) & \text{by Lemma~\ref{thm:r-gamma-monotone}} \\ 
& \iff \rgamma(\rval_1) \cap S \subseteq \rgamma(\rval_2) \cap S &  \\ 
& \implies \ralpha(\rgamma(\rval_1) \cap S) \rvord \ralpha(\rgamma(\rval_2) \cap S) & \text{by Lemma~\ref{thm:r-v-alpha-monotone}} \\ 
& \iff \rupdate{\rval_1}{\cnode}{\rval} \rvord \rupdate{\rval_2}{\cnode}{\rval} &  \text{by def. of $\rupdate{\cdot}{\cdot}{\cdot}$} 
\end{align*}
}%
\end{proof}

\begin{lemma}\label{thm:r-n-strength-monotone-2}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, $\rval'_1 \in \rvalues[\rscope_0]$, $\rval'_2 \in \rvalues[\rscope_0]$, and $\cnode \in \cnodes$. 
Then $\rval_1 \rvord \rval_2 \wedge \rval'_1 \rvord \rval'_2 \implies \rupdate{\rval_1}{\cnode}{\rval'_1} \rvord \rupdate{\rval_2}{\cnode}{\rval'_2}$.
\end{lemma}
\begin{proof}
In the below calculational proof, let $S_1 = \setc{\pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma(\rval'_1)}$
and $S_2 = \setc{\pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma(\rval'_2)}$. 

First note that $\rval'_1 \rvord \rval'_2$ implies by Lemma~\ref{thm:r-gamma-monotone} that $\rgamma(\rval'_1) \subseteq \rgamma(\rval'_2)$.
Hence, $S_1 \subseteq S_2$.
%
{\small
\begin{align*}
\rval_1 \rvord \rval_2 & \implies \rgamma(\rval_1) \subseteq \rgamma(\rval_2) & \text{by Lemma~\ref{thm:r-gamma-monotone}} \\ 
& \iff \rgamma(\rval_1) \cap S_1 \subseteq \rgamma(\rval_2) \cap S_2 &  \text{by $S_1 \subseteq S_2$}\\ 
& \implies \ralpha(\rgamma(\rval_1) \cap S_1) \rvord \ralpha(\rgamma(\rval_2) \cap S_2) & \text{by mono. of $\ralpha$} \\ 
& \iff \rupdate{\rval_1}{\cnode}{\rval} \rvord \rupdate{\rval_2}{\cnode}{\rval} &  \text{by def. of $\rupdate{\cdot}{\cdot}{\cdot}$} 
\end{align*}
}%
\end{proof}



\begin{lemma}\label{thm:r-neq-strength-monotone}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, $\cnode_1 \in \cnodes$, and $\cnode_2 \in \cnodes$. 
Then $\rval_1 \rvord \rval_2 \implies \requality{\rval_1}{\cnode_1}{\cnode_2} \rvord \requality{\rval_2}{\cnode_1}{\cnode_2}$.
\end{lemma}
\begin{proof}
Similar as for Lemma~\ref{thm:r-n-strength-monotone}.
\end{proof}


\begin{lemma}\label{thm:r-veq-strength-monotone}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, and $\cnode \in \cnodes$. 
Then $\rval_1 \rvord \rval_2 \implies \requality{\rval_1}{\nu}{\cnode} \rvord \requality{\rval_2}{\nu}{\cnode}$.
\end{lemma}
\begin{proof}
Similar as for Lemma~\ref{thm:r-n-strength-monotone}.
\end{proof}


\begin{lemma}\label{thm:r-map-strength-monotone}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, and $\rmap \in \rmaps$. 
Then $\rval_1 \rvord \rval_2 \implies \rstrengthen{\rval_1}{\rmap} \rvord \rstrengthen{\rval_2}{\rmap}$.
\end{lemma}
\begin{proof}
The result follows from Lemma~\ref{thm:r-n-strength-monotone} and the monotonicity of meets.
\end{proof}


\begin{lemma}\label{thm:r-map-strength-monotone-2}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, $\rmap_1 \in \rmaps$, and $\rmap_2 \in \rmaps$. 
Then $\rval_1 \rvord \rval_2 \wedge \rmap_1 \rmord \rmap_2 \implies \rstrengthen{\rval_1}{\rmap_1} \rvord \rstrengthen{\rval_2}{\rmap_2}$.
\end{lemma}
\begin{proof}
The result follows from Lemma~\ref{thm:r-n-strength-monotone-2} and the monotonicity of meets.
\end{proof}


\begin{lemma}\label{thm:r-rescope-monotone}
Let $\rval_1 \in \rvalues$, $\rval_2 \in \rvalues$, and $\rscope'$ be a scope. 
Then $\rval_1 \rvord \rval_2 \implies \rstrengthen{\rval_1}{\rscope'} \rvord \rstrengthen{\rval_2}{\rscope'}$.
\end{lemma}
\begin{proof}
Similar as for Lemma~\ref{thm:r-n-strength-monotone}.
\end{proof}


\input{proofs/r-structural}


\subsubsection{Propagation and Transformer}

\begin{zproof*}[of Lemma~\ref{thm:r-prop-increasing-monotone}]\end{zproof*}
\begin{proof}
For the increasing property, the proof goes by structural induction on both 
relational arguments of $\rprop$ and it closely follows the proof of 
Lemma~\ref{thm:c-prop-increase}. Regarding monotonicity, the proof 
goes by structural induction on the relational arguments of $\rprop$, 
closely follows the proof of Lemma~\ref{thm:c-prop-monotone}, and 
relies on Lemma~\ref{thm:r-n-strength-monotone-2} (introduced later).
\end{proof}

\begin{zproof*}[of Lemma~\ref{thm:r-step-increasing-monotone}]\end{zproof*}
\begin{proof}
The increasing property of $\Rtrans{\cdot}$ is obvious. Regarding monotonicity,
the proof goes by structural induction on program expressions and it closely
follows the proof of Lemma~\ref{thm:c-step-monotone}. The proof relies on
Lemma~\ref{thm:r-prop-increasing-monotone} as well as 
Lemma~\ref{thm:r-map-strength-monotone-2},~\ref{thm:r-veq-strength-monotone},~\ref{thm:r-rescope-monotone}, and~\ref{thm:r-neq-strength-monotone}.
\end{proof}


\paragraph{Range of Computation}

\begin{lemma}~\label{thm:r-frame}
Let $\rmap$ and $\rmap_1$ be relational maps, $\cenv$ an environment, and $e^\ell$ an expression of a program $p$. 
If $\domvalid(\ell, p, \cenv)$ and $\Rtrans[\fuel]{e^\ell}(\cenv)(\rmap) = \rmap_1$, then 
$\forall \cnode. \rmap(\cnode) \not = \rmap_1(\cnode) \implies \cnode \in \crange_p(\cn{\cenv}{\ell})$.
\end{lemma}
\begin{proof}
The same as in the proof of Lemma~\ref{thm:c-frame}.
\end{proof}


The same result about the range of computation can be shown.
\begin{lemma}~\label{thm:r-framer}
Let $\rmap$ and $\rmap_1$ be relational maps, $\cenv$ an environment, and $e^\ell$ an expression of a program $p$. 
If $\domvalid(\ell, p, \cenv)$ and $\Rtrans[\fuel]{e^\ell}(\cenv)(\cmap) = \rmap_1$, then 
$\forall \cnode. \rmap(\cnode) \not = \rmap_1(\cnode) \implies \cnode \in \cranger_p(\cn{\cenv}{\ell})$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:c-framer}.
\end{proof}
%

\input{proofs/r-semantics-soundness}


==> proofs/r-structural.tex <==
\paragraph{Structural Strengthening}

We also here provide a structural definition of strengthening and argue its soundness.
First, whenever $\cnode \not \in \rscope$, then 
$\supdate{\rval_{\pscope}}{\cnode}{\rval} \Def= \rval$. 
Otherwise, 
%
\[\begin{array}{l l}
\supdate{\rval}{\cnode}{\rbot} & \Def= \rbot\\[1ex]
\supdate{\rval}{\cnode}{\rval'} & \Def= \rval \ind[3] \text{if } \rval \in \{\rbot, \rerr\} \text{ or } \rval' \in \{\rerr\} \cup \rtables[]\\[1ex]
%
\supdate{\rel_1}{\cnode}{\rel_2} &\Def= \rupdate{\rel_1}{\cnode}{\rel_2} \\[1ex]
% 
\supdate{\rtable}{\cnode}{\rval} &\Def=  \Lambda \ccsite. 
\pair{\supdate{\pi_1(\rtable(\ccsite))}{\cnode}{\rval}}{\supdate{\pi_2(\rtable(\ccsite))}{\cnode}{\exists \ccsite.\,\rval}} \ind[1]\;\; \rval \in \rels[]
\end{array}\]
%
It can be shown that the structural strengthening is an overapproximation of the ordinary one.
%
\begin{lemma}~\label{thm:r-structural-soundness}
Let $\rval \in \rvalues[]$, $\rval' \in \rvalues[]$, and $\cnode \in \cnodes$.
Then, $\rupdate{\rval}{\cnode}{\rval'} \rvord \supdate{\rval}{\cnode}{\rval'}$.
\end{lemma}
\begin{proof}
When $\cnode \not \in \rscope$, the argument is trivial by Lemma~\ref{thm:r-n-strengthening}. Otherwise, if $\rval' = \rbot$, the result
follows by the fact monotonicity of $\ralpha$ and
by the definition of $\rgamma$.
The proof is carried by structural induction on $\rval$. First, for the cases
where $\rval' \in \{\rerr\} \cup \rtables[]$, the result follows immediately
by Lemma~\ref{thm:r-n-strengthening}. For the rest of the proof, we thus assume
that $\rval' \in \rels[]$.

For the base cases when $\rval \in \{\rbot, \rerr\}$ the result again follows easily
from Lemma~\ref{thm:r-n-strengthening}. For the base case $\rval \in \rels[]$, the
argument is trivial. For the induction case when $\rval \in \rtables$, we have the following:
%
\[\begin{array}{@{}r}
\{ \pair{\cmap}{\ctable}\;|\; 
\forall \ccsite.\; \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) {=} \pair{\rval_i}{\rval_o} 
        \wedge \pair{\cmap_i}{\cval_i} \in \rgamma[](\rval_i) \\
        \wedge\; \pair{\cmap_o}{\cval_o} \in \rgamma[](\rval_o)
        \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i]\} \cap \mathcal{M} \\[1ex]
{\small \textbf{where } \mathcal{M} = \setc{ \pair{\cmap'[\cnode \mapsto \cval']}{\cval}}{\pair{\cmap'}{\cval'} \in \rgamma[](\rval')}} \\[1ex]
%
= \{\pair{\cmap}{\ctable}\;|\; 
\forall \ccsite.\; \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) {=} \pair{\rval_i}{\rval_o} 
        \wedge \pair{\cmap_i}{\cval_i} \in \rgamma[](\rval_i) \\
        \wedge\; \pair{\cmap_o}{\cval_o} \in \rgamma[](\rval_o)
        \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i] \wedge
        \pair{\cmap}{\ctable} \in \mathcal{M}\} \\
%
= \{\pair{\cmap}{\ctable}\;|\; 
\forall \ccsite.\; \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) {=} \pair{\rval_i}{\rval_o} 
        \wedge \pair{\cmap_i}{\cval_i} \in (\rgamma[](\rval_i) \cap \mathcal{M}) \\
        \wedge\; \pair{\cmap_o}{\cval_o} \in \rgamma[](\rval_o)  \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap 
        \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i] \wedge \cmap \in \mathcal{M}\} \\
{\small \textbf{by $\ccsite$ not in the scope of $\rval_i$ and def.\ of $\mathcal{M}$ (values)}} \\[1ex]
%
= \{\pair{\cmap}{\ctable}\;|\; 
\forall \ccsite.\; \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) {=} \pair{\rval_i}{\rval_o} 
        \wedge \pair{\cmap_i}{\cval_i} \in (\rgamma[](\rval_i) \cap \mathcal{M}) \\
        \wedge\; \pair{\cmap_o}{\cval_o} \in (\rgamma[](\rval_o) \cap \mathcal{M}^{\ccsite}) \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap 
        \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i]\} \\
{\small \textbf{where } \mathcal{M}^{\ccsite} = \setc{\pair{\cmap[\ccsite \mapsto \cval']}{\cval}}{\pair{\cmap}{\cval} \in \mathcal{M} \wedge \cval' \in \cvalues}} \\[1ex]
%
\subseteq \{\pair{\cmap}{\ctable}\;|\; 
\forall \ccsite.\; \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) {=} \pair{\rval_i}{\rval_o} 
        \wedge \pair{\cmap_i}{\cval_i} \in \rgamma[](\rupdate{\rval_i}{\cnode}{\rval'}) \\
        \wedge\; \pair{\cmap_o}{\cval_o} \in \rgamma[](\rupdate{\rval_o}{\cnode}{\exists \ccsite.\,\rval'}) \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap 
        \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i]\} \\
{\small \textbf{by the def.\ of $\rupdate{\cdot}{\cdot}{\cdot}$, def.\ of $\exists \cdot.\,\cdot$, and Proposition~\ref{prop:galois-connections}}} \\[1ex]
%
= \{\pair{\cmap}{\ctable}\;|\; 
\forall \ccsite.\; \ctable(\ccsite) {=} \pair{\cval_i}{\cval_o} \wedge \rtable(\ccsite) {=} \pair{\rval_i}{\rval_o} 
        \wedge \pair{\cmap_i}{\cval_i} \in \rgamma[](\supdate{\rval_i}{\cnode}{\rval'}) \\
        \wedge\; \pair{\cmap_o}{\cval_o} \in \rgamma[](\supdate{\rval_o}{\cnode}{\exists \ccsite.\,\rval'}) \wedge \cmap_i =_{\setminus \{\ccsite\}} \cmap 
        \wedge \cmap_o {=} \cmap_i[\ccsite \mapsto \cval_i]\} \\
{\small \textbf{by i.h.\ and Proposition~\ref{prop:galois-connections}}}\\[1ex]
= \cmap'
\end{array}\]
%
We then have that 
$\rupdate{\rval}{\cnode}{\rval'} \rvord \ralpha[](\cmap' \cup \rgamma(\rbot)) = \ralpha(\rgamma(\supdate{\rval}{\cnode}{\rval'})) \rvord \supdate{\rval}{\cnode}{\rval'}$
by Proposition~\ref{prop:galois-connections}.
%
\end{proof}


==> proofs/t-semantics.tex <==
% !TEX root = ../../thesis.tex
\clearpage
\subsection{Data Flow Refinement Type Semantics Proofs}
\label{sec:proofs-rt-semantics}

As usual, we first provide the definitions of refinement type meet and 
join. 
\begin{definition}
\[\begin{array}{cc}
\tyrel[\basetype]{\paramelem_1} \tvjoin[] \tyrel[\basetype]{\paramelem_2} \Def= \tyrel[\basetype]{\paramelem_1 \;\paramjoin[]\; \paramelem_2} &
\tbot \tvjoin[] \tval \Def= \tval \quad\quad \tval \tvjoin[] \tbot \Def= \tval \\
\ttab{\tval_1}{\tval_2} \tvjoin[] \ttab{\tval_3}{\tval_4} \Def= 
	\ttab{\tval_1\tvjoin[]\tval_3}{\tval_2\tvjoin[]\tval_4} 
& \quad\tval_1 \tvjoin[] \tval_2 \Def= \terr \quad \text{(otherwise)}
\end{array}\]
\end{definition}
A depth $\cvdepth$ of a refinement type value is defined 
in the similar way as for the values of the collapsed semantics. 
We can now prove the correctness of the meet and join operators.
%
\begin{lemma}\label{thm:tvjoin}
Let $V \in \powerset(\tvalues)$. Then, $\tvjoin[] V = \mi{lub} (V)$ and 
$\tvmeet[] V = \mi{glb} (V)$ subject to $\tvord[]$.
\end{lemma}
\begin{proof}
Similar to the proof of Lemma~\ref{thm:rvjoin}, the proof is carried by case analysis on elements 
of $U$ and induction on the minimum depth thereof when $U$ consists of refinement function types only.
\end{proof}


\begin{zproof*}[of Lemma~\ref{thm:t-meet-morph-values} (Complete Meet Morphism of $\tvgamma$)]\end{zproof*}
Let $U \in \powerset(\tvalues)$ and let $\pscope$ be an abstract scope. 
We need to show that $\tvgamma[](\tvmeet U) = \pvmeet[\tval \in U] \tvgamma[](\tval)$.
\begin{proof}
We carry the proof by case analysis on elements of $U$ and induction on the minimum depth
thereof when $U$ consists of tables only. 

We first consider the trivial (base) cases where $U$ is not a set of multiple refinement function types.
\begin{itemize}
\small
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}

\item $U = \emptyset$. Here, $\tvgamma[](\tvmeet[] \emptyset) = \tvgamma[](\terr) = \perr = \pvmeet[] \emptyset$.
\item $U= \{\tval\}$. Trivial.
\item $\tyrel[\cdot]{\cdot} \in U, \ttable \in U$. We have $\tvmeet[] \{\tyrel[\cdot]{\cdot}, \ttable\} = \tbot$
        and since $\tbot$ is the bottom element, $\tvmeet[] U = \tbot$. Similarly,
	$\tvgamma[](\tyrel[\cdot]{\cdot}) \pvmeet[] \tvgamma[](\ttable) = \pbot = \tvgamma[](\tbot)$ so by the 
        definition of $\pvmeet[]$ we have $\pvmeet[\tval \in U] \tvgamma[](\tval) = \rbot$.
\item $\tyrel[\basetype_1]{\cdot} \in U, \tyrel[\basetype_2]{\cdot} \in U$, and $\basetype_1 \not= \basetype_2$.
 Similar to the previous case.


\item $\exists \basetype.\,\forall \tval \in U.\,\tval = \tyrel{\cdot}$. Here,
{\footnotesize \begin{gather*}
\tvgamma[](\tvmeet[] U) = \tvgamma[](\tvmeet[\tyrelv \in U] \tyrelv) \\
= \setc{\pdmap}{\pdmap \in \paramgamma(\parammeet[] \setc{\paramelem}{\tyrel{\paramelem} \in U}) \wedge \pdmap(\nu) \in \gamma_B(\basetype)}\\
\ind[21] \textbf{\scriptsize [by def. of $\tvgamma[]$ and $\tvmeet[]$]} \\
= \bigcap_{\tyrel{\paramelem} \in U} \setc{\pdmap}{\pdmap \in \paramgamma(\paramelem) \wedge \pdmap(\nu) \in \gamma_B(\basetype)}\\
\ind[10] \textbf{\scriptsize [by the complete meet-morphism of $\paramgamma$]} \\
=  \bigcap_{\tval \in U} \tvgamma[](\tval) = \pvmeet[\tval \in U] \tvgamma[](\tval)
\ind[10] \textbf{\scriptsize [by def. of $\tvgamma[]$ and $\pvmeet[]$]}
\end{gather*}}%


\item $\terr \in U$. Here, $ \tvmeet[] U = \tvmeet[] (U/\{\terr\})$ and $\pvmeet[\tval \in U] \tvgamma[](\tval) = \pvmeet[\tval \in U, \tval \not = \terr] \tvgamma[](\tval)$ since $\tvgamma[](\terr) = \perr$. The set $U/\{\terr\}$ either falls into one of the above cases or consists of multiple tables, which is the case we show next.
\end{itemize}


Let $U \subseteq \ttables$ and $|U| > 1$. Let $d$ be the minimum depth of any table in $U$.
{\footnotesize
\begin{gather*}
\tvgamma[](\tvmeet[] U) = \tvgamma[](\ttab{\tvmeet[] \setc{\pi_1(\ptio(\ttable))}{\ttable \in U}}{\tvmeet[] \setc{\pi_2(\ptio(\ttable))}{\ttable \in U}}) \\
\ind[15] \textbf{\scriptsize [by def. of $\tvmeet[]$]} \\
= \ptab{\tvgamma[](\tvmeet[] \setc{\pi_1(\ptio(\ttable))}{\ttable \in U})}{\tvgamma[](\tvmeet[] \setc{\pi_2(\ptio(\ttable))}{\ttable \in U})} \\
\ind[15] \textbf{\scriptsize [by def. of $\tvgamma[]$]} \\
= \ptab{\pvmeet[] \setc{\tvgamma[](\pi_1(\ptio(\ttable)))}{\ttable \in U}}{\pvmeet[] \setc{\tvgamma[](\pi_2(\ptio(\ttable)))}{\ttable \in U}} \\
\textbf{\scriptsize [by i.h. on the min. depth of $\setc{\pi_1(\ptio(\ttable)))}{\ttable \in U}$ and $\setc{\pi_2(\ptio(\ttable)))}{\ttable \in U}$]} \\
= \pvmeet[\tval \in U] \tvgamma[](\tval) \ind[9] \textbf{\scriptsize [by def. of $\pvmeet[]$]}
\end{gather*}}%
\end{proof}



\subsubsection{Domain Operations}


\begin{lemma}~\label{thm:t-structural-soundness}
Structural strengthening operations are sound.
\end{lemma}
\begin{proof}
The proof goes by structural induction on the type being strengthened.
The proof shows that structural strengthening on types overapproximates the
structural strengthening on collapsed values. The argument then follows from
Lemma~\ref{thm:cl-structural-soundness}.
\end{proof}

%\begin{lemma}~\label{thm:t-v-strengthening}
%The structural strengthening operations on types are monotone, idempotent, and strengthening.
%\end{lemma}
%\begin{proof}
%The results follow from the properties of strengthening operations on collapsed values and
%the definition of strengthening operations on types as the best abstractions of their collapsed
%counterparts.
%\end{proof}

It can be also shown that the structural strengthening indeed
performs a strengthening given certain assumptions.
\begin{lemma}~\label{thm:t-v-strengthening}
Let the set of types $\tvalues$ be instantiated with an abstract domain
of type refinements $\paramdomain$ with the strengthening property
$\forall \paramelem \in \paramdomain, \paramelem_1 \in \paramdomain.
\rupdate{\paramelem}{\absn}{\paramelem_1} \paramord \paramelem$.
Let $\tval \in \tvalues$ and $\tval_1 \in \tvalues$. Then,
$\rupdate{\tval}{\absn}{\tval_1} \tvord \tval$ where
strengthening $\rupdate{\cdot}{\cdot}$ is defined structurally
as shown in Figure~\ref{fig:structural-ops-types}.
\end{lemma}
\begin{proof}
The proof goes by structural induction on $\tval$ and case analysis of $\tval_1$.
For the cases where $\tval \in \{\tbot, \terr\}$ or $\tval_1 \in \{\tbot, \terr\} \cup \ttables[]$,
the argument is trivial. For the case when both $\tval$ and $\tval_1$ are 
basic refinement types, the argument follows from the strengthening property
of abstract domain elements. The case when $\tval \in \ttables[]$ and $\tval_1 \in \tyrels[]$
follows from the i.h.
\end{proof}


We can also show that strengthening is monotone assuming that refinement
domain strengthening and rescoping operations are monotone.
\begin{lemma}~\label{thm:t-v-strengthening-monotone}
Let $\tval \in \tvalues$, $\tval' \in \tvalues$, $\tval_1 \in \tvalues$, 
$\tval_2 \in \tvalues$, and $\absn \in \absns$. Assuming that strengthening operations on 
refinement domain $\paramdomain$ are monotone, then 
$\tval_1 \tvord[] \tval_2 \wedge \tval \tvord[] \tval' {\implies} \rupdate{\tval_1}{\absn}{\tval} \tvord[] \rupdate{\tval_2}{\absn}{\tval'}$. 
\end{lemma}
\begin{proof}
When $\absn \not\in \pscope$, the argument is straightforward.
The proof goes by structural induction on $\tval_1$ and $\tval_2$.
But, let us first discuss the cases of $\tval$ and $\tval'$.
When $\tval = \tbot$, the argument is trivial. The same applies
when $\tval \in \ttables$ or $\tval = \terr$. Whenever
$\tval' = \terr$ or $\tval' \in \ttables$, the argument goes
by Lemma~\ref{thm:t-v-strengthening}. 
We can thus carry the induction argument by just considering the cases where
$\tval, \tval' \in \tyrels[]$. Let 
$\tval = \tyrel[\basetype_0]{\paramelem_0}$ and
$\tval' = \tyrel[\basetype_0]{\paramelem'_0}$. 
Let us cover the base cases first.
\begin{itemize}
\item $\tval_1 = \tbot$. Here, $\rupdate{\tval_1}{\absn}{\tval} = \tbot$ and the
result follows trivially.
\item $\tval_2 =  \tbot$. Then it must be that $\tval_1 = \tbot$ and the result follows from the
previously analyzed case.
\item $\tval_2 = \terr$. We have $\rupdate{\tval_2}{\absn}{\tval} = \terr$ and the result holds
trivially.
\item $\tval_1 = \terr$. Then, $\tval_2 = \terr$ which is the case already covered.  
\item $\tval_1 = \tyrel{\paramelem_1}, \tval_2 = \tyrel{\paramelem_2},$ where 
$\paramelem_1 \paramord[] \paramelem_2$. We have 
$\rupdate{\tval_1}{\absn}{\tval} = \tyrel{\rupdate{\paramelem_1}{\absn}{\paramelem_0}}$ and
$\rupdate{\tval_2}{\absn}{\tval} = \tyrel{\rupdate{\paramelem_2}{\absn}{\paramelem'_0}}$.
The result then follows from the monotonicity of the refinement strengthening.
\end{itemize}

For the induction case where $\tval_1 \in \ttables[]$ and $\tval_2 \in \ttables[]$, the
argument follows straightforwardly from the i.h. and monotonicity of the
refinement domain rescoping operation.
\end{proof}


\subsubsection{Abstract Propagation and Transformer}

\begin{zproof*}[of Lemma~\ref{thm:t-prop-increasing-monotone}]\end{zproof*}
\begin{proof}
The increasing property follows easily by the structural induction on both type arguments of $\tprop$.
Regarding monotonicity, the argument goes on structural induction on the argument to $\tprop$
by closely following that of Lemma~\ref{thm:c-prop-monotone} and it relies on 
Lemma~\ref{thm:t-v-strengthening-monotone}.
\end{proof}


\begin{zproof*}[of Lemma~\ref{thm:t-step-increasing-monotone}]\end{zproof*}
\begin{proof}
The increasing property follows trivially. The argument for monotonicity follows that of
Lemma~\ref{thm:c-step-monotone} and it relies on the monotonicity of $\tprop$
established by Lemma~\ref{thm:t-prop-increasing-monotone}.
\end{proof}


\begin{lemma}~\label{thm:rt-finite-nodes}
  For all programs $e$, either $\tcoll[e](\pnode) =\tmap_{\terr}$ 
    or the set $\pset{\pnode \in \pnodes}{\tcoll[e](\pnode) \neq \tbot}$ is finite.
\end{lemma}
\begin{proof}
The proof is the same as the proof of Lemma~\ref{lem:finite-nodes}.
\end{proof}


\subsubsection{Widenings}

We next prove main properties regarding the widening operators of the general refinement type sematnics.

\begin{lemma}~\label{thm:sh-ord}
Let $\tval_1 \in \tvalues$, $\tval_2 \in \tvalues$ such that $\tval_1 \tvord \tval_2$.
Then, $\shape(\tval_1) \tvord \shape(\tval_2)$.
\end{lemma}
\begin{proof}
The proof easily follows by structural induction on both $\tval_1$ and $\tval_2$.
\end{proof}

%\begin{lemma}~\label{thm:sh-wid-join}
%Let $\tval_1 \in \tvalues$, $\tval_2 \in \tvalues$, and $\tval = \tval_1 \tvjoin \tval_2$.
%Then, $\shape(\tval_1) \tvord \shape(\tval)$ and $\shape(\tval_2) \tvord \shape(\tval)$.   
%\end{lemma}
%\begin{proof}
%The proof follows from the basic properties of joins (increasiveness) and Lemma~\ref{thm:sh-ord}.
%\end{proof}
%
\begin{lemma}~\label{thm:sh-t-wid-depth}
Let $\paramwid$ be a widening operator for the domain of abstract refinements $\paramdomain$
used to instantiate the set of types $\tvalues$ and the widening operator $\trelwid$. Also, let
$\tval_1 \in \tvalues$, $\tval_2 \in \tvalues$, and $\tval = \tval_1 \trelwid \tval_2$.
Then, $\cvdepth(\tval) \leq \m{max}(\cvdepth(\tval_1), \cvdepth(\tval_2))$.   
\end{lemma}
\begin{proof}
The proof goes by structural induction on both $\tval_1$ and $\tval_2$ and
it relies on the properties of the $\shape$ function.
\end{proof}
%
%\begin{lemma}~\label{thm:sh-comp-wid}
%Let $\twid$ be the composite widening operator for the domain of abstract refinements 
%$\paramdomain$ used to instantiate the set of types $\tvalues$ and let $\shapewid$ be
%the corresponding shape widening operator. Also, let
%$\tval_1 \in \tvalues$, $\tval_2 \in \tvalues$, and $\tval = \tval_1 \twid \tval_2$.
%Then, $\shape(\tval_1) \tvord \shape(\tval)$ and $\shape(\tval_2) \twid \shape(\tval)$.   
%\end{lemma}
%\begin{proof}
%Recall that $\tval_1 \twid \tval_2 \Def= \tval_1 \trelwid (\tval_1 \shapewid \tval_2)$.
%Now, $\shape(\tval_1) \tvord \shape(\tval_1 \shapewid \tval_2)$ and
%$\shape(\tval_2) \tvord \shape(\tval_1 \shapewid \tval_2)$ by Lemma~\ref{thm:sh-ord} and
%the fact that $\shapewid$ is an upper bound operator. By Lemma~\ref{thm:sh-t-wid} it
%follows then that $\shape(\tval_1) \tvord \shape(\tval)$ and $\shape(\tval_2) \twid \shape(\tval)$.  % 
%Alternatively, $\twid$ is an upper bound operator by definition, so the result
%immediately follows from Lemma~\ref{thm:sh-ord}.
%\end{proof}


\begin{zproof*}[of Lemma~\ref{lem:type-widening}]\end{zproof*}
\begin{proof}
The upper bound property of $\twid$ directly follows from the upper bound properties
of $\trelwid$ and $\shapewid$.
Let $\tval_0 \tvord \tval_1 \tvord \dots$ be an increasing sequence of types.
Let $y^i$ be the sequence of types defined by $y_0 = \tval_0$ and 
$y_{i} = y_{i-1} \twid \tval_{i-1}$ for all $i>0$. By $\twid$ being an upper bound operator 
it follows that $y_0 \tvord y_1 \tvord \dots$. By Lemma~\ref{thm:sh-ord}, it is then 
the case that $\shape(y_0) \tvord \shape(y_1) \tvord \dots$. 
Now, $\trelwid$ increases the shape of the two argument types by being increasing and 
by Lemma~\ref{thm:sh-ord}, but only by introducing $\terr$ (Lemma~\ref{thm:sh-t-wid-depth}). 
Hence, either $\trelwid$ eventually produces $\terr$ in the sequence $y^i$, thus stabilizing it, 
or it eventually stops affecting the shape of types in $y^i$. In that case, the shape 
of $y^i$ eventually stabilizes by the widening properties of $\shapewid$. The whole $y^i$ 
then stabilizes by the widening operator property of $\paramwid$ and the definition of $\trelwid$.
\end{proof}






==> rel-struct.tex <==
% !TEX root = main.tex
\section{Systems of Structures}
\label{sec:rel-struct}

The collecting semantics provides extremely rich information about actual program 
executions. For each function, the semantics can tell exactly what are the inputs passed 
to the function in the program, the results the function returns on these inputs, 
and details on how this function was passed to other functions during the execution.
This information implicitly contains information on how functions behaved when 
passed as arguments to other functions. Clearly, statically computing this program 
semantics is impossible.

In this section, we introduce a \textit{system of elementary structures} that 
effectively computes an overapproximation of the collecting semantics by keeping 
track of only certain kind of information about concrete program behaviors. That is, 
this system dictates the information structure, i.e., what kind of information 
about program behaviors is being tracked during the analysis, while the refinement 
type systems improve the analysis precision by refining the information being tracked. 
We piggyback on the system of elementary structures later on in Section~\ref{sec:gen-refinement-system} 
to create a general refinement type system. Therefore, choosing a system of 
structures can be seen as a first design choice in creating a refinement type system. 

\subsection{Elementary Structures}

The first simplification the system of elementary structures introduces is the
abstraction of sets of program values by \textit{elementary structures} shown below. 
We assume we are given a finite set of base structures $\sbase \in \Sbases$,
where $\sbool \in \Sbases$, and a concretization function 
$\gamma_{\Sbases}:\Sbases \to \powerset{\Vals}$, 
assumed to be disjoint for simplicity, that tells us what values each structure abstracts over. 

\[\begin{array}{r l}
s, q ::= &  \sbase \qd|\qd \unrs \qd|\qd \anys \qd|\qd J:s_1 \tto \dots \tto s_l \\[1ex]
\multicolumn{2}{r}{\quad\quad\quad\text{elementary structures } \Structs \qd (2 \leq l \leq k + 1, J \subseteq I)} 
\end{array}\]

\noindent Closure structures $J:s_1 \tto \dots \tto s_l$ intuitvely stand for
closures of functions in $J$ such that next $l-1$ arguments passed to the closure
comply with structures $s_1$ to $s_{l-1}$, respectively, and once all the arguments
have been passed, the functions in $J$ return values complying with $s_l$. Note how
closure structures do not talk about argument histories nor arguments 
already seen by the corresponding closures. This is another simplification w.r.t. the 
concrete semantics. Our system of structures only cares about how closures behave
in the future, i.e., once they are passed to other functions. A possible direction 
in which the existing refinement type systems can be extended is to consider a 
system of structures that can in addition infer invariants on how argument functions 
behaved prior to being passed to a calee function. We leave investigation of such 
powerful structures as future work. 

Structures $\unrs$ and $\anys$ informally represent non-termination value and a
set of all values, respectively. Function structures $s_f$ will be used to assign
(abstract) structural meaning to functions, whereas program structures $\vec{S}$
are used to abstract programs. The intuition we provided here is made formal
in Figure~\ref{fig:gamma-rstructures} in the form of concretization functions.

\begin{figure*}[t]
\[\begin{array}{l l}
\nfscon:\Nfstructs \to \Rels^n & \nfscon(\vec{S}) \triangleq \langle \fscon(\vecat{\vec{S}}{1}), \dots, \fscon(\vecat{\vec{S}}{n})\rangle \\[2ex]


\fscon: \Fstructs \to \Rels &
\fscon(s_1 \tto \dots \tto s_{k+1}) \triangleq \{\langle \env,v\rangle \;|\; \env \in \Envs \wedge (par(\env) \Rightarrow v = \unr) \wedge
				(\forall i \leq k.\; arg(\env, i) \in \scon(s_i)) \wedge v \in \scon(s_{k+1})\} \\[3ex]
%\multicolumn{2}{r}{\;\wedge\; \forall C \in his(\env), c \in C.\; fits(c, \vec{S})\}} \\[2ex]



\scon: \Structs \to \powerset{\Vals} & 
		\scon(\anys) \triangleq \Vals \quad\quad \scon(\unrs) \triangleq \{\bot\} \quad\quad 
		\scon(\sbase) \triangleq \gamma_B(\sbase) \cup \{\bot\}\\[1ex]

&\scon(J:s_1 \tto \dots \tto s_l) \triangleq \{ [j\;\env] \;|\; j \in J \wedge m = k+1-l \wedge lai(\env) = m \;\wedge \\[0.5ex]
%(\forall C \in his(\env), c \in C.\; fits(c, \vec{S}))  \;\wedge\\[0.5ex]
\multicolumn{2}{r}{\forall \langle \env_1, v \rangle \in \fscon(\vecat{\vec{S}}{j}).\; \prefix(\env, \env_1) \Rightarrow
		(\forall 1 \leq i < l.\; arg(\env_1, m + i) \in \scon(s_i)) \wedge v \in \scon(s_l)\} \cup \{\bot\}} \\[3ex]



& \prefix(\langle\his{}{C_0}, \dots, \his{\vz_l}{C_l}, \unr, \dots,\unr\rangle, 
			\langle\his{}{D_0},  \dots, \his{\wz_m}{D_m}, \unr, \dots,\unr\rangle)\iff\\[0.5ex]
\multicolumn{2}{r}{l \leq m \wedge C_l \subseteq D_l \wedge \vz_l = \wz_l \wedge \forall 1 \leq i \leq l -1.\;\vh_i = \wh_i} 
%& fits(c, \vec{S}) \iff \exists i, \env, v.\; c= [i\;\env] \wedge \langle \env, v\rangle \in \fscon(\vecat{\vec{S}}{i})
\end{array}\]
\label{fig:gamma-rstructures}
\caption{Concretization function for elementary structures}
\end{figure*}


For the purposes of giving the definition of the abstract transformer later on, we 
will need the join (lub) $\slubs:\Structs \times \Structs \to \Structs$ operator for structures, 
given as follows:

\[\begin{array}{r l l}
s \slubs q \triangleq& s & \textbf{if $q = \unrs$} \\[0.5ex]
\triangleq & q & \textbf{if $s = \unrs$} \\[0.5ex]
%\triangleq & \anys & \text{if $s = \anys$ or $q = \anys$} \\[0.5ex]
\triangleq & J_1 \cup J_2: s_1 \slubs q_1 \tto \dots \tto s_l \slubs q_l& \\[0.25ex] 
\multicolumn{3}{r}{\textbf{if } s = J_1: s_1 \tto \dots \tto s_l \textbf{ and } q =  J_2: q_1 \tto \dots \tto q_l} \\[1ex]
\triangleq & s & \textbf{if } s = q = \sbase\\[0.25ex]
%\triangleq & \sbase & \text{if } s = q = \sbase \\[0.5ex]
%\triangleq & \sbool & \text{if } s = q = \sbool \\[0.5ex]
\triangleq & \anys & \textbf{otherwise}
\end{array}\]

\paragraph{Environments.} Abstract structural environments 
$\senv \in \Senvs \triangleq \Structs^k$ are vectors of $k$ 
structures. The empty environment is defined as 
$\senv_{\bot} \triangleq \langle \unrs, \dots, \unrs \rangle$. 
The join operator on environments $\senvlubs: \Senvs \times \Senvs \to \Senvs$
is a pointwise lifting of the join operator on single structures.
We will use symbol $\senvec$ to range over vectors of $n$ structure 
environments. 

\paragraph{Relations.} Semantic domains used for assigning 
abstract meaning to program functions are program structures $\sec{S}$ 
which are vectors of $n$ function structures. 

\[\begin{array}{l r}
s_f ::= s_1 \tto \dots \tto s_{k+1} & \text{function structure $\Fstructs$} \\[1ex]
\vec{S} \in \Nfstructs & \Repeat{5}{\quad}\text{program structures}  
\end{array}\]

\noindent A function structure, on the other hand, is a closure structure of length $k+1$.
The join operator $\nfslubs: \Nfstructs \times \Nfstructs \to \Nfstructs$ on such 
vectors is a simple pointwise vector extension of the join operator on single structures.


\subsection{Abstract Semantics}

\paragraph{Abstract transformer.}
The abstract transformer for the system of relational structures
$\astrans{\cdot}: \Exp \to \Nfstructs \to \Senvs \to (\Senvs \times \Structs \times (\Senvs)^n)$ is
defined below.

\begin{figure}[h!]
\centering
\begin{tabular}{l l l}
$\astrans{x_i}(\vec{S})(\senv)$ &$\triangleq$&  $\langle \senv, \vecat{\senv}{i}, \senvbot^n \rangle$ \\[1.5ex]

%---constant---
$\astrans{b}(\vec{S})(\senv)$ &$\triangleq$& 
	$\begin{cases}
		\langle \senv, \sbase, \senvbot^n \rangle & \textbf{if } b \in \gamma_B(\sbase)\\
		\langle \senv, \anys, \senvbot^n \rangle & \textbf{otherwise}
		\end{cases}$\\[3ex]

%---function names---
$\astrans{f_i}(\vec{S})(\senv)$ &$\triangleq$& $\langle \senv, \{i\}:\vecat{\vec{S}}{i}, \senvbot^n \rangle$ \\[1.5ex]

%---if-then-else---
$\astrans{\ifte{e}{e_1}{e_2}}(\vec{S})(\senv)$ &$\triangleq$& \\[0.5ex]
\multicolumn{3}{l}{\quad$\Mlet \langle \senv, s_0, \senvec_0 \rangle = \astrans{e}(\vec{S})(\senv) \Min$}\\[0.5ex]	
\multicolumn{3}{l}{\quad$\Mlet \langle \senv, s_1, \senvec_1 \rangle = \astrans{e_1}(\vec{S})(\senv) \Min$}\\[0.5ex]	
\multicolumn{3}{l}{\quad$\Mlet \langle \senv, s_2, \senvec_2 \rangle = \astrans{e_2}(\vec{S})(\senv) \Min$}\\[0.5ex]	

\multicolumn{3}{l}{\quad\quad $\Mif s_0  = \unrs \vee s_0 = \anys \;\Mthen \langle \senv, s_0, \senvec_0  \rangle$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad $\Melse \Mif s_0  \not = \sbool\;\Mthen \langle \senv, \anys, \senvec_0 \rangle$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad $\Melse \langle \senv, s_1 \slubs s_2, \senvec_0 \vec{\senvlubs} \senvec_1 \vec{\senvlubs} \senvec_2 \rangle$}\\[2ex]

%---function application---
$\astrans{e_1(e_2)}(\vec{S})(\senv)$ &$\triangleq$& \\[0.5ex]	
\multicolumn{3}{l}{\quad$\Mlet \langle \senv, s_1, \senvec_1 \rangle = \astrans{e_1}(\vec{S})(\senv) \Min$}\\[0.5ex]	
\multicolumn{3}{l}{\quad$\Mlet \langle \senv, s_2, \senvec_2 \rangle = \astrans{e_2}(\vec{S})(\senv) \Min$}\\[0.5ex]	

\multicolumn{3}{l}{\quad\quad $\Mif s_1  = \unrs \vee s_1 = \anys \;\Mthen \langle \senv, s_1, \senvec_1  \rangle$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad $\Melse \Mif s_1 = \sbase \;\Mthen \langle \senv, \anys, \senvec_1  \rangle$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad $\Melse \Mif s_2 = \unrs \vee s_2 = \anys \;\Mthen \langle \senv, s_2, \senvec_2  \rangle$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad $\Melse$}\\[0.5ex]

\multicolumn{3}{l}{\quad\quad\quad $\Mlet s_1 = J:q_1 \tto q_2 \tto \dots \tto q_l \Min$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad\quad $\Mlet s = \Mif l = 2 \;\Mthen q_l \;\Melse q_2 \tto \dots \tto q_l \Min$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad\quad $\Mlet \senv_0 = \vecupd{\senvbot}{(k+1-l)}{s_2}  \Min$}\\[0.5ex]
\multicolumn{3}{l}{\quad\quad\quad\quad $\langle \senv, s, 
			\senvec_1 \vec{\senvlubs} \senvec_2 \vec{\senvlubs}
				\vecupd{\senvbot^n}{J}{\senv_0}\rangle$}
\end{tabular}
\caption{Abstract transformer for the structure system}
\label{fig:abstract-structure-transformer}
\end{figure}


\paragraph{Collecting semantics.}
The abstract (structure) collecting semantics 
$\ascoll{\cdot}:\Progs \to \Senvs^n \to \Nfstructs$ is as follows.


\[\begin{array}{@{}l}
\scoll{f_1\; x_1\cdots x_k =e_1\dots f_n\;x_1\cdots x_k = e_n}(\senvec_0) \triangleq \\[1ex]
\mathbf{lfp}^{\srelord}_{\vec{er_s}(\senvec_0)}\; \lambda \vec{S}.\; \vec{S} \quad\nfslubs\;\\[1ex]
\multicolumn{1}{r}{\langle rel_s(e_1, \vec{S}, re_s(\vecat{\vec{S}}{1})), \dots, rel_s(e_1, \vec{S}, re_s(\vecat{\vec{S}}{n}))\rangle \;\nfslubs} \\[1ex]
\multicolumn{1}{r}{er_s(env_s(e_1, \vec{S}, re_s(\vecat{\vec{S}}{1}))) \;\nfslubs \;\cdots \;\nfslubs}\\[1ex]
\multicolumn{1}{r}{er_s(env_s(e_1, \vec{S}, re_s(\vecat{\vec{S}}{n})))} \\[3ex]

er_s(\langle s_1, \dots, s_k \rangle) \triangleq s_1 \tto \dots s_k \tto \unrs \\[1ex]

re_s(s_1 \tto \dots \tto s_k \tto s_{k+1}) \triangleq \langle s_1, \dots, s_k \rangle \\[1ex]

rel_s(e, \vec{S}, \senv) \triangleq s_1 \tto \dots \tto s_k \tto s \\[0.5ex]
\multicolumn{1}{r}{\textbf{where } \senv = \langle s_1, \dots, s_k \rangle \textbf{ and } 
	\exists \vec{\senv}.\;\strans{e}(\vec{S})(\senv)= \langle \senv, s, \vec{\senv} \rangle}\\[1ex]

envs_s(e, \vec{S}, \senv) \triangleq \vec{\senv} \qd\quad\quad\textbf{where } 
		\exists s.\;\strans{e}(\vec{S})(\senv)= \langle \senv, s, \vec{\senv} \rangle 
\end{array}\]

